Prior Convictions: Black-Box Adversarial Attacks with Bandits and Priors

We study the problem of generating adversarial examples in a black-box setting in which only loss-oracle access to a model is available. We introduce a framework that conceptually unifies much of the existing work on black-box attacks, and we demonstrate that the current state-of-the-art methods are optimal in a natural sense. Despite this optimality, we show how to improve black-box attacks by bringing a new element into the problem: gradient priors. We give a bandit optimization-based algorithm that allows us to seamlessly integrate any such priors, and we explicitly identify and incorporate two examples. The resulting methods use two to four times fewer queries and fail two to five times less often than the current state-of-the-art.

==> fig/data/avgq-vs-success-2/banditst-l2-cdf.tex <==
0 0.281216
0 0.283995
0 0.287492
6.000000 0.288951
7.000000 0.291243
8.000000 0.293326
9.600000 0.288344
10.333333 0.289474
11.142858 0.292392
11.142858 0.297224
13.111111 0.298736
14.000000 0.296533
14.909091 0.297083
14.909091 0.300000
16.000000 0.300322
17.076923 0.301642
17.076923 0.304312
17.076923 0.306962
17.076923 0.309612
17.076923 0.312240
17.076923 0.314861
17.076923 0.317467
19.000000 0.316464
20.799999 0.316104
22.500000 0.315074
22.500000 0.317417
24.235294 0.318284
28.700001 0.308697
28.700001 0.310893
30.095238 0.310502
30.095238 0.312632
32.869564 0.310465
32.869564 0.312559
35.520000 0.311640
36.769230 0.310803
36.769230 0.312840
36.769230 0.314808
38.148148 0.311991
38.148148 0.313919
39.571430 0.311188
39.571430 0.313066
41.034481 0.309216
41.034481 0.310917
42.533333 0.310859
42.533333 0.312562
45.500000 0.307107
45.500000 0.308815
45.500000 0.310420
45.500000 0.312009
47.090908 0.308512
48.647060 0.307203
50.171429 0.307116
50.171429 0.308600
51.722221 0.306104
51.722221 0.307595
51.722221 0.309085
53.351353 0.309334
53.351353 0.310754
53.351353 0.312172
53.351353 0.313611
53.351353 0.315042
53.351353 0.316532
53.351353 0.317987
53.351353 0.319455
53.351353 0.320877
53.351353 0.322321
53.351353 0.323756
53.351353 0.325132
53.351353 0.326531
55.578949 0.321918
55.578949 0.323286
55.578949 0.324626
55.578949 0.325932
55.578949 0.327250
55.578949 0.328538
60.299999 0.326816
60.299999 0.328093
60.299999 0.329335
62.634148 0.326451
62.634148 0.327643
62.634148 0.328847
62.634148 0.330038
65.047623 0.327533
65.047623 0.328717
65.047623 0.329946
65.047623 0.331160
65.047623 0.332352
65.047623 0.333543
65.047623 0.334792
65.047623 0.336056
65.047623 0.337282
67.767441 0.333846
67.767441 0.335026
67.767441 0.336244
67.767441 0.337478
70.545456 0.335897
73.244446 0.331111
73.244446 0.332293
78.468086 0.329946
78.468086 0.331157
81.000000 0.329782
81.000000 0.330975
81.000000 0.332183
83.551018 0.331480
86.040001 0.331182
86.040001 0.332373
86.040001 0.333580
86.040001 0.334758
86.040001 0.335861
86.040001 0.336957
86.040001 0.338022
86.040001 0.339064
88.745094 0.337763
88.745094 0.338805
91.423080 0.336383
91.423080 0.337411
91.423080 0.338464
91.423080 0.339607
94.150940 0.338848
94.150940 0.339910
94.150940 0.341012
94.150940 0.342094
94.150940 0.343124
94.150940 0.344150
94.150940 0.345148
94.150940 0.346160
97.074074 0.344506
97.074074 0.345441
97.074074 0.346375
97.074074 0.347343
97.074074 0.348294
100.072731 0.345381
100.072731 0.346270
100.072731 0.347208
103.071426 0.344768
103.071426 0.345674
103.071426 0.346591
103.071426 0.347563
103.071426 0.348518
103.071426 0.349465
103.071426 0.350439
103.071426 0.351412
106.245613 0.350807
106.245613 0.351746
106.245613 0.352674
106.245613 0.353644
106.245613 0.354611
109.482758 0.353389
109.482758 0.354339
109.482758 0.355285
109.482758 0.356239
109.482758 0.357192
109.482758 0.358076
109.482758 0.358915
109.482758 0.359797
112.881355 0.355517
112.881355 0.356461
119.475410 0.351471
122.645164 0.351170
122.645164 0.352059
122.645164 0.352951
122.645164 0.353852
125.841270 0.349804
125.841270 0.350682
129.000000 0.349139
132.092300 0.342580
132.092300 0.343503
132.092300 0.344436
132.092300 0.345344
132.092300 0.346234
132.092300 0.347112
135.272720 0.342607
135.272720 0.343509
135.272720 0.344395
135.272720 0.345260
135.272720 0.346145
135.272720 0.347038
135.272720 0.347900
138.567169 0.343379
138.567169 0.344195
138.567169 0.345022
138.567169 0.345887
138.567169 0.346721
138.567169 0.347526
141.941177 0.347167
141.941177 0.348033
141.941177 0.348894
148.571426 0.346659
151.774643 0.344983
151.774643 0.345835
151.774643 0.346692
151.774643 0.347527
155.000000 0.343259
158.164383 0.342787
158.164383 0.343634
158.164383 0.344486
158.164383 0.345317
158.164383 0.346133
161.378372 0.345557
161.378372 0.346344
161.378372 0.347115
161.378372 0.347842
161.378372 0.348603
164.639999 0.346581
164.639999 0.347387
164.639999 0.348212
164.639999 0.349071
167.921051 0.348286
167.921051 0.349050
174.333328 0.343662
174.333328 0.344468
177.468353 0.343777
177.468353 0.344554
177.468353 0.345331
177.468353 0.346101
177.468353 0.346864
177.468353 0.347632
177.468353 0.348422
177.468353 0.349196
177.468353 0.349958
177.468353 0.350706
177.468353 0.351456
177.468353 0.352220
177.468353 0.353053
180.850006 0.352136
180.850006 0.352900
180.850006 0.353674
180.850006 0.354447
180.850006 0.355246
184.271606 0.352430
184.271606 0.353216
184.271606 0.353956
184.271606 0.354703
184.271606 0.355456
184.271606 0.356216
184.271606 0.356970
184.271606 0.357713
184.271606 0.358412
184.271606 0.359120
184.271606 0.359853
184.271606 0.360571
184.271606 0.361310
184.271606 0.362067
191.542175 0.359817
191.542175 0.360550
191.542175 0.361303
191.542175 0.362011
191.542175 0.362723
191.542175 0.363439
191.542175 0.364175
191.542175 0.364871
191.542175 0.365592
191.542175 0.366289
191.542175 0.366993
191.542175 0.367735
195.333328 0.366966
195.333328 0.367699
195.333328 0.368405
195.333328 0.369105
199.129410 0.364459
199.129410 0.365173
199.129410 0.365907
199.129410 0.366638
199.129410 0.367326
199.129410 0.368009
199.129410 0.368694
199.129410 0.369384
203.023254 0.365826
203.023254 0.366535
203.023254 0.367229
203.023254 0.367913
203.023254 0.368600
203.023254 0.369334
203.023254 0.370081
203.023254 0.370823
203.023254 0.371527
203.023254 0.372202
203.023254 0.372873
203.023254 0.373513
203.023254 0.374152
203.023254 0.374817
203.023254 0.375496
207.172409 0.374493
207.172409 0.375134
211.272720 0.370677
211.272720 0.371329
211.272720 0.371977
211.272720 0.372613
211.272720 0.373255
211.272720 0.373907
215.415726 0.370476
215.415726 0.371162
215.415726 0.371834
215.415726 0.372522
215.415726 0.373226
215.415726 0.373913
215.415726 0.374588
215.415726 0.375296
215.415726 0.375976
215.415726 0.376683
219.688889 0.373497
219.688889 0.374187
223.912094 0.373553
223.912094 0.374255
223.912094 0.374959
228.108688 0.373472
228.108688 0.374125
232.258072 0.372431
236.340424 0.371178
236.340424 0.371875
236.340424 0.372583
236.340424 0.373260
236.340424 0.373931
236.340424 0.374613
236.340424 0.375283
236.340424 0.375962
236.340424 0.376613
236.340424 0.377240
236.340424 0.377881
236.340424 0.378507
236.340424 0.379167
236.340424 0.379800
236.340424 0.380416
236.340424 0.381040
236.340424 0.381688
236.340424 0.382335
236.340424 0.383020
236.340424 0.383750
236.340424 0.384457
236.340424 0.385199
236.340424 0.385916
236.340424 0.386599
236.340424 0.387295
236.340424 0.387980
236.340424 0.388630
236.340424 0.389277
240.926315 0.387038
240.926315 0.387691
240.926315 0.388318
245.479172 0.385051
249.958755 0.384192
249.958755 0.384802
249.958755 0.385416
249.958755 0.386011
249.958755 0.386595
249.958755 0.387187
249.958755 0.387777
249.958755 0.388357
249.958755 0.389013
249.958755 0.389651
249.958755 0.390271
254.571426 0.387667
254.571426 0.388286
254.571426 0.388890
254.571426 0.389502
254.571426 0.390108
254.571426 0.390735
254.571426 0.391382
254.571426 0.392004
254.571426 0.392635
254.571426 0.393252
254.571426 0.393927
259.313141 0.391903
259.313141 0.392516
259.313141 0.393181
259.313141 0.393893
264.040009 0.388571
264.040009 0.389194
264.040009 0.389846
264.040009 0.390521
264.040009 0.391210
264.040009 0.391890
264.040009 0.392525
264.040009 0.393129
264.040009 0.393737
264.040009 0.394328
264.040009 0.394919
264.040009 0.395528
264.040009 0.396163
264.040009 0.396800
264.040009 0.397425
264.040009 0.398066
264.040009 0.398743
264.040009 0.399404
269.029694 0.395162
269.029694 0.395769
269.029694 0.396379
269.029694 0.396981
274.000000 0.391060
274.000000 0.391650
278.912628 0.386981
283.750000 0.385278
288.514282 0.376359
288.514282 0.376931
288.514282 0.377501
288.514282 0.378077
288.514282 0.378680
288.514282 0.379273
288.514282 0.379886
288.514282 0.380493
288.514282 0.381100
288.514282 0.381699
293.377350 0.376303
293.377350 0.376881
293.377350 0.377495
293.377350 0.378065
293.377350 0.378631
293.377350 0.379185
293.377350 0.379737
293.377350 0.380269
293.377350 0.380832
293.377350 0.381384
293.377350 0.381907
293.377350 0.382434
293.377350 0.382971
293.377350 0.383498
293.377350 0.384032
293.377350 0.384574
293.377350 0.385147
293.377350 0.385683
293.377350 0.386220
293.377350 0.386768
293.377350 0.387313
293.377350 0.387863
293.377350 0.388428
293.377350 0.388994
293.377350 0.389567
293.377350 0.390151
293.377350 0.390712
298.654205 0.389630
298.654205 0.390184
298.654205 0.390746
298.654205 0.391306
303.907410 0.386648
303.907410 0.387198
303.907410 0.387775
303.907410 0.388348
309.137604 0.386831
309.137604 0.387406
309.137604 0.387977
309.137604 0.388538
319.459473 0.385060
319.459473 0.385610
319.459473 0.386150
319.459473 0.386670
324.553558 0.384999
324.553558 0.385495
324.553558 0.385985
324.553558 0.386481
324.553558 0.386991
324.553558 0.387483
324.553558 0.387963
324.553558 0.388444
324.553558 0.388973
324.553558 0.389491
324.553558 0.390008
324.553558 0.390540
324.553558 0.391100
329.787598 0.386990
329.787598 0.387519
329.787598 0.388047
329.787598 0.388580
335.000000 0.387553
340.139130 0.383868
340.139130 0.384362
340.139130 0.384875
340.139130 0.385404
340.139130 0.385918
340.139130 0.386418
340.139130 0.386911
340.139130 0.387388
345.327576 0.381159
345.327576 0.381654
345.327576 0.382168
345.327576 0.382672
345.327576 0.383190
345.327576 0.383730
345.327576 0.384248
345.327576 0.384758
345.327576 0.385261
345.327576 0.385745
345.327576 0.386227
345.327576 0.386743
345.327576 0.387254
345.327576 0.387767
345.327576 0.388294
345.327576 0.388805
345.327576 0.389340
345.327576 0.389875
345.327576 0.390404
345.327576 0.390937
345.327576 0.391437
345.327576 0.391938
345.327576 0.392455
345.327576 0.392959
345.327576 0.393528
350.854706 0.391100
350.854706 0.391636
350.854706 0.392145
350.854706 0.392640
350.854706 0.393129
350.854706 0.393619
350.854706 0.394113
350.854706 0.394620
350.854706 0.395141
350.854706 0.395662
350.854706 0.396196
350.854706 0.396725
350.854706 0.397246
350.854706 0.397751
350.854706 0.398273
356.542358 0.396551
356.542358 0.397079
356.542358 0.397610
356.542358 0.398139
356.542358 0.398658
356.542358 0.399217
356.542358 0.399732
362.252106 0.393838
362.252106 0.394309
362.252106 0.394755
373.487610 0.386327
373.487610 0.386773
373.487610 0.387209
373.487610 0.387673
373.487610 0.388153
379.049194 0.380752
379.049194 0.381199
379.049194 0.381662
379.049194 0.382131
384.585358 0.379010
384.585358 0.379482
384.585358 0.379948
390.080658 0.378695
390.080658 0.379184
390.080658 0.379676
390.080658 0.380143
390.080658 0.380601
390.080658 0.381061
390.080658 0.381524
390.080658 0.381977
390.080658 0.382436
395.631989 0.379865
395.631989 0.380333
395.631989 0.380793
395.631989 0.381239
395.631989 0.381666
395.631989 0.382106
395.631989 0.382528
395.631989 0.382950
395.631989 0.383349
395.631989 0.383764
395.631989 0.384171
395.631989 0.384577
395.631989 0.384987
395.631989 0.385420
395.631989 0.385872
401.333344 0.384997
401.333344 0.385418
401.333344 0.385843
401.333344 0.386292
401.333344 0.386729
401.333344 0.387155
401.333344 0.387561
401.333344 0.387972
401.333344 0.388380
401.333344 0.388790
401.333344 0.389194
401.333344 0.389602
407.133850 0.385772
407.133850 0.386171
407.133850 0.386578
407.133850 0.386992
407.133850 0.387419
407.133850 0.387847
407.133850 0.388279
407.133850 0.388688
407.133850 0.389104
407.133850 0.389543
407.133850 0.389994
407.133850 0.390450
407.133850 0.390935
407.133850 0.391389
407.133850 0.391842
413.078125 0.387103
413.078125 0.387545
413.078125 0.388008
413.078125 0.388433
413.078125 0.388876
413.078125 0.389325
413.078125 0.389748
413.078125 0.390159
413.078125 0.390547
413.078125 0.390936
413.078125 0.391357
413.078125 0.391799
413.078125 0.392231
413.078125 0.392675
413.078125 0.393125
413.078125 0.393546
413.078125 0.393970
413.078125 0.394389
413.078125 0.394822
413.078125 0.395277
413.078125 0.395734
413.078125 0.396195
413.078125 0.396652
413.078125 0.397097
413.078125 0.397532
413.078125 0.397986
413.078125 0.398433
413.078125 0.398873
413.078125 0.399314
413.078125 0.399745
413.078125 0.400189
413.078125 0.400614
413.078125 0.401019
413.078125 0.401411
413.078125 0.401828
413.078125 0.402250
413.078125 0.402665
413.078125 0.403096
413.078125 0.403531
413.078125 0.403948
413.078125 0.404367
413.078125 0.404790
413.078125 0.405229
413.078125 0.405662
413.078125 0.406091
413.078125 0.406537
413.078125 0.406977
413.078125 0.407393
413.078125 0.407816
413.078125 0.408233
413.078125 0.408652
413.078125 0.409075
413.078125 0.409493
413.078125 0.409908
413.078125 0.410331
413.078125 0.410759
413.078125 0.411191
413.078125 0.411606
413.078125 0.412026
413.078125 0.412475
419.860474 0.400457
426.553833 0.398348
426.553833 0.398759
426.553833 0.399160
426.553833 0.399560
426.553833 0.399959
426.553833 0.400343
426.553833 0.400744
426.553833 0.401183
426.553833 0.401608
426.553833 0.402036
426.553833 0.402454
426.553833 0.402887
426.553833 0.403333
426.553833 0.403764
426.553833 0.404196
433.374054 0.400095
433.374054 0.400508
433.374054 0.400912
433.374054 0.401314
433.374054 0.401709
433.374054 0.402121
433.374054 0.402523
433.374054 0.402914
433.374054 0.403319
433.374054 0.403718
433.374054 0.404114
433.374054 0.404500
433.374054 0.404881
433.374054 0.405248
433.374054 0.405640
433.374054 0.406021
433.374054 0.406422
433.374054 0.406807
433.374054 0.407200
433.374054 0.407587
433.374054 0.407980
433.374054 0.408357
433.374054 0.408731
433.374054 0.409110
433.374054 0.409489
440.469696 0.407593
440.469696 0.407972
440.469696 0.408368
440.469696 0.408753
440.469696 0.409144
440.469696 0.409532
440.469696 0.409911
440.469696 0.410282
440.469696 0.410654
440.469696 0.411030
440.469696 0.411404
440.469696 0.411768
440.469696 0.412130
440.469696 0.412485
440.469696 0.412830
440.469696 0.413204
440.469696 0.413572
440.469696 0.413944
440.469696 0.414338
440.469696 0.414747
440.469696 0.415159
440.469696 0.415579
440.469696 0.416001
447.804504 0.407480
447.804504 0.407891
447.804504 0.408331
447.804504 0.408785
447.804504 0.409225
447.804504 0.409664
447.804504 0.410088
455.134338 0.408952
455.134338 0.409360
455.134338 0.409768
462.399994 0.405699
462.399994 0.406105
462.399994 0.406500
462.399994 0.406890
462.399994 0.407269
462.399994 0.407670
462.399994 0.408099
462.399994 0.408520
462.399994 0.408944
462.399994 0.409354
462.399994 0.409746
462.399994 0.410135
469.735291 0.406675
469.735291 0.407050
469.735291 0.407432
469.735291 0.407843
469.735291 0.408264
469.735291 0.408687
477.051086 0.407363
477.051086 0.407765
477.051086 0.408149
477.051086 0.408522
484.318848 0.406762
484.318848 0.407130
484.318848 0.407496
484.318848 0.407849
484.318848 0.408212
484.318848 0.408587
498.714294 0.406123
498.714294 0.406490
498.714294 0.406848
498.714294 0.407224
498.714294 0.407608
498.714294 0.407983
498.714294 0.408365
498.714294 0.408740
498.714294 0.409120
498.714294 0.409493
498.714294 0.409868
498.714294 0.410244
498.714294 0.410610
498.714294 0.410989
498.714294 0.411376
498.714294 0.411763
498.714294 0.412161
498.714294 0.412546
498.714294 0.412921
498.714294 0.413287
498.714294 0.413647
498.714294 0.414020
498.714294 0.414406
498.714294 0.414785
498.714294 0.415155
498.714294 0.415532
498.714294 0.415927
498.714294 0.416318
498.714294 0.416696
506.170227 0.412660
506.170227 0.413037
506.170227 0.413417
506.170227 0.413809
506.170227 0.414205
506.170227 0.414590
506.170227 0.414984
506.170227 0.415366
506.170227 0.415753
506.170227 0.416141
506.170227 0.416541
506.170227 0.416950
506.170227 0.417368
506.170227 0.417779
506.170227 0.418191
506.170227 0.418565
506.170227 0.418940
506.170227 0.419299
506.170227 0.419642
506.170227 0.419979
506.170227 0.420328
506.170227 0.420671
506.170227 0.421015
506.170227 0.421367
506.170227 0.421702
506.170227 0.422054
506.170227 0.422440
506.170227 0.422823
506.170227 0.423186
506.170227 0.423544
506.170227 0.423900
506.170227 0.424270
506.170227 0.424636
506.170227 0.424994
506.170227 0.425348
506.170227 0.425714
506.170227 0.426064
514.042236 0.421056
514.042236 0.421407
514.042236 0.421747
514.042236 0.422074
514.042236 0.422407
514.042236 0.422743
514.042236 0.423064
514.042236 0.423391
514.042236 0.423735
514.042236 0.424088
514.042236 0.424455
514.042236 0.424821
514.042236 0.425184
514.042236 0.425547
514.042236 0.425903
514.042236 0.426270
514.042236 0.426622
514.042236 0.426980
514.042236 0.427330
514.042236 0.427688
514.042236 0.428039
514.042236 0.428411
514.042236 0.428766
514.042236 0.429111
514.042236 0.429461
514.042236 0.429822
514.042236 0.430178
514.042236 0.430544
514.042236 0.430911
514.042236 0.431264
514.042236 0.431612
514.042236 0.431971
514.042236 0.432326
514.042236 0.432680
514.042236 0.433034
514.042236 0.433406
514.042236 0.433778
530.486084 0.430517
530.486084 0.430872
530.486084 0.431253
530.486084 0.431643
530.486084 0.432039
530.486084 0.432464
530.486084 0.432877
530.486084 0.433275
538.648254 0.432033
538.648254 0.432387
538.648254 0.432749
538.648254 0.433133
538.648254 0.433516
538.648254 0.433889
538.648254 0.434252
538.648254 0.434616
538.648254 0.434987
546.821899 0.426545
546.821899 0.426922
546.821899 0.427294
546.821899 0.427679
546.821899 0.428052
546.821899 0.428422
546.821899 0.428791
546.821899 0.429147
546.821899 0.429497
546.821899 0.429845
546.821899 0.430204
546.821899 0.430557
546.821899 0.430907
546.821899 0.431267
546.821899 0.431625
546.821899 0.431982
546.821899 0.432354
546.821899 0.432724
546.821899 0.433097
546.821899 0.433464
546.821899 0.433830
546.821899 0.434182
546.821899 0.434530
546.821899 0.434872
546.821899 0.435227
546.821899 0.435567
546.821899 0.435904
546.821899 0.436251
546.821899 0.436611
546.821899 0.436975
546.821899 0.437368
546.821899 0.437744
546.821899 0.438113
546.821899 0.438462
546.821899 0.438828
546.821899 0.439186
546.821899 0.439550
546.821899 0.439902
555.401367 0.437492
555.401367 0.437830
555.401367 0.438173
555.401367 0.438506
555.401367 0.438838
555.401367 0.439172
563.945923 0.433466
563.945923 0.433795
563.945923 0.434117
563.945923 0.434452
563.945923 0.434786
563.945923 0.435116
563.945923 0.435438
563.945923 0.435786
563.945923 0.436128
563.945923 0.436463
563.945923 0.436785
563.945923 0.437099
563.945923 0.437431
563.945923 0.437790
563.945923 0.438152
563.945923 0.438509
563.945923 0.438851
563.945923 0.439167
563.945923 0.439515
563.945923 0.439879
563.945923 0.440228
563.945923 0.440578
563.945923 0.440917
563.945923 0.441251
563.945923 0.441599
563.945923 0.441942
563.945923 0.442283
563.945923 0.442643
563.945923 0.443001
563.945923 0.443343
563.945923 0.443676
563.945923 0.444001
563.945923 0.444318
563.945923 0.444629
563.945923 0.444955
563.945923 0.445298
563.945923 0.445625
563.945923 0.445954
563.945923 0.446263
563.945923 0.446567
563.945923 0.446877
563.945923 0.447182
563.945923 0.447497
563.945923 0.447823
563.945923 0.448158
563.945923 0.448503
563.945923 0.448854
563.945923 0.449220
563.945923 0.449580
573.033569 0.447737
573.033569 0.448098
573.033569 0.448457
573.033569 0.448806
573.033569 0.449157
573.033569 0.449503
573.033569 0.449852
573.033569 0.450196
573.033569 0.450542
573.033569 0.450894
573.033569 0.451247
573.033569 0.451596
573.033569 0.451962
573.033569 0.452322
573.033569 0.452668
573.033569 0.453001
573.033569 0.453351
573.033569 0.453722
573.033569 0.454080
573.033569 0.454437
573.033569 0.454798
573.033569 0.455173
573.033569 0.455537
573.033569 0.455912
573.033569 0.456287
573.033569 0.456661
582.346680 0.455504
582.346680 0.455874
591.562927 0.454351
591.562927 0.454719
591.562927 0.455071
591.562927 0.455410
591.562927 0.455758
591.562927 0.456092
591.562927 0.456430
591.562927 0.456766
591.562927 0.457109
591.562927 0.457471
591.562927 0.457810
591.562927 0.458148
591.562927 0.458514
591.562927 0.458877
591.562927 0.459230
591.562927 0.459579
591.562927 0.459922
591.562927 0.460263
591.562927 0.460608
591.562927 0.460954
591.562927 0.461305
591.562927 0.461661
591.562927 0.462004
591.562927 0.462350
591.562927 0.462706
591.562927 0.463042
591.562927 0.463393
591.562927 0.463738
591.562927 0.464089
591.562927 0.464429
591.562927 0.464770
591.562927 0.465118
591.562927 0.465472
591.562927 0.465801
591.562927 0.466131
591.562927 0.466472
591.562927 0.466811
591.562927 0.467161
591.562927 0.467512
591.562927 0.467873
591.562927 0.468236
591.562927 0.468586
591.562927 0.468940
591.562927 0.469323
591.562927 0.469689
591.562927 0.470044
591.562927 0.470385
591.562927 0.470728
591.562927 0.471083
591.562927 0.471438
591.562927 0.471802
591.562927 0.472183
591.562927 0.472561
591.562927 0.472944
591.562927 0.473324
591.562927 0.473702
591.562927 0.474090
591.562927 0.474455
601.421082 0.471482
601.421082 0.471853
611.176453 0.465685
620.818176 0.464012
620.818176 0.464381
620.818176 0.464761
620.818176 0.465130
620.818176 0.465493
620.818176 0.465852
620.818176 0.466226
620.818176 0.466617
620.818176 0.466992
620.818176 0.467344
620.818176 0.467682
620.818176 0.468032
620.818176 0.468378
620.818176 0.468712
620.818176 0.469046
620.818176 0.469385
620.818176 0.469722
620.818176 0.470058
620.818176 0.470386
620.818176 0.470696
620.818176 0.471022
620.818176 0.471348
620.818176 0.471679
620.818176 0.472013
620.818176 0.472342
620.818176 0.472660
620.818176 0.472991
620.818176 0.473322
620.818176 0.473641
620.818176 0.473959
620.818176 0.474283
620.818176 0.474597
620.818176 0.474927
620.818176 0.475271
620.818176 0.475612
620.818176 0.475974
620.818176 0.476337
620.818176 0.476701
620.818176 0.477067
620.818176 0.477446
620.818176 0.477802
620.818176 0.478157
620.818176 0.478495
630.890320 0.476545
630.890320 0.476897
630.890320 0.477254
630.890320 0.477613
630.890320 0.477978
630.890320 0.478348
630.890320 0.478705
630.890320 0.479058
630.890320 0.479395
630.890320 0.479718
630.890320 0.480050
630.890320 0.480388
630.890320 0.480726
630.890320 0.481069
630.890320 0.481409
630.890320 0.481757
630.890320 0.482108
630.890320 0.482450
630.890320 0.482797
630.890320 0.483141
630.890320 0.483488
630.890320 0.483840
630.890320 0.484189
630.890320 0.484530
630.890320 0.484859
630.890320 0.485187
630.890320 0.485518
630.890320 0.485868
630.890320 0.486210
630.890320 0.486546
630.890320 0.486888
630.890320 0.487234
630.890320 0.487582
630.890320 0.487933
630.890320 0.488276
630.890320 0.488617
630.890320 0.488962
630.890320 0.489315
630.890320 0.489672
630.890320 0.490022
630.890320 0.490356
630.890320 0.490677
630.890320 0.491015
630.890320 0.491334
641.397461 0.485340
641.397461 0.485661
641.397461 0.485992
641.397461 0.486310
641.397461 0.486631
641.397461 0.486956
641.397461 0.487294
641.397461 0.487631
641.397461 0.487974
641.397461 0.488329
641.397461 0.488687
641.397461 0.489037
641.397461 0.489377
641.397461 0.489728
641.397461 0.490070
641.397461 0.490401
641.397461 0.490724
651.987244 0.486328
662.455688 0.483365
672.805054 0.476361
672.805054 0.476714
672.805054 0.477046
672.805054 0.477371
672.805054 0.477683
672.805054 0.478005
672.805054 0.478314
672.805054 0.478629
672.805054 0.478961
672.805054 0.479285
672.805054 0.479598
672.805054 0.479907
672.805054 0.480219
672.805054 0.480528
672.805054 0.480862
672.805054 0.481189
683.224976 0.475371
683.224976 0.475701
683.224976 0.476024
683.224976 0.476342
683.224976 0.476650
683.224976 0.476952
683.224976 0.477255
683.224976 0.477585
683.224976 0.477904
683.224976 0.478205
683.224976 0.478520
683.224976 0.478843
683.224976 0.479167
683.224976 0.479496
683.224976 0.479846
683.224976 0.480206
683.224976 0.480549
683.224976 0.480885
683.224976 0.481219
683.224976 0.481554
683.224976 0.481889
683.224976 0.482219
693.788818 0.480828
693.788818 0.481156
693.788818 0.481479
693.788818 0.481796
693.788818 0.482105
693.788818 0.482419
693.788818 0.482737
693.788818 0.483051
693.788818 0.483364
693.788818 0.483694
693.788818 0.484023
693.788818 0.484331
693.788818 0.484658
693.788818 0.484961
693.788818 0.485262
693.788818 0.485562
693.788818 0.485859
693.788818 0.486166
693.788818 0.486485
693.788818 0.486799
693.788818 0.487119
693.788818 0.487448
693.788818 0.487765
693.788818 0.488092
693.788818 0.488437
693.788818 0.488769
693.788818 0.489095
693.788818 0.489427
693.788818 0.489758
693.788818 0.490093
693.788818 0.490419
693.788818 0.490731
693.788818 0.491031
693.788818 0.491344
693.788818 0.491645
693.788818 0.491947
693.788818 0.492249
693.788818 0.492572
693.788818 0.492889
693.788818 0.493215
693.788818 0.493543
693.788818 0.493879
693.788818 0.494204
693.788818 0.494526
693.788818 0.494864
693.788818 0.495190
693.788818 0.495529
693.788818 0.495868
693.788818 0.496197
693.788818 0.496535
693.788818 0.496876
693.788818 0.497223
693.788818 0.497559
693.788818 0.497893
693.788818 0.498217
693.788818 0.498532
693.788818 0.498848
693.788818 0.499150
693.788818 0.499479
693.788818 0.499797
693.788818 0.500130
693.788818 0.500454
693.788818 0.500762
693.788818 0.501071
693.788818 0.501371
693.788818 0.501681
693.788818 0.501978
693.788818 0.502294
693.788818 0.502617
693.788818 0.502943
693.788818 0.503259
693.788818 0.503580
693.788818 0.503878
705.123474 0.501639
705.123474 0.501927
705.123474 0.502236
705.123474 0.502549
705.123474 0.502853
705.123474 0.503169
705.123474 0.503477
705.123474 0.503806
705.123474 0.504134
705.123474 0.504469
705.123474 0.504810
705.123474 0.505163
705.123474 0.505511
705.123474 0.505865
705.123474 0.506221
716.503052 0.498138
716.503052 0.498493
716.503052 0.498858
716.503052 0.499211
716.503052 0.499557
716.503052 0.499885
716.503052 0.500223
716.503052 0.500552
716.503052 0.500876
716.503052 0.501196
716.503052 0.501493
716.503052 0.501780
716.503052 0.502091
716.503052 0.502398
716.503052 0.502710
716.503052 0.503023
716.503052 0.503347
716.503052 0.503674
727.963440 0.500383
727.963440 0.500711
739.309082 0.500074
739.309082 0.500406
739.309082 0.500714
739.309082 0.501027
739.309082 0.501349
739.309082 0.501653
739.309082 0.501971
739.309082 0.502292
739.309082 0.502616
739.309082 0.502937
739.309082 0.503252
739.309082 0.503566
739.309082 0.503881
739.309082 0.504220
739.309082 0.504554
739.309082 0.504892
739.309082 0.505241
739.309082 0.505588
739.309082 0.505941
739.309082 0.506295
739.309082 0.506649
739.309082 0.506994
739.309082 0.507323
739.309082 0.507658
739.309082 0.507995
739.309082 0.508327
739.309082 0.508658
739.309082 0.508989
739.309082 0.509332
739.309082 0.509666
739.309082 0.509983
739.309082 0.510306
739.309082 0.510634
739.309082 0.510955
739.309082 0.511276
739.309082 0.511597
739.309082 0.511911
739.309082 0.512220
739.309082 0.512535
739.309082 0.512845
739.309082 0.513169
739.309082 0.513488
739.309082 0.513819
739.309082 0.514151
739.309082 0.514486
739.309082 0.514823
739.309082 0.515158
739.309082 0.515478
739.309082 0.515799
739.309082 0.516122
739.309082 0.516433
739.309082 0.516754
739.309082 0.517076
739.309082 0.517396
739.309082 0.517705
739.309082 0.518020
739.309082 0.518328
739.309082 0.518628
739.309082 0.518928
739.309082 0.519249
739.309082 0.519567
739.309082 0.519893
739.309082 0.520221
739.309082 0.520547
739.309082 0.520869
739.309082 0.521191
739.309082 0.521510
739.309082 0.521825
739.309082 0.522126
739.309082 0.522420
739.309082 0.522709
739.309082 0.523003
739.309082 0.523313
739.309082 0.523617
739.309082 0.523942
739.309082 0.524307
739.309082 0.524669
739.309082 0.525032
739.309082 0.525377
739.309082 0.525723
751.481934 0.516590
751.481934 0.516941
751.481934 0.517281
751.481934 0.517616
751.481934 0.517950
751.481934 0.518274
751.481934 0.518592
751.481934 0.518915
751.481934 0.519224
751.481934 0.519525
751.481934 0.519820
751.481934 0.520122
751.481934 0.520426
751.481934 0.520749
763.676636 0.518520
763.676636 0.518838
763.676636 0.519155
763.676636 0.519463
763.676636 0.519769
763.676636 0.520069
763.676636 0.520365
763.676636 0.520669
763.676636 0.520991
763.676636 0.521294
763.676636 0.521598
763.676636 0.521901
763.676636 0.522201
763.676636 0.522510
763.676636 0.522817
763.676636 0.523124
763.676636 0.523418
763.676636 0.523725
763.676636 0.524032
775.952393 0.516851
775.952393 0.517159
775.952393 0.517470
775.952393 0.517790
775.952393 0.518099
775.952393 0.518406
775.952393 0.518706
775.952393 0.518996
775.952393 0.519287
775.952393 0.519583
775.952393 0.519893
775.952393 0.520203
775.952393 0.520518
788.236694 0.517284
788.236694 0.517594
788.236694 0.517923
788.236694 0.518235
788.236694 0.518526
788.236694 0.518825
788.236694 0.519123
788.236694 0.519421
788.236694 0.519718
788.236694 0.520030
788.236694 0.520344
788.236694 0.520656
800.517639 0.517253
800.517639 0.517562
800.517639 0.517853
800.517639 0.518143
800.517639 0.518421
800.517639 0.518707
800.517639 0.518990
800.517639 0.519271
800.517639 0.519558
800.517639 0.519844
800.517639 0.520117
800.517639 0.520393
800.517639 0.520674
800.517639 0.520957
800.517639 0.521245
800.517639 0.521530
800.517639 0.521815
800.517639 0.522094
800.517639 0.522373
800.517639 0.522636
800.517639 0.522898
800.517639 0.523191
800.517639 0.523473
800.517639 0.523751
800.517639 0.524047
800.517639 0.524357
800.517639 0.524657
800.517639 0.524970
800.517639 0.525273
800.517639 0.525560
800.517639 0.525844
800.517639 0.526144
800.517639 0.526450
800.517639 0.526761
800.517639 0.527067
800.517639 0.527374
800.517639 0.527674
800.517639 0.527975
800.517639 0.528279
800.517639 0.528591
800.517639 0.528893
800.517639 0.529193
800.517639 0.529487
800.517639 0.529772
800.517639 0.530052
800.517639 0.530334
800.517639 0.530612
800.517639 0.530882
800.517639 0.531150
800.517639 0.531430
800.517639 0.531717
800.517639 0.532005
800.517639 0.532293
800.517639 0.532572
800.517639 0.532856
800.517639 0.533154
800.517639 0.533470
800.517639 0.533780
800.517639 0.534065
800.517639 0.534366
800.517639 0.534690
800.517639 0.535003
800.517639 0.535316
800.517639 0.535630
800.517639 0.535951
800.517639 0.536291
800.517639 0.536619
800.517639 0.536949
800.517639 0.537275
800.517639 0.537602
800.517639 0.537922
800.517639 0.538248
800.517639 0.538571
800.517639 0.538884
800.517639 0.539183
800.517639 0.539479
800.517639 0.539791
800.517639 0.540102
800.517639 0.540403
800.517639 0.540697
800.517639 0.540987
800.517639 0.541274
813.614014 0.537317
813.614014 0.537586
813.614014 0.537874
813.614014 0.538148
813.614014 0.538423
813.614014 0.538699
813.614014 0.538985
813.614014 0.539283
813.614014 0.539578
813.614014 0.539868
813.614014 0.540163
813.614014 0.540443
813.614014 0.540717
813.614014 0.541001
813.614014 0.541292
813.614014 0.541589
813.614014 0.541882
813.614014 0.542167
813.614014 0.542461
813.614014 0.542748
813.614014 0.543033
813.614014 0.543323
813.614014 0.543621
813.614014 0.543917
813.614014 0.544217
813.614014 0.544504
813.614014 0.544789
813.614014 0.545074
813.614014 0.545362
813.614014 0.545647
813.614014 0.545933
813.614014 0.546234
813.614014 0.546543
813.614014 0.546870
813.614014 0.547188
813.614014 0.547521
813.614014 0.547842
813.614014 0.548144
827.000000 0.543275
827.000000 0.543579
827.000000 0.543876
827.000000 0.544171
827.000000 0.544462
840.289001 0.541009
840.289001 0.541304
840.289001 0.541602
840.289001 0.541893
840.289001 0.542184
840.289001 0.542478
840.289001 0.542776
840.289001 0.543077
840.289001 0.543368
840.289001 0.543665
840.289001 0.543975
840.289001 0.544293
840.289001 0.544620
840.289001 0.544934
840.289001 0.545244
840.289001 0.545565
840.289001 0.545892
840.289001 0.546202
840.289001 0.546512
840.289001 0.546831
840.289001 0.547143
840.289001 0.547453
840.289001 0.547767
840.289001 0.548084
840.289001 0.548381
840.289001 0.548678
840.289001 0.548988
840.289001 0.549307
840.289001 0.549613
840.289001 0.549901
840.289001 0.550175
840.289001 0.550465
840.289001 0.550752
840.289001 0.551027
840.289001 0.551313
840.289001 0.551586
840.289001 0.551876
840.289001 0.552159
840.289001 0.552441
840.289001 0.552729
840.289001 0.553018
840.289001 0.553314
840.289001 0.553615
840.289001 0.553912
840.289001 0.554207
840.289001 0.554494
840.289001 0.554793
840.289001 0.555080
840.289001 0.555357
840.289001 0.555639
854.000000 0.552154
854.000000 0.552427
854.000000 0.552698
854.000000 0.552978
854.000000 0.553259
854.000000 0.553545
854.000000 0.553825
854.000000 0.554113
854.000000 0.554402
854.000000 0.554697
854.000000 0.555006
854.000000 0.555312
854.000000 0.555622
854.000000 0.555918
854.000000 0.556214
854.000000 0.556499
854.000000 0.556785
854.000000 0.557065
854.000000 0.557346
854.000000 0.557632
854.000000 0.557931
854.000000 0.558226
854.000000 0.558514
854.000000 0.558803
854.000000 0.559087
854.000000 0.559376
854.000000 0.559675
854.000000 0.559963
854.000000 0.560246
854.000000 0.560527
854.000000 0.560829
854.000000 0.561129
854.000000 0.561428
854.000000 0.561733
854.000000 0.562033
854.000000 0.562321
854.000000 0.562608
854.000000 0.562899
854.000000 0.563185
854.000000 0.563467
854.000000 0.563742
854.000000 0.564019
854.000000 0.564302
854.000000 0.564598
854.000000 0.564911
854.000000 0.565219
854.000000 0.565515
854.000000 0.565814
868.102844 0.549067
868.102844 0.549361
868.102844 0.549663
868.102844 0.549960
868.102844 0.550248
868.102844 0.550536
868.102844 0.550823
868.102844 0.551105
868.102844 0.551406
868.102844 0.551729
868.102844 0.552046
868.102844 0.552359
868.102844 0.552663
868.102844 0.552966
868.102844 0.553279
868.102844 0.553577
868.102844 0.553861
868.102844 0.554134
868.102844 0.554401
868.102844 0.554663
868.102844 0.554917
868.102844 0.555171
868.102844 0.555435
868.102844 0.555695
868.102844 0.555955
868.102844 0.556229
868.102844 0.556518
868.102844 0.556831
868.102844 0.557135
868.102844 0.557454
868.102844 0.557749
868.102844 0.558046
868.102844 0.558339
868.102844 0.558635
882.431824 0.552949
882.431824 0.553223
882.431824 0.553521
882.431824 0.553797
882.431824 0.554064
882.431824 0.554346
882.431824 0.554644
882.431824 0.554935
882.431824 0.555227
882.431824 0.555536
882.431824 0.555830
882.431824 0.556115
882.431824 0.556403
882.431824 0.556692
882.431824 0.556992
882.431824 0.557287
882.431824 0.557600
882.431824 0.557913
882.431824 0.558204
882.431824 0.558517
882.431824 0.558815
882.431824 0.559131
882.431824 0.559435
882.431824 0.559734
882.431824 0.560034
882.431824 0.560337
882.431824 0.560647
882.431824 0.560963
882.431824 0.561271
882.431824 0.561587
882.431824 0.561901
882.431824 0.562211
882.431824 0.562530
882.431824 0.562854
896.983032 0.562259
896.983032 0.562572
896.983032 0.562868
896.983032 0.563174
911.415710 0.555759
911.415710 0.556053
911.415710 0.556366
911.415710 0.556678
911.415710 0.556981
911.415710 0.557307
925.754211 0.552631
925.754211 0.552932
925.754211 0.553231
925.754211 0.553527
925.754211 0.553825
925.754211 0.554115
925.754211 0.554407
925.754211 0.554703
925.754211 0.554988
925.754211 0.555299
925.754211 0.555624
925.754211 0.555940
925.754211 0.556258
925.754211 0.556579
925.754211 0.556924
925.754211 0.557256
925.754211 0.557579
925.754211 0.557903
925.754211 0.558209
925.754211 0.558504
925.754211 0.558791
925.754211 0.559085
925.754211 0.559375
925.754211 0.559678
925.754211 0.559977
925.754211 0.560270
925.754211 0.560574
925.754211 0.560884
925.754211 0.561187
925.754211 0.561502
925.754211 0.561828
925.754211 0.562135
925.754211 0.562432
925.754211 0.562734
925.754211 0.563048
925.754211 0.563356
925.754211 0.563659
925.754211 0.563951
925.754211 0.564239
925.754211 0.564532
925.754211 0.564829
925.754211 0.565131
925.754211 0.565443
925.754211 0.565752
925.754211 0.566051
925.754211 0.566339
925.754211 0.566619
925.754211 0.566900
925.754211 0.567184
925.754211 0.567467
925.754211 0.567742
925.754211 0.568016
925.754211 0.568281
925.754211 0.568549
925.754211 0.568827
925.754211 0.569105
925.754211 0.569387
925.754211 0.569660
925.754211 0.569937
925.754211 0.570214
925.754211 0.570484
925.754211 0.570754
925.754211 0.571041
925.754211 0.571337
925.754211 0.571634
925.754211 0.571943
925.754211 0.572250
925.754211 0.572574
925.754211 0.572881
925.754211 0.573198
925.754211 0.573502
925.754211 0.573796
925.754211 0.574097
925.754211 0.574388
925.754211 0.574686
925.754211 0.574991
925.754211 0.575303
925.754211 0.575632
925.754211 0.575979
925.754211 0.576309
925.754211 0.576625
925.754211 0.576946
925.754211 0.577256
925.754211 0.577565
925.754211 0.577868
925.754211 0.578184
925.754211 0.578484
925.754211 0.578792
925.754211 0.579097
925.754211 0.579398
925.754211 0.579696
925.754211 0.579992
925.754211 0.580292
925.754211 0.580609
940.977783 0.579565
940.977783 0.579876
940.977783 0.580190
940.977783 0.580510
940.977783 0.580846
940.977783 0.581200
940.977783 0.581550
940.977783 0.581892
956.121521 0.579264
956.121521 0.579573
971.120850 0.578651
971.120850 0.578955
971.120850 0.579254
971.120850 0.579547
971.120850 0.579824
971.120850 0.580103
971.120850 0.580380
971.120850 0.580659
986.043701 0.577254
986.043701 0.577541
986.043701 0.577819
986.043701 0.578116
986.043701 0.578415
986.043701 0.578713
986.043701 0.579017
986.043701 0.579324
986.043701 0.579620
986.043701 0.579907
986.043701 0.580185
986.043701 0.580465
986.043701 0.580748
986.043701 0.581033
986.043701 0.581310
986.043701 0.581590
986.043701 0.581884
986.043701 0.582178
986.043701 0.582456
986.043701 0.582756
1001.021729 0.578238
1001.021729 0.578531
1001.021729 0.578817
1001.021729 0.579105
1001.021729 0.579395
1001.021729 0.579679
1001.021729 0.579965
1001.021729 0.580247
1001.021729 0.580536
1001.021729 0.580811
1001.021729 0.581094
1001.021729 0.581380
1001.021729 0.581671
1001.021729 0.581953
1001.021729 0.582256
1001.021729 0.582570
1001.021729 0.582862
1001.021729 0.583151
1016.032410 0.575702
1016.032410 0.575982
1016.032410 0.576259
1016.032410 0.576559
1016.032410 0.576858
1016.032410 0.577163
1016.032410 0.577462
1016.032410 0.577765
1016.032410 0.578053
1016.032410 0.578337
1016.032410 0.578620
1016.032410 0.578905
1016.032410 0.579198
1016.032410 0.579489
1045.871704 0.574054
1045.871704 0.574344
1045.871704 0.574633
1045.871704 0.574908
1045.871704 0.575187
1045.871704 0.575470
1045.871704 0.575755
1045.871704 0.576033
1045.871704 0.576308
1045.871704 0.576586
1045.871704 0.576867
1045.871704 0.577151
1045.871704 0.577429
1045.871704 0.577717
1045.871704 0.578005
1045.871704 0.578294
1045.871704 0.578573
1045.871704 0.578850
1045.871704 0.579131
1045.871704 0.579412
1045.871704 0.579690
1045.871704 0.579960
1045.871704 0.580244
1045.871704 0.580524
1045.871704 0.580798
1045.871704 0.581079
1045.871704 0.581371
1045.871704 0.581660
1045.871704 0.581943
1045.871704 0.582226
1045.871704 0.582515
1045.871704 0.582800
1045.871704 0.583070
1045.871704 0.583346
1045.871704 0.583622
1045.871704 0.583894
1045.871704 0.584169
1045.871704 0.584426
1045.871704 0.584684
1045.871704 0.584938
1045.871704 0.585196
1060.989380 0.577182
1060.989380 0.577487
1060.989380 0.577779
1060.989380 0.578064
1060.989380 0.578335
1060.989380 0.578606
1060.989380 0.578884
1060.989380 0.579155
1060.989380 0.579436
1060.989380 0.579736
1060.989380 0.580028
1060.989380 0.580311
1060.989380 0.580582
1060.989380 0.580838
1060.989380 0.581106
1060.989380 0.581369
1060.989380 0.581632
1060.989380 0.581891
1060.989380 0.582165
1060.989380 0.582434
1060.989380 0.582697
1060.989380 0.582963
1060.989380 0.583227
1060.989380 0.583519
1060.989380 0.583796
1060.989380 0.584075
1060.989380 0.584344
1060.989380 0.584605
1060.989380 0.584881
1076.254028 0.574153
1076.254028 0.574408
1076.254028 0.574673
1076.254028 0.574942
1076.254028 0.575205
1076.254028 0.575481
1076.254028 0.575747
1076.254028 0.576028
1076.254028 0.576319
1076.254028 0.576606
1091.463135 0.574482
1091.463135 0.574743
1091.463135 0.574998
1091.463135 0.575256
1091.463135 0.575503
1091.463135 0.575759
1091.463135 0.576032
1091.463135 0.576304
1091.463135 0.576582
1091.463135 0.576848
1091.463135 0.577119
1091.463135 0.577399
1091.463135 0.577690
1091.463135 0.577975
1091.463135 0.578254
1091.463135 0.578520
1091.463135 0.578786
1091.463135 0.579056
1091.463135 0.579329
1106.712036 0.571886
1106.712036 0.572162
1106.712036 0.572428
1106.712036 0.572705
1106.712036 0.572975
1106.712036 0.573255
1106.712036 0.573538
1106.712036 0.573819
1106.712036 0.574096
1106.712036 0.574381
1106.712036 0.574676
1106.712036 0.574956
1106.712036 0.575262
1106.712036 0.575572
1106.712036 0.575871
1106.712036 0.576174
1106.712036 0.576470
1106.712036 0.576767
1106.712036 0.577076
1106.712036 0.577382
1106.712036 0.577690
1106.712036 0.577987
1106.712036 0.578273
1106.712036 0.578563
1106.712036 0.578847
1106.712036 0.579135
1106.712036 0.579427
1106.712036 0.579711
1106.712036 0.579990
1106.712036 0.580270
1106.712036 0.580549
1106.712036 0.580834
1106.712036 0.581123
1106.712036 0.581429
1106.712036 0.581733
1106.712036 0.582031
1106.712036 0.582319
1106.712036 0.582609
1106.712036 0.582905
1106.712036 0.583202
1106.712036 0.583496
1106.712036 0.583779
1106.712036 0.584061
1106.712036 0.584357
1106.712036 0.584657
1106.712036 0.584951
1106.712036 0.585239
1106.712036 0.585527
1106.712036 0.585818
1106.712036 0.586111
1106.712036 0.586406
1106.712036 0.586691
1106.712036 0.586995
1106.712036 0.587297
1106.712036 0.587588
1106.712036 0.587874
1106.712036 0.588149
1106.712036 0.588425
1106.712036 0.588705
1106.712036 0.588967
1106.712036 0.589226
1106.712036 0.589505
1106.712036 0.589806
1106.712036 0.590110
1106.712036 0.590417
1106.712036 0.590714
1106.712036 0.591001
1106.712036 0.591292
1106.712036 0.591576
1106.712036 0.591861
1106.712036 0.592142
1106.712036 0.592427
1106.712036 0.592701
1106.712036 0.592991
1106.712036 0.593276
1106.712036 0.593560
1106.712036 0.593857
1106.712036 0.594135
1106.712036 0.594403
1106.712036 0.594663
1106.712036 0.594913
1106.712036 0.595185
1106.712036 0.595455
1106.712036 0.595726
1106.712036 0.595994
1106.712036 0.596263
1106.712036 0.596525
1106.712036 0.596800
1106.712036 0.597085
1106.712036 0.597357
1122.739624 0.590517
1122.739624 0.590798
1122.739624 0.591082
1122.739624 0.591364
1122.739624 0.591638
1122.739624 0.591919
1122.739624 0.592188
1138.673584 0.591166
1154.453613 0.590292
1154.453613 0.590589
1154.453613 0.590892
1154.453613 0.591190
1154.453613 0.591471
1154.453613 0.591753
1154.453613 0.592029
1170.143555 0.581950
1170.143555 0.582214
1170.143555 0.582478
1170.143555 0.582733
1170.143555 0.582975
1170.143555 0.583202
1170.143555 0.583441
1170.143555 0.583684
1170.143555 0.583939
1185.765259 0.582822
1185.765259 0.583084
1185.765259 0.583345
1185.765259 0.583600
1185.765259 0.583858
1185.765259 0.584116
1185.765259 0.584381
1185.765259 0.584659
1185.765259 0.584939
1185.765259 0.585220
1185.765259 0.585500
1185.765259 0.585771
1185.765259 0.586038
1185.765259 0.586309
1185.765259 0.586579
1185.765259 0.586837
1185.765259 0.587116
1185.765259 0.587381
1185.765259 0.587656
1185.765259 0.587927
1185.765259 0.588193
1185.765259 0.588477
1185.765259 0.588761
1185.765259 0.589036
1185.765259 0.589310
1185.765259 0.589587
1185.765259 0.589857
1185.765259 0.590123
1185.765259 0.590387
1185.765259 0.590647
1185.765259 0.590906
1185.765259 0.591165
1185.765259 0.591410
1185.765259 0.591649
1185.765259 0.591897
1185.765259 0.592146
1185.765259 0.592396
1185.765259 0.592645
1185.765259 0.592896
1185.765259 0.593153
1185.765259 0.593408
1185.765259 0.593659
1185.765259 0.593919
1185.765259 0.594167
1185.765259 0.594421
1185.765259 0.594664
1185.765259 0.594913
1201.705566 0.590455
1201.705566 0.590700
1201.705566 0.590942
1201.705566 0.591209
1201.705566 0.591474
1201.705566 0.591742
1201.705566 0.592006
1201.705566 0.592271
1201.705566 0.592531
1201.705566 0.592811
1201.705566 0.593088
1201.705566 0.593370
1201.705566 0.593642
1201.705566 0.593901
1201.705566 0.594164
1201.705566 0.594428
1201.705566 0.594701
1201.705566 0.594976
1201.705566 0.595245
1201.705566 0.595509
1201.705566 0.595766
1201.705566 0.596019
1201.705566 0.596272
1201.705566 0.596527
1201.705566 0.596779
1201.705566 0.597041
1201.705566 0.597306
1201.705566 0.597575
1201.705566 0.597852
1201.705566 0.598162
1201.705566 0.598465
1201.705566 0.598772
1201.705566 0.599074
1201.705566 0.599359
1201.705566 0.599650
1201.705566 0.599927
1201.705566 0.600195
1201.705566 0.600465
1201.705566 0.600740
1201.705566 0.601020
1201.705566 0.601296
1217.899048 0.596070
1217.899048 0.596353
1217.899048 0.596629
1217.899048 0.596912
1233.969849 0.595744
1233.969849 0.596007
1233.969849 0.596267
1233.969849 0.596538
1233.969849 0.596804
1233.969849 0.597089
1233.969849 0.597383
1233.969849 0.597672
1233.969849 0.597953
1233.969849 0.598226
1233.969849 0.598494
1233.969849 0.598768
1233.969849 0.599039
1233.969849 0.599304
1233.969849 0.599567
1233.969849 0.599833
1233.969849 0.600093
1233.969849 0.600356
1233.969849 0.600609
1233.969849 0.600869
1233.969849 0.601147
1233.969849 0.601425
1233.969849 0.601730
1233.969849 0.602039
1233.969849 0.602356
1233.969849 0.602664
1233.969849 0.602965
1233.969849 0.603263
1233.969849 0.603565
1233.969849 0.603858
1233.969849 0.604152
1233.969849 0.604445
1233.969849 0.604731
1233.969849 0.605013
1233.969849 0.605305
1233.969849 0.605597
1233.969849 0.605888
1233.969849 0.606177
1233.969849 0.606450
1233.969849 0.606737
1233.969849 0.607014
1233.969849 0.607282
1233.969849 0.607541
1233.969849 0.607807
1233.969849 0.608068
1233.969849 0.608332
1233.969849 0.608598
1233.969849 0.608855
1233.969849 0.609117
1233.969849 0.609397
1233.969849 0.609670
1233.969849 0.609931
1233.969849 0.610186
1233.969849 0.610452
1233.969849 0.610722
1233.969849 0.610996
1233.969849 0.611271
1233.969849 0.611532
1233.969849 0.611791
1233.969849 0.612044
1233.969849 0.612306
1233.969849 0.612565
1233.969849 0.612819
1233.969849 0.613075
1233.969849 0.613326
1233.969849 0.613594
1233.969849 0.613878
1233.969849 0.614143
1233.969849 0.614411
1233.969849 0.614667
1233.969849 0.614932
1233.969849 0.615202
1233.969849 0.615485
1233.969849 0.615770
1233.969849 0.616059
1233.969849 0.616357
1233.969849 0.616659
1233.969849 0.616962
1233.969849 0.617260
1233.969849 0.617569
1233.969849 0.617864
1233.969849 0.618158
1250.699951 0.617410
1250.699951 0.617706
1250.699951 0.617999
1250.699951 0.618285
1250.699951 0.618559
1250.699951 0.618834
1267.323364 0.607560
1267.323364 0.607845
1267.323364 0.608123
1267.323364 0.608405
1267.323364 0.608689
1267.323364 0.608977
1267.323364 0.609264
1267.323364 0.609537
1267.323364 0.609805
1267.323364 0.610083
1267.323364 0.610367
1267.323364 0.610656
1267.323364 0.610928
1267.323364 0.611192
1267.323364 0.611465
1267.323364 0.611740
1267.323364 0.612001
1267.323364 0.612259
1267.323364 0.612518
1267.323364 0.612779
1267.323364 0.613036
1267.323364 0.613289
1267.323364 0.613547
1267.323364 0.613815
1267.323364 0.614076
1267.323364 0.614345
1267.323364 0.614621
1267.323364 0.614898
1267.323364 0.615166
1267.323364 0.615430
1267.323364 0.615705
1267.323364 0.615982
1267.323364 0.616256
1267.323364 0.616518
1267.323364 0.616776
1267.323364 0.617038
1267.323364 0.617302
1267.323364 0.617557
1267.323364 0.617803
1267.323364 0.618056
1267.323364 0.618305
1267.323364 0.618548
1267.323364 0.618789
1267.323364 0.619040
1267.323364 0.619297
1267.323364 0.619563
1267.323364 0.619831
1267.323364 0.620104
1267.323364 0.620376
1267.323364 0.620668
1267.323364 0.620957
1267.323364 0.621252
1267.323364 0.621544
1267.323364 0.621852
1267.323364 0.622155
1267.323364 0.622438
1267.323364 0.622726
1267.323364 0.622997
1267.323364 0.623264
1267.323364 0.623543
1267.323364 0.623817
1267.323364 0.624089
1267.323364 0.624350
1267.323364 0.624604
1267.323364 0.624859
1267.323364 0.625114
1267.323364 0.625370
1267.323364 0.625657
1267.323364 0.625958
1267.323364 0.626258
1267.323364 0.626544
1267.323364 0.626829
1267.323364 0.627120
1267.323364 0.627408
1267.323364 0.627697
1267.323364 0.627967
1267.323364 0.628246
1267.323364 0.628531
1267.323364 0.628821
1267.323364 0.629116
1267.323364 0.629401
1267.323364 0.629674
1267.323364 0.629950
1267.323364 0.630217
1267.323364 0.630487
1267.323364 0.630762
1267.323364 0.631048
1267.323364 0.631325
1267.323364 0.631593
1267.323364 0.631871
1267.323364 0.632156
1267.323364 0.632440
1267.323364 0.632710
1267.323364 0.633002
1284.712891 0.627309
1284.712891 0.627597
1284.712891 0.627884
1284.712891 0.628161
1284.712891 0.628430
1284.712891 0.628693
1284.712891 0.628964
1284.712891 0.629231
1302.009888 0.621176
1302.009888 0.621434
1302.009888 0.621695
1302.009888 0.621954
1302.009888 0.622200
1302.009888 0.622443
1302.009888 0.622700
1302.009888 0.622961
1302.009888 0.623214
1302.009888 0.623452
1302.009888 0.623689
1302.009888 0.623926
1302.009888 0.624176
1302.009888 0.624430
1302.009888 0.624697
1302.009888 0.624968
1302.009888 0.625232
1302.009888 0.625491
1302.009888 0.625759
1302.009888 0.626029
1302.009888 0.626319
1302.009888 0.626601
1302.009888 0.626878
1302.009888 0.627149
1302.009888 0.627426
1302.009888 0.627689
1302.009888 0.627944
1302.009888 0.628225
1302.009888 0.628508
1302.009888 0.628784
1302.009888 0.629073
1302.009888 0.629365
1302.009888 0.629647
1319.460815 0.618291
1319.460815 0.618567
1319.460815 0.618853
1319.460815 0.619124
1319.460815 0.619398
1319.460815 0.619665
1319.460815 0.619923
1319.460815 0.620183
1319.460815 0.620451
1319.460815 0.620703
1319.460815 0.620964
1319.460815 0.621231
1319.460815 0.621487
1319.460815 0.621743
1319.460815 0.622012
1319.460815 0.622282
1319.460815 0.622555
1319.460815 0.622829
1319.460815 0.623097
1319.460815 0.623375
1319.460815 0.623647
1319.460815 0.623915
1319.460815 0.624186
1319.460815 0.624437
1319.460815 0.624689
1319.460815 0.624945
1319.460815 0.625213
1319.460815 0.625500
1319.460815 0.625791
1319.460815 0.626082
1319.460815 0.626358
1319.460815 0.626648
1319.460815 0.626933
1319.460815 0.627225
1319.460815 0.627519
1319.460815 0.627822
1319.460815 0.628119
1319.460815 0.628416
1319.460815 0.628719
1319.460815 0.629015
1319.460815 0.629296
1319.460815 0.629565
1319.460815 0.629837
1319.460815 0.630118
1319.460815 0.630425
1319.460815 0.630724
1319.460815 0.631028
1319.460815 0.631323
1319.460815 0.631609
1319.460815 0.631897
1319.460815 0.632191
1319.460815 0.632493
1319.460815 0.632812
1319.460815 0.633115
1319.460815 0.633413
1319.460815 0.633698
1319.460815 0.633963
1319.460815 0.634228
1319.460815 0.634483
1319.460815 0.634746
1319.460815 0.635028
1319.460815 0.635305
1319.460815 0.635605
1319.460815 0.635891
1319.460815 0.636178
1319.460815 0.636472
1319.460815 0.636778
1319.460815 0.637088
1319.460815 0.637393
1319.460815 0.637678
1319.460815 0.637958
1319.460815 0.638221
1319.460815 0.638497
1319.460815 0.638774
1319.460815 0.639063
1319.460815 0.639351
1319.460815 0.639619
1319.460815 0.639885
1319.460815 0.640134
1319.460815 0.640392
1319.460815 0.640664
1319.460815 0.640930
1319.460815 0.641184
1319.460815 0.641464
1319.460815 0.641734
1319.460815 0.642015
1319.460815 0.642317
1319.460815 0.642605
1319.460815 0.642886
1319.460815 0.643180
1319.460815 0.643457
1319.460815 0.643725
1319.460815 0.643974
1319.460815 0.644231
1319.460815 0.644485
1319.460815 0.644733
1319.460815 0.644977
1319.460815 0.645233
1319.460815 0.645523
1319.460815 0.645813
1319.460815 0.646079
1319.460815 0.646351
1319.460815 0.646633
1319.460815 0.646907
1319.460815 0.647180
1319.460815 0.647456
1319.460815 0.647719
1319.460815 0.647993
1319.460815 0.648257
1337.804932 0.641522
1337.804932 0.641781
1337.804932 0.642049
1356.000000 0.629280
1356.000000 0.629558
1356.000000 0.629849
1356.000000 0.630131
1356.000000 0.630404
1356.000000 0.630671
1356.000000 0.630940
1356.000000 0.631196
1356.000000 0.631461
1356.000000 0.631734
1356.000000 0.632025
1356.000000 0.632304
1356.000000 0.632573
1356.000000 0.632826
1356.000000 0.633089
1356.000000 0.633361
1356.000000 0.633620
1356.000000 0.633870
1356.000000 0.634125
1356.000000 0.634377
1356.000000 0.634644
1356.000000 0.634922
1356.000000 0.635201
1356.000000 0.635487
1356.000000 0.635757
1356.000000 0.636034
1374.270508 0.633974
1374.270508 0.634258
1374.270508 0.634539
1374.270508 0.634826
1374.270508 0.635105
1374.270508 0.635386
1374.270508 0.635659
1374.270508 0.635937
1374.270508 0.636224
1374.270508 0.636502
1374.270508 0.636772
1374.270508 0.637037
1374.270508 0.637310
1374.270508 0.637572
1374.270508 0.637838
1374.270508 0.638097
1374.270508 0.638369
1392.528809 0.632770
1392.528809 0.633039
1392.528809 0.633302
1392.528809 0.633566
1392.528809 0.633825
1392.528809 0.634086
1392.528809 0.634344
1392.528809 0.634602
1392.528809 0.634852
1392.528809 0.635108
1392.528809 0.635363
1392.528809 0.635620
1392.528809 0.635876
1392.528809 0.636152
1392.528809 0.636423
1392.528809 0.636679
1392.528809 0.636938
1392.528809 0.637199
1410.784668 0.625121
1428.876221 0.622596
1428.876221 0.622856
1428.876221 0.623118
1428.876221 0.623378
1428.876221 0.623632
1428.876221 0.623895
1428.876221 0.624161
1428.876221 0.624420
1428.876221 0.624688
1428.876221 0.624963
1446.890991 0.624116
1446.890991 0.624374
1446.890991 0.624629
1446.890991 0.624883
1446.890991 0.625138
1446.890991 0.625399
1446.890991 0.625666
1464.801880 0.624047
1464.801880 0.624293
1464.801880 0.624548
1464.801880 0.624793
1464.801880 0.625035
1464.801880 0.625283
1464.801880 0.625512
1464.801880 0.625744
1464.801880 0.625975
1464.801880 0.626216
1464.801880 0.626463
1464.801880 0.626719
1464.801880 0.626968
1464.801880 0.627208
1464.801880 0.627453
1464.801880 0.627698
1464.801880 0.627946
1464.801880 0.628197
1464.801880 0.628446
1464.801880 0.628703
1464.801880 0.628954
1464.801880 0.629199
1464.801880 0.629462
1464.801880 0.629717
1464.801880 0.629967
1464.801880 0.630232
1464.801880 0.630496
1464.801880 0.630760
1464.801880 0.631021
1464.801880 0.631270
1464.801880 0.631526
1464.801880 0.631797
1464.801880 0.632043
1464.801880 0.632288
1464.801880 0.632530
1464.801880 0.632795
1464.801880 0.633071
1464.801880 0.633354
1464.801880 0.633644
1464.801880 0.633921
1464.801880 0.634192
1464.801880 0.634458
1464.801880 0.634721
1464.801880 0.634981
1464.801880 0.635260
1464.801880 0.635532
1464.801880 0.635799
1464.801880 0.636072
1464.801880 0.636348
1464.801880 0.636625
1464.801880 0.636896
1464.801880 0.637165
1464.801880 0.637427
1464.801880 0.637682
1464.801880 0.637961
1464.801880 0.638229
1464.801880 0.638526
1464.801880 0.638807
1464.801880 0.639084
1464.801880 0.639349
1464.801880 0.639605
1464.801880 0.639882
1464.801880 0.640181
1464.801880 0.640462
1464.801880 0.640739
1464.801880 0.640997
1464.801880 0.641251
1464.801880 0.641498
1464.801880 0.641736
1464.801880 0.641969
1464.801880 0.642212
1464.801880 0.642448
1464.801880 0.642708
1464.801880 0.642977
1464.801880 0.643260
1464.801880 0.643557
1464.801880 0.643837
1464.801880 0.644126
1464.801880 0.644406
1464.801880 0.644680
1464.801880 0.644960
1483.305176 0.639642
1483.305176 0.639913
1483.305176 0.640172
1483.305176 0.640433
1483.305176 0.640702
1483.305176 0.640975
1483.305176 0.641236
1483.305176 0.641482
1483.305176 0.641734
1483.305176 0.641995
1483.305176 0.642257
1483.305176 0.642531
1483.305176 0.642803
1483.305176 0.643061
1483.305176 0.643313
1483.305176 0.643556
1483.305176 0.643796
1483.305176 0.644044
1483.305176 0.644281
1483.305176 0.644523
1483.305176 0.644775
1483.305176 0.645036
1483.305176 0.645288
1483.305176 0.645536
1483.305176 0.645779
1483.305176 0.646014
1483.305176 0.646255
1483.305176 0.646496
1483.305176 0.646738
1483.305176 0.646995
1483.305176 0.647239
1501.925293 0.646429
1501.925293 0.646684
1501.925293 0.646935
1501.925293 0.647166
1501.925293 0.647414
1501.925293 0.647679
1520.427856 0.640060
1520.427856 0.640321
1520.427856 0.640571
1520.427856 0.640827
1520.427856 0.641086
1520.427856 0.641343
1538.814819 0.639507
1538.814819 0.639762
1538.814819 0.640034
1538.814819 0.640294
1538.814819 0.640551
1538.814819 0.640798
1557.087524 0.632597
1557.087524 0.632837
1557.087524 0.633074
1557.087524 0.633303
1557.087524 0.633532
1557.087524 0.633768
1557.087524 0.634014
1557.087524 0.634258
1557.087524 0.634506
1557.087524 0.634767
1557.087524 0.635028
1557.087524 0.635285
1557.087524 0.635552
1557.087524 0.635822
1557.087524 0.636099
1557.087524 0.636368
1557.087524 0.636640
1557.087524 0.636898
1557.087524 0.637171
1557.087524 0.637447
1557.087524 0.637721
1557.087524 0.637981
1557.087524 0.638223
1557.087524 0.638451
1557.087524 0.638671
1557.087524 0.638905
1557.087524 0.639153
1557.087524 0.639404
1557.087524 0.639640
1557.087524 0.639875
1557.087524 0.640113
1557.087524 0.640357
1557.087524 0.640605
1557.087524 0.640850
1557.087524 0.641094
1557.087524 0.641330
1557.087524 0.641571
1557.087524 0.641810
1557.087524 0.642046
1557.087524 0.642277
1557.087524 0.642527
1557.087524 0.642766
1557.087524 0.643011
1557.087524 0.643237
1557.087524 0.643478
1557.087524 0.643712
1557.087524 0.643967
1557.087524 0.644217
1557.087524 0.644471
1557.087524 0.644715
1557.087524 0.644965
1557.087524 0.645212
1557.087524 0.645454
1557.087524 0.645708
1557.087524 0.645969
1557.087524 0.646228
1557.087524 0.646494
1557.087524 0.646741
1557.087524 0.647003
1557.087524 0.647249
1557.087524 0.647493
1557.087524 0.647729
1557.087524 0.647976
1557.087524 0.648232
1557.087524 0.648519
1557.087524 0.648793
1557.087524 0.649065
1557.087524 0.649338
1557.087524 0.649602
1557.087524 0.649877
1557.087524 0.650141
1557.087524 0.650406
1557.087524 0.650680
1557.087524 0.650946
1557.087524 0.651230
1557.087524 0.651501
1557.087524 0.651773
1557.087524 0.652053
1557.087524 0.652323
1557.087524 0.652596
1557.087524 0.652866
1557.087524 0.653148
1557.087524 0.653426
1557.087524 0.653696
1557.087524 0.653984
1557.087524 0.654268
1557.087524 0.654564
1557.087524 0.654852
1557.087524 0.655131
1557.087524 0.655389
1576.018311 0.654289
1576.018311 0.654545
1576.018311 0.654813
1576.018311 0.655079
1576.018311 0.655341
1576.018311 0.655592
1594.831055 0.654811
1594.831055 0.655047
1594.831055 0.655284
1594.831055 0.655518
1594.831055 0.655755
1594.831055 0.655999
1594.831055 0.656234
1594.831055 0.656495
1594.831055 0.656754
1594.831055 0.656989
1594.831055 0.657228
1594.831055 0.657478
1594.831055 0.657727
1594.831055 0.657976
1594.831055 0.658215
1594.831055 0.658459
1594.831055 0.658693
1594.831055 0.658943
1594.831055 0.659190
1594.831055 0.659442
1594.831055 0.659698
1594.831055 0.659955
1594.831055 0.660219
1594.831055 0.660469
1594.831055 0.660717
1594.831055 0.660962
1613.709106 0.647216
1613.709106 0.647475
1613.709106 0.647760
1613.709106 0.648032
1613.709106 0.648278
1613.709106 0.648538
1613.709106 0.648795
1613.709106 0.649052
1613.709106 0.649304
1613.709106 0.649546
1613.709106 0.649783
1613.709106 0.650018
1613.709106 0.650260
1613.709106 0.650497
1613.709106 0.650744
1613.709106 0.650998
1613.709106 0.651260
1613.709106 0.651530
1613.709106 0.651825
1613.709106 0.652101
1613.709106 0.652368
1613.709106 0.652619
1613.709106 0.652890
1613.709106 0.653168
1613.709106 0.653447
1613.709106 0.653749
1613.709106 0.654050
1613.709106 0.654343
1632.669678 0.647520
1651.468506 0.645934
1651.468506 0.646215
1651.468506 0.646486
1651.468506 0.646765
1651.468506 0.647033
1651.468506 0.647305
1651.468506 0.647577
1651.468506 0.647842
1651.468506 0.648104
1651.468506 0.648352
1651.468506 0.648605
1651.468506 0.648868
1651.468506 0.649118
1651.468506 0.649359
1651.468506 0.649597
1651.468506 0.649835
1651.468506 0.650077
1651.468506 0.650319
1651.468506 0.650566
1651.468506 0.650818
1651.468506 0.651069
1651.468506 0.651318
1651.468506 0.651569
1651.468506 0.651816
1651.468506 0.652050
1651.468506 0.652282
1651.468506 0.652518
1651.468506 0.652769
1651.468506 0.653019
1651.468506 0.653279
1651.468506 0.653537
1651.468506 0.653805
1651.468506 0.654080
1651.468506 0.654345
1651.468506 0.654605
1651.468506 0.654856
1651.468506 0.655092
1651.468506 0.655337
1651.468506 0.655576
1651.468506 0.655810
1651.468506 0.656046
1651.468506 0.656291
1651.468506 0.656541
1651.468506 0.656789
1651.468506 0.657027
1651.468506 0.657265
1651.468506 0.657499
1651.468506 0.657742
1651.468506 0.657976
1651.468506 0.658216
1651.468506 0.658445
1651.468506 0.658689
1651.468506 0.658936
1651.468506 0.659194
1651.468506 0.659442
1651.468506 0.659689
1651.468506 0.659937
1651.468506 0.660183
1651.468506 0.660445
1651.468506 0.660705
1651.468506 0.660967
1651.468506 0.661230
1651.468506 0.661500
1651.468506 0.661740
1651.468506 0.661977
1651.468506 0.662232
1651.468506 0.662480
1651.468506 0.662723
1651.468506 0.662967
1651.468506 0.663232
1651.468506 0.663481
1651.468506 0.663728
1651.468506 0.663974
1651.468506 0.664217
1651.468506 0.664451
1651.468506 0.664686
1670.780273 0.656075
1670.780273 0.656299
1670.780273 0.656522
1670.780273 0.656746
1670.780273 0.656978
1670.780273 0.657206
1670.780273 0.657436
1670.780273 0.657663
1670.780273 0.657885
1670.780273 0.658102
1670.780273 0.658336
1670.780273 0.658578
1670.780273 0.658810
1670.780273 0.659052
1670.780273 0.659296
1670.780273 0.659532
1670.780273 0.659775
1670.780273 0.660026
1670.780273 0.660260
1670.780273 0.660492
1670.780273 0.660735
1670.780273 0.660995
1670.780273 0.661239
1709.297729 0.657312
1709.297729 0.657552
1709.297729 0.657794
1709.297729 0.658036
1709.297729 0.658277
1709.297729 0.658526
1709.297729 0.658767
1709.297729 0.659000
1709.297729 0.659240
1709.297729 0.659483
1709.297729 0.659742
1709.297729 0.659990
1709.297729 0.660233
1709.297729 0.660484
1709.297729 0.660739
1709.297729 0.661004
1709.297729 0.661262
1709.297729 0.661530
1709.297729 0.661785
1709.297729 0.662040
1709.297729 0.662300
1709.297729 0.662565
1709.297729 0.662824
1709.297729 0.663061
1709.297729 0.663299
1709.297729 0.663548
1709.297729 0.663784
1709.297729 0.664014
1709.297729 0.664248
1709.297729 0.664482
1709.297729 0.664728
1709.297729 0.664986
1709.297729 0.665235
1709.297729 0.665480
1709.297729 0.665710
1709.297729 0.665943
1709.297729 0.666167
1709.297729 0.666385
1709.297729 0.666631
1709.297729 0.666872
1709.297729 0.667110
1709.297729 0.667350
1709.297729 0.667590
1709.297729 0.667840
1709.297729 0.668096
1709.297729 0.668336
1709.297729 0.668571
1709.297729 0.668793
1709.297729 0.669022
1709.297729 0.669257
1709.297729 0.669515
1709.297729 0.669762
1709.297729 0.670013
1709.297729 0.670250
1709.297729 0.670494
1709.297729 0.670739
1709.297729 0.670987
1709.297729 0.671242
1709.297729 0.671494
1709.297729 0.671749
1709.297729 0.672003
1709.297729 0.672264
1709.297729 0.672531
1709.297729 0.672811
1709.297729 0.673075
1709.297729 0.673328
1709.297729 0.673589
1709.297729 0.673848
1709.297729 0.674105
1709.297729 0.674383
1709.297729 0.674645
1709.297729 0.674899
1709.297729 0.675152
1709.297729 0.675402
1709.297729 0.675661
1709.297729 0.675902
1728.973511 0.667581
1728.973511 0.667800
1728.973511 0.668016
1728.973511 0.668242
1728.973511 0.668481
1728.973511 0.668729
1728.973511 0.668980
1728.973511 0.669232
1728.973511 0.669478
1728.973511 0.669722
1728.973511 0.669976
1728.973511 0.670236
1728.973511 0.670500
1728.973511 0.670753
1728.973511 0.671004
1728.973511 0.671239
1728.973511 0.671467
1728.973511 0.671707
1728.973511 0.671938
1748.643188 0.670546
1748.643188 0.670782
1748.643188 0.671030
1748.643188 0.671297
1748.643188 0.671569
1748.643188 0.671837
1748.643188 0.672098
1748.643188 0.672355
1748.643188 0.672617
1748.643188 0.672873
1748.643188 0.673128
1748.643188 0.673392
1748.643188 0.673661
1748.643188 0.673919
1748.643188 0.674178
1748.643188 0.674436
1748.643188 0.674704
1748.643188 0.674959
1748.643188 0.675205
1748.643188 0.675434
1748.643188 0.675656
1748.643188 0.675873
1748.643188 0.676098
1748.643188 0.676341
1748.643188 0.676611
1748.643188 0.676901
1748.643188 0.677186
1748.643188 0.677454
1748.643188 0.677709
1748.643188 0.677951
1748.643188 0.678200
1748.643188 0.678456
1748.643188 0.678720
1748.643188 0.678985
1748.643188 0.679259
1748.643188 0.679533
1748.643188 0.679793
1748.643188 0.680055
1748.643188 0.680317
1748.643188 0.680574
1748.643188 0.680824
1748.643188 0.681063
1748.643188 0.681299
1748.643188 0.681532
1748.643188 0.681767
1748.643188 0.682016
1748.643188 0.682263
1748.643188 0.682519
1748.643188 0.682764
1748.643188 0.683015
1748.643188 0.683259
1748.643188 0.683506
1748.643188 0.683738
1748.643188 0.683973
1748.643188 0.684206
1748.643188 0.684442
1748.643188 0.684691
1748.643188 0.684931
1748.643188 0.685186
1748.643188 0.685451
1748.643188 0.685704
1748.643188 0.685954
1748.643188 0.686218
1748.643188 0.686468
1748.643188 0.686707
1748.643188 0.686944
1748.643188 0.687183
1748.643188 0.687429
1748.643188 0.687676
1768.745605 0.686111
1768.745605 0.686342
1768.745605 0.686586
1768.745605 0.686840
1768.745605 0.687087
1768.745605 0.687353
1768.745605 0.687608
1768.745605 0.687893
1768.745605 0.688157
1768.745605 0.688418
1768.745605 0.688688
1768.745605 0.688955
1768.745605 0.689220
1768.745605 0.689481
1768.745605 0.689738
1768.745605 0.689982
1768.745605 0.690214
1768.745605 0.690460
1768.745605 0.690701
1768.745605 0.690941
1768.745605 0.691173
1768.745605 0.691404
1768.745605 0.691622
1768.745605 0.691832
1768.745605 0.692043
1768.745605 0.692248
1768.745605 0.692455
1768.745605 0.692678
1768.745605 0.692913
1768.745605 0.693131
1768.745605 0.693373
1768.745605 0.693636
1768.745605 0.693915
1788.960693 0.688583
1788.960693 0.688837
1788.960693 0.689088
1788.960693 0.689341
1788.960693 0.689601
1788.960693 0.689859
1788.960693 0.690117
1788.960693 0.690378
1788.960693 0.690641
1788.960693 0.690899
1788.960693 0.691147
1788.960693 0.691402
1788.960693 0.691649
1788.960693 0.691888
1788.960693 0.692150
1788.960693 0.692424
1788.960693 0.692691
1788.960693 0.692966
1788.960693 0.693242
1788.960693 0.693510
1788.960693 0.693773
1788.960693 0.694038
1788.960693 0.694306
1788.960693 0.694568
1788.960693 0.694823
1788.960693 0.695055
1788.960693 0.695279
1788.960693 0.695514
1788.960693 0.695748
1788.960693 0.695963
1788.960693 0.696180
1788.960693 0.696398
1788.960693 0.696633
1788.960693 0.696859
1788.960693 0.697092
1788.960693 0.697324
1788.960693 0.697565
1788.960693 0.697803
1788.960693 0.698041
1788.960693 0.698279
1788.960693 0.698529
1788.960693 0.698766
1788.960693 0.698997
1788.960693 0.699232
1788.960693 0.699469
1788.960693 0.699710
1788.960693 0.699953
1788.960693 0.700188
1788.960693 0.700435
1788.960693 0.700689
1809.434814 0.698499
1829.740234 0.694244
1829.740234 0.694475
1829.740234 0.694708
1829.740234 0.694928
1829.740234 0.695145
1829.740234 0.695368
1829.740234 0.695594
1829.740234 0.695809
1829.740234 0.696043
1829.740234 0.696274
1829.740234 0.696519
1829.740234 0.696767
1829.740234 0.697020
1829.740234 0.697282
1829.740234 0.697545
1829.740234 0.697803
1829.740234 0.698052
1829.740234 0.698293
1829.740234 0.698542
1829.740234 0.698797
1829.740234 0.699061
1829.740234 0.699328
1829.740234 0.699582
1829.740234 0.699838
1829.740234 0.700080
1829.740234 0.700328
1829.740234 0.700583
1829.740234 0.700845
1829.740234 0.701132
1829.740234 0.701421
1829.740234 0.701706
1829.740234 0.701980
1829.740234 0.702254
1829.740234 0.702525
1829.740234 0.702775
1829.740234 0.703027
1829.740234 0.703285
1829.740234 0.703552
1829.740234 0.703822
1829.740234 0.704074
1829.740234 0.704311
1829.740234 0.704547
1829.740234 0.704789
1829.740234 0.705021
1829.740234 0.705264
1829.740234 0.705524
1829.740234 0.705781
1829.740234 0.706050
1829.740234 0.706315
1829.740234 0.706568
1829.740234 0.706828
1829.740234 0.707075
1850.318970 0.691283
1850.318970 0.691523
1850.318970 0.691762
1850.318970 0.692003
1850.318970 0.692243
1850.318970 0.692498
1850.318970 0.692754
1850.318970 0.692999
1850.318970 0.693243
1850.318970 0.693487
1870.806885 0.693088
1870.806885 0.693348
1870.806885 0.693612
1870.806885 0.693867
1870.806885 0.694135
1870.806885 0.694402
1870.806885 0.694661
1870.806885 0.694923
1870.806885 0.695179
1870.806885 0.695440
1891.205078 0.685270
1891.205078 0.685535
1891.205078 0.685789
1891.205078 0.686048
1891.205078 0.686300
1891.205078 0.686566
1891.205078 0.686843
1891.205078 0.687116
1891.205078 0.687381
1891.205078 0.687652
1891.205078 0.687914
1891.205078 0.688166
1891.205078 0.688419
1891.205078 0.688668
1891.205078 0.688907
1891.205078 0.689162
1891.205078 0.689407
1891.205078 0.689663
1891.205078 0.689941
1891.205078 0.690202
1891.205078 0.690459
1891.205078 0.690715
1891.205078 0.690978
1891.205078 0.691234
1891.205078 0.691509
1891.205078 0.691760
1891.205078 0.691997
1891.205078 0.692238
1891.205078 0.692463
1891.205078 0.692696
1891.205078 0.692923
1891.205078 0.693134
1891.205078 0.693356
1891.205078 0.693575
1891.205078 0.693796
1891.205078 0.694020
1891.205078 0.694238
1891.205078 0.694466
1891.205078 0.694688
1891.205078 0.694921
1891.205078 0.695169
1891.205078 0.695420
1891.205078 0.695675
1891.205078 0.695923
1891.205078 0.696192
1891.205078 0.696456
1891.205078 0.696718
1891.205078 0.696985
1891.205078 0.697255
1891.205078 0.697531
1891.205078 0.697798
1911.863770 0.696760
1911.863770 0.696997
1911.863770 0.697232
1911.863770 0.697461
1911.863770 0.697697
1911.863770 0.697944
1911.863770 0.698193
1911.863770 0.698454
1911.863770 0.698711
1911.863770 0.698952
1911.863770 0.699200
1911.863770 0.699452
1911.863770 0.699706
1911.863770 0.699954
1911.863770 0.700201
1911.863770 0.700420
1911.863770 0.700659
1911.863770 0.700908
1911.863770 0.701152
1911.863770 0.701397
1911.863770 0.701627
1911.863770 0.701854
1911.863770 0.702093
1911.863770 0.702325
1911.863770 0.702570
1911.863770 0.702811
1911.863770 0.703043
1911.863770 0.703271
1911.863770 0.703504
1911.863770 0.703738
1911.863770 0.703968
1911.863770 0.704198
1911.863770 0.704427
1911.863770 0.704662
1911.863770 0.704900
1911.863770 0.705137
1911.863770 0.705381
1911.863770 0.705632
1911.863770 0.705887
1911.863770 0.706137
1911.863770 0.706394
1911.863770 0.706632
1911.863770 0.706872
1911.863770 0.707122
1911.863770 0.707371
1911.863770 0.707642
1911.863770 0.707911
1911.863770 0.708171
1911.863770 0.708433
1911.863770 0.708690
1911.863770 0.708946
1911.863770 0.709193
1911.863770 0.709434
1911.863770 0.709689
1911.863770 0.709964
1911.863770 0.710234
1911.863770 0.710490
1911.863770 0.710743
1911.863770 0.711021
1911.863770 0.711287
1911.863770 0.711552
1932.864380 0.702701
1932.864380 0.702935
1932.864380 0.703171
1932.864380 0.703394
1932.864380 0.703624
1932.864380 0.703836
1932.864380 0.704056
1932.864380 0.704271
1932.864380 0.704493
1932.864380 0.704718
1932.864380 0.704956
1932.864380 0.705198
1932.864380 0.705427
1932.864380 0.705654
1932.864380 0.705878
1953.814331 0.705566
1953.814331 0.705787
1953.814331 0.706006
1953.814331 0.706224
1953.814331 0.706451
1953.814331 0.706674
1953.814331 0.706888
1953.814331 0.707113
1953.814331 0.707345
1953.814331 0.707587
1953.814331 0.707823
1953.814331 0.708056
1953.814331 0.708295
1953.814331 0.708535
1953.814331 0.708780
1953.814331 0.709017
1953.814331 0.709266
1953.814331 0.709503
1953.814331 0.709738
1953.814331 0.709977
1953.814331 0.710220
1953.814331 0.710456
1953.814331 0.710692
1953.814331 0.710933
1953.814331 0.711180
1953.814331 0.711406
1953.814331 0.711627
1953.814331 0.711849
1953.814331 0.712080
1953.814331 0.712319
1953.814331 0.712544
1953.814331 0.712762
1953.814331 0.712976
1974.865601 0.710505
1974.865601 0.710724
1974.865601 0.710969
1974.865601 0.711210
1974.865601 0.711441
1974.865601 0.711672
1974.865601 0.711901
1974.865601 0.712139
1974.865601 0.712384
1974.865601 0.712616
1974.865601 0.712845
1974.865601 0.713085
1974.865601 0.713329
1974.865601 0.713578
1974.865601 0.713834
1974.865601 0.714079
1974.865601 0.714330
1974.865601 0.714582
1974.865601 0.714831
1974.865601 0.715063
1974.865601 0.715291
1974.865601 0.715524
1974.865601 0.715756
1974.865601 0.715987
1974.865601 0.716227
1974.865601 0.716470
1974.865601 0.716706
1974.865601 0.716944
1974.865601 0.717182
1974.865601 0.717422
1974.865601 0.717647
1974.865601 0.717865
1974.865601 0.718087
1974.865601 0.718302
1974.865601 0.718535
1974.865601 0.718782
1974.865601 0.719028
1974.865601 0.719277
1974.865601 0.719529
1974.865601 0.719782
1974.865601 0.720026
1974.865601 0.720262
1974.865601 0.720498
1974.865601 0.720750
1974.865601 0.721004
1974.865601 0.721271
1974.865601 0.721543
1974.865601 0.721810
1974.865601 0.722059
1974.865601 0.722307
1974.865601 0.722559
1974.865601 0.722814
1974.865601 0.723056
1974.865601 0.723285
1996.192505 0.722308
1996.192505 0.722530
1996.192505 0.722766
1996.192505 0.723007
1996.192505 0.723245
1996.192505 0.723490
1996.192505 0.723745
1996.192505 0.724005
1996.192505 0.724262
1996.192505 0.724529
1996.192505 0.724793
1996.192505 0.725035
2017.441650 0.721993
2017.441650 0.722224
2017.441650 0.722463
2017.441650 0.722692
2017.441650 0.722914
2017.441650 0.723149
2017.441650 0.723375
2017.441650 0.723615
2017.441650 0.723859
2017.441650 0.724097
2017.441650 0.724342
2017.441650 0.724595
2017.441650 0.724831
2017.441650 0.725062
2017.441650 0.725292
2017.441650 0.725530
2017.441650 0.725770
2017.441650 0.726005
2017.441650 0.726229
2017.441650 0.726451
2017.441650 0.726675
2017.441650 0.726920
2017.441650 0.727153
2017.441650 0.727399
2017.441650 0.727636
2017.441650 0.727876
2017.441650 0.728114
2017.441650 0.728358
2017.441650 0.728597
2017.441650 0.728835
2017.441650 0.729060
2017.441650 0.729271
2017.441650 0.729485
2017.441650 0.729708
2017.441650 0.729918
2017.441650 0.730148
2017.441650 0.730383
2017.441650 0.730610
2017.441650 0.730848
2017.441650 0.731071
2017.441650 0.731298
2017.441650 0.731539
2017.441650 0.731796
2017.441650 0.732051
2017.441650 0.732308
2017.441650 0.732550
2017.441650 0.732797
2017.441650 0.733031
2017.441650 0.733266
2017.441650 0.733500
2017.441650 0.733738
2017.441650 0.733977
2017.441650 0.734215
2017.441650 0.734448
2017.441650 0.734674
2017.441650 0.734907
2017.441650 0.735144
2017.441650 0.735370
2017.441650 0.735599
2017.441650 0.735828
2017.441650 0.736051
2017.441650 0.736275
2017.441650 0.736498
2017.441650 0.736716
2017.441650 0.736926
2017.441650 0.737145
2017.441650 0.737373
2017.441650 0.737604
2017.441650 0.737849
2017.441650 0.738095
2017.441650 0.738344
2017.441650 0.738589
2017.441650 0.738821
2017.441650 0.739058
2017.441650 0.739291
2017.441650 0.739530
2017.441650 0.739773
2017.441650 0.740014
2017.441650 0.740260
2017.441650 0.740503
2017.441650 0.740745
2017.441650 0.740996
2017.441650 0.741244
2017.441650 0.741485
2017.441650 0.741716
2017.441650 0.741954
2017.441650 0.742194
2017.441650 0.742427
2017.441650 0.742666
2017.441650 0.742907
2017.441650 0.743155
2017.441650 0.743408
2017.441650 0.743667
2017.441650 0.743924
2017.441650 0.744168
2017.441650 0.744401
2017.441650 0.744629
2017.441650 0.744871
2017.441650 0.745111
2017.441650 0.745345
2017.441650 0.745572
2017.441650 0.745796
2017.441650 0.746026
2017.441650 0.746257
2017.441650 0.746486
2017.441650 0.746721
2017.441650 0.746958
2017.441650 0.747206
2017.441650 0.747438
2017.441650 0.747658
2017.441650 0.747896
2017.441650 0.748125
2017.441650 0.748362
2017.441650 0.748608
2017.441650 0.748858
2039.468872 0.735119
2039.468872 0.735353
2039.468872 0.735587
2039.468872 0.735814
2039.468872 0.736037
2039.468872 0.736269
2039.468872 0.736502
2039.468872 0.736734
2039.468872 0.736959
2039.468872 0.737180
2039.468872 0.737410
2039.468872 0.737634
2039.468872 0.737849
2039.468872 0.738056
2039.468872 0.738268
2039.468872 0.738479
2039.468872 0.738687
2039.468872 0.738903
2039.468872 0.739116
2039.468872 0.739343
2061.479248 0.737947
2061.479248 0.738197
2061.479248 0.738440
2061.479248 0.738695
2061.479248 0.738948
2061.479248 0.739201
2061.479248 0.739441
2061.479248 0.739692
2061.479248 0.739950
2061.479248 0.740208
2061.479248 0.740469
2061.479248 0.740723
2061.479248 0.740981
2061.479248 0.741241
2061.479248 0.741500
2061.479248 0.741765
2083.440430 0.737159
2083.440430 0.737414
2083.440430 0.737654
2083.440430 0.737884
2083.440430 0.738105
2083.440430 0.738324
2083.440430 0.738561
2083.440430 0.738798
2083.440430 0.739032
2083.440430 0.739257
2083.440430 0.739488
2083.440430 0.739726
2083.440430 0.739966
2083.440430 0.740205
2083.440430 0.740444
2083.440430 0.740678
2083.440430 0.740917
2083.440430 0.741134
2105.368896 0.729273
2105.368896 0.729492
2105.368896 0.729711
2105.368896 0.729927
2105.368896 0.730150
2105.368896 0.730370
2105.368896 0.730577
2105.368896 0.730779
2105.368896 0.730989
2105.368896 0.731219
2105.368896 0.731448
2105.368896 0.731674
2105.368896 0.731892
2105.368896 0.732106
2105.368896 0.732327
2105.368896 0.732536
2105.368896 0.732751
2105.368896 0.732971
2105.368896 0.733186
2105.368896 0.733408
2105.368896 0.733641
2105.368896 0.733866
2105.368896 0.734096
2105.368896 0.734334
2105.368896 0.734566
2105.368896 0.734815
2105.368896 0.735067
2105.368896 0.735323
2105.368896 0.735576
2105.368896 0.735821
2105.368896 0.736073
2105.368896 0.736315
2105.368896 0.736549
2105.368896 0.736780
2105.368896 0.737010
2105.368896 0.737236
2105.368896 0.737451
2105.368896 0.737661
2105.368896 0.737877
2105.368896 0.738096
2105.368896 0.738321
2105.368896 0.738553
2105.368896 0.738780
2105.368896 0.739014
2105.368896 0.739235
2105.368896 0.739460
2105.368896 0.739676
2105.368896 0.739893
2105.368896 0.740118
2105.368896 0.740336
2105.368896 0.740560
2105.368896 0.740776
2105.368896 0.740996
2105.368896 0.741213
2105.368896 0.741433
2105.368896 0.741653
2105.368896 0.741879
2105.368896 0.742121
2105.368896 0.742343
2105.368896 0.742567
2105.368896 0.742789
2105.368896 0.743011
2105.368896 0.743226
2105.368896 0.743441
2105.368896 0.743653
2105.368896 0.743879
2105.368896 0.744107
2105.368896 0.744327
2105.368896 0.744559
2105.368896 0.744785
2105.368896 0.745016
2105.368896 0.745235
2105.368896 0.745453
2105.368896 0.745677
2105.368896 0.745899
2105.368896 0.746122
2105.368896 0.746349
2105.368896 0.746581
2105.368896 0.746812
2105.368896 0.747059
2105.368896 0.747292
2105.368896 0.747527
2105.368896 0.747754
2105.368896 0.747976
2105.368896 0.748184
2105.368896 0.748400
2105.368896 0.748619
2105.368896 0.748856
2105.368896 0.749099
2105.368896 0.749334
2105.368896 0.749557
2105.368896 0.749777
2105.368896 0.750007
2105.368896 0.750233
2105.368896 0.750449
2105.368896 0.750679
2105.368896 0.750923
2105.368896 0.751156
2105.368896 0.751389
2105.368896 0.751627
2105.368896 0.751862
2105.368896 0.752089
2105.368896 0.752335
2105.368896 0.752570
2105.368896 0.752820
2105.368896 0.753079
2105.368896 0.753326
2105.368896 0.753570
2105.368896 0.753811
2105.368896 0.754044
2105.368896 0.754296
2105.368896 0.754542
2105.368896 0.754793
2105.368896 0.755042
2105.368896 0.755288
2105.368896 0.755535
2105.368896 0.755786
2105.368896 0.756034
2128.081543 0.754735
2128.081543 0.754980
2128.081543 0.755212
2128.081543 0.755443
2128.081543 0.755694
2128.081543 0.755930
2128.081543 0.756173
2128.081543 0.756415
2150.674805 0.755705
2150.674805 0.755942
2150.674805 0.756181
2150.674805 0.756425
2150.674805 0.756659
2150.674805 0.756889
2150.674805 0.757110
2150.674805 0.757329
2150.674805 0.757561
2150.674805 0.757813
2150.674805 0.758069
2150.674805 0.758320
2150.674805 0.758559
2150.674805 0.758798
2150.674805 0.759033
2150.674805 0.759275
2150.674805 0.759505
2150.674805 0.759746
2150.674805 0.760001
2150.674805 0.760238
2150.674805 0.760476
2150.674805 0.760714
2150.674805 0.760944
2150.674805 0.761180
2150.674805 0.761409
2150.674805 0.761643
2150.674805 0.761871
2150.674805 0.762094
2150.674805 0.762347
2150.674805 0.762607
2150.674805 0.762853
2150.674805 0.763101
2150.674805 0.763342
2150.674805 0.763588
2150.674805 0.763821
2150.674805 0.764041
2150.674805 0.764272
2150.674805 0.764509
2150.674805 0.764738
2150.674805 0.764973
2150.674805 0.765201
2150.674805 0.765433
2150.674805 0.765662
2150.674805 0.765881
2150.674805 0.766122
2150.674805 0.766369
2150.674805 0.766597
2150.674805 0.766810
2150.674805 0.767032
2150.674805 0.767247
2150.674805 0.767457
2150.674805 0.767671
2150.674805 0.767890
2150.674805 0.768108
2173.522217 0.763176
2173.522217 0.763402
2173.522217 0.763643
2173.522217 0.763885
2173.522217 0.764130
2173.522217 0.764376
2173.522217 0.764612
2173.522217 0.764840
2173.522217 0.765071
2173.522217 0.765303
2173.522217 0.765537
2173.522217 0.765766
2173.522217 0.766009
2173.522217 0.766260
2173.522217 0.766512
2173.522217 0.766780
2173.522217 0.767028
2173.522217 0.767262
2173.522217 0.767483
2173.522217 0.767700
2173.522217 0.767924
2173.522217 0.768138
2173.522217 0.768359
2173.522217 0.768577
2173.522217 0.768808
2173.522217 0.769047
2173.522217 0.769279
2173.522217 0.769503
2173.522217 0.769720
2173.522217 0.769951
2173.522217 0.770193
2173.522217 0.770437
2173.522217 0.770680
2173.522217 0.770938
2173.522217 0.771209
2173.522217 0.771472
2173.522217 0.771725
2173.522217 0.771980
2173.522217 0.772220
2173.522217 0.772446
2173.522217 0.772683
2173.522217 0.772923
2173.522217 0.773177
2173.522217 0.773428
2173.522217 0.773658
2173.522217 0.773887
2173.522217 0.774103
2173.522217 0.774316
2173.522217 0.774548
2173.522217 0.774784
2173.522217 0.775004
2173.522217 0.775237
2173.522217 0.775465
2173.522217 0.775698
2173.522217 0.775923
2173.522217 0.776137
2173.522217 0.776348
2173.522217 0.776578
2173.522217 0.776811
2173.522217 0.777046
2173.522217 0.777287
2173.522217 0.777529
2173.522217 0.777785
2173.522217 0.778038
2173.522217 0.778291
2173.522217 0.778538
2173.522217 0.778779
2173.522217 0.779024
2173.522217 0.779257
2173.522217 0.779486
2173.522217 0.779710
2173.522217 0.779935
2173.522217 0.780155
2173.522217 0.780389
2173.522217 0.780624
2173.522217 0.780850
2173.522217 0.781077
2173.522217 0.781309
2173.522217 0.781550
2173.522217 0.781804
2173.522217 0.782047
2173.522217 0.782304
2173.522217 0.782569
2173.522217 0.782838
2173.522217 0.783101
2173.522217 0.783358
2173.522217 0.783608
2173.522217 0.783848
2173.522217 0.784085
2173.522217 0.784337
2173.522217 0.784607
2173.522217 0.784854
2173.522217 0.785092
2173.522217 0.785331
2173.522217 0.785562
2173.522217 0.785785
2173.522217 0.786011
2173.522217 0.786218
2173.522217 0.786427
2173.522217 0.786655
2173.522217 0.786880
2173.522217 0.787094
2173.522217 0.787305
2173.522217 0.787520
2173.522217 0.787745
2173.522217 0.787974
2173.522217 0.788205
2173.522217 0.788438
2173.522217 0.788688
2173.522217 0.788944
2173.522217 0.789202
2173.522217 0.789457
2173.522217 0.789725
2173.522217 0.789979
2173.522217 0.790229
2173.522217 0.790474
2173.522217 0.790722
2173.522217 0.790960
2173.522217 0.791202
2173.522217 0.791449
2173.522217 0.791692
2173.522217 0.791925
2173.522217 0.792165
2173.522217 0.792403
2173.522217 0.792639
2173.522217 0.792870
2173.522217 0.793106
2173.522217 0.793344
2173.522217 0.793596
2173.522217 0.793846
2173.522217 0.794089
2173.522217 0.794338
2173.522217 0.794568
2173.522217 0.794792
2173.522217 0.795021
2173.522217 0.795241
2173.522217 0.795466
2173.522217 0.795696
2173.522217 0.795925
2173.522217 0.796152
2173.522217 0.796385
2173.522217 0.796615
2173.522217 0.796829
2173.522217 0.797055
2173.522217 0.797288
2173.522217 0.797514
2173.522217 0.797723
2173.522217 0.797934
2173.522217 0.798134
2173.522217 0.798341
2173.522217 0.798543
2173.522217 0.798753
2173.522217 0.798966
2173.522217 0.799170
2173.522217 0.799375
2173.522217 0.799584
2173.522217 0.799791
2173.522217 0.800000
2173.522217 0.800206
2173.522217 0.800411
2173.522217 0.800612
2173.522217 0.800815
2173.522217 0.801030
2173.522217 0.801254
2173.522217 0.801477
2173.522217 0.801712
2173.522217 0.801944
2173.522217 0.802178
2173.522217 0.802417
2173.522217 0.802652
2173.522217 0.802894
2173.522217 0.803123
2173.522217 0.803363
2173.522217 0.803620
2173.522217 0.803865
2173.522217 0.804099
2173.522217 0.804327
2173.522217 0.804545
2173.522217 0.804761
2173.522217 0.804981
2173.522217 0.805204
2173.522217 0.805422
2173.522217 0.805643
2173.522217 0.805875
2173.522217 0.806101
2173.522217 0.806338
2173.522217 0.806568
2173.522217 0.806804
2173.522217 0.807052
2173.522217 0.807300
2173.522217 0.807543
2173.522217 0.807789
2173.522217 0.808029
2173.522217 0.808269
2173.522217 0.808513
2173.522217 0.808760
2173.522217 0.808996
2173.522217 0.809229
2173.522217 0.809446
2173.522217 0.809677
2173.522217 0.809909
2173.522217 0.810153
2173.522217 0.810399
2173.522217 0.810645
2173.522217 0.810871
2173.522217 0.811092
2173.522217 0.811326
2173.522217 0.811555
2173.522217 0.811787
2173.522217 0.812019
2173.522217 0.812245
2173.522217 0.812469
2173.522217 0.812705
2173.522217 0.812937
2173.522217 0.813181
2173.522217 0.813413
2173.522217 0.813638
2173.522217 0.813871
2173.522217 0.814109
2173.522217 0.814340
2173.522217 0.814570
2173.522217 0.814799
2173.522217 0.815042
2173.522217 0.815276
2173.522217 0.815516
2173.522217 0.815755
2173.522217 0.816000
2173.522217 0.816247
2173.522217 0.816486
2173.522217 0.816709
2173.522217 0.816951
2198.048340 0.803001
2198.048340 0.803241
2198.048340 0.803480
2198.048340 0.803718
2198.048340 0.803960
2198.048340 0.804190
2198.048340 0.804424
2198.048340 0.804661
2198.048340 0.804913
2198.048340 0.805174
2198.048340 0.805435
2198.048340 0.805695
2198.048340 0.805946
2198.048340 0.806197
2198.048340 0.806440
2198.048340 0.806682
2198.048340 0.806921
2198.048340 0.807148
2198.048340 0.807371
2198.048340 0.807586
2198.048340 0.807797
2198.048340 0.808012
2198.048340 0.808225
2198.048340 0.808448
2198.048340 0.808680
2198.048340 0.808906
2198.048340 0.809127
2198.048340 0.809347
2198.048340 0.809556
2198.048340 0.809765
2198.048340 0.809978
2198.048340 0.810196
2198.048340 0.810414
2198.048340 0.810626
2198.048340 0.810833
2198.048340 0.811036
2198.048340 0.811256
2198.048340 0.811480
2198.048340 0.811700
2198.048340 0.811923
2198.048340 0.812163
2198.048340 0.812405
2198.048340 0.812639
2198.048340 0.812864
2198.048340 0.813110
2198.048340 0.813349
2198.048340 0.813584
2198.048340 0.813812
2198.048340 0.814049
2222.770996 0.806734
2222.770996 0.806972
2222.770996 0.807214
2222.770996 0.807446
2222.770996 0.807695
2222.770996 0.807928
2222.770996 0.808157
2222.770996 0.808393
2222.770996 0.808618
2222.770996 0.808841
2222.770996 0.809061
2222.770996 0.809285
2222.770996 0.809509
2222.770996 0.809731
2222.770996 0.809979
2222.770996 0.810228
2222.770996 0.810467
2222.770996 0.810706
2222.770996 0.810932
2222.770996 0.811168
2222.770996 0.811391
2222.770996 0.811626
2222.770996 0.811871
2222.770996 0.812117
2222.770996 0.812363
2222.770996 0.812613
2222.770996 0.812863
2222.770996 0.813125
2222.770996 0.813371
2222.770996 0.813610
2222.770996 0.813845
2222.770996 0.814094
2222.770996 0.814325
2222.770996 0.814578
2222.770996 0.814835
2222.770996 0.815078
2222.770996 0.815320
2222.770996 0.815561
2222.770996 0.815805
2222.770996 0.816038
2222.770996 0.816289
2222.770996 0.816532
2222.770996 0.816784
2222.770996 0.817025
2222.770996 0.817266
2222.770996 0.817498
2222.770996 0.817734
2222.770996 0.817971
2222.770996 0.818203
2222.770996 0.818431
2222.770996 0.818660
2222.770996 0.818908
2222.770996 0.819164
2222.770996 0.819416
2222.770996 0.819668
2222.770996 0.819918
2222.770996 0.820159
2222.770996 0.820399
2222.770996 0.820641
2222.770996 0.820873
2222.770996 0.821103
2222.770996 0.821325
2222.770996 0.821539
2222.770996 0.821758
2222.770996 0.821980
2222.770996 0.822205
2247.823975 0.822413
2247.823975 0.822651
2247.823975 0.822890
2247.823975 0.823120
2247.823975 0.823359
2247.823975 0.823596
2247.823975 0.823831
2247.823975 0.824070
2247.823975 0.824310
2247.823975 0.824554
2247.823975 0.824807
2247.823975 0.825065
2247.823975 0.825346
2247.823975 0.825611
2247.823975 0.825865
2247.823975 0.826118
2247.823975 0.826368
2247.823975 0.826641
2247.823975 0.826896
2247.823975 0.827137
2247.823975 0.827405
2247.823975 0.827666
2247.823975 0.827911
2247.823975 0.828163
2247.823975 0.828416
2247.823975 0.828661
2247.823975 0.828899
2247.823975 0.829147
2247.823975 0.829411
2247.823975 0.829678
2247.823975 0.829937
2247.823975 0.830189
2247.823975 0.830433
2247.823975 0.830672
2272.948242 0.818411
2272.948242 0.818637
2272.948242 0.818861
2272.948242 0.819081
2297.904785 0.809860
2297.904785 0.810111
2297.904785 0.810346
2297.904785 0.810579
2297.904785 0.810818
2297.904785 0.811064
2297.904785 0.811306
2297.904785 0.811566
2297.904785 0.811814
2297.904785 0.812057
2297.904785 0.812294
2297.904785 0.812529
2297.904785 0.812752
2297.904785 0.812986
2297.904785 0.813225
2297.904785 0.813459
2322.790527 0.806806
2322.790527 0.807048
2322.790527 0.807291
2322.790527 0.807536
2322.790527 0.807782
2322.790527 0.808015
2322.790527 0.808238
2322.790527 0.808462
2322.790527 0.808678
2322.790527 0.808915
2322.790527 0.809147
2322.790527 0.809366
2322.790527 0.809593
2322.790527 0.809809
2322.790527 0.810031
2322.790527 0.810245
2322.790527 0.810471
2322.790527 0.810699
2322.790527 0.810923
2322.790527 0.811144
2322.790527 0.811367
2322.790527 0.811591
2322.790527 0.811815
2322.790527 0.812049
2322.790527 0.812271
2322.790527 0.812521
2322.790527 0.812769
2347.692871 0.808686
2347.692871 0.808931
2347.692871 0.809175
2347.692871 0.809414
2347.692871 0.809670
2347.692871 0.809928
2347.692871 0.810172
2347.692871 0.810398
2347.692871 0.810612
2347.692871 0.810836
2347.692871 0.811097
2347.692871 0.811356
2347.692871 0.811617
2347.692871 0.811881
2347.692871 0.812148
2347.692871 0.812400
2347.692871 0.812652
2347.692871 0.812890
2347.692871 0.813121
2347.692871 0.813344
2347.692871 0.813563
2347.692871 0.813772
2347.692871 0.813986
2347.692871 0.814197
2347.692871 0.814407
2347.692871 0.814623
2347.692871 0.814838
2347.692871 0.815045
2347.692871 0.815246
2347.692871 0.815451
2347.692871 0.815664
2347.692871 0.815893
2347.692871 0.816120
2347.692871 0.816364
2347.692871 0.816608
2347.692871 0.816836
2347.692871 0.817063
2347.692871 0.817282
2347.692871 0.817501
2347.692871 0.817722
2347.692871 0.817946
2347.692871 0.818158
2347.692871 0.818384
2347.692871 0.818607
2347.692871 0.818831
2347.692871 0.819053
2347.692871 0.819266
2347.692871 0.819485
2347.692871 0.819720
2347.692871 0.819970
2347.692871 0.820213
2347.692871 0.820455
2347.692871 0.820688
2347.692871 0.820922
2347.692871 0.821152
2347.692871 0.821383
2347.692871 0.821614
2347.692871 0.821849
2347.692871 0.822081
2347.692871 0.822315
2347.692871 0.822549
2347.692871 0.822784
2347.692871 0.823029
2347.692871 0.823281
2347.692871 0.823531
2347.692871 0.823799
2347.692871 0.824048
2347.692871 0.824284
2347.692871 0.824508
2347.692871 0.824730
2347.692871 0.824953
2347.692871 0.825175
2347.692871 0.825400
2347.692871 0.825638
2347.692871 0.825875
2347.692871 0.826111
2347.692871 0.826362
2347.692871 0.826625
2347.692871 0.826865
2347.692871 0.827099
2347.692871 0.827331
2347.692871 0.827558
2347.692871 0.827786
2347.692871 0.828017
2347.692871 0.828231
2347.692871 0.828450
2347.692871 0.828675
2347.692871 0.828910
2347.692871 0.829140
2347.692871 0.829356
2347.692871 0.829581
2347.692871 0.829804
2347.692871 0.830026
2347.692871 0.830242
2347.692871 0.830453
2347.692871 0.830661
2347.692871 0.830904
2347.692871 0.831131
2347.692871 0.831357
2347.692871 0.831582
2347.692871 0.831794
2347.692871 0.832007
2347.692871 0.832221
2347.692871 0.832442
2347.692871 0.832657
2347.692871 0.832887
2347.692871 0.833109
2347.692871 0.833342
2347.692871 0.833595
2347.692871 0.833859
2347.692871 0.834132
2347.692871 0.834399
2347.692871 0.834652
2347.692871 0.834899
2347.692871 0.835152
2347.692871 0.835421
2347.692871 0.835694
2347.692871 0.835950
2347.692871 0.836210
2347.692871 0.836447
2347.692871 0.836695
2347.692871 0.836946
2347.692871 0.837186
2347.692871 0.837430
2347.692871 0.837674
2347.692871 0.837906
2347.692871 0.838132
2347.692871 0.838383
2347.692871 0.838637
2347.692871 0.838880
2347.692871 0.839145
2347.692871 0.839401
2347.692871 0.839650
2347.692871 0.839893
2347.692871 0.840134
2347.692871 0.840367
2347.692871 0.840598
2347.692871 0.840813
2347.692871 0.841028
2347.692871 0.841233
2347.692871 0.841436
2347.692871 0.841645
2347.692871 0.841868
2347.692871 0.842086
2347.692871 0.842309
2347.692871 0.842561
2347.692871 0.842810
2347.692871 0.843058
2347.692871 0.843310
2347.692871 0.843545
2347.692871 0.843779
2347.692871 0.844003
2347.692871 0.844226
2347.692871 0.844447
2347.692871 0.844675
2347.692871 0.844897
2347.692871 0.845128
2347.692871 0.845358
2347.692871 0.845583
2347.692871 0.845807
2347.692871 0.846039
2347.692871 0.846271
2347.692871 0.846503
2373.678467 0.845046
2373.678467 0.845255
2373.678467 0.845484
2373.678467 0.845693
2373.678467 0.845887
2373.678467 0.846083
2373.678467 0.846303
2373.678467 0.846519
2373.678467 0.846753
2373.678467 0.846991
2373.678467 0.847234
2373.678467 0.847470
2373.678467 0.847702
2373.678467 0.847932
2373.678467 0.848180
2373.678467 0.848422
2373.678467 0.848656
2373.678467 0.848879
2373.678467 0.849097
2373.678467 0.849329
2373.678467 0.849559
2373.678467 0.849787
2373.678467 0.850019
2373.678467 0.850251
2373.678467 0.850492
2373.678467 0.850710
2373.678467 0.850926
2373.678467 0.851130
2373.678467 0.851337
2373.678467 0.851550
2373.678467 0.851778
2373.678467 0.852006
2373.678467 0.852228
2373.678467 0.852447
2373.678467 0.852657
2373.678467 0.852870
2373.678467 0.853076
2373.678467 0.853268
2373.678467 0.853457
2373.678467 0.853655
2373.678467 0.853865
2373.678467 0.854085
2373.678467 0.854320
2373.678467 0.854565
2373.678467 0.854817
2373.678467 0.855054
2373.678467 0.855296
2373.678467 0.855531
2373.678467 0.855748
2373.678467 0.855963
2373.678467 0.856177
2373.678467 0.856387
2373.678467 0.856605
2373.678467 0.856844
2373.678467 0.857090
2373.678467 0.857322
2373.678467 0.857567
2373.678467 0.857809
2373.678467 0.858068
2373.678467 0.858342
2373.678467 0.858602
2373.678467 0.858860
2373.678467 0.859102
2373.678467 0.859346
2373.678467 0.859611
2373.678467 0.859874
2373.678467 0.860143
2373.678467 0.860418
2373.678467 0.860686
2373.678467 0.860935
2373.678467 0.861181
2373.678467 0.861419
2373.678467 0.861645
2373.678467 0.861864
2373.678467 0.862082
2373.678467 0.862288
2373.678467 0.862518
2373.678467 0.862760
2373.678467 0.863003
2373.678467 0.863260
2373.678467 0.863516
2373.678467 0.863773
2373.678467 0.864033
2373.678467 0.864280
2373.678467 0.864545
2373.678467 0.864803
2373.678467 0.865060
2373.678467 0.865320
2373.678467 0.865566
2373.678467 0.865793
2373.678467 0.866007
2373.678467 0.866234
2373.678467 0.866459
2373.678467 0.866702
2373.678467 0.866942
2373.678467 0.867183
2373.678467 0.867436
2400.218750 0.856171
2400.218750 0.856447
2400.218750 0.856706
2400.218750 0.856950
2400.218750 0.857184
2400.218750 0.857441
2400.218750 0.857699
2400.218750 0.857959
2400.218750 0.858223
2400.218750 0.858483
2400.218750 0.858743
2400.218750 0.858985
2400.218750 0.859235
2400.218750 0.859485
2400.218750 0.859746
2400.218750 0.860007
2400.218750 0.860252
2400.218750 0.860498
2400.218750 0.860758
2400.218750 0.861016
2400.218750 0.861262
2400.218750 0.861504
2426.723633 0.853601
2426.723633 0.853882
2426.723633 0.854147
2453.046631 0.851085
2479.173828 0.838781
2479.173828 0.839013
2479.173828 0.839247
2479.173828 0.839484
2479.173828 0.839717
2479.173828 0.839951
2479.173828 0.840197
2479.173828 0.840443
2505.161621 0.834223
2505.161621 0.834439
2505.161621 0.834665
2505.161621 0.834908
2505.161621 0.835139
2505.161621 0.835378
2505.161621 0.835605
2505.161621 0.835823
2505.161621 0.836028
2505.161621 0.836221
2505.161621 0.836426
2505.161621 0.836638
2505.161621 0.836836
2505.161621 0.837029
2505.161621 0.837230
2505.161621 0.837429
2531.072754 0.835957
2531.072754 0.836173
2531.072754 0.836374
2531.072754 0.836599
2531.072754 0.836838
2531.072754 0.837075
2531.072754 0.837325
2531.072754 0.837564
2531.072754 0.837799
2531.072754 0.838015
2531.072754 0.838247
2531.072754 0.838465
2531.072754 0.838683
2531.072754 0.838897
2531.072754 0.839102
2531.072754 0.839302
2531.072754 0.839491
2531.072754 0.839681
2531.072754 0.839871
2531.072754 0.840065
2531.072754 0.840260
2531.072754 0.840460
2531.072754 0.840662
2531.072754 0.840886
2531.072754 0.841119
2531.072754 0.841351
2531.072754 0.841577
2531.072754 0.841793
2531.072754 0.842004
2531.072754 0.842221
2531.072754 0.842439
2531.072754 0.842658
2531.072754 0.842884
2531.072754 0.843124
2531.072754 0.843363
2531.072754 0.843607
2531.072754 0.843841
2531.072754 0.844093
2531.072754 0.844341
2531.072754 0.844584
2531.072754 0.844840
2531.072754 0.845083
2531.072754 0.845325
2531.072754 0.845568
2531.072754 0.845814
2531.072754 0.846050
2531.072754 0.846285
2531.072754 0.846507
2531.072754 0.846736
2531.072754 0.846951
2531.072754 0.847176
2531.072754 0.847397
2531.072754 0.847635
2531.072754 0.847880
2531.072754 0.848113
2531.072754 0.848324
2531.072754 0.848521
2531.072754 0.848735
2531.072754 0.848954
2531.072754 0.849179
2531.072754 0.849402
2531.072754 0.849615
2531.072754 0.849825
2531.072754 0.850029
2531.072754 0.850237
2531.072754 0.850455
2531.072754 0.850676
2531.072754 0.850895
2531.072754 0.851117
2531.072754 0.851332
2531.072754 0.851573
2531.072754 0.851823
2531.072754 0.852063
2531.072754 0.852297
2531.072754 0.852539
2531.072754 0.852782
2531.072754 0.853027
2531.072754 0.853265
2531.072754 0.853497
2531.072754 0.853711
2531.072754 0.853919
2531.072754 0.854134
2531.072754 0.854360
2531.072754 0.854591
2531.072754 0.854814
2531.072754 0.855055
2531.072754 0.855295
2531.072754 0.855540
2531.072754 0.855773
2531.072754 0.856015
2531.072754 0.856259
2531.072754 0.856503
2531.072754 0.856756
2531.072754 0.856995
2531.072754 0.857230
2531.072754 0.857472
2531.072754 0.857697
2531.072754 0.857904
2531.072754 0.858105
2531.072754 0.858290
2531.072754 0.858477
2531.072754 0.858671
2531.072754 0.858863
2531.072754 0.859061
2531.072754 0.859271
2531.072754 0.859474
2531.072754 0.859666
2531.072754 0.859860
2531.072754 0.860047
2531.072754 0.860240
2531.072754 0.860446
2531.072754 0.860647
2531.072754 0.860846
2531.072754 0.861050
2531.072754 0.861247
2531.072754 0.861454
2531.072754 0.861664
2531.072754 0.861875
2531.072754 0.862079
2531.072754 0.862293
2531.072754 0.862497
2531.072754 0.862712
2531.072754 0.862938
2531.072754 0.863157
2531.072754 0.863382
2531.072754 0.863597
2531.072754 0.863811
2531.072754 0.864027
2531.072754 0.864237
2531.072754 0.864454
2531.072754 0.864674
2531.072754 0.864881
2531.072754 0.865094
2531.072754 0.865329
2531.072754 0.865561
2531.072754 0.865805
2531.072754 0.866034
2531.072754 0.866267
2531.072754 0.866506
2531.072754 0.866726
2531.072754 0.866942
2531.072754 0.867150
2531.072754 0.867360
2531.072754 0.867585
2531.072754 0.867814
2531.072754 0.868049
2531.072754 0.868275
2531.072754 0.868515
2531.072754 0.868761
2531.072754 0.868998
2531.072754 0.869244
2531.072754 0.869477
2531.072754 0.869705
2531.072754 0.869935
2531.072754 0.870169
2531.072754 0.870406
2531.072754 0.870649
2531.072754 0.870915
2531.072754 0.871171
2531.072754 0.871408
2531.072754 0.871654
2558.015381 0.873223
2558.015381 0.873470
2558.015381 0.873700
2558.015381 0.873939
2558.015381 0.874160
2558.015381 0.874402
2584.798584 0.867496
2584.798584 0.867742
2584.798584 0.867975
2584.798584 0.868206
2584.798584 0.868469
2584.798584 0.868734
2584.798584 0.868997
2584.798584 0.869246
2584.798584 0.869491
2584.798584 0.869742
2584.798584 0.869980
2584.798584 0.870220
2584.798584 0.870458
2584.798584 0.870686
2584.798584 0.870925
2584.798584 0.871152
2584.798584 0.871372
2584.798584 0.871588
2584.798584 0.871810
2584.798584 0.872049
2584.798584 0.872296
2584.798584 0.872541
2584.798584 0.872782
2584.798584 0.873012
2584.798584 0.873233
2584.798584 0.873452
2584.798584 0.873676
2584.798584 0.873905
2584.798584 0.874130
2584.798584 0.874368
2584.798584 0.874597
2584.798584 0.874823
2584.798584 0.875043
2584.798584 0.875252
2584.798584 0.875468
2584.798584 0.875682
2584.798584 0.875919
2584.798584 0.876155
2584.798584 0.876379
2584.798584 0.876599
2584.798584 0.876825
2584.798584 0.877052
2584.798584 0.877285
2584.798584 0.877516
2584.798584 0.877760
2584.798584 0.877988
2584.798584 0.878203
2584.798584 0.878440
2584.798584 0.878683
2584.798584 0.878936
2584.798584 0.879178
2584.798584 0.879406
2584.798584 0.879619
2584.798584 0.879839
2584.798584 0.880061
2584.798584 0.880274
2584.798584 0.880498
2584.798584 0.880730
2584.798584 0.880963
2584.798584 0.881193
2584.798584 0.881426
2584.798584 0.881647
2584.798584 0.881863
2584.798584 0.882076
2584.798584 0.882294
2584.798584 0.882506
2584.798584 0.882716
2584.798584 0.882923
2584.798584 0.883150
2584.798584 0.883377
2584.798584 0.883594
2584.798584 0.883814
2584.798584 0.884038
2584.798584 0.884279
2584.798584 0.884512
2584.798584 0.884746
2584.798584 0.884977
2584.798584 0.885213
2584.798584 0.885465
2584.798584 0.885719
2584.798584 0.885982
2584.798584 0.886233
2584.798584 0.886480
2584.798584 0.886734
2584.798584 0.886991
2584.798584 0.887231
2584.798584 0.887462
2584.798584 0.887694
2584.798584 0.887936
2584.798584 0.888186
2584.798584 0.888448
2584.798584 0.888698
2584.798584 0.888926
2584.798584 0.889155
2584.798584 0.889375
2584.798584 0.889588
2584.798584 0.889797
2584.798584 0.890001
2584.798584 0.890207
2584.798584 0.890414
2584.798584 0.890622
2584.798584 0.890826
2584.798584 0.891040
2584.798584 0.891259
2584.798584 0.891469
2584.798584 0.891687
2584.798584 0.891914
2584.798584 0.892133
2584.798584 0.892365
2584.798584 0.892607
2584.798584 0.892829
2584.798584 0.893042
2584.798584 0.893250
2584.798584 0.893465
2584.798584 0.893693
2584.798584 0.893942
2584.798584 0.894183
2584.798584 0.894421
2584.798584 0.894662
2584.798584 0.894903
2584.798584 0.895143
2584.798584 0.895390
2584.798584 0.895615
2584.798584 0.895839
2584.798584 0.896060
2584.798584 0.896277
2584.798584 0.896501
2584.798584 0.896723
2584.798584 0.896947
2584.798584 0.897180
2584.798584 0.897401
2584.798584 0.897616
2584.798584 0.897833
2584.798584 0.898069
2584.798584 0.898293
2584.798584 0.898532
2584.798584 0.898757
2584.798584 0.898973
2584.798584 0.899203
2584.798584 0.899420
2584.798584 0.899636
2584.798584 0.899853
2584.798584 0.900066
2584.798584 0.900286
2584.798584 0.900504
2584.798584 0.900719
2584.798584 0.900943
2584.798584 0.901175
2584.798584 0.901423
2584.798584 0.901660
2584.798584 0.901886
2584.798584 0.902108
2584.798584 0.902325
2584.798584 0.902533
2584.798584 0.902734
2584.798584 0.902940
2584.798584 0.903154
2584.798584 0.903379
2584.798584 0.903613
2584.798584 0.903843
2584.798584 0.904084
2584.798584 0.904329
2584.798584 0.904584
2584.798584 0.904831
2584.798584 0.905087
2584.798584 0.905325
2584.798584 0.905558
2584.798584 0.905777
2584.798584 0.906004
2584.798584 0.906218
2584.798584 0.906426
2584.798584 0.906639
2584.798584 0.906861
2584.798584 0.907087
2584.798584 0.907309
2584.798584 0.907526
2584.798584 0.907741
2584.798584 0.907956
2584.798584 0.908170
2584.798584 0.908398
2584.798584 0.908635
2584.798584 0.908881
2584.798584 0.909120
2584.798584 0.909351
2584.798584 0.909572
2584.798584 0.909784
2584.798584 0.910008
2584.798584 0.910224
2584.798584 0.910485
2584.798584 0.910748
2584.798584 0.911000
2584.798584 0.911255
2584.798584 0.911497
2584.798584 0.911751
2584.798584 0.912016
2584.798584 0.912281
2584.798584 0.912526
2584.798584 0.912772
2584.798584 0.913007
2584.798584 0.913235


==> fig/data/avgq-vs-success-2/banditst-linf-cdf.tex <==
0.000000 0.280978
1.000000 0.276461
2.000000 0.268539
2.571429 0.271547
4.833333 0.264450
5.571429 0.268174
6.000000 0.275129
6.500000 0.283401
9.391304 0.273253
10.384615 0.276650
10.384615 0.279373
10.384615 0.282842
10.888889 0.283973
10.888889 0.286936
11.500000 0.287836
11.500000 0.290598
11.500000 0.293434
12.275862 0.292777
13.066667 0.291717
13.066667 0.294719
13.935484 0.295856
13.935484 0.299050
13.935484 0.301551
13.935484 0.304447
16.000000 0.299101
16.000000 0.303178
16.000000 0.306704
16.000000 0.309931
16.000000 0.312607
16.000000 0.316021
17.294117 0.316400
18.571428 0.316213
21.027027 0.316896
21.027027 0.320208
21.027027 0.322954
21.027027 0.325936
22.368422 0.327411
23.692308 0.325257
25.000000 0.323663
25.000000 0.326356
25.000000 0.329287
25.000000 0.332340
26.439024 0.333701
26.439024 0.336442
26.439024 0.339094
27.952381 0.339645
32.222221 0.335070
32.222221 0.337487
33.608696 0.334482
33.608696 0.336999
36.375000 0.334042
37.714287 0.334611
37.714287 0.336517
37.714287 0.338218
37.714287 0.339693
40.549019 0.334878
40.549019 0.336878
41.961540 0.334959
41.961540 0.337117
41.961540 0.339258
41.961540 0.341479
41.961540 0.343725
41.961540 0.345888
41.961540 0.347927
46.654545 0.343689
46.654545 0.345874
46.654545 0.348407
46.654545 0.351127
48.250000 0.350244
48.250000 0.352450
49.859650 0.347655
49.859650 0.349920
49.859650 0.352742
49.859650 0.355428
49.859650 0.357709
53.254238 0.352211
54.900002 0.350361
58.096775 0.344584
58.096775 0.347440
58.096775 0.349945
59.714287 0.348485
59.714287 0.350506
59.714287 0.352348
61.375000 0.352957
63.015385 0.353273
64.636360 0.353171
66.238808 0.352248
66.238808 0.353861
66.238808 0.355420
66.238808 0.357297
66.238808 0.359288
66.238808 0.361246
66.238808 0.363355
72.985916 0.358415
72.985916 0.360177
72.985916 0.362083
77.810814 0.355748
77.810814 0.357595
77.810814 0.359417
79.413330 0.359312
79.413330 0.360711
79.413330 0.362302
79.413330 0.364299
81.078949 0.363488
81.078949 0.365467
81.078949 0.367256
81.078949 0.369076
81.078949 0.370838
81.078949 0.372904
82.857140 0.368187
82.857140 0.369946
82.857140 0.371635
82.857140 0.373532
82.857140 0.375772
84.717949 0.374983
86.556961 0.375285
86.556961 0.377192
86.556961 0.379494
86.556961 0.381771
86.556961 0.383682
88.474998 0.382694
88.474998 0.384588
88.474998 0.386683
90.419754 0.385022
92.341461 0.384020
92.341461 0.385964
94.265060 0.386332
94.265060 0.388106
94.265060 0.389885
98.117645 0.384020
98.117645 0.386792
98.117645 0.389186
98.117645 0.391174
98.117645 0.393181
98.117645 0.394692
102.068962 0.393455
102.068962 0.395178
104.022728 0.395567
104.022728 0.397866
105.977531 0.398212
107.911110 0.392100
107.911110 0.393660
107.911110 0.395344
107.911110 0.397096
107.911110 0.398610
107.911110 0.400253
107.911110 0.401679
109.956047 0.399770
109.956047 0.401225
109.956047 0.402922
109.956047 0.404719
109.956047 0.406504
112.065216 0.403532
112.065216 0.405192
112.065216 0.406845
114.193550 0.406961
114.193550 0.408164
114.193550 0.409679
114.193550 0.411626
114.193550 0.413395
114.193550 0.414961
114.193550 0.416702
116.425529 0.417156
116.425529 0.419178
116.425529 0.420973
116.425529 0.422981
116.425529 0.424843
116.425529 0.426768
118.736839 0.419548
118.736839 0.421508
123.298965 0.414871
123.298965 0.417183
123.298965 0.419401
123.298965 0.421697
123.298965 0.423998
127.878784 0.418197
127.878784 0.420523
127.878784 0.422488
130.160004 0.417158
130.160004 0.418379
132.435638 0.417603
132.435638 0.418707
132.435638 0.419931
132.435638 0.420836
132.435638 0.421596
132.435638 0.422818
132.435638 0.424466
132.435638 0.425371
132.435638 0.426395
132.435638 0.427914
132.435638 0.429313
132.435638 0.430823
132.435638 0.432336
132.435638 0.433625
132.435638 0.434853
132.435638 0.435888
132.435638 0.437307
132.435638 0.438698
132.435638 0.440170
132.435638 0.441775
132.435638 0.443419
132.435638 0.445034
132.435638 0.446626
135.117645 0.446478
135.117645 0.448498
135.117645 0.450379
137.805832 0.450758
137.805832 0.452369
137.805832 0.453790
140.500000 0.452428
140.500000 0.453615
140.500000 0.455158
140.500000 0.456266
140.500000 0.457744
140.500000 0.459263
140.500000 0.460510
146.000000 0.458754
146.000000 0.460754
146.000000 0.462367
148.728973 0.458569
148.728973 0.459748
151.444443 0.456850
151.444443 0.457849
151.444443 0.458518
151.444443 0.459044
154.183487 0.454969
154.183487 0.455871
154.183487 0.457014
154.183487 0.458634
154.183487 0.460602
156.963638 0.459366
156.963638 0.461718
156.963638 0.463754
156.963638 0.465836
159.765762 0.466588
159.765762 0.468551
162.553574 0.469231
162.553574 0.470840
162.553574 0.472347
162.553574 0.474064
162.553574 0.475662
165.380524 0.474790
165.380524 0.476529
165.380524 0.478262
165.380524 0.480270
168.228073 0.479127
168.228073 0.480722
168.228073 0.482276
168.228073 0.483807
171.095657 0.481561
171.095657 0.483018
171.095657 0.484491
171.095657 0.485876
171.095657 0.486836
174.000000 0.479932
174.000000 0.480876
174.000000 0.482211
174.000000 0.483772
174.000000 0.485266
176.940170 0.484934
176.940170 0.486126
176.940170 0.487668
182.773102 0.484310
182.773102 0.485425
182.773102 0.486703
182.773102 0.487902
182.773102 0.489407
182.773102 0.490831
182.773102 0.492270
182.773102 0.493267
185.750000 0.492762
185.750000 0.494398
185.750000 0.496253
185.750000 0.498409
188.743805 0.498296
188.743805 0.500088
191.721313 0.498919
191.721313 0.500570
194.682922 0.501554
197.612900 0.501737
197.612900 0.503267
203.396820 0.498732
203.396820 0.500436
203.396820 0.502443
203.396820 0.504337
203.396820 0.506399
203.396820 0.508650
203.396820 0.511061
203.396820 0.513189
206.346451 0.510330
212.139542 0.506041
212.139542 0.508203
212.139542 0.510259
212.139542 0.511904
212.139542 0.513885
212.139542 0.515637
212.139542 0.517768
212.139542 0.519733
218.000000 0.517849
218.000000 0.519249
218.000000 0.521141
218.000000 0.523218
218.000000 0.524727
220.939392 0.524788
223.849625 0.524363
223.849625 0.526240
223.849625 0.528237
223.849625 0.529974
226.776123 0.525116
226.776123 0.527071
226.776123 0.528920
226.776123 0.530846
226.776123 0.532501
226.776123 0.533743
226.776123 0.535584
226.776123 0.537778
226.776123 0.539829
229.792587 0.538242
229.792587 0.540084
232.794113 0.541039
232.794113 0.542174
232.794113 0.543786
232.794113 0.545614
232.794113 0.548092
232.794113 0.549997
232.794113 0.551965
232.794113 0.553390
238.898544 0.549839
238.898544 0.551452
238.898544 0.552890
241.928055 0.548217
241.928055 0.549717
244.942856 0.549774
247.929077 0.547548
253.804199 0.540854
256.694458 0.542392
256.694458 0.544600
256.694458 0.546395
256.694458 0.548264
256.694458 0.550154
256.694458 0.551520
256.694458 0.552754
256.694458 0.554044
256.694458 0.554819
256.694458 0.555943
256.694458 0.556852
256.694458 0.557609
259.710358 0.552455
259.710358 0.553996
259.710358 0.555188
259.710358 0.556473
259.710358 0.558135
259.710358 0.559495
259.710358 0.560568
265.809509 0.556580
265.809509 0.558309
268.824310 0.552312
271.812073 0.552741
274.773346 0.553635
274.773346 0.555392
274.773346 0.557751
277.735107 0.553403
277.735107 0.555205
277.735107 0.557103
277.735107 0.559738
280.710541 0.556441
280.710541 0.558918
283.673218 0.559985
286.610382 0.556405
289.522583 0.557402
292.410248 0.556717
292.410248 0.559423
292.410248 0.561909
298.151886 0.558579
298.151886 0.561048
298.151886 0.563522
301.006287 0.559312
301.006287 0.561419
301.006287 0.563772
301.006287 0.566226
303.875000 0.564041
303.875000 0.565598
303.875000 0.567216
303.875000 0.568609
306.757751 0.564692
306.757751 0.566679
309.629639 0.566207
309.629639 0.567489
309.629639 0.568347
309.629639 0.569693
309.629639 0.571102
309.629639 0.572192
309.629639 0.573383
309.629639 0.574838
309.629639 0.576320
309.629639 0.577541
309.629639 0.578503
309.629639 0.579791
309.629639 0.580433
309.629639 0.581056
309.629639 0.582183
309.629639 0.583202
309.629639 0.584189
315.682922 0.574526
315.682922 0.574885
315.682922 0.575113
315.682922 0.576216
315.682922 0.576989
315.682922 0.577936
315.682922 0.579123
315.682922 0.580188
315.682922 0.581035
315.682922 0.582222
315.682922 0.583454
315.682922 0.585032
315.682922 0.586453
315.682922 0.587781
318.824249 0.582065
318.824249 0.582767
318.824249 0.583438
321.963867 0.581334
325.077850 0.581274
325.077850 0.582349
325.077850 0.583338
328.190491 0.582255
328.190491 0.583067
328.190491 0.584085
331.301788 0.580661
331.301788 0.581524
334.399994 0.574345
334.399994 0.575978
334.399994 0.578117
334.399994 0.580143
334.399994 0.581951
337.520477 0.579152
340.616272 0.575748
340.616272 0.577218
340.616272 0.578615
340.616272 0.580170
340.616272 0.581494
343.734100 0.581586
343.734100 0.583210
343.734100 0.584378
343.734100 0.586011
343.734100 0.587264
343.734100 0.589218
346.885071 0.589976
346.885071 0.591745
346.885071 0.593747
346.885071 0.595170
346.885071 0.596005
353.193176 0.586635
356.305084 0.585850
356.305084 0.586532
356.305084 0.587461
356.305084 0.588595
356.305084 0.590150
359.438202 0.591011
359.438202 0.592195
359.438202 0.593780
359.438202 0.595267
359.438202 0.597234
359.438202 0.598314
359.438202 0.599577
359.438202 0.600814
359.438202 0.602580
359.438202 0.605345
359.438202 0.607779
359.438202 0.610294
362.670380 0.611560
362.670380 0.614039
365.888885 0.614827
369.082886 0.611835
372.252747 0.602588
372.252747 0.604370
378.532623 0.596366
378.532623 0.597258
381.643250 0.590785
381.643250 0.591414
381.643250 0.592464
381.643250 0.593473
384.763428 0.592830
384.763428 0.593711
384.763428 0.595328
384.763428 0.597187
384.763428 0.598860
384.763428 0.600674
384.763428 0.602512
387.925140 0.598699
387.925140 0.601073
391.074463 0.602034
397.294739 0.588964
397.294739 0.589991
397.294739 0.591145
397.294739 0.592416
397.294739 0.593944
400.408386 0.589568
400.408386 0.590947
403.510406 0.591392
406.590668 0.584604
406.590668 0.585970
406.590668 0.587696
406.590668 0.589257
406.590668 0.590540
406.590668 0.592162
406.590668 0.593835
406.590668 0.595770
406.590668 0.597919
406.590668 0.600186
409.742279 0.596938
409.742279 0.598977
409.742279 0.600646
412.892303 0.601365
412.892303 0.603160
416.030609 0.597586
416.030609 0.598568
416.030609 0.600135
416.030609 0.601608
416.030609 0.602623
416.030609 0.603667
419.197968 0.600586
419.197968 0.602166
422.353546 0.602071
422.353546 0.603110
422.353546 0.604125
422.353546 0.605225
422.353546 0.607047
422.353546 0.608185
422.353546 0.609736
422.353546 0.611283
422.353546 0.612720
422.353546 0.613252
425.577881 0.612808
425.577881 0.614032
425.577881 0.614857
425.577881 0.615769
425.577881 0.617307
428.820007 0.611310
428.820007 0.612129
428.820007 0.612927
428.820007 0.613991
428.820007 0.615347
428.820007 0.616713
428.820007 0.618280
428.820007 0.619678
428.820007 0.621304
428.820007 0.623087
428.820007 0.624422
428.820007 0.625609
428.820007 0.626483
428.820007 0.627703
428.820007 0.628262
428.820007 0.629277
428.820007 0.630357
428.820007 0.631500
428.820007 0.633311
435.584167 0.628954
435.584167 0.630615
435.584167 0.632235
438.945801 0.631720
438.945801 0.632638
438.945801 0.633836
438.945801 0.635211
438.945801 0.636420
438.945801 0.638218
438.945801 0.639817
438.945801 0.641434
438.945801 0.643125
442.362732 0.642664
445.756104 0.640610
445.756104 0.641544
445.756104 0.643229
445.756104 0.644579
445.756104 0.645891
445.756104 0.647718
445.756104 0.649001
445.756104 0.650369
445.756104 0.651650
445.756104 0.652430
445.756104 0.654310
445.756104 0.655896
445.756104 0.657412
445.756104 0.658975
445.756104 0.660717
445.756104 0.662184
445.756104 0.663452
445.756104 0.664436
445.756104 0.665430
445.756104 0.667235
445.756104 0.668829
445.756104 0.669672
445.756104 0.670276
445.756104 0.670960
445.756104 0.671864
445.756104 0.673030
445.756104 0.674136
445.756104 0.675406
445.756104 0.676887
445.756104 0.678445
445.756104 0.679812
445.756104 0.681697
445.756104 0.683709
445.756104 0.685583
449.446594 0.681602
449.446594 0.682993
449.446594 0.684276
449.446594 0.685013
449.446594 0.685101
449.446594 0.685552
449.446594 0.686046
449.446594 0.687271
449.446594 0.688072
449.446594 0.688984
449.446594 0.689385
449.446594 0.689906
449.446594 0.690799
449.446594 0.692733
449.446594 0.694792
449.446594 0.697050
449.446594 0.698996
453.265686 0.696208
453.265686 0.698795
457.067322 0.694978
460.842102 0.689255
460.842102 0.691424
460.842102 0.693302
460.842102 0.695319
464.619049 0.696592
464.619049 0.698651
464.619049 0.700384
464.619049 0.702825
468.398102 0.694040
468.398102 0.695462
472.160370 0.693552
472.160370 0.695543
475.906097 0.688414
475.906097 0.690130
475.906097 0.690905
475.906097 0.692627
475.906097 0.694308
475.906097 0.695296
479.672882 0.685062
479.672882 0.686300
483.423248 0.682432
483.423248 0.683390
483.423248 0.683954
483.423248 0.684456
483.423248 0.685064
483.423248 0.685440
490.930878 0.674310
494.642212 0.673906
494.642212 0.674924
502.000000 0.668696
502.000000 0.668968
502.000000 0.668958
505.656097 0.659306
505.656097 0.660117
505.656097 0.660591
505.656097 0.660852
505.656097 0.661163
505.656097 0.661405
505.656097 0.661000
505.656097 0.660791
505.656097 0.660608
505.656097 0.660960
505.656097 0.661928
505.656097 0.663158
505.656097 0.664090
509.396393 0.664158
509.396393 0.665007
509.396393 0.665624
509.396393 0.666409
513.139038 0.659810
513.139038 0.660708
513.139038 0.661508
513.139038 0.662405
513.139038 0.662948
513.139038 0.663867
513.139038 0.665425
513.139038 0.667162
513.139038 0.669224
513.139038 0.670831
513.139038 0.673093
513.139038 0.675024
513.139038 0.676497
516.964294 0.677677
524.530945 0.672057
524.530945 0.673241
524.530945 0.674027
524.530945 0.675290
524.530945 0.676242
524.530945 0.677621
524.530945 0.678797
524.530945 0.679892
524.530945 0.681006
528.343628 0.679976
528.343628 0.680251
528.343628 0.680765
528.343628 0.681518
528.343628 0.682452
528.343628 0.683638
528.343628 0.684240
532.184204 0.678417
532.184204 0.678777
532.184204 0.679342
532.184204 0.680135
532.184204 0.681439
532.184204 0.682442
532.184204 0.684229
532.184204 0.685627
536.061157 0.680109
536.061157 0.681273
536.061157 0.682260
536.061157 0.683372
536.061157 0.684014
536.061157 0.685330
536.061157 0.686707
536.061157 0.688268
536.061157 0.689804
536.061157 0.691325
536.061157 0.693638
536.061157 0.695405
536.061157 0.696687
536.061157 0.698108
536.061157 0.700180
536.061157 0.701805
536.061157 0.703530
540.052185 0.694506
544.017334 0.689470
544.017334 0.690927
547.965515 0.689240
547.965515 0.691073
547.965515 0.692439
547.965515 0.694372
547.965515 0.696345
547.965515 0.698306
547.965515 0.699902
547.965515 0.701392
551.948486 0.700631
551.948486 0.701847
551.948486 0.703390
551.948486 0.705125
551.948486 0.706916
551.948486 0.709110
551.948486 0.710405
559.931885 0.702980
559.931885 0.704686
559.931885 0.705784
567.831238 0.698181
567.831238 0.699470
567.831238 0.700110
567.831238 0.701217
567.831238 0.702051
571.773132 0.694212
571.773132 0.695434
571.773132 0.697091
571.773132 0.697807
571.773132 0.699074
571.773132 0.699828
579.658325 0.685738
579.658325 0.686143
579.658325 0.686765
579.658325 0.686921
579.658325 0.687283
579.658325 0.687171
579.658325 0.687469
579.658325 0.687634
579.658325 0.688122
579.658325 0.689322
579.658325 0.691033
579.658325 0.692942
579.658325 0.694321
579.658325 0.695455
579.658325 0.697305
579.658325 0.698910
579.658325 0.700591
579.658325 0.702578
579.658325 0.704324
579.658325 0.705801
579.658325 0.707280
579.658325 0.708816
579.658325 0.710264
579.658325 0.711543
579.658325 0.713016
579.658325 0.713942
579.658325 0.714726
579.658325 0.715900
583.784241 0.716460
583.784241 0.717426
583.784241 0.718281
583.784241 0.719681
583.784241 0.720768
587.917358 0.713938
587.917358 0.715034
587.917358 0.716110
587.917358 0.717223
587.917358 0.718635
587.917358 0.720169
592.065857 0.718735
592.065857 0.720201
592.065857 0.722300
592.065857 0.724510
592.065857 0.726278
596.221313 0.723479
596.221313 0.724712
596.221313 0.725873
604.479675 0.715066
604.479675 0.716276
604.479675 0.717216
604.479675 0.717892
604.479675 0.718062
604.479675 0.719135
604.479675 0.720255
604.479675 0.720557
604.479675 0.720119
604.479675 0.720087
604.479675 0.719939
604.479675 0.719845
604.479675 0.719615
604.479675 0.719226
604.479675 0.718246
604.479675 0.717740
604.479675 0.717511
604.479675 0.717700
604.479675 0.718640
604.479675 0.719956
604.479675 0.720996
604.479675 0.722465
604.479675 0.723697
608.744934 0.722780
608.744934 0.724770
608.744934 0.726617
608.744934 0.729202
608.744934 0.731647
608.744934 0.734019
608.744934 0.736252
613.032288 0.726119
613.032288 0.726996
613.032288 0.728176
613.032288 0.729765
613.032288 0.730829
613.032288 0.732182
613.032288 0.733300
613.032288 0.734375
613.032288 0.735727
613.032288 0.737357
613.032288 0.738784
613.032288 0.740371
613.032288 0.741964
613.032288 0.743548
613.032288 0.745253
613.032288 0.746795
613.032288 0.748062
613.032288 0.749513
613.032288 0.750748
613.032288 0.751502
613.032288 0.751500
613.032288 0.752159
613.032288 0.753163
617.469910 0.751055
617.469910 0.752147
617.469910 0.753505
617.469910 0.755489
617.469910 0.757122
617.469910 0.758788
617.469910 0.760674
617.469910 0.761813
617.469910 0.763390
617.469910 0.764404
621.952026 0.754276
621.952026 0.755135
621.952026 0.756215
621.952026 0.757248
621.952026 0.757687
621.952026 0.758246
621.952026 0.758521
621.952026 0.758638
621.952026 0.758817
621.952026 0.759192
621.952026 0.759774
621.952026 0.760041
621.952026 0.760720
621.952026 0.761763
621.952026 0.762578
621.952026 0.763223
621.952026 0.764318
621.952026 0.765591
621.952026 0.766140
621.952026 0.766683
621.952026 0.767805
621.952026 0.769943
626.573730 0.770951
626.573730 0.773220
626.573730 0.775521
626.573730 0.777062
626.573730 0.778320
626.573730 0.779430
626.573730 0.780276
626.573730 0.781271
626.573730 0.782952
626.573730 0.784675
626.573730 0.786348
626.573730 0.788044
626.573730 0.789547
626.573730 0.790628
626.573730 0.791509
626.573730 0.792975
626.573730 0.793616
626.573730 0.793701
626.573730 0.793904
626.573730 0.793830
631.317444 0.787499
631.317444 0.787755
631.317444 0.788536
631.317444 0.788826
631.317444 0.789858
631.317444 0.790977
631.317444 0.792421
631.317444 0.793839
631.317444 0.795311
631.317444 0.796620
631.317444 0.797945
631.317444 0.799334
631.317444 0.800437
631.317444 0.800906
631.317444 0.802437
631.317444 0.803987
631.317444 0.805620
631.317444 0.806874
631.317444 0.808100
631.317444 0.809543
631.317444 0.811364
631.317444 0.813407
631.317444 0.814788
631.317444 0.815272
631.317444 0.816140
636.221313 0.816347
636.221313 0.817305
636.221313 0.818040
636.221313 0.818422
636.221313 0.818819
636.221313 0.819018
636.221313 0.819481
636.221313 0.818998
636.221313 0.819387
636.221313 0.819933
636.221313 0.820681
636.221313 0.821551
636.221313 0.822709
636.221313 0.823525
636.221313 0.824489
636.221313 0.825216
636.221313 0.825912
636.221313 0.827014
636.221313 0.828001
636.221313 0.829500
636.221313 0.831241
636.221313 0.832208
636.221313 0.832452
636.221313 0.832752
641.275574 0.822617
641.275574 0.823675
641.275574 0.824498
641.275574 0.825387
651.328125 0.816245
651.328125 0.816221
651.328125 0.816172
651.328125 0.816028
651.328125 0.815617
651.328125 0.815587
651.328125 0.815861
651.328125 0.816191
651.328125 0.816492
651.328125 0.816911
651.328125 0.817531
651.328125 0.818341
651.328125 0.819036
651.328125 0.819343
656.404663 0.812986
656.404663 0.813362
656.404663 0.813805
656.404663 0.813953
656.404663 0.814541
656.404663 0.815279
656.404663 0.816159
656.404663 0.816961
656.404663 0.818023
661.511658 0.815179
661.511658 0.816534
661.511658 0.817803
661.511658 0.819349
661.511658 0.821274
661.511658 0.823686
661.511658 0.825609
661.511658 0.827305
666.640930 0.829934
666.640930 0.832126
671.746155 0.824275
671.746155 0.824998
671.746155 0.825484
671.746155 0.826269
671.746155 0.827204
671.746155 0.828607
671.746155 0.829810
671.746155 0.830831
671.746155 0.831688
671.746155 0.832279
671.746155 0.833191
671.746155 0.834046
671.746155 0.835013
671.746155 0.835657
671.746155 0.836472
671.746155 0.836898
671.746155 0.837753
671.746155 0.838184
671.746155 0.838562
671.746155 0.839106
671.746155 0.839949
671.746155 0.841124
671.746155 0.842115
671.746155 0.842983
671.746155 0.843313
671.746155 0.843575
671.746155 0.844272
671.746155 0.845338
671.746155 0.846478
671.746155 0.847900
671.746155 0.849792
677.049805 0.846758
677.049805 0.847762
677.049805 0.849059
677.049805 0.850905
677.049805 0.852098
677.049805 0.852376
677.049805 0.852742
677.049805 0.852800
687.657776 0.835301
692.909119 0.835020
692.909119 0.836423
698.135864 0.836364
698.135864 0.837358
698.135864 0.837742
698.135864 0.838574
698.135864 0.839324
698.135864 0.839897
698.135864 0.840866
698.135864 0.842515
698.135864 0.844022
698.135864 0.845761
698.135864 0.847676
698.135864 0.849524
698.135864 0.851404
698.135864 0.852639
698.135864 0.854242
698.135864 0.855843
698.135864 0.857789
698.135864 0.860094
698.135864 0.862063
698.135864 0.863585
698.135864 0.864921
698.135864 0.865897
698.135864 0.866807
698.135864 0.868420
698.135864 0.869378
698.135864 0.870451
698.135864 0.871805
698.135864 0.872918
698.135864 0.874629
698.135864 0.875898
698.135864 0.876793
698.135864 0.878060
698.135864 0.879326
698.135864 0.880686
698.135864 0.881943
698.135864 0.883160
698.135864 0.885106
698.135864 0.886544
698.135864 0.887746
698.135864 0.888954
698.135864 0.889912
698.135864 0.890858
698.135864 0.892175
698.135864 0.893190
698.135864 0.894090
703.661682 0.867807
709.153564 0.862251
709.153564 0.862964
709.153564 0.864060
709.153564 0.864943
709.153564 0.865708
709.153564 0.866206
709.153564 0.866888
709.153564 0.867744
709.153564 0.868976
709.153564 0.870513
709.153564 0.872409
709.153564 0.873788
709.153564 0.875591
709.153564 0.877553
714.708984 0.873712
714.708984 0.875018
714.708984 0.876572
714.708984 0.878305
714.708984 0.879684
714.708984 0.880895
714.708984 0.881885
714.708984 0.882794
714.708984 0.883707
714.708984 0.884984
720.297424 0.882724
720.297424 0.883171
720.297424 0.883176
720.297424 0.883622
720.297424 0.884614
720.297424 0.885804
720.297424 0.886766
720.297424 0.888059
720.297424 0.889189
720.297424 0.890508
720.297424 0.891632
720.297424 0.892825
720.297424 0.893896
720.297424 0.894459
720.297424 0.894900
720.297424 0.895767
720.297424 0.896769
720.297424 0.898007
720.297424 0.899466
720.297424 0.900710
720.297424 0.901927
720.297424 0.903310
720.297424 0.905084
720.297424 0.906930
720.297424 0.908783
720.297424 0.910309
720.297424 0.912658
720.297424 0.915179
720.297424 0.917106
726.059265 0.909757
726.059265 0.911400
726.059265 0.914258
726.059265 0.915967
726.059265 0.917927
726.059265 0.920330
726.059265 0.922863
726.059265 0.925100
726.059265 0.926904
726.059265 0.928579
726.059265 0.930182
726.059265 0.931846
726.059265 0.933424
726.059265 0.935072
726.059265 0.936373
731.889282 0.923250
731.889282 0.923209
731.889282 0.924172
731.889282 0.925002
731.889282 0.925592
731.889282 0.926432
737.720581 0.919677
737.720581 0.920388
737.720581 0.920772
737.720581 0.920891
737.720581 0.921215
737.720581 0.921741
737.720581 0.922815
737.720581 0.924285
743.567749 0.921577
743.567749 0.923132
743.567749 0.924810
743.567749 0.926483
743.567749 0.927745
743.567749 0.929129
743.567749 0.930310
743.567749 0.931367
743.567749 0.932572
743.567749 0.933602
743.567749 0.934349
743.567749 0.934757
743.567749 0.936509
743.567749 0.937764
743.567749 0.938782
743.567749 0.940315
743.567749 0.942046
743.567749 0.943474
749.503662 0.924039
749.503662 0.925189
749.503662 0.926986
749.503662 0.928428
749.503662 0.930312
749.503662 0.932015
749.503662 0.933018
749.503662 0.934202
749.503662 0.935834
755.461792 0.923234
755.461792 0.924707
755.461792 0.925931
755.461792 0.927053
755.461792 0.928382
755.461792 0.929869
755.461792 0.930841
755.461792 0.931787
755.461792 0.932202
755.461792 0.933457
755.461792 0.934256
761.456543 0.930358
761.456543 0.931243
761.456543 0.931854
761.456543 0.932149
761.456543 0.932301
761.456543 0.932735
761.456543 0.933109
761.456543 0.933392
761.456543 0.933686
761.456543 0.933818
761.456543 0.934413
761.456543 0.935064
761.456543 0.936122
761.456543 0.936981
761.456543 0.937798
761.456543 0.938650
761.456543 0.939582
761.456543 0.940491
761.456543 0.940915
761.456543 0.941320
761.456543 0.941736
761.456543 0.942616
761.456543 0.942991
761.456543 0.943388
761.456543 0.943732
761.456543 0.944361
761.456543 0.945372
761.456543 0.946267
761.456543 0.946716
761.456543 0.947085
761.456543 0.948075
761.456543 0.948699
761.456543 0.949194
761.456543 0.950215
761.456543 0.950576
761.456543 0.951203
761.456543 0.951982
761.456543 0.953595
761.456543 0.955774
761.456543 0.957093
761.456543 0.958320
761.456543 0.958932
761.456543 0.959771
761.456543 0.960514
761.456543 0.961446
761.456543 0.962884
761.456543 0.964165
761.456543 0.965667
761.456543 0.968004
761.456543 0.970017
761.456543 0.971668
761.456543 0.973449
761.456543 0.975019
774.079163 0.954705
774.079163 0.955369
774.079163 0.956271
774.079163 0.957098
774.079163 0.957548
774.079163 0.958193
774.079163 0.959629
774.079163 0.961002
780.379944 0.953114
780.379944 0.954514
780.379944 0.955315
780.379944 0.955747
780.379944 0.956699
780.379944 0.957691
780.379944 0.957788
780.379944 0.958487
780.379944 0.959553
786.700012 0.956859
786.700012 0.957621
786.700012 0.959330
786.700012 0.960765
793.003540 0.961276
793.003540 0.963109
793.003540 0.964426
793.003540 0.965941
793.003540 0.967835
793.003540 0.969094
793.003540 0.970840
793.003540 0.972441
793.003540 0.974361
793.003540 0.977085
793.003540 0.979067
793.003540 0.980524
793.003540 0.982602
793.003540 0.985455
793.003540 0.987566
799.368774 0.971893
799.368774 0.973632
799.368774 0.975157
799.368774 0.976389
799.368774 0.977616
799.368774 0.978271
799.368774 0.978033
799.368774 0.978185
799.368774 0.978789
799.368774 0.978817
799.368774 0.979479
805.766785 0.978202
805.766785 0.978381
805.766785 0.978639
805.766785 0.978654
805.766785 0.978998
805.766785 0.979012
805.766785 0.979093
805.766785 0.979163
805.766785 0.979585
805.766785 0.980354
805.766785 0.981112
805.766785 0.981389
805.766785 0.981566
805.766785 0.982035
805.766785 0.982852
812.225342 0.980549
818.645630 0.982242
818.645630 0.982932
825.034973 0.972117
825.034973 0.971727
825.034973 0.971306
825.034973 0.971892
825.034973 0.973015
825.034973 0.973758
825.034973 0.974435
825.034973 0.975425
825.034973 0.976976
825.034973 0.978083
825.034973 0.979148
825.034973 0.980679
825.034973 0.982077
825.034973 0.983209
825.034973 0.984171
825.034973 0.985445
825.034973 0.987049
831.498230 0.973108
831.498230 0.974138
831.498230 0.975607
831.498230 0.976707
831.498230 0.978001
831.498230 0.979472
831.498230 0.980553
831.498230 0.982121
831.498230 0.984420
831.498230 0.986281
831.498230 0.988133
831.498230 0.990620
831.498230 0.992549
831.498230 0.993816
831.498230 0.995145
831.498230 0.995859
831.498230 0.996250
831.498230 0.995964
831.498230 0.995810
831.498230 0.995656
831.498230 0.994525
831.498230 0.994172
831.498230 0.993660
831.498230 0.993731
831.498230 0.993892
831.498230 0.994540
831.498230 0.995995
831.498230 0.996804
831.498230 0.997803
831.498230 0.999225
831.498230 1.000386
831.498230 1.001638
831.498230 1.002905
831.498230 1.004075
831.498230 1.004571
831.498230 1.005313
831.498230 1.007021
831.498230 1.008395
831.498230 1.010719
831.498230 1.012663
831.498230 1.014020
831.498230 1.014939
831.498230 1.015825
831.498230 1.016476
831.498230 1.017253
831.498230 1.018029
831.498230 1.018846
831.498230 1.019832
831.498230 1.021171
838.256958 1.005454
838.256958 1.006657
844.982727 1.000078
844.982727 1.002481
844.982727 1.004408
844.982727 1.005949
844.982727 1.007721
844.982727 1.009557
844.982727 1.010952
844.982727 1.011978
851.717224 0.998265
851.717224 0.999349
851.717224 1.000599
851.717224 1.001355
851.717224 1.002204
851.717224 1.002489
851.717224 1.003453
851.717224 1.004098
851.717224 1.005694
851.717224 1.006884
851.717224 1.007054
858.481079 1.009444
858.481079 1.010276
858.481079 1.011393
858.481079 1.012433
858.481079 1.013299
858.481079 1.014075
858.481079 1.014886
858.481079 1.015798
858.481079 1.015820
858.481079 1.016162
858.481079 1.016289
858.481079 1.017348
858.481079 1.018304
858.481079 1.019643
858.481079 1.019920
858.481079 1.020870
858.481079 1.021761
858.481079 1.022833
858.481079 1.023149
858.481079 1.024098
858.481079 1.025080
858.481079 1.026889
858.481079 1.028256
858.481079 1.029538
865.363037 1.023591
865.363037 1.025409
865.363037 1.026485
865.363037 1.027848
865.363037 1.028642
865.363037 1.030039
865.363037 1.030333
865.363037 1.031697
865.363037 1.032915
865.363037 1.034312
865.363037 1.035172
865.363037 1.035784
865.363037 1.035628
865.363037 1.034993
865.363037 1.034708
865.363037 1.035682
865.363037 1.036454
865.363037 1.037569
865.363037 1.038179
865.363037 1.038858
865.363037 1.040490
865.363037 1.042469
865.363037 1.044252
865.363037 1.046096
865.363037 1.047566
865.363037 1.048632
865.363037 1.050098
865.363037 1.051181
865.363037 1.052609
865.363037 1.053987
865.363037 1.055406
865.363037 1.056482
865.363037 1.056750
865.363037 1.058300
865.363037 1.059260
865.363037 1.059521
865.363037 1.059906
865.363037 1.060284
865.363037 1.061655
865.363037 1.061954
865.363037 1.062783
865.363037 1.063095
865.363037 1.063794
865.363037 1.064991
865.363037 1.066197
865.363037 1.067693
865.363037 1.069368
865.363037 1.070545
865.363037 1.071743
865.363037 1.072866
865.363037 1.073681
865.363037 1.074274
865.363037 1.075707
865.363037 1.076489
865.363037 1.077533
865.363037 1.079240
865.363037 1.080504
865.363037 1.082515
872.593872 1.059969
872.593872 1.062163
872.593872 1.064345
872.593872 1.066111
872.593872 1.067576
872.593872 1.069598
872.593872 1.070818
872.593872 1.071844
872.593872 1.072993
872.593872 1.074997
872.593872 1.076869
872.593872 1.077885
872.593872 1.079980
872.593872 1.081956
872.593872 1.084019
872.593872 1.085655
872.593872 1.086745
872.593872 1.087490
872.593872 1.087480
872.593872 1.087433
872.593872 1.087939
872.593872 1.088934
872.593872 1.090042
872.593872 1.090526
872.593872 1.091826
872.593872 1.092322
872.593872 1.091730
872.593872 1.092702
887.288147 1.082110
887.288147 1.082520
887.288147 1.083522
894.581055 1.082213
894.581055 1.083382
894.581055 1.084923
894.581055 1.085727
894.581055 1.087759
901.858582 1.067722
901.858582 1.069036
901.858582 1.070784
901.858582 1.072744
901.858582 1.075155
901.858582 1.077493
909.127502 1.061963
909.127502 1.062492
909.127502 1.063374
909.127502 1.064883
909.127502 1.066220
909.127502 1.068020
909.127502 1.069351
909.127502 1.069687
909.127502 1.070099
909.127502 1.070841
909.127502 1.072356
909.127502 1.073956
909.127502 1.074871
909.127502 1.076094
909.127502 1.077643
909.127502 1.078462
909.127502 1.080013
909.127502 1.082070
909.127502 1.082870
909.127502 1.084731
909.127502 1.085988
909.127502 1.087325
909.127502 1.088495
909.127502 1.090538
916.508362 1.088017
916.508362 1.088987
916.508362 1.090737
916.508362 1.092486
916.508362 1.093554
916.508362 1.093936
916.508362 1.093998
916.508362 1.094782
916.508362 1.095251
916.508362 1.095815
916.508362 1.096212
916.508362 1.096473
923.919983 1.068456
923.919983 1.069230
931.295654 1.065076
931.295654 1.065268
931.295654 1.065155
931.295654 1.065099
931.295654 1.065790
931.295654 1.067756
931.295654 1.069604
931.295654 1.072022
931.295654 1.074064
931.295654 1.075455
938.688721 1.063732
938.688721 1.064175
938.688721 1.064738
938.688721 1.065445
946.059387 1.060053
953.388184 1.028685
953.388184 1.028285
953.388184 1.027727
953.388184 1.026934
953.388184 1.025695
953.388184 1.024936
953.388184 1.024706
953.388184 1.025289
953.388184 1.026510
953.388184 1.027545
953.388184 1.027901
953.388184 1.028057
953.388184 1.027919
953.388184 1.027662
953.388184 1.028168
953.388184 1.029008
953.388184 1.030331
953.388184 1.031298
953.388184 1.032419
953.388184 1.033788
953.388184 1.034665
953.388184 1.035793
953.388184 1.037096
953.388184 1.038293
953.388184 1.039860
953.388184 1.041005
953.388184 1.041978
953.388184 1.042556
960.852478 1.027538
960.852478 1.028500
960.852478 1.029024
960.852478 1.029767
968.294128 1.012835
975.693787 0.972337
975.693787 0.972988
975.693787 0.973689
975.693787 0.974732
975.693787 0.975416
975.693787 0.976481
975.693787 0.977487
975.693787 0.978722
975.693787 0.979477
975.693787 0.980520
975.693787 0.981248
975.693787 0.981580
975.693787 0.981928
975.693787 0.981943
975.693787 0.982136
975.693787 0.982536
975.693787 0.982813
975.693787 0.983554
975.693787 0.983831
975.693787 0.984707
975.693787 0.985625
975.693787 0.987023
975.693787 0.987850
975.693787 0.988548
975.693787 0.989421
975.693787 0.990296
975.693787 0.990698
975.693787 0.990959
975.693787 0.991083
975.693787 0.991061
975.693787 0.991205
975.693787 0.991191
975.693787 0.990633
975.693787 0.990402
975.693787 0.990665
975.693787 0.991272
975.693787 0.993171
983.285706 0.996034
983.285706 0.997491
983.285706 0.998719
983.285706 1.000739
983.285706 1.001918
983.285706 1.003065
983.285706 1.004532
983.285706 1.005972
983.285706 1.007043
983.285706 1.008614
983.285706 1.010187
983.285706 1.011741
983.285706 1.013216
983.285706 1.014234
983.285706 1.015023
983.285706 1.015743
983.285706 1.017022
983.285706 1.018456
983.285706 1.020055
990.951477 1.010740
990.951477 1.011598
990.951477 1.012274
990.951477 1.012238
990.951477 1.011980
990.951477 1.012138
990.951477 1.011897
990.951477 1.012394
990.951477 1.012633
990.951477 1.013864
990.951477 1.014457
990.951477 1.014621
990.951477 1.015069
990.951477 1.016227
990.951477 1.017810
990.951477 1.019169
990.951477 1.021042
990.951477 1.022866
990.951477 1.025166
990.951477 1.026087
990.951477 1.027125
990.951477 1.027444
990.951477 1.027947
990.951477 1.028410
990.951477 1.029102
990.951477 1.029384
998.735474 1.014742
998.735474 1.015910
998.735474 1.017076
998.735474 1.017744
998.735474 1.019316
998.735474 1.020329
998.735474 1.021560
998.735474 1.022296
998.735474 1.022978
998.735474 1.024239
998.735474 1.025406
998.735474 1.025769
998.735474 1.026522
998.735474 1.027314
998.735474 1.028183
998.735474 1.029288
998.735474 1.030462
998.735474 1.031747
998.735474 1.032492
998.735474 1.033377
998.735474 1.033810
998.735474 1.034257
998.735474 1.033788
998.735474 1.033468
998.735474 1.033506
998.735474 1.033964
998.735474 1.034785
998.735474 1.035869
998.735474 1.037121
998.735474 1.038465
998.735474 1.040119
998.735474 1.041587
1006.675232 1.014827
1006.675232 1.016011
1006.675232 1.017105
1006.675232 1.017767
1006.675232 1.019702
1006.675232 1.021166
1006.675232 1.021953
1006.675232 1.022974
1006.675232 1.024113
1006.675232 1.025582
1006.675232 1.027266
1006.675232 1.029650
1006.675232 1.031643
1006.675232 1.033130
1006.675232 1.034126
1006.675232 1.035087
1006.675232 1.036095
1014.673096 1.037923
1014.673096 1.039380
1014.673096 1.040194
1014.673096 1.041236
1014.673096 1.042048
1014.673096 1.043025
1014.673096 1.044176
1014.673096 1.044698
1014.673096 1.045343
1014.673096 1.046046
1014.673096 1.046733
1014.673096 1.047248
1014.673096 1.047463
1014.673096 1.048306
1014.673096 1.049206
1014.673096 1.050520
1014.673096 1.051664
1014.673096 1.052305
1014.673096 1.053317
1014.673096 1.054397
1014.673096 1.055105
1014.673096 1.056299
1014.673096 1.057008
1014.673096 1.057234
1014.673096 1.057629
1014.673096 1.058519
1014.673096 1.060423
1014.673096 1.062012
1022.798706 1.048994
1022.798706 1.049488
1022.798706 1.050290
1022.798706 1.051354
1022.798706 1.051931
1022.798706 1.052694
1022.798706 1.053543
1022.798706 1.053715
1022.798706 1.054222
1022.798706 1.054906
1022.798706 1.055335
1030.942627 1.051315
1030.942627 1.051991
1030.942627 1.051852
1030.942627 1.051744
1030.942627 1.051605
1030.942627 1.051545
1030.942627 1.051676
1030.942627 1.050550
1030.942627 1.049917
1030.942627 1.050187
1030.942627 1.050104
1030.942627 1.050807
1030.942627 1.051348
1030.942627 1.051470
1030.942627 1.051850
1030.942627 1.052269
1030.942627 1.051625
1030.942627 1.051867
1030.942627 1.051921
1030.942627 1.052660
1039.161865 1.050579
1047.335449 1.037742
1055.463745 1.038087
1055.463745 1.038466
1055.463745 1.038966
1055.463745 1.039477
1055.463745 1.039538
1063.572388 1.042950
1063.572388 1.043519
1063.572388 1.043854
1063.572388 1.044200
1063.572388 1.044911
1071.661499 1.022774
1071.661499 1.022929
1071.661499 1.023412
1071.661499 1.023533
1071.661499 1.024033
1071.661499 1.024996
1071.661499 1.026165
1071.661499 1.027088
1071.661499 1.028464
1071.661499 1.029305
1071.661499 1.030141
1071.661499 1.031929
1071.661499 1.033828
1071.661499 1.035746
1071.661499 1.037284
1071.661499 1.039077
1071.661499 1.041206
1071.661499 1.043283
1071.661499 1.044445
1071.661499 1.044985
1071.661499 1.046411
1071.661499 1.047976
1071.661499 1.049756
1071.661499 1.051143
1071.661499 1.052616
1071.661499 1.053940
1071.661499 1.055497
1071.661499 1.055792
1071.661499 1.056912
1071.661499 1.058380
1071.661499 1.060380
1071.661499 1.061705
1071.661499 1.063238
1071.661499 1.064378
1071.661499 1.065035
1071.661499 1.065795
1071.661499 1.066099
1071.661499 1.066857
1071.661499 1.068118
1071.661499 1.069333
1071.661499 1.070056
1071.661499 1.070518
1071.661499 1.070775
1071.661499 1.070274
1071.661499 1.070622
1071.661499 1.070811
1071.661499 1.071288
1071.661499 1.072117
1071.661499 1.072635
1071.661499 1.073852
1071.661499 1.075360
1071.661499 1.076473
1071.661499 1.077613
1071.661499 1.078292
1071.661499 1.078906
1080.043701 1.063424
1080.043701 1.064459
1080.043701 1.065897
1080.043701 1.066767
1080.043701 1.067702
1080.043701 1.068076
1080.043701 1.068797
1080.043701 1.068647
1080.043701 1.068180
1080.043701 1.068217
1080.043701 1.067813
1080.043701 1.067759
1080.043701 1.068861
1080.043701 1.070124
1080.043701 1.070880
1080.043701 1.072781
1080.043701 1.074313
1080.043701 1.075829
1080.043701 1.077259
1080.043701 1.079157
1080.043701 1.080460
1080.043701 1.080714
1080.043701 1.081123
1080.043701 1.081387
1080.043701 1.082016
1080.043701 1.082438
1080.043701 1.082196
1080.043701 1.082305
1080.043701 1.082969
1080.043701 1.083337
1080.043701 1.083579
1080.043701 1.083647
1080.043701 1.085140
1080.043701 1.086129
1080.043701 1.086879
1080.043701 1.087698
1080.043701 1.088271
1080.043701 1.088873
1080.043701 1.089232
1080.043701 1.089558
1080.043701 1.089413
1080.043701 1.089782
1080.043701 1.090307
1080.043701 1.091210
1080.043701 1.093072
1080.043701 1.095613
1080.043701 1.097956
1088.666626 1.077147
1088.666626 1.079783
1097.248413 1.067834
1097.248413 1.069175
1097.248413 1.070839
1105.795654 1.060796
1105.795654 1.062405
1105.795654 1.064287
1105.795654 1.065694
1105.795654 1.066369
1105.795654 1.067233
1105.795654 1.067949
1105.795654 1.068595
1105.795654 1.068873
1105.795654 1.069314
1105.795654 1.069288
1105.795654 1.069393
1105.795654 1.069642
1105.795654 1.069715
1105.795654 1.070244
1105.795654 1.071181
1105.795654 1.071875
1105.795654 1.072931
1105.795654 1.073610
1105.795654 1.074196
1105.795654 1.075415
1105.795654 1.076182
1105.795654 1.077315
1105.795654 1.078037
1105.795654 1.078835
1105.795654 1.079611
1105.795654 1.080614
1105.795654 1.081351
1105.795654 1.081932
1105.795654 1.082437
1105.795654 1.083166
1105.795654 1.084092
1105.795654 1.085325
1105.795654 1.086517
1105.795654 1.087660
1105.795654 1.088569
1105.795654 1.089771
1105.795654 1.091501
1105.795654 1.092639
1105.795654 1.093909
1105.795654 1.094718
1105.795654 1.095492
1105.795654 1.096390
1105.795654 1.097569
1105.795654 1.098618
1105.795654 1.099589
1105.795654 1.100098
1105.795654 1.100444
1105.795654 1.100672
1105.795654 1.100881
1105.795654 1.100987
1105.795654 1.100866
1105.795654 1.100931
1105.795654 1.101485
1105.795654 1.101992
1105.795654 1.102271
1105.795654 1.102674
1105.795654 1.103588
1105.795654 1.104327
1105.795654 1.104116
1105.795654 1.104616
1105.795654 1.104028
1105.795654 1.103683
1105.795654 1.103464
1105.795654 1.102837
1105.795654 1.102179
1105.795654 1.101940
1105.795654 1.101995
1105.795654 1.102180
1105.795654 1.102854
1105.795654 1.103199
1105.795654 1.103966
1114.734619 1.086463
1114.734619 1.087702
1114.734619 1.089057
1114.734619 1.090273
1114.734619 1.090962
1114.734619 1.092232
1114.734619 1.093678
1114.734619 1.094700
1114.734619 1.095922
1114.734619 1.097614
1114.734619 1.098386
1114.734619 1.099588
1114.734619 1.100982
1114.734619 1.102172
1114.734619 1.103146
1114.734619 1.104019
1114.734619 1.104780
1114.734619 1.105110
1114.734619 1.105808
1114.734619 1.106583
1114.734619 1.107244
1114.734619 1.107900
1114.734619 1.108459
1114.734619 1.109460
1114.734619 1.110739
1114.734619 1.111224
1114.734619 1.111695
1114.734619 1.112881
1114.734619 1.113804
1114.734619 1.115139
1114.734619 1.115655
1114.734619 1.116493
1114.734619 1.117465
1114.734619 1.118010
1114.734619 1.118724
1114.734619 1.120050
1114.734619 1.121563
1114.734619 1.122692
1114.734619 1.124236
1114.734619 1.125640
1114.734619 1.126294
1114.734619 1.126901
1114.734619 1.127741
1114.734619 1.128780
1114.734619 1.130394
1114.734619 1.131162
1114.734619 1.131411
1114.734619 1.131651
1114.734619 1.132016
1114.734619 1.132495
1123.926147 1.084708
1123.926147 1.085049
1123.926147 1.085168
1123.926147 1.085385
1123.926147 1.085510
1123.926147 1.086429
1123.926147 1.087469
1123.926147 1.087994
1133.110474 1.094634
1133.110474 1.094906
1133.110474 1.095289
1133.110474 1.095073
1133.110474 1.096018
1133.110474 1.096602
1133.110474 1.097402
1133.110474 1.098200
1133.110474 1.098959
1133.110474 1.099907
1133.110474 1.100685
1133.110474 1.101727
1133.110474 1.102554
1133.110474 1.103309
1133.110474 1.104041
1142.330322 1.106356
1142.330322 1.107881
1142.330322 1.108468
1142.330322 1.109680
1142.330322 1.110884
1142.330322 1.112018
1142.330322 1.112847
1142.330322 1.113934
1142.330322 1.114595
1142.330322 1.115586
1142.330322 1.116499
1142.330322 1.117563
1142.330322 1.118009
1142.330322 1.118103
1142.330322 1.118421
1142.330322 1.119145
1142.330322 1.120057
1142.330322 1.121163
1142.330322 1.122293
1142.330322 1.122943
1142.330322 1.123387
1142.330322 1.124206
1142.330322 1.125142
1142.330322 1.126009
1142.330322 1.126660
1142.330322 1.127447
1142.330322 1.128302
1142.330322 1.129300
1142.330322 1.130494
1142.330322 1.131873
1142.330322 1.132816
1142.330322 1.133084
1142.330322 1.133360
1142.330322 1.133262
1142.330322 1.132978
1142.330322 1.133629
1142.330322 1.134147
1142.330322 1.135040
1142.330322 1.135814
1142.330322 1.136575
1142.330322 1.137123
1142.330322 1.137360
1142.330322 1.137460
1142.330322 1.138077
1151.762207 1.124934
1151.762207 1.125279
1151.762207 1.125774
1151.762207 1.125679
1151.762207 1.125179
1151.762207 1.124896
1151.762207 1.125210
1151.762207 1.125940
1151.762207 1.127324
1151.762207 1.129331
1151.762207 1.131398
1151.762207 1.132875
1151.762207 1.134190
1151.762207 1.136171
1151.762207 1.137634
1151.762207 1.139078
1151.762207 1.139883
1151.762207 1.140805
1151.762207 1.141210
1151.762207 1.141473
1151.762207 1.141845
1151.762207 1.142017
1151.762207 1.142013
1151.762207 1.141630
1151.762207 1.141421
1151.762207 1.141211
1151.762207 1.140578
1151.762207 1.140217
1151.762207 1.139852
1151.762207 1.139531
1151.762207 1.139763
1151.762207 1.139901
1151.762207 1.139899
1151.762207 1.139930
1151.762207 1.141013
1151.762207 1.142042
1151.762207 1.142742
1151.762207 1.143508
1151.762207 1.144516
1151.762207 1.145740
1151.762207 1.146821
1151.762207 1.147715
1151.762207 1.149136
1151.762207 1.150323
1151.762207 1.151683
1151.762207 1.152531
1151.762207 1.153579
1151.762207 1.154001
1151.762207 1.154371
1151.762207 1.154451
1151.762207 1.154970
1151.762207 1.155472
1151.762207 1.156103
1151.762207 1.157018
1151.762207 1.158006
1151.762207 1.158437
1151.762207 1.158775
1151.762207 1.160043
1151.762207 1.160871
1151.762207 1.161656
1151.762207 1.162704
1151.762207 1.163806
1151.762207 1.164915
1151.762207 1.166079
1151.762207 1.166744
1161.531860 1.157595
1161.531860 1.158060
1161.531860 1.158584
1161.531860 1.159713
1161.531860 1.161118
1161.531860 1.162637
1161.531860 1.163662
1161.531860 1.164268
1161.531860 1.164803
1161.531860 1.164785
1161.531860 1.165078
1161.531860 1.165241
1161.531860 1.165287
1161.531860 1.165242
1161.531860 1.165260
1161.531860 1.165622
1161.531860 1.165692
1161.531860 1.165859
1161.531860 1.166645
1161.531860 1.168140
1161.531860 1.170057
1161.531860 1.171166
1161.531860 1.172413
1161.531860 1.173595
1161.531860 1.174577
1161.531860 1.175815
1161.531860 1.176535
1161.531860 1.177025
1161.531860 1.177765
1161.531860 1.178948
1161.531860 1.179694
1161.531860 1.180419
1161.531860 1.181338
1161.531860 1.182728
1161.531860 1.183892
1161.531860 1.185034
1161.531860 1.186717
1161.531860 1.188357
1161.531860 1.189831
1161.531860 1.190570
1161.531860 1.191502
1161.531860 1.192275
1161.531860 1.193051
1161.531860 1.193723
1161.531860 1.194787
1161.531860 1.195960
1161.531860 1.197170
1161.531860 1.197819
1161.531860 1.198952
1161.531860 1.200570
1161.531860 1.201925
1161.531860 1.203540
1161.531860 1.204625
1161.531860 1.205908
1161.531860 1.206712
1161.531860 1.207407
1161.531860 1.207991
1161.531860 1.208501
1161.531860 1.208854
1161.531860 1.209328
1161.531860 1.209994
1161.531860 1.210361
1161.531860 1.210904
1171.624268 1.191765
1171.624268 1.192294
1171.624268 1.193629
1171.624268 1.194293
1171.624268 1.194606
1171.624268 1.195353
1171.624268 1.196000
1171.624268 1.196867
1171.624268 1.197806
1171.624268 1.198933
1171.624268 1.199549
1171.624268 1.200030
1171.624268 1.201671
1171.624268 1.202962
1171.624268 1.204288
1171.624268 1.205269
1171.624268 1.205981
1171.624268 1.206875
1171.624268 1.207636
1171.624268 1.208744
1171.624268 1.209238
1171.624268 1.209660
1171.624268 1.210135
1171.624268 1.210411
1171.624268 1.210843
1171.624268 1.211049
1171.624268 1.211171
1171.624268 1.210745
1171.624268 1.210917
1171.624268 1.210883
1171.624268 1.210856
1171.624268 1.210701
1171.624268 1.211273
1171.624268 1.211838
1171.624268 1.212460
1171.624268 1.212952
1171.624268 1.213872
1171.624268 1.214588
1171.624268 1.214835
1171.624268 1.215348
1171.624268 1.215654
1171.624268 1.215839
1171.624268 1.216185
1171.624268 1.216226
1171.624268 1.216297
1171.624268 1.216984
1171.624268 1.217836
1171.624268 1.218569
1171.624268 1.218938
1171.624268 1.219816
1171.624268 1.220133
1171.624268 1.220516
1171.624268 1.220979
1171.624268 1.220989
1171.624268 1.221463
1171.624268 1.220828
1171.624268 1.220946
1171.624268 1.222004
1171.624268 1.223074
1171.624268 1.224829
1171.624268 1.226157
1171.624268 1.227210
1171.624268 1.228318
1171.624268 1.229690
1171.624268 1.230854
1171.624268 1.232176
1171.624268 1.233020
1171.624268 1.233844
1171.624268 1.234836
1171.624268 1.236138
1171.624268 1.236668
1171.624268 1.237300
1171.624268 1.238021
1182.096680 1.229989
1182.096680 1.231515
1182.096680 1.232934
1182.096680 1.233947
1182.096680 1.235001
1182.096680 1.235965
1182.096680 1.236707
1182.096680 1.236880
1182.096680 1.236718
1182.096680 1.236899
1182.096680 1.237086
1182.096680 1.237743
1182.096680 1.238280
1182.096680 1.238086
1182.096680 1.237799
1182.096680 1.237916
1182.096680 1.238307
1182.096680 1.238376
1182.096680 1.238430
1182.096680 1.238488
1182.096680 1.238171
1182.096680 1.238328
1182.096680 1.238440
1182.096680 1.238209
1182.096680 1.237985
1182.096680 1.237722
1182.096680 1.237342
1182.096680 1.236962
1182.096680 1.236402
1182.096680 1.237045
1182.096680 1.237537
1182.096680 1.237121
1182.096680 1.236430
1182.096680 1.236740
1182.096680 1.236802
1182.096680 1.236886
1182.096680 1.237645
1182.096680 1.238007
1182.096680 1.238482
1182.096680 1.239221
1182.096680 1.240361
1182.096680 1.241254
1182.096680 1.242354
1182.096680 1.242966
1182.096680 1.243778
1182.096680 1.244552
1182.096680 1.245504
1182.096680 1.246596
1182.096680 1.248215
1182.096680 1.249128
1182.096680 1.250597
1182.096680 1.251151
1182.096680 1.251330
1182.096680 1.251270
1182.096680 1.251741
1182.096680 1.252271
1182.096680 1.252544
1182.096680 1.252852
1182.096680 1.253412
1182.096680 1.254354
1182.096680 1.255415
1182.096680 1.256580
1182.096680 1.258287
1182.096680 1.259603
1182.096680 1.260231
1182.096680 1.260820
1182.096680 1.261340
1182.096680 1.262170
1182.096680 1.262908
1182.096680 1.263749
1182.096680 1.264284
1182.096680 1.264664
1182.096680 1.265654
1182.096680 1.265692
1182.096680 1.265469
1182.096680 1.265889
1182.096680 1.265970
1182.096680 1.266010
1182.096680 1.266121
1182.096680 1.266549
1182.096680 1.266988
1182.096680 1.267225
1182.096680 1.267062
1182.096680 1.266926
1193.012085 1.241627
1193.012085 1.241266
1193.012085 1.241560
1193.012085 1.242047
1193.012085 1.242242
1193.012085 1.242807
1193.012085 1.243273
1193.012085 1.243676
1193.012085 1.244026
1193.012085 1.244587
1193.012085 1.245663
1193.012085 1.246801
1193.012085 1.247274
1193.012085 1.248436
1193.012085 1.249362
1193.012085 1.250387
1193.012085 1.251545
1193.012085 1.252634
1193.012085 1.253803
1193.012085 1.255651
1193.012085 1.257282
1193.012085 1.258813
1193.012085 1.259829
1193.012085 1.261087
1193.012085 1.262237
1193.012085 1.263382
1193.012085 1.264553
1193.012085 1.265582
1193.012085 1.266790
1193.012085 1.267856
1193.012085 1.268669
1193.012085 1.269406
1193.012085 1.270044
1193.012085 1.270289
1193.012085 1.270437
1193.012085 1.271158
1193.012085 1.271375
1193.012085 1.272379
1193.012085 1.272250
1193.012085 1.272511
1193.012085 1.272468
1193.012085 1.272808
1193.012085 1.272686
1193.012085 1.272984
1193.012085 1.273081
1193.012085 1.272949
1193.012085 1.273484
1193.012085 1.272942
1193.012085 1.273557
1193.012085 1.273853
1193.012085 1.273952
1193.012085 1.274770
1193.012085 1.275573
1193.012085 1.276329
1193.012085 1.276989
1193.012085 1.277756
1193.012085 1.277955
1193.012085 1.278055
1193.012085 1.278309
1193.012085 1.278747
1193.012085 1.279264
1193.012085 1.279096
1193.012085 1.279249
1193.012085 1.279854
1193.012085 1.279634
1193.012085 1.279973
1193.012085 1.280767
1193.012085 1.281214
1193.012085 1.281508
1193.012085 1.281315
1193.012085 1.280954
1193.012085 1.280892
1193.012085 1.281309
1193.012085 1.282096
1193.012085 1.282488
1193.012085 1.282640
1193.012085 1.282807
1204.324341 1.268044
1204.324341 1.268623
1204.324341 1.269293
1204.324341 1.269751
1204.324341 1.271162
1204.324341 1.273197
1204.324341 1.275144
1204.324341 1.276421
1204.324341 1.277529
1204.324341 1.278162
1204.324341 1.279177
1215.634766 1.282456
1215.634766 1.282449
1215.634766 1.283005
1215.634766 1.283042
1215.634766 1.283873
1215.634766 1.284608
1215.634766 1.285637
1215.634766 1.287198
1215.634766 1.288651
1215.634766 1.289782
1215.634766 1.290768
1215.634766 1.290958
1215.634766 1.291261
1215.634766 1.291438
1215.634766 1.292029
1215.634766 1.292789
1215.634766 1.293416
1215.634766 1.294797
1215.634766 1.296378
1215.634766 1.297540
1215.634766 1.298988
1227.002930 1.306426
1227.002930 1.307218
1227.002930 1.308037
1227.002930 1.309141
1227.002930 1.309854
1227.002930 1.310527
1227.002930 1.311678
1227.002930 1.312217
1238.351196 1.264864
1238.351196 1.265951
1238.351196 1.266751
1238.351196 1.267418
1238.351196 1.267841
1238.351196 1.268653
1238.351196 1.269049
1238.351196 1.269359
1238.351196 1.270255
1238.351196 1.271889
1238.351196 1.273311
1238.351196 1.274380
1238.351196 1.275919
1238.351196 1.277804
1238.351196 1.280190
1238.351196 1.281913
1238.351196 1.283500
1238.351196 1.284858
1238.351196 1.285943
1238.351196 1.286147
1238.351196 1.286370
1238.351196 1.286724
1238.351196 1.287032
1238.351196 1.286627
1238.351196 1.287058
1238.351196 1.287415
1238.351196 1.288242
1238.351196 1.289078
1238.351196 1.289984
1238.351196 1.290642
1238.351196 1.291153
1238.351196 1.291613
1238.351196 1.291915
1238.351196 1.292064
1238.351196 1.292729
1238.351196 1.293451
1238.351196 1.294009
1238.351196 1.294656
1238.351196 1.295114
1238.351196 1.296860
1238.351196 1.297954
1238.351196 1.299131
1238.351196 1.301117
1238.351196 1.302833
1238.351196 1.304221
1249.899170 1.264511
1249.899170 1.264873
1249.899170 1.265496
1249.899170 1.265690
1249.899170 1.266133
1249.899170 1.266684
1249.899170 1.267820
1249.899170 1.269609
1249.899170 1.270897
1249.899170 1.272495
1249.899170 1.273833
1249.899170 1.275169
1249.899170 1.276200
1249.899170 1.276524
1249.899170 1.278053
1249.899170 1.279715
1249.899170 1.280494
1249.899170 1.280488
1249.899170 1.280462
1249.899170 1.280756
1249.899170 1.280231
1249.899170 1.280360
1249.899170 1.280252
1249.899170 1.280842
1261.520752 1.286296
1261.520752 1.287062
1261.520752 1.287649
1261.520752 1.288446
1261.520752 1.289394
1261.520752 1.290225
1261.520752 1.291549
1261.520752 1.291839
1261.520752 1.292492
1261.520752 1.292717
1261.520752 1.293473
1261.520752 1.294874
1261.520752 1.295745
1261.520752 1.296531
1261.520752 1.297367
1261.520752 1.298204
1261.520752 1.298563
1261.520752 1.299636
1261.520752 1.300039
1261.520752 1.301040
1261.520752 1.300595
1261.520752 1.300605
1261.520752 1.301087
1261.520752 1.301514
1261.520752 1.301963
1261.520752 1.301900
1261.520752 1.301727
1261.520752 1.301904
1261.520752 1.302674
1261.520752 1.302871
1261.520752 1.303254
1261.520752 1.303660
1261.520752 1.304157
1273.268433 1.281165
1273.268433 1.281317
1273.268433 1.281225
1273.268433 1.280466
1273.268433 1.279824
1273.268433 1.279549
1273.268433 1.279461
1273.268433 1.280040
1273.268433 1.280600
1273.268433 1.281265
1273.268433 1.281761
1273.268433 1.282494
1273.268433 1.283553
1273.268433 1.284818
1273.268433 1.285647
1273.268433 1.286268
1273.268433 1.288056
1273.268433 1.288699
1273.268433 1.290020
1273.268433 1.291532
1273.268433 1.293015
1273.268433 1.293907
1273.268433 1.294538
1273.268433 1.295213
1273.268433 1.296290
1273.268433 1.296798
1273.268433 1.297405
1273.268433 1.297945
1273.268433 1.298503
1273.268433 1.298678
1285.123535 1.304760
1285.123535 1.305848
1285.123535 1.307091
1285.123535 1.308419
1285.123535 1.310709
1285.123535 1.312773
1285.123535 1.314228
1285.123535 1.315758
1285.123535 1.317323
1285.123535 1.318559
1296.967773 1.289823
1296.967773 1.290889
1296.967773 1.292266
1296.967773 1.293149
1296.967773 1.294362
1296.967773 1.294567
1296.967773 1.295654
1296.967773 1.297086
1296.967773 1.298671
1296.967773 1.299289
1308.801147 1.274288
1308.801147 1.274884
1308.801147 1.275782
1308.801147 1.276607
1308.801147 1.277017
1308.801147 1.277022
1308.801147 1.276788
1308.801147 1.276555
1308.801147 1.276664
1308.801147 1.277008
1308.801147 1.277254
1308.801147 1.277628
1308.801147 1.278841
1308.801147 1.279806
1308.801147 1.280799
1308.801147 1.281530
1308.801147 1.281928
1308.801147 1.282139
1308.801147 1.282312
1308.801147 1.282681
1308.801147 1.281911
1308.801147 1.282844
1308.801147 1.283549
1308.801147 1.284590
1308.801147 1.285262
1308.801147 1.286237
1308.801147 1.287465
1308.801147 1.288599
1308.801147 1.289832
1308.801147 1.291425
1308.801147 1.292518
1308.801147 1.294029
1308.801147 1.295344
1308.801147 1.296384
1308.801147 1.298235
1308.801147 1.298951
1308.801147 1.300036
1308.801147 1.300662
1308.801147 1.301300
1308.801147 1.301670
1308.801147 1.301916
1308.801147 1.302335
1308.801147 1.302369
1308.801147 1.302485
1308.801147 1.302381
1308.801147 1.302803
1308.801147 1.303643
1308.801147 1.303838
1308.801147 1.304543
1308.801147 1.305313
1308.801147 1.306086
1308.801147 1.307204
1308.801147 1.307346
1308.801147 1.308062
1308.801147 1.308606
1308.801147 1.309594
1308.801147 1.310042
1308.801147 1.310724
1308.801147 1.311587
1308.801147 1.312701
1308.801147 1.313465
1308.801147 1.314319
1308.801147 1.315793
1308.801147 1.316676
1308.801147 1.317572
1308.801147 1.318494
1308.801147 1.318769
1308.801147 1.319104
1308.801147 1.319748
1308.801147 1.320708
1308.801147 1.322275
1308.801147 1.323974
1308.801147 1.325217
1308.801147 1.326107
1308.801147 1.328044
1308.801147 1.329228
1308.801147 1.330738
1308.801147 1.332415
1308.801147 1.333319
1308.801147 1.334302
1308.801147 1.335217
1308.801147 1.335216
1308.801147 1.335147
1308.801147 1.335476
1308.801147 1.335563
1308.801147 1.335327
1308.801147 1.335661
1308.801147 1.336088
1308.801147 1.336546
1308.801147 1.337152
1308.801147 1.337295
1308.801147 1.337737
1308.801147 1.338688
1308.801147 1.339545
1308.801147 1.340573
1308.801147 1.340299
1308.801147 1.340877
1308.801147 1.341878
1308.801147 1.342923
1308.801147 1.344263
1308.801147 1.344847
1308.801147 1.345101
1308.801147 1.344960
1308.801147 1.345093
1308.801147 1.345820
1308.801147 1.345850
1308.801147 1.346512
1308.801147 1.347297
1308.801147 1.347981
1308.801147 1.348429
1308.801147 1.350268
1308.801147 1.351376
1308.801147 1.352605
1308.801147 1.353675
1308.801147 1.355837
1308.801147 1.357442
1308.801147 1.358810
1308.801147 1.360112
1308.801147 1.361393
1308.801147 1.362272
1308.801147 1.363442
1308.801147 1.364269
1308.801147 1.364446
1308.801147 1.365243
1308.801147 1.365787
1308.801147 1.366425
1321.300293 1.354493
1333.732544 1.352157
1346.098511 1.348798
1346.098511 1.348667
1346.098511 1.349019
1346.098511 1.349224
1346.098511 1.348964
1346.098511 1.348891
1346.098511 1.348360
1346.098511 1.348415
1346.098511 1.348072
1346.098511 1.347878
1346.098511 1.348018
1346.098511 1.348208
1346.098511 1.348023
1346.098511 1.348333
1346.098511 1.348310
1346.098511 1.348503
1346.098511 1.349154
1346.098511 1.350530
1358.497070 1.324052
1358.497070 1.324541
1358.497070 1.325011
1358.497070 1.325292
1358.497070 1.325744
1358.497070 1.326199
1358.497070 1.326968
1358.497070 1.328163
1358.497070 1.328182
1358.497070 1.328106
1358.497070 1.328335
1358.497070 1.329042
1358.497070 1.329626
1358.497070 1.330398
1358.497070 1.330439
1358.497070 1.329973
1358.497070 1.329836
1358.497070 1.329637
1358.497070 1.329568
1358.497070 1.329583
1358.497070 1.330469
1358.497070 1.331181
1358.497070 1.332316
1358.497070 1.333422
1358.497070 1.334097
1358.497070 1.335502
1358.497070 1.336660
1358.497070 1.337039
1358.497070 1.338214
1358.497070 1.338232
1358.497070 1.338147
1358.497070 1.338143
1358.497070 1.339096
1358.497070 1.339929
1358.497070 1.341104
1358.497070 1.341824
1358.497070 1.342207
1358.497070 1.342908
1358.497070 1.343249
1358.497070 1.343760
1358.497070 1.343907
1358.497070 1.344501
1358.497070 1.344987
1358.497070 1.345382
1358.497070 1.345930
1358.497070 1.345933
1358.497070 1.345658
1358.497070 1.344981
1358.497070 1.344939
1358.497070 1.345222
1358.497070 1.346078
1358.497070 1.346117
1358.497070 1.345731
1358.497070 1.345144
1358.497070 1.344410
1358.497070 1.344412
1358.497070 1.343821
1358.497070 1.343989
1358.497070 1.343390
1358.497070 1.343349
1358.497070 1.343458
1358.497070 1.343586
1358.497070 1.344344
1358.497070 1.344565
1358.497070 1.345005
1358.497070 1.345571
1358.497070 1.345897
1358.497070 1.346367
1358.497070 1.346604
1358.497070 1.346846
1358.497070 1.347056
1358.497070 1.347812
1358.497070 1.348201
1358.497070 1.348413
1358.497070 1.349377
1358.497070 1.350877
1358.497070 1.351992
1358.497070 1.352581
1358.497070 1.353262
1358.497070 1.353706
1358.497070 1.355063
1358.497070 1.356106
1358.497070 1.356891
1358.497070 1.358287
1358.497070 1.359304
1358.497070 1.360084
1358.497070 1.360781
1358.497070 1.361469
1358.497070 1.362465
1358.497070 1.363827
1358.497070 1.364999
1358.497070 1.366440
1358.497070 1.366936
1358.497070 1.367087
1358.497070 1.366961
1358.497070 1.367438
1358.497070 1.367718
1358.497070 1.367638
1358.497070 1.367898
1358.497070 1.368249
1358.497070 1.368220
1358.497070 1.368039
1358.497070 1.368418
1358.497070 1.367892
1358.497070 1.367570
1358.497070 1.367002
1358.497070 1.366561
1358.497070 1.366296
1358.497070 1.366055
1358.497070 1.365646
1358.497070 1.365288
1358.497070 1.365268
1358.497070 1.365568
1358.497070 1.365543
1358.497070 1.365180
1358.497070 1.364564
1358.497070 1.364549
1358.497070 1.364968
1358.497070 1.365893
1358.497070 1.366787
1358.497070 1.367831
1358.497070 1.368561
1358.497070 1.369015
1358.497070 1.369667
1358.497070 1.370873
1358.497070 1.371320
1358.497070 1.372071
1358.497070 1.372425
1358.497070 1.372868
1358.497070 1.373593
1358.497070 1.374261
1358.497070 1.374474
1358.497070 1.374407
1358.497070 1.374050
1358.497070 1.373769
1358.497070 1.374198
1358.497070 1.374871
1358.497070 1.375219
1358.497070 1.375559
1358.497070 1.376340
1358.497070 1.377314
1358.497070 1.377976
1358.497070 1.378458
1358.497070 1.379089
1358.497070 1.380449
1358.497070 1.381671
1358.497070 1.382401
1358.497070 1.382743
1358.497070 1.383761
1358.497070 1.386025
1358.497070 1.387650
1358.497070 1.388689
1358.497070 1.390251
1358.497070 1.391617
1358.497070 1.393616
1358.497070 1.395690
1358.497070 1.397247
1358.497070 1.399908
1358.497070 1.401789
1358.497070 1.403226
1358.497070 1.404017
1358.497070 1.405174
1358.497070 1.405234
1358.497070 1.405454
1358.497070 1.405686
1358.497070 1.405964
1358.497070 1.405858
1358.497070 1.406334
1358.497070 1.406563
1358.497070 1.406607
1358.497070 1.405718
1358.497070 1.405729
1358.497070 1.406943
1358.497070 1.407868
1358.497070 1.409140
1358.497070 1.410821
1358.497070 1.413156
1358.497070 1.415051
1358.497070 1.416052
1358.497070 1.417294
1358.497070 1.417422
1358.497070 1.418083
1358.497070 1.419468
1358.497070 1.420553
1358.497070 1.421877
1358.497070 1.423496
1358.497070 1.424252
1358.497070 1.424029
1358.497070 1.424186
1358.497070 1.425498
1358.497070 1.426644
1358.497070 1.427086
1358.497070 1.427758
1358.497070 1.428347
1358.497070 1.428894
1358.497070 1.430416
1358.497070 1.431764
1358.497070 1.432370
1358.497070 1.433964
1358.497070 1.435141
1358.497070 1.437203
1358.497070 1.438851
1358.497070 1.440364
1358.497070 1.441682
1358.497070 1.443217
1358.497070 1.444540
1358.497070 1.446001
1358.497070 1.446752
1358.497070 1.446924
1358.497070 1.447587
1358.497070 1.448075
1358.497070 1.448257
1358.497070 1.448627
1358.497070 1.448809
1358.497070 1.449232
1358.497070 1.449524
1358.497070 1.449586
1358.497070 1.449743
1358.497070 1.449190
1358.497070 1.449824
1358.497070 1.449817
1358.497070 1.449333
1358.497070 1.450358
1358.497070 1.451106
1358.497070 1.450637
1358.497070 1.450372
1358.497070 1.451094
1358.497070 1.451590
1358.497070 1.452463
1358.497070 1.454121
1358.497070 1.455243
1358.497070 1.455975
1358.497070 1.456696
1358.497070 1.457138
1358.497070 1.457385
1358.497070 1.457415
1358.497070 1.457636
1358.497070 1.457712
1358.497070 1.457460
1358.497070 1.456754
1358.497070 1.455701
1358.497070 1.454999
1358.497070 1.454409
1358.497070 1.453400
1358.497070 1.453940
1358.497070 1.453991
1358.497070 1.454314
1358.497070 1.454883
1358.497070 1.455216
1358.497070 1.455646
1358.497070 1.455254
1358.497070 1.454342
1358.497070 1.453844
1358.497070 1.453140
1358.497070 1.452342
1358.497070 1.451790
1358.497070 1.451461
1358.497070 1.450876
1358.497070 1.451066
1358.497070 1.451963
1358.497070 1.452775
1358.497070 1.453691
1358.497070 1.454746
1358.497070 1.455572
1358.497070 1.455691
1358.497070 1.456095
1358.497070 1.456318
1358.497070 1.457172
1358.497070 1.457262
1358.497070 1.457346
1358.497070 1.458198
1358.497070 1.459267
1358.497070 1.459596
1358.497070 1.460188
1358.497070 1.461683
1358.497070 1.463358
1358.497070 1.464686
1358.497070 1.465620
1358.497070 1.466408
1358.497070 1.466879
1358.497070 1.467916
1358.497070 1.468975
1358.497070 1.470102
1358.497070 1.470696
1358.497070 1.471152
1358.497070 1.471026
1358.497070 1.471696
1358.497070 1.472485
1358.497070 1.473394
1358.497070 1.474041
1358.497070 1.475060
1358.497070 1.475923
1358.497070 1.476938
1358.497070 1.477743
1358.497070 1.477788
1358.497070 1.477937
1358.497070 1.478798
1358.497070 1.479092
1358.497070 1.480011
1358.497070 1.480304
1358.497070 1.480145
1358.497070 1.480663
1358.497070 1.481326
1358.497070 1.483105
1358.497070 1.485817
1358.497070 1.488388
1358.497070 1.490911
1358.497070 1.493335
1358.497070 1.495343
1358.497070 1.496145
1358.497070 1.497380
1358.497070 1.498709
1358.497070 1.500081
1358.497070 1.501033
1358.497070 1.502045
1358.497070 1.502787
1358.497070 1.503525
1358.497070 1.504079
1358.497070 1.504137
1358.497070 1.504209
1358.497070 1.504943
1358.497070 1.506043
1358.497070 1.507192
1358.497070 1.508136
1358.497070 1.508790
1358.497070 1.509448
1358.497070 1.509241
1358.497070 1.509428
1358.497070 1.509657
1358.497070 1.509477
1358.497070 1.508588
1358.497070 1.507977
1358.497070 1.507316
1358.497070 1.506603
1358.497070 1.506700
1358.497070 1.506312
1358.497070 1.506802
1358.497070 1.507145
1358.497070 1.507450
1358.497070 1.507831
1358.497070 1.508357
1358.497070 1.508316
1358.497070 1.508089
1358.497070 1.507994
1358.497070 1.508236
1358.497070 1.508533
1358.497070 1.509672
1358.497070 1.510767
1358.497070 1.511910
1358.497070 1.513120
1358.497070 1.514156
1358.497070 1.515338
1358.497070 1.516919
1358.497070 1.517722
1358.497070 1.517964
1358.497070 1.518458
1358.497070 1.518960
1358.497070 1.519436
1358.497070 1.519983
1358.497070 1.520697
1358.497070 1.521289
1358.497070 1.521476
1358.497070 1.521390
1358.497070 1.521282
1358.497070 1.521375
1358.497070 1.520998
1358.497070 1.521157
1358.497070 1.520340
1358.497070 1.519822
1358.497070 1.519833
1358.497070 1.519797
1358.497070 1.519806
1358.497070 1.519831
1358.497070 1.520348
1358.497070 1.521088
1358.497070 1.522066
1358.497070 1.523095
1358.497070 1.524088
1358.497070 1.524796
1358.497070 1.525779
1358.497070 1.525929
1358.497070 1.527079
1358.497070 1.528108
1358.497070 1.529094
1358.497070 1.530741
1358.497070 1.531945
1358.497070 1.533554
1358.497070 1.535358
1358.497070 1.536966
1358.497070 1.538620
1358.497070 1.541182
1358.497070 1.543006
1358.497070 1.543782
1358.497070 1.544259
1358.497070 1.545245
1358.497070 1.546931
1358.497070 1.548525
1358.497070 1.549522
1358.497070 1.551387
1358.497070 1.553103
1358.497070 1.554472
1358.497070 1.555102
1358.497070 1.556257
1358.497070 1.557315
1358.497070 1.557325
1358.497070 1.558755
1358.497070 1.559863
1358.497070 1.560954
1358.497070 1.561213
1358.497070 1.561692
1358.497070 1.562626
1358.497070 1.563549
1358.497070 1.564221
1358.497070 1.564438
1358.497070 1.564687
1358.497070 1.564724
1358.497070 1.565168
1358.497070 1.564919
1358.497070 1.565300
1358.497070 1.565960
1358.497070 1.566096
1358.497070 1.566071
1358.497070 1.566999
1358.497070 1.567873
1358.497070 1.569297
1358.497070 1.570122
1358.497070 1.570904
1358.497070 1.570935
1358.497070 1.571464
1358.497070 1.571948
1358.497070 1.572138
1358.497070 1.572627
1358.497070 1.572863
1358.497070 1.572626
1358.497070 1.571869
1358.497070 1.571416
1358.497070 1.571493
1358.497070 1.571299
1358.497070 1.572072
1358.497070 1.572070
1358.497070 1.572577
1373.365967 1.569928
1373.365967 1.569987
1373.365967 1.570428
1373.365967 1.570748
1373.365967 1.570658
1373.365967 1.570312
1373.365967 1.570779
1373.365967 1.571633
1373.365967 1.573297
1373.365967 1.574923
1373.365967 1.575927
1373.365967 1.576744
1373.365967 1.577846
1373.365967 1.578636
1373.365967 1.579787
1373.365967 1.580638
1373.365967 1.580808
1373.365967 1.580826
1373.365967 1.581075
1373.365967 1.580341
1373.365967 1.579231
1373.365967 1.579089
1373.365967 1.578059
1373.365967 1.577372
1373.365967 1.577049
1373.365967 1.577442
1373.365967 1.577936
1373.365967 1.578718
1373.365967 1.579518
1373.365967 1.580436
1373.365967 1.580947
1373.365967 1.580825
1373.365967 1.581672
1373.365967 1.583419
1373.365967 1.584019
1373.365967 1.584432
1373.365967 1.585221
1373.365967 1.586715
1373.365967 1.588028
1373.365967 1.589229
1373.365967 1.590863
1373.365967 1.592638
1373.365967 1.594352
1373.365967 1.596497
1373.365967 1.598497
1373.365967 1.600876
1373.365967 1.602819
1373.365967 1.604542
1373.365967 1.606612
1373.365967 1.608791
1373.365967 1.611052
1373.365967 1.612579
1373.365967 1.613836
1373.365967 1.614542
1373.365967 1.614609
1373.365967 1.614986
1373.365967 1.614449
1373.365967 1.614457
1373.365967 1.614061
1373.365967 1.614058
1373.365967 1.613639
1373.365967 1.614204
1373.365967 1.614398
1373.365967 1.614179
1373.365967 1.614351
1373.365967 1.614933
1373.365967 1.615223
1373.365967 1.615030
1373.365967 1.614619
1373.365967 1.614548
1373.365967 1.614837
1373.365967 1.615212
1373.365967 1.615713
1373.365967 1.616649
1373.365967 1.617054
1388.580444 1.555048
1388.580444 1.554493
1388.580444 1.553988
1388.580444 1.553302
1388.580444 1.553375
1388.580444 1.553303
1388.580444 1.553154
1388.580444 1.553158
1388.580444 1.553660
1388.580444 1.554347
1388.580444 1.555373
1388.580444 1.555216
1388.580444 1.555184
1388.580444 1.555298
1388.580444 1.555389
1388.580444 1.556075
1388.580444 1.557071
1388.580444 1.556401
1388.580444 1.556245
1388.580444 1.556061
1388.580444 1.555903
1388.580444 1.556117
1388.580444 1.557170
1388.580444 1.557042
1388.580444 1.556808
1388.580444 1.556745
1388.580444 1.557249
1388.580444 1.558097
1388.580444 1.559056
1388.580444 1.559949
1388.580444 1.560189
1388.580444 1.560174
1388.580444 1.559781
1388.580444 1.559549
1388.580444 1.559369
1388.580444 1.559635
1388.580444 1.560432
1388.580444 1.561891
1388.580444 1.563391
1388.580444 1.564223
1388.580444 1.565018
1388.580444 1.566244
1388.580444 1.568042
1388.580444 1.570017
1388.580444 1.572142
1388.580444 1.573985
1388.580444 1.575856
1388.580444 1.577014
1388.580444 1.578925
1388.580444 1.579978
1388.580444 1.582058
1388.580444 1.583496
1388.580444 1.584685
1388.580444 1.586569
1388.580444 1.587949
1404.022949 1.589166
1404.022949 1.590062
1404.022949 1.590663
1404.022949 1.591350
1404.022949 1.591634
1404.022949 1.592085
1404.022949 1.593104
1404.022949 1.594551
1404.022949 1.595803
1404.022949 1.597837
1404.022949 1.599658
1404.022949 1.601054
1404.022949 1.602205
1404.022949 1.603030
1404.022949 1.603913
1404.022949 1.604489
1404.022949 1.603627
1404.022949 1.602969
1404.022949 1.602195
1404.022949 1.602413
1404.022949 1.602279
1404.022949 1.603166
1404.022949 1.604125
1404.022949 1.604786
1404.022949 1.606118
1404.022949 1.607195
1404.022949 1.607577
1404.022949 1.608187
1404.022949 1.609262
1404.022949 1.610511
1404.022949 1.611763
1404.022949 1.612560
1404.022949 1.613538
1404.022949 1.615024
1404.022949 1.616247
1404.022949 1.617322
1404.022949 1.618238
1404.022949 1.619428
1404.022949 1.619607
1404.022949 1.619472
1404.022949 1.618516
1404.022949 1.618143
1404.022949 1.617975
1404.022949 1.618096
1404.022949 1.618125
1404.022949 1.618636
1404.022949 1.619237
1404.022949 1.619495
1404.022949 1.619486
1404.022949 1.619132
1404.022949 1.619115
1404.022949 1.619711
1419.674316 1.573696
1419.674316 1.573496
1419.674316 1.573254
1419.674316 1.572583
1419.674316 1.573824
1419.674316 1.574163
1419.674316 1.574472
1419.674316 1.575602
1419.674316 1.576337
1419.674316 1.577189
1419.674316 1.578518
1419.674316 1.579698
1419.674316 1.581081
1419.674316 1.581692
1419.674316 1.582360
1419.674316 1.582714
1419.674316 1.583017
1419.674316 1.583119
1419.674316 1.583050
1419.674316 1.583053
1419.674316 1.583134
1419.674316 1.583316
1419.674316 1.583319
1419.674316 1.583394
1419.674316 1.583431
1419.674316 1.584336
1419.674316 1.585410
1435.390259 1.576620
1435.390259 1.576699
1435.390259 1.575983
1435.390259 1.575743
1435.390259 1.576704
1435.390259 1.577460
1435.390259 1.577822
1435.390259 1.578131
1435.390259 1.578080
1435.390259 1.579132
1435.390259 1.580016
1451.079590 1.552952
1451.079590 1.552849
1451.079590 1.553244
1451.079590 1.554016
1451.079590 1.554411
1451.079590 1.554464
1451.079590 1.553921
1451.079590 1.553594
1451.079590 1.552850
1451.079590 1.552919
1451.079590 1.553847
1451.079590 1.554484
1451.079590 1.555412
1451.079590 1.556548
1451.079590 1.557694
1451.079590 1.557525
1451.079590 1.557552
1451.079590 1.557378
1451.079590 1.558536
1451.079590 1.559709
1451.079590 1.560889
1451.079590 1.561896
1451.079590 1.562766
1451.079590 1.562834
1451.079590 1.563085
1451.079590 1.563273
1451.079590 1.563980
1451.079590 1.565020
1451.079590 1.565903
1451.079590 1.566561
1451.079590 1.567224
1451.079590 1.567824
1451.079590 1.568325
1451.079590 1.568214
1451.079590 1.568618
1451.079590 1.569069
1451.079590 1.569497
1451.079590 1.570614
1451.079590 1.570891
1451.079590 1.571272
1451.079590 1.572185
1451.079590 1.573103
1466.917847 1.512488
1466.917847 1.513645
1466.917847 1.514636
1466.917847 1.515629
1466.917847 1.515718
1466.917847 1.515843
1466.917847 1.515218
1466.917847 1.515384
1466.917847 1.514616
1466.917847 1.513949
1466.917847 1.513183
1466.917847 1.512232
1466.917847 1.512111
1466.917847 1.512367
1466.917847 1.512593
1466.917847 1.513157
1466.917847 1.513343
1466.917847 1.513351
1466.917847 1.513984
1466.917847 1.514464
1466.917847 1.515734
1466.917847 1.517020
1466.917847 1.518538
1466.917847 1.519217
1466.917847 1.519885
1466.917847 1.521312
1466.917847 1.521907
1466.917847 1.522218
1466.917847 1.522659
1466.917847 1.522891
1466.917847 1.523346
1466.917847 1.522891
1466.917847 1.522747
1466.917847 1.523214
1466.917847 1.523878
1466.917847 1.525167
1466.917847 1.526543
1466.917847 1.527558
1466.917847 1.529054
1466.917847 1.530075
1466.917847 1.531001
1466.917847 1.531390
1466.917847 1.532279
1466.917847 1.533873
1466.917847 1.535520
1466.917847 1.536830
1466.917847 1.538093
1466.917847 1.539713
1466.917847 1.540481
1466.917847 1.541022
1466.917847 1.542143
1466.917847 1.542714
1466.917847 1.543526
1466.917847 1.544912
1466.917847 1.546018
1466.917847 1.547480
1466.917847 1.548867
1466.917847 1.549729
1466.917847 1.550953
1466.917847 1.552196
1466.917847 1.551922
1466.917847 1.551526
1466.917847 1.551254
1466.917847 1.551430
1466.917847 1.551853
1466.917847 1.552549
1466.917847 1.553258
1466.917847 1.554084
1483.050903 1.541032
1483.050903 1.541705
1499.104248 1.520189
1499.104248 1.521444
1499.104248 1.522678
1499.104248 1.523642
1499.104248 1.524381
1499.104248 1.524757
1499.104248 1.525301
1499.104248 1.525742
1499.104248 1.526739
1499.104248 1.527721
1499.104248 1.528441
1499.104248 1.529298
1499.104248 1.530659
1499.104248 1.531684
1499.104248 1.532198
1499.104248 1.532800
1499.104248 1.532595
1499.104248 1.532904
1499.104248 1.532592
1499.104248 1.532496
1499.104248 1.533204
1499.104248 1.533164
1499.104248 1.532962
1499.104248 1.532724
1499.104248 1.532849
1499.104248 1.532083
1499.104248 1.532442
1499.104248 1.532745
1499.104248 1.532724
1499.104248 1.532510
1499.104248 1.532625
1499.104248 1.533075
1499.104248 1.533798
1499.104248 1.534311
1499.104248 1.534004
1499.104248 1.534110
1499.104248 1.534024
1499.104248 1.534444
1499.104248 1.534896
1499.104248 1.534375
1499.104248 1.534235
1499.104248 1.534091
1499.104248 1.533995
1499.104248 1.532908
1499.104248 1.532265
1499.104248 1.531595
1499.104248 1.530871
1499.104248 1.530498
1499.104248 1.530165
1499.104248 1.530859
1499.104248 1.531121
1499.104248 1.530540
1499.104248 1.530643
1499.104248 1.531560
1499.104248 1.532339
1499.104248 1.533035
1499.104248 1.534466
1499.104248 1.535588
1499.104248 1.536683
1499.104248 1.537113
1499.104248 1.537268
1499.104248 1.537318
1499.104248 1.537704
1515.421387 1.485971
1515.421387 1.485917
1515.421387 1.485559
1515.421387 1.485501
1515.421387 1.484922
1515.421387 1.484958
1515.421387 1.484713
1515.421387 1.484230
1515.421387 1.484400
1515.421387 1.484922
1515.421387 1.485569
1515.421387 1.486632
1515.421387 1.487439
1515.421387 1.487892
1515.421387 1.488428
1515.421387 1.489325
1515.421387 1.490819
1515.421387 1.492238
1515.421387 1.493863
1515.421387 1.495306
1515.421387 1.496676
1515.421387 1.497310
1515.421387 1.498460
1515.421387 1.499922
1515.421387 1.500571
1515.421387 1.501185
1515.421387 1.501121
1515.421387 1.501099
1515.421387 1.501558
1515.421387 1.501804
1515.421387 1.502808
1515.421387 1.503971
1515.421387 1.505497
1515.421387 1.506594
1531.837524 1.476977
1531.837524 1.477275
1531.837524 1.477285
1531.837524 1.478506
1531.837524 1.479513
1531.837524 1.480465
1531.837524 1.481019
1531.837524 1.482126
1531.837524 1.482339
1531.837524 1.482154
1531.837524 1.483661
1531.837524 1.483279
1531.837524 1.483675
1531.837524 1.484079
1531.837524 1.484588
1531.837524 1.484911
1531.837524 1.484728
1531.837524 1.485928
1531.837524 1.486990
1531.837524 1.487813
1531.837524 1.488183
1531.837524 1.488965
1531.837524 1.490151
1531.837524 1.491480
1531.837524 1.492796
1531.837524 1.493720
1531.837524 1.494611
1531.837524 1.496586
1531.837524 1.497182
1531.837524 1.497953
1531.837524 1.498381
1531.837524 1.499370
1531.837524 1.500188
1531.837524 1.500805
1531.837524 1.501362
1531.837524 1.502380
1531.837524 1.503422
1531.837524 1.503548
1531.837524 1.503614
1531.837524 1.503795
1531.837524 1.504284
1531.837524 1.504433
1531.837524 1.504613
1531.837524 1.505446
1531.837524 1.506271
1548.413452 1.477218
1548.413452 1.477564
1548.413452 1.477300
1548.413452 1.478177
1548.413452 1.478523
1548.413452 1.478419
1548.413452 1.479120
1548.413452 1.479172
1548.413452 1.479774
1548.413452 1.480064
1548.413452 1.479730
1548.413452 1.479475
1548.413452 1.479049
1548.413452 1.478257
1548.413452 1.477867
1548.413452 1.478032
1548.413452 1.478175
1548.413452 1.478745
1548.413452 1.479046
1548.413452 1.479168
1548.413452 1.479394
1548.413452 1.479863
1548.413452 1.480221
1548.413452 1.480889
1548.413452 1.482262
1548.413452 1.483349
1548.413452 1.483029
1548.413452 1.483617
1548.413452 1.484203
1548.413452 1.484734
1548.413452 1.484522
1548.413452 1.485070
1548.413452 1.486143
1548.413452 1.487669
1548.413452 1.488346
1548.413452 1.488091
1548.413452 1.488270
1548.413452 1.487977
1548.413452 1.488491
1548.413452 1.488570
1548.413452 1.488472
1548.413452 1.488259
1548.413452 1.488804
1548.413452 1.489274
1548.413452 1.489681
1548.413452 1.489556
1548.413452 1.490185
1548.413452 1.490534
1548.413452 1.491608
1548.413452 1.492676
1548.413452 1.493726
1548.413452 1.494909
1548.413452 1.495714
1548.413452 1.496704
1548.413452 1.498206
1548.413452 1.499870
1548.413452 1.500278
1548.413452 1.501992
1548.413452 1.504076
1548.413452 1.505846
1548.413452 1.508053
1548.413452 1.509508
1548.413452 1.510362
1548.413452 1.511423
1548.413452 1.512434
1548.413452 1.513258
1548.413452 1.513593
1548.413452 1.514108
1548.413452 1.514200
1548.413452 1.513974
1548.413452 1.513557
1548.413452 1.513381
1548.413452 1.513027
1548.413452 1.512643
1548.413452 1.513222
1548.413452 1.513050
1548.413452 1.513180
1548.413452 1.512532
1548.413452 1.512867
1548.413452 1.513007
1548.413452 1.512539
1548.413452 1.511970
1548.413452 1.511244
1548.413452 1.510569
1548.413452 1.510633
1548.413452 1.510305
1548.413452 1.509894
1548.413452 1.508304
1548.413452 1.507479
1548.413452 1.507264
1548.413452 1.505611
1548.413452 1.504496
1548.413452 1.505151
1548.413452 1.505180
1548.413452 1.505898
1548.413452 1.506482
1548.413452 1.507456
1548.413452 1.508312
1548.413452 1.508755
1548.413452 1.509102
1548.413452 1.509646
1548.413452 1.510598
1548.413452 1.512076
1548.413452 1.512819
1548.413452 1.513602
1548.413452 1.514353
1548.413452 1.514298
1565.493042 1.494848
1565.493042 1.495931
1565.493042 1.496692
1565.493042 1.497622
1565.493042 1.498767
1565.493042 1.499612
1565.493042 1.500161
1565.493042 1.501594
1565.493042 1.502386
1565.493042 1.503310
1565.493042 1.504489
1565.493042 1.504872
1565.493042 1.505330
1565.493042 1.505971
1565.493042 1.506810
1565.493042 1.507298
1565.493042 1.508595
1565.493042 1.509515
1565.493042 1.510706
1565.493042 1.511122
1565.493042 1.512383
1565.493042 1.513284
1565.493042 1.513255
1565.493042 1.513230
1565.493042 1.513259
1565.493042 1.513646
1565.493042 1.513966
1565.493042 1.514132
1565.493042 1.514467
1565.493042 1.514690
1565.493042 1.515171
1565.493042 1.515445
1565.493042 1.516114
1565.493042 1.516716
1565.493042 1.517287
1565.493042 1.518494
1565.493042 1.519412
1565.493042 1.520567
1565.493042 1.520766
1565.493042 1.521400
1565.493042 1.521819
1565.493042 1.522394
1565.493042 1.522862
1565.493042 1.523966
1565.493042 1.524857
1565.493042 1.525738
1565.493042 1.526042
1565.493042 1.526786
1565.493042 1.526892
1565.493042 1.527750
1565.493042 1.527666
1565.493042 1.528157
1565.493042 1.527997
1565.493042 1.528133
1565.493042 1.528214
1565.493042 1.529436
1565.493042 1.530573
1565.493042 1.533071
1565.493042 1.535141
1565.493042 1.536319
1565.493042 1.536984
1565.493042 1.537394
1565.493042 1.537092
1565.493042 1.537152
1565.493042 1.537671
1565.493042 1.538932
1565.493042 1.540381
1565.493042 1.542311
1565.493042 1.543919
1565.493042 1.545624
1565.493042 1.547076
1565.493042 1.548708
1565.493042 1.549327
1565.493042 1.550462
1565.493042 1.551641
1565.493042 1.553154
1565.493042 1.554266
1565.493042 1.555128
1565.493042 1.556021
1565.493042 1.556172
1565.493042 1.556445
1565.493042 1.556816
1565.493042 1.557064
1565.493042 1.557331
1565.493042 1.557485
1565.493042 1.557764
1565.493042 1.557884
1565.493042 1.558256
1565.493042 1.558215
1565.493042 1.557734
1565.493042 1.557246
1565.493042 1.556789
1565.493042 1.556504
1565.493042 1.557006
1565.493042 1.557095
1565.493042 1.557348
1565.493042 1.558064
1565.493042 1.558473
1565.493042 1.560022
1565.493042 1.561091
1565.493042 1.562537
1565.493042 1.563689
1565.493042 1.564454
1565.493042 1.564569
1565.493042 1.564699
1565.493042 1.566288
1565.493042 1.567089
1565.493042 1.567896
1565.493042 1.568339
1565.493042 1.568440
1565.493042 1.568584
1565.493042 1.569272
1565.493042 1.570130
1565.493042 1.571390
1565.493042 1.572952
1565.493042 1.575102
1565.493042 1.577150
1565.493042 1.578540
1565.493042 1.580429
1565.493042 1.581753
1565.493042 1.583360
1565.493042 1.584946
1565.493042 1.585617
1565.493042 1.586342
1565.493042 1.586207
1565.493042 1.586107
1565.493042 1.586461
1565.493042 1.587003
1565.493042 1.586752
1565.493042 1.587147
1565.493042 1.587357
1565.493042 1.587819
1565.493042 1.587534
1565.493042 1.587097
1565.493042 1.586652
1565.493042 1.587395
1565.493042 1.587867
1565.493042 1.588993
1565.493042 1.590364
1565.493042 1.591261
1565.493042 1.592063
1565.493042 1.593222
1565.493042 1.595047
1565.493042 1.596349
1565.493042 1.597668
1565.493042 1.597859
1565.493042 1.598229
1565.493042 1.599565
1583.300049 1.540557
1583.300049 1.540765
1583.300049 1.541766
1583.300049 1.542845
1583.300049 1.543944
1583.300049 1.544625
1583.300049 1.544919
1583.300049 1.545436
1583.300049 1.545800
1583.300049 1.546529
1583.300049 1.547174
1583.300049 1.547239
1583.300049 1.546952
1583.300049 1.546829
1583.300049 1.546613
1583.300049 1.546554
1583.300049 1.546099
1583.300049 1.545724
1583.300049 1.544990
1583.300049 1.544785
1583.300049 1.544265
1583.300049 1.544584
1583.300049 1.544826
1583.300049 1.545477
1583.300049 1.545890
1583.300049 1.546697
1583.300049 1.547660
1583.300049 1.549348
1583.300049 1.551059
1583.300049 1.552318
1583.300049 1.553007
1583.300049 1.554168
1583.300049 1.554503
1583.300049 1.554898
1583.300049 1.555718
1583.300049 1.556884
1583.300049 1.558358
1583.300049 1.559591
1583.300049 1.560153
1583.300049 1.561084
1583.300049 1.561967
1583.300049 1.562493
1583.300049 1.563491
1583.300049 1.564609
1583.300049 1.566658
1583.300049 1.568229
1583.300049 1.569433
1583.300049 1.570236
1583.300049 1.571053
1583.300049 1.571720
1583.300049 1.572419
1583.300049 1.573165
1583.300049 1.574233
1601.301880 1.498330
1601.301880 1.498507
1601.301880 1.499359
1601.301880 1.499686
1601.301880 1.500166
1601.301880 1.500907
1601.301880 1.501041
1601.301880 1.501397
1601.301880 1.501193
1601.301880 1.501353
1601.301880 1.501119
1601.301880 1.500747
1601.301880 1.500774
1601.301880 1.499785
1601.301880 1.499019
1601.301880 1.498665
1601.301880 1.498827
1601.301880 1.498013
1601.301880 1.497959
1601.301880 1.497979
1601.301880 1.497499
1601.301880 1.496229
1601.301880 1.495076
1601.301880 1.494955
1601.301880 1.495219
1601.301880 1.495548
1601.301880 1.495612
1601.301880 1.495325
1601.301880 1.496689
1601.301880 1.497428
1601.301880 1.498377
1601.301880 1.498649
1601.301880 1.499031
1601.301880 1.499066
1601.301880 1.499249
1601.301880 1.498555
1601.301880 1.497567
1601.301880 1.498178
1601.301880 1.498957
1601.301880 1.499428
1601.301880 1.499750
1601.301880 1.500278
1601.301880 1.500071
1601.301880 1.499462
1601.301880 1.499041
1601.301880 1.499334
1601.301880 1.500229
1601.301880 1.500980
1601.301880 1.501186
1601.301880 1.502041
1601.301880 1.503299
1601.301880 1.504178
1601.301880 1.505666
1601.301880 1.506758
1601.301880 1.507780
1601.301880 1.508602
1601.301880 1.508750
1601.301880 1.509492
1601.301880 1.510457
1601.301880 1.511343
1601.301880 1.511555
1601.301880 1.511318
1601.301880 1.510737
1601.301880 1.510162
1601.301880 1.509429
1601.301880 1.509544
1601.301880 1.509366
1601.301880 1.509541
1601.301880 1.509929
1601.301880 1.509852
1601.301880 1.510255
1601.301880 1.509940
1601.301880 1.508984
1601.301880 1.508705
1601.301880 1.508604
1601.301880 1.508224
1601.301880 1.508453
1601.301880 1.509289
1601.301880 1.509736
1601.301880 1.510130
1601.301880 1.509827
1601.301880 1.509646
1601.301880 1.510115
1601.301880 1.509951
1601.301880 1.509948
1601.301880 1.509817
1601.301880 1.509904
1601.301880 1.510250
1601.301880 1.510544
1601.301880 1.511003
1601.301880 1.511547
1601.301880 1.512368
1601.301880 1.513287
1601.301880 1.513330
1601.301880 1.513959
1601.301880 1.515534
1601.301880 1.516861
1601.301880 1.518495
1601.301880 1.519916
1601.301880 1.520849
1601.301880 1.521424
1601.301880 1.521935
1619.767944 1.523784
1619.767944 1.524688
1619.767944 1.525898
1619.767944 1.527460
1619.767944 1.528393
1619.767944 1.529159
1619.767944 1.529256
1619.767944 1.529702
1619.767944 1.529503
1619.767944 1.530073
1638.187378 1.534109
1638.187378 1.534773
1656.516479 1.526011
1656.516479 1.526298
1656.516479 1.527045
1656.516479 1.527628
1656.516479 1.527874
1656.516479 1.527667
1656.516479 1.529534
1656.516479 1.531309
1656.516479 1.532585
1656.516479 1.534186
1656.516479 1.535591
1656.516479 1.536805
1656.516479 1.538806
1656.516479 1.539664
1656.516479 1.540297
1656.516479 1.540952
1656.516479 1.540593
1656.516479 1.541654
1656.516479 1.542405
1656.516479 1.543053
1656.516479 1.543242
1656.516479 1.543265
1656.516479 1.543828
1656.516479 1.544699
1656.516479 1.545818
1656.516479 1.545923
1656.516479 1.546116
1656.516479 1.546826
1656.516479 1.547587
1656.516479 1.548433
1656.516479 1.549771
1656.516479 1.551098
1656.516479 1.552014
1656.516479 1.552461
1656.516479 1.553575
1656.516479 1.554528
1656.516479 1.554723
1656.516479 1.555088
1656.516479 1.555477
1656.516479 1.555694
1656.516479 1.555672
1656.516479 1.556898
1656.516479 1.558027
1656.516479 1.558897
1656.516479 1.560436
1656.516479 1.562467
1656.516479 1.563295
1656.516479 1.564544
1656.516479 1.565662
1656.516479 1.566655
1656.516479 1.566622
1656.516479 1.567098
1656.516479 1.567300
1656.516479 1.567832
1656.516479 1.568244
1656.516479 1.567592
1656.516479 1.566599
1656.516479 1.566138
1656.516479 1.565576
1656.516479 1.565259
1656.516479 1.565533
1656.516479 1.565115
1656.516479 1.564722
1656.516479 1.564599
1656.516479 1.564835
1656.516479 1.565149
1656.516479 1.565888
1656.516479 1.565679
1656.516479 1.566916
1656.516479 1.566902
1656.516479 1.567753
1656.516479 1.568036
1656.516479 1.567869
1656.516479 1.568106
1656.516479 1.567725
1656.516479 1.568517
1656.516479 1.568149
1656.516479 1.568211
1656.516479 1.567793
1656.516479 1.567945
1656.516479 1.568419
1656.516479 1.568836
1656.516479 1.569015
1656.516479 1.569404
1656.516479 1.569723
1656.516479 1.570264
1656.516479 1.569573
1656.516479 1.568458
1656.516479 1.567291
1656.516479 1.566297
1656.516479 1.565359
1656.516479 1.564931
1656.516479 1.565165
1656.516479 1.564717
1656.516479 1.564750
1656.516479 1.564504
1656.516479 1.564644
1656.516479 1.563603
1656.516479 1.563003
1656.516479 1.561513
1656.516479 1.561101
1656.516479 1.559855
1656.516479 1.559103
1656.516479 1.559114
1656.516479 1.559960
1656.516479 1.560106
1656.516479 1.560094
1656.516479 1.560910
1656.516479 1.562101
1656.516479 1.563258
1656.516479 1.564378
1656.516479 1.565722
1656.516479 1.567619
1656.516479 1.570357
1656.516479 1.572230
1656.516479 1.573426
1656.516479 1.574973
1656.516479 1.575913
1656.516479 1.576894
1656.516479 1.578356
1656.516479 1.579853
1656.516479 1.580884
1656.516479 1.582568
1656.516479 1.583581
1656.516479 1.585190
1656.516479 1.587338
1656.516479 1.588852
1656.516479 1.589656
1656.516479 1.590699
1656.516479 1.591099
1656.516479 1.590769
1656.516479 1.590856
1656.516479 1.591092
1656.516479 1.592070
1656.516479 1.593487
1656.516479 1.594324
1656.516479 1.595364
1656.516479 1.596381
1656.516479 1.597588
1656.516479 1.599075
1656.516479 1.600004
1656.516479 1.601380
1656.516479 1.602409
1656.516479 1.604331
1656.516479 1.606562
1656.516479 1.609361
1656.516479 1.612031
1656.516479 1.614015
1656.516479 1.615727
1656.516479 1.617119
1656.516479 1.618888
1656.516479 1.620860
1656.516479 1.622283
1656.516479 1.623410
1656.516479 1.625563
1675.594482 1.594033
1675.594482 1.594887
1675.594482 1.595757
1675.594482 1.596700
1675.594482 1.597831
1675.594482 1.599688
1675.594482 1.600443
1675.594482 1.600709
1675.594482 1.600029
1675.594482 1.599965
1675.594482 1.599748
1675.594482 1.598666
1675.594482 1.596956
1675.594482 1.595760
1675.594482 1.594871
1675.594482 1.593843
1675.594482 1.592420
1675.594482 1.591695
1675.594482 1.590773
1675.594482 1.590435
1675.594482 1.590355
1675.594482 1.589724
1675.594482 1.589873
1675.594482 1.589961
1675.594482 1.588686
1675.594482 1.588194
1675.594482 1.587746
1675.594482 1.587138
1675.594482 1.587342
1675.594482 1.586902
1675.594482 1.587062
1675.594482 1.586187
1675.594482 1.584924
1675.594482 1.584176
1675.594482 1.583571
1675.594482 1.583756
1675.594482 1.584316
1675.594482 1.584488
1675.594482 1.584134
1675.594482 1.583554
1675.594482 1.583180
1675.594482 1.583024
1675.594482 1.583469
1675.594482 1.584450
1675.594482 1.585466
1675.594482 1.586100
1675.594482 1.587623
1675.594482 1.588400
1675.594482 1.589898
1675.594482 1.590703
1675.594482 1.591552
1675.594482 1.591091
1675.594482 1.591013
1675.594482 1.590644
1675.594482 1.590414
1675.594482 1.591053
1675.594482 1.592143
1675.594482 1.593605
1675.594482 1.595753
1675.594482 1.598155
1675.594482 1.600264
1675.594482 1.601547
1694.907104 1.631983
1694.907104 1.633987
1694.907104 1.634733
1694.907104 1.636206
1694.907104 1.637148
1694.907104 1.638497
1694.907104 1.639211
1694.907104 1.639345
1694.907104 1.639282
1694.907104 1.639650
1694.907104 1.640649
1694.907104 1.641629
1694.907104 1.642309
1694.907104 1.642982
1694.907104 1.644339
1694.907104 1.646370
1694.907104 1.647870
1694.907104 1.649633
1694.907104 1.650983
1694.907104 1.651277
1694.907104 1.651828
1694.907104 1.652609
1694.907104 1.653165
1694.907104 1.653476
1694.907104 1.653113
1694.907104 1.652521
1694.907104 1.652293
1694.907104 1.652824
1694.907104 1.654327
1694.907104 1.655863
1694.907104 1.657357
1694.907104 1.658736
1714.288818 1.613558
1714.288818 1.614931
1714.288818 1.615774
1714.288818 1.616404
1714.288818 1.616520
1714.288818 1.615787
1714.288818 1.614637
1714.288818 1.613270
1714.288818 1.611798
1714.288818 1.610459
1714.288818 1.610809
1714.288818 1.610507
1714.288818 1.610298
1714.288818 1.609948
1714.288818 1.609485
1714.288818 1.608854
1714.288818 1.608443
1714.288818 1.608513
1714.288818 1.607602
1714.288818 1.607253
1714.288818 1.608109
1714.288818 1.609099
1714.288818 1.609391
1714.288818 1.609336
1714.288818 1.609869
1714.288818 1.610007
1714.288818 1.609538
1714.288818 1.608889
1714.288818 1.609362
1714.288818 1.609537
1714.288818 1.609356
1714.288818 1.609213
1714.288818 1.609449
1714.288818 1.610598
1714.288818 1.610978
1714.288818 1.612368
1714.288818 1.613217
1714.288818 1.613234
1714.288818 1.613237
1714.288818 1.613482
1714.288818 1.614024
1714.288818 1.613815
1714.288818 1.614422
1714.288818 1.614084
1714.288818 1.614334
1714.288818 1.614665
1714.288818 1.615084
1714.288818 1.614912
1714.288818 1.615359
1714.288818 1.615918
1714.288818 1.616300
1714.288818 1.617460
1714.288818 1.617810
1714.288818 1.618357
1714.288818 1.619684
1714.288818 1.621037
1714.288818 1.622390
1714.288818 1.622753
1714.288818 1.623089
1714.288818 1.624050
1714.288818 1.625603
1714.288818 1.626189
1714.288818 1.626805
1714.288818 1.627179
1714.288818 1.628191
1714.288818 1.628821
1714.288818 1.630363
1714.288818 1.632153
1714.288818 1.634190
1714.288818 1.635736
1714.288818 1.636961
1714.288818 1.637929
1714.288818 1.638944
1714.288818 1.639937
1714.288818 1.640745
1714.288818 1.642305
1714.288818 1.643442
1714.288818 1.645012
1714.288818 1.645572
1714.288818 1.645471
1714.288818 1.646001
1714.288818 1.645856
1714.288818 1.646110
1714.288818 1.646197
1714.288818 1.646924
1714.288818 1.647204
1714.288818 1.647559
1714.288818 1.648379
1714.288818 1.649432
1714.288818 1.650250
1714.288818 1.649987
1714.288818 1.650636
1714.288818 1.650681
1714.288818 1.651109
1714.288818 1.651606
1714.288818 1.652371
1714.288818 1.652593
1714.288818 1.652501
1714.288818 1.652368
1714.288818 1.652361
1714.288818 1.652746
1714.288818 1.653436
1714.288818 1.653805
1714.288818 1.653710
1714.288818 1.653922
1714.288818 1.653707
1714.288818 1.654511
1714.288818 1.655091
1714.288818 1.656690
1714.288818 1.657524
1714.288818 1.658708
1714.288818 1.658810
1714.288818 1.659108
1714.288818 1.659098
1714.288818 1.659675
1714.288818 1.660128
1714.288818 1.659860
1714.288818 1.659462
1714.288818 1.659174
1714.288818 1.659392
1714.288818 1.659265
1714.288818 1.660235
1714.288818 1.660937
1714.288818 1.661637
1714.288818 1.661738
1714.288818 1.661870
1714.288818 1.662848
1714.288818 1.663290
1714.288818 1.663593
1714.288818 1.664545
1714.288818 1.666325
1714.288818 1.667913
1714.288818 1.669812
1714.288818 1.671496
1714.288818 1.673581
1734.298950 1.679171
1734.298950 1.680193
1734.298950 1.680946
1734.298950 1.681334
1734.298950 1.681031
1734.298950 1.680657
1734.298950 1.680222
1734.298950 1.680158
1734.298950 1.680343
1734.298950 1.680246
1734.298950 1.680528
1734.298950 1.680828
1734.298950 1.680965
1734.298950 1.680684
1734.298950 1.680529
1734.298950 1.680307
1734.298950 1.679683
1734.298950 1.679675
1734.298950 1.679369
1734.298950 1.678800
1734.298950 1.678571
1734.298950 1.678363
1734.298950 1.677821
1734.298950 1.677791
1734.298950 1.678698
1734.298950 1.679380
1734.298950 1.679830
1734.298950 1.680514
1734.298950 1.680446
1734.298950 1.680508
1734.298950 1.680762
1734.298950 1.681711
1734.298950 1.683064
1734.298950 1.684264
1734.298950 1.686386
1734.298950 1.687932
1734.298950 1.688834
1734.298950 1.690080
1734.298950 1.691329
1734.298950 1.693103
1734.298950 1.694715
1734.298950 1.696108
1734.298950 1.697434
1734.298950 1.698065
1734.298950 1.698490
1734.298950 1.698336
1734.298950 1.698243
1734.298950 1.698723
1734.298950 1.698882
1734.298950 1.699105
1734.298950 1.698807
1734.298950 1.698607
1734.298950 1.698826
1734.298950 1.699212
1734.298950 1.699315
1734.298950 1.699440
1734.298950 1.699165
1734.298950 1.699291
1734.298950 1.699039
1734.298950 1.699493
1734.298950 1.700373
1734.298950 1.700927
1734.298950 1.701084
1734.298950 1.701905
1734.298950 1.703241
1734.298950 1.703930
1734.298950 1.704496
1734.298950 1.705032
1734.298950 1.706273
1734.298950 1.707391
1734.298950 1.708550
1734.298950 1.709513
1734.298950 1.709892
1734.298950 1.710245
1734.298950 1.711088
1734.298950 1.711093
1734.298950 1.711447
1734.298950 1.712282
1734.298950 1.713135
1734.298950 1.713203
1734.298950 1.713328
1734.298950 1.714025
1734.298950 1.714366
1734.298950 1.715271
1734.298950 1.716853
1734.298950 1.717548
1734.298950 1.718167
1734.298950 1.719028
1734.298950 1.720469
1734.298950 1.721911
1734.298950 1.722947
1734.298950 1.724033
1734.298950 1.724385
1734.298950 1.724951
1734.298950 1.726720
1734.298950 1.728630
1734.298950 1.730290
1734.298950 1.731275
1734.298950 1.732356
1734.298950 1.733385
1734.298950 1.734331
1734.298950 1.734546
1734.298950 1.735450
1734.298950 1.735602
1734.298950 1.736744
1734.298950 1.737623
1734.298950 1.739217
1734.298950 1.739960
1734.298950 1.740987
1734.298950 1.742237
1734.298950 1.743549
1734.298950 1.744574
1734.298950 1.745620
1754.812988 1.635831
1754.812988 1.635776
1754.812988 1.635976
1754.812988 1.635820
1754.812988 1.635461
1754.812988 1.635654
1754.812988 1.635007
1754.812988 1.634807
1754.812988 1.635111
1754.812988 1.635349
1754.812988 1.635398
1754.812988 1.634742
1754.812988 1.633480
1754.812988 1.632611
1754.812988 1.631138
1754.812988 1.630425
1754.812988 1.630047
1754.812988 1.629579
1754.812988 1.628566
1754.812988 1.628253
1754.812988 1.627973
1754.812988 1.627886
1754.812988 1.628919
1754.812988 1.629709
1754.812988 1.630681
1754.812988 1.631342
1754.812988 1.631193
1754.812988 1.631213
1754.812988 1.631779
1754.812988 1.632504
1754.812988 1.633653
1754.812988 1.634488
1754.812988 1.635870
1754.812988 1.636295
1754.812988 1.637109
1754.812988 1.637355
1754.812988 1.636822
1754.812988 1.636438
1754.812988 1.637149
1754.812988 1.637762
1754.812988 1.637948
1754.812988 1.637883
1754.812988 1.638254
1754.812988 1.637916
1754.812988 1.638211
1754.812988 1.637703
1754.812988 1.638535
1754.812988 1.638189
1754.812988 1.637853
1754.812988 1.637399
1754.812988 1.636868
1754.812988 1.635954
1754.812988 1.635119
1754.812988 1.635100
1754.812988 1.635060
1754.812988 1.635215
1754.812988 1.635186
1754.812988 1.635355
1754.812988 1.635846
1754.812988 1.636090
1754.812988 1.637114
1754.812988 1.638397
1754.812988 1.639680
1754.812988 1.640438
1754.812988 1.640882
1754.812988 1.641639
1754.812988 1.641922
1754.812988 1.642684
1754.812988 1.643177
1754.812988 1.643991
1754.812988 1.643172
1754.812988 1.642712
1754.812988 1.642681
1754.812988 1.642777
1754.812988 1.642121
1754.812988 1.642372
1754.812988 1.642798
1754.812988 1.643129
1754.812988 1.643209
1754.812988 1.643980
1754.812988 1.645066
1754.812988 1.645715
1754.812988 1.646160
1754.812988 1.646894
1754.812988 1.646848
1754.812988 1.647721
1754.812988 1.648618
1754.812988 1.649316
1754.812988 1.649701
1754.812988 1.650904
1754.812988 1.651921
1754.812988 1.652813
1754.812988 1.653617
1754.812988 1.654572
1754.812988 1.656144
1754.812988 1.656760
1754.812988 1.657324
1754.812988 1.658295
1754.812988 1.659376
1754.812988 1.660284
1754.812988 1.661184
1754.812988 1.662228
1754.812988 1.664244
1754.812988 1.665416
1754.812988 1.666526
1754.812988 1.668139
1754.812988 1.668789
1754.812988 1.669710
1754.812988 1.671206
1754.812988 1.672217
1754.812988 1.673296
1754.812988 1.673841
1754.812988 1.674194
1754.812988 1.675127
1754.812988 1.675451
1754.812988 1.675758
1754.812988 1.675895
1754.812988 1.676512
1754.812988 1.677678
1754.812988 1.678575
1754.812988 1.679602
1754.812988 1.680602
1754.812988 1.681226
1754.812988 1.681901
1754.812988 1.682596
1754.812988 1.683232
1754.812988 1.684204
1754.812988 1.684655
1754.812988 1.685270
1754.812988 1.685653
1754.812988 1.685823
1754.812988 1.686407
1754.812988 1.686778
1754.812988 1.687265
1754.812988 1.687692
1754.812988 1.687998
1754.812988 1.687875
1754.812988 1.687980
1754.812988 1.688247
1754.812988 1.688405
1754.812988 1.688448
1754.812988 1.689314
1754.812988 1.689601
1754.812988 1.690190
1754.812988 1.690734
1754.812988 1.691069
1754.812988 1.691283
1754.812988 1.691710
1754.812988 1.692100
1754.812988 1.691914
1754.812988 1.691892
1754.812988 1.692647
1754.812988 1.693842
1754.812988 1.694452
1754.812988 1.695744
1754.812988 1.696819
1754.812988 1.697626
1754.812988 1.699503
1754.812988 1.700736
1754.812988 1.701465
1754.812988 1.701996
1754.812988 1.702053
1754.812988 1.702865
1754.812988 1.703960
1754.812988 1.704574
1754.812988 1.704903
1754.812988 1.706164
1754.812988 1.706531
1754.812988 1.706486
1754.812988 1.706588
1754.812988 1.706806
1754.812988 1.706720
1754.812988 1.706749
1754.812988 1.706304
1754.812988 1.706102
1754.812988 1.705824
1754.812988 1.704990
1754.812988 1.704961
1754.812988 1.705938
1754.812988 1.706443
1754.812988 1.706508
1754.812988 1.707434
1754.812988 1.707780
1754.812988 1.708117
1754.812988 1.708275
1754.812988 1.707983
1754.812988 1.707152
1754.812988 1.705931
1754.812988 1.704619
1754.812988 1.703954
1754.812988 1.703210
1754.812988 1.703202
1754.812988 1.703382
1754.812988 1.703637
1754.812988 1.703492
1754.812988 1.703319
1754.812988 1.703819
1754.812988 1.703901
1754.812988 1.705039
1754.812988 1.705840
1754.812988 1.706220
1754.812988 1.706698
1754.812988 1.706704
1754.812988 1.705982
1754.812988 1.705648
1754.812988 1.705046
1754.812988 1.704334
1754.812988 1.703977
1754.812988 1.704283
1754.812988 1.704879
1754.812988 1.706169
1754.812988 1.706520
1754.812988 1.707325
1754.812988 1.708304
1754.812988 1.709445
1754.812988 1.710514
1754.812988 1.711167
1754.812988 1.711291
1754.812988 1.711499
1754.812988 1.712333
1754.812988 1.712382
1754.812988 1.712419
1754.812988 1.712881
1754.812988 1.713504
1754.812988 1.713768
1754.812988 1.714596
1754.812988 1.715363
1754.812988 1.716046
1754.812988 1.715614
1754.812988 1.715180
1754.812988 1.715081
1776.464844 1.633538
1776.464844 1.633329
1776.464844 1.633511
1776.464844 1.633551
1776.464844 1.633637
1776.464844 1.634210
1776.464844 1.634611
1776.464844 1.635780
1776.464844 1.636460
1776.464844 1.637042
1776.464844 1.637873
1776.464844 1.638506
1776.464844 1.638796
1776.464844 1.639917
1776.464844 1.641022
1776.464844 1.641901
1776.464844 1.643199
1776.464844 1.644241
1776.464844 1.644927
1776.464844 1.645670
1776.464844 1.646835
1776.464844 1.648652
1776.464844 1.649135
1776.464844 1.649400
1776.464844 1.649569
1776.464844 1.650105
1776.464844 1.650538
1776.464844 1.650337
1776.464844 1.650734
1776.464844 1.651165
1776.464844 1.650441
1776.464844 1.649751
1776.464844 1.648848
1776.464844 1.648369
1776.464844 1.647363
1776.464844 1.647628
1776.464844 1.646775
1776.464844 1.646644
1776.464844 1.647088
1776.464844 1.647930
1776.464844 1.649624
1776.464844 1.650746
1776.464844 1.650989
1776.464844 1.651620
1776.464844 1.652115
1776.464844 1.652120
1776.464844 1.652147
1776.464844 1.651865
1776.464844 1.651707
1776.464844 1.651070
1776.464844 1.651214
1776.464844 1.650443
1776.464844 1.650254
1776.464844 1.649867
1776.464844 1.649817
1776.464844 1.649428
1776.464844 1.649744
1776.464844 1.649262
1776.464844 1.648606
1776.464844 1.648878
1776.464844 1.649470
1776.464844 1.649979
1776.464844 1.649848
1776.464844 1.650133
1776.464844 1.649719
1776.464844 1.649885
1776.464844 1.650068
1776.464844 1.650439
1776.464844 1.650599
1776.464844 1.650761
1776.464844 1.651053
1776.464844 1.651059
1776.464844 1.651415
1776.464844 1.651698
1776.464844 1.651183
1776.464844 1.650353
1776.464844 1.650492
1776.464844 1.650385
1776.464844 1.650550
1776.464844 1.650997
1776.464844 1.650810
1776.464844 1.649686
1776.464844 1.649386
1776.464844 1.648296
1776.464844 1.648478
1776.464844 1.648440
1776.464844 1.648539
1776.464844 1.648456
1776.464844 1.648481
1776.464844 1.647866
1776.464844 1.647790
1776.464844 1.648568
1776.464844 1.649632
1776.464844 1.649981
1776.464844 1.650750
1776.464844 1.651523
1776.464844 1.652199
1776.464844 1.653127
1776.464844 1.654331
1776.464844 1.655216
1776.464844 1.657783
1798.544434 1.579546
1798.544434 1.582024
1798.544434 1.584931
1798.544434 1.587106
1798.544434 1.589066
1798.544434 1.589946
1798.544434 1.589826
1798.544434 1.589427
1798.544434 1.589755
1798.544434 1.589558
1798.544434 1.590429
1798.544434 1.590552
1798.544434 1.590572
1798.544434 1.590040
1798.544434 1.590185
1798.544434 1.590239
1798.544434 1.590286


==> fig/data/avgq-vs-success-2/banditstd-l2-cdf.tex <==
0 0.283590
2.000000 0.285482
3.000000 0.290213
4.000000 0.291170
5.333333 0.287684
6.500000 0.288786
7.600000 0.290410
8.000000 0.299123
9.263158 0.303386
10.095238 0.309590
12.296296 0.308128
12.642858 0.317273
13.400000 0.322070
13.806452 0.327433
14.250000 0.331067
15.176471 0.332566
15.176471 0.338779
17.157894 0.335540
18.536585 0.333499
19.441860 0.332781
19.909090 0.333280
20.400000 0.336389
20.913044 0.340067
21.958334 0.341252
21.958334 0.346878
21.958334 0.352373
21.958334 0.357851
23.240000 0.352917
24.500000 0.355223
24.500000 0.359706
24.500000 0.364048
25.888889 0.360025
25.888889 0.364302
26.618181 0.367418
28.070175 0.366680
28.793104 0.364098
30.233334 0.360033
30.950819 0.361044
30.950819 0.364616
32.444443 0.357842
32.444443 0.361258
32.444443 0.364786
33.250000 0.363710
34.061539 0.366166
34.061539 0.369802
36.529411 0.367464
36.529411 0.371108
37.362320 0.373444
37.362320 0.377171
37.362320 0.380900
37.362320 0.384566
38.285713 0.386303
40.111111 0.384558
41.013699 0.385762
42.799999 0.382790
43.684212 0.380350
43.684212 0.383463
43.684212 0.386737
44.623375 0.386854
45.564102 0.386680
45.564102 0.389833
47.474998 0.385998
48.419754 0.386663
48.419754 0.389311
50.337349 0.384608
50.337349 0.387136
50.337349 0.389699
54.183907 0.377450
55.113636 0.373235
55.113636 0.375748
55.113636 0.378391
57.044445 0.374423
57.044445 0.377152
57.044445 0.379691
57.044445 0.382328
57.044445 0.385037
57.044445 0.387665
57.044445 0.390458
58.131866 0.385526
61.319149 0.377842
61.319149 0.380139
62.378948 0.381033
62.378948 0.383500
62.378948 0.386012
63.479168 0.387160
64.577316 0.384008
65.673470 0.384921
67.839996 0.378579
69.960785 0.370078
69.960785 0.372384
71.029129 0.372810
71.029129 0.375098
71.029129 0.377547
72.134613 0.373482
72.134613 0.375978
73.257141 0.376874
73.257141 0.379463
73.257141 0.381940
73.257141 0.384372
74.433960 0.381287
74.433960 0.383748
75.626167 0.381858
76.814812 0.381769
76.814812 0.384130
76.814812 0.386492
76.814812 0.388828
76.814812 0.391218
76.814812 0.393491
76.814812 0.395619
76.814812 0.397836
76.814812 0.400145
78.146790 0.400653
79.472725 0.401128
80.792793 0.398886
82.107140 0.399390
82.107140 0.401434
82.107140 0.403516
83.451324 0.399201
83.451324 0.401171
84.807014 0.397108
86.156525 0.396152
87.500000 0.396679
88.837608 0.395159
91.478989 0.390477
92.783333 0.390960
92.783333 0.392979
92.783333 0.394883
94.115700 0.395181
94.115700 0.397155
94.115700 0.399336
94.115700 0.401448
94.115700 0.403546
94.115700 0.405611
94.115700 0.407666
95.540985 0.402668
96.959351 0.402881
96.959351 0.404835
99.792000 0.399032
101.190475 0.395821
101.190475 0.397797
101.190475 0.399760
101.190475 0.401702
101.190475 0.403636
102.645668 0.399907
104.093750 0.393547
105.534882 0.390239
105.534882 0.391918
105.534882 0.393665
107.000000 0.389167
107.000000 0.390811
107.000000 0.392488
108.488548 0.390312
108.488548 0.392026
108.488548 0.393636
108.488548 0.395197
108.488548 0.396810
110.030304 0.391461
110.030304 0.392956
110.030304 0.394482
110.030304 0.396049
110.030304 0.397677
111.624062 0.396472
111.624062 0.398110
111.624062 0.399786
111.624062 0.401393
111.624062 0.403004
111.624062 0.404628
111.624062 0.406238
111.624062 0.407878
111.624062 0.409508
113.328362 0.409499
115.022224 0.409869
116.705879 0.409026
116.705879 0.410686
116.705879 0.412377
116.705879 0.414117
116.705879 0.415797
116.705879 0.417489
116.705879 0.419203
116.705879 0.420958
116.705879 0.422683
118.496353 0.422051
120.275360 0.417405
120.275360 0.419159
120.275360 0.420821
120.275360 0.422485
122.086334 0.419862
122.086334 0.421544
123.900002 0.417756
123.900002 0.419284
125.716309 0.414538
125.716309 0.415991
125.716309 0.417573
125.716309 0.419245
129.384613 0.414516
129.384613 0.416124
131.208328 0.411681
131.208328 0.413306
131.208328 0.414977
131.208328 0.416682
131.208328 0.418323
131.208328 0.419987
133.089661 0.418156
133.089661 0.419763
133.089661 0.421347
133.089661 0.422891
133.089661 0.424397
133.089661 0.425928
133.089661 0.427356
133.089661 0.428730
133.089661 0.430125
133.089661 0.431587
133.089661 0.433153
135.095886 0.428397
137.088440 0.426691
137.088440 0.428112
137.088440 0.429641
137.088440 0.431170
137.088440 0.432659
137.088440 0.434129
137.088440 0.435609
141.181213 0.431094
141.181213 0.432483
141.181213 0.434005
141.181213 0.435526
141.181213 0.436995
141.181213 0.438440
141.181213 0.439905
141.181213 0.441291
143.293335 0.436345
145.390732 0.436064
145.390732 0.437327
145.390732 0.438596
149.581696 0.421967
149.581696 0.423380
149.581696 0.424704
149.581696 0.426045
149.581696 0.427389
149.581696 0.428709
149.581696 0.429958
151.727280 0.429052
151.727280 0.430264
151.727280 0.431572
151.727280 0.432830
151.727280 0.434047
151.727280 0.435259
151.727280 0.436401
151.727280 0.437581
151.727280 0.438832
153.961288 0.431556
153.961288 0.432779
153.961288 0.434043
153.961288 0.435260
153.961288 0.436540
153.961288 0.437816
153.961288 0.439086
153.961288 0.440307
153.961288 0.441604
153.961288 0.442937
153.961288 0.444205
153.961288 0.445437
153.961288 0.446695
153.961288 0.447986
153.961288 0.449325
153.961288 0.450592
156.371796 0.442225
156.371796 0.443525
156.371796 0.444917
156.371796 0.446267
156.371796 0.447745
158.815292 0.446731
161.240509 0.443832
161.240509 0.445274
161.240509 0.446772
161.240509 0.448246
161.240509 0.449709
161.240509 0.451224
161.240509 0.452707
161.240509 0.454252
161.240509 0.455767
161.240509 0.457252
163.761002 0.456456
166.262497 0.455711
166.262497 0.457048
166.262497 0.458317
166.262497 0.459537
166.262497 0.460753
166.262497 0.461997
166.262497 0.463320
166.262497 0.464632
166.262497 0.465944
166.262497 0.467261
166.262497 0.468588
166.262497 0.469878
166.262497 0.471122
166.262497 0.472365
168.906830 0.471264
171.530869 0.469585
174.134964 0.468076
174.134964 0.469554
174.134964 0.471037
174.134964 0.472502
174.134964 0.473977
174.134964 0.475423
174.134964 0.476841
176.792679 0.476411
179.430298 0.473482
179.430298 0.474804
179.430298 0.476149
179.430298 0.477384
179.430298 0.478655
179.430298 0.479861
179.430298 0.481027
179.430298 0.482162
182.132523 0.477679
182.132523 0.478861
182.132523 0.480032
182.132523 0.481200
182.132523 0.482322
184.862274 0.475728
184.862274 0.476780
184.862274 0.477823
184.862274 0.478891
184.862274 0.479964
184.862274 0.481050
184.862274 0.482130
184.862274 0.483255
184.862274 0.484401
184.862274 0.485578
187.678574 0.483292
187.678574 0.484573
187.678574 0.485849
187.678574 0.487215
193.305878 0.481825
193.305878 0.483107
193.305878 0.484347
193.305878 0.485581
193.305878 0.486822
193.305878 0.488104
193.305878 0.489343
193.305878 0.490511
196.163742 0.490500
196.163742 0.491699
201.826584 0.488270
201.826584 0.489367
201.826584 0.490516
201.826584 0.491623
204.655167 0.490828
204.655167 0.491978
207.474289 0.483889
207.474289 0.484960
207.474289 0.486043
207.474289 0.487172
207.474289 0.488335
207.474289 0.489504
207.474289 0.490665
210.340912 0.490124
210.340912 0.491385
210.340912 0.492741
210.340912 0.494113
210.340912 0.495483
210.340912 0.496742
210.340912 0.497899
210.340912 0.498992
210.340912 0.500126
210.340912 0.501219
213.288132 0.491879
213.288132 0.493000
213.288132 0.494152
213.288132 0.495274
213.288132 0.496411
213.288132 0.497568
213.288132 0.498718
216.280899 0.497790
216.280899 0.498920
216.280899 0.500087
216.280899 0.501236
216.280899 0.502323
219.296097 0.501553
219.296097 0.502644
219.296097 0.503731
219.296097 0.504885
219.296097 0.506021
219.296097 0.507206
222.344452 0.501856
222.344452 0.503107
222.344452 0.504415
222.344452 0.505641
222.344452 0.506946
228.450546 0.498799
228.450546 0.500051
228.450546 0.501276
228.450546 0.502454
228.450546 0.503625
228.450546 0.504793
228.450546 0.505917
231.530060 0.501992
231.530060 0.503112
231.530060 0.504291
231.530060 0.505449
231.530060 0.506588
231.530060 0.507667
234.641312 0.507182
234.641312 0.508217
234.641312 0.509226
234.641312 0.510248
234.641312 0.511262
234.641312 0.512292
234.641312 0.513347
234.641312 0.514423
234.641312 0.515567
234.641312 0.516652
234.641312 0.517707
234.641312 0.518804
234.641312 0.519974
234.641312 0.521112
234.641312 0.522306
234.641312 0.523436
234.641312 0.524604
234.641312 0.525708
237.913513 0.522627
241.161285 0.522516
241.161285 0.523595
241.161285 0.524726
241.161285 0.525922
241.161285 0.527041
241.161285 0.528198
241.161285 0.529339
241.161285 0.530493
241.161285 0.531606
241.161285 0.532764
241.161285 0.533872
241.161285 0.535032
241.161285 0.536243
241.161285 0.537398
241.161285 0.538611
241.161285 0.539811
241.161285 0.540960
241.161285 0.542141
244.566849 0.537238
244.566849 0.538364
247.957443 0.538136
247.957443 0.539309
247.957443 0.540415
247.957443 0.541592
247.957443 0.542848
247.957443 0.544074
247.957443 0.545366
247.957443 0.546648
247.957443 0.547836
247.957443 0.548962
247.957443 0.550140
247.957443 0.551265
247.957443 0.552596
247.957443 0.553889
247.957443 0.555136
247.957443 0.556412
247.957443 0.557683
247.957443 0.558909
247.957443 0.560026
247.957443 0.561222
247.957443 0.562434
251.534393 0.555457
251.534393 0.556680
251.534393 0.557887
251.534393 0.559118
255.115784 0.551984
255.115784 0.553170
258.680634 0.549948
258.680634 0.551181
258.680634 0.552409
258.680634 0.553657
258.680634 0.554905
258.680634 0.556130
258.680634 0.557480
258.680634 0.558773
262.291656 0.555267
262.291656 0.556480
262.291656 0.557598
262.291656 0.558608
262.291656 0.559599
262.291656 0.560647
262.291656 0.561817
262.291656 0.562997
262.291656 0.564137
262.291656 0.565257
262.291656 0.566411
262.291656 0.567562
262.291656 0.568683
262.291656 0.569860
262.291656 0.571023
262.291656 0.572079
262.291656 0.573079
262.291656 0.574101
262.291656 0.575129
266.062164 0.572779
266.062164 0.573773
266.062164 0.574829
266.062164 0.575970
266.062164 0.577107
266.062164 0.578232
266.062164 0.579429
269.865967 0.571455
269.865967 0.572649
269.865967 0.573845
269.865967 0.575097
269.865967 0.576243
269.865967 0.577328
269.865967 0.578397
269.865967 0.579477
273.712830 0.572402
273.712830 0.573587
273.712830 0.574718
273.712830 0.575772
273.712830 0.576802
273.712830 0.577769
273.712830 0.578759
273.712830 0.579774
273.712830 0.580728
273.712830 0.581665
277.622437 0.573074
277.622437 0.574120
281.512695 0.569048
281.512695 0.570003
281.512695 0.570960
281.512695 0.571998
285.404053 0.568188
285.404053 0.569335
285.404053 0.570427
285.404053 0.571595
289.296478 0.569959
289.296478 0.571036
293.170013 0.568795
293.170013 0.569828
293.170013 0.570846
293.170013 0.571934
293.170013 0.573111
293.170013 0.574257
293.170013 0.575314
293.170013 0.576363
293.170013 0.577411
293.170013 0.578439
297.104492 0.578555
297.104492 0.579626
297.104492 0.580690
297.104492 0.581679
297.104492 0.582697
297.104492 0.583767
297.104492 0.584805
297.104492 0.585817
297.104492 0.586769
297.104492 0.587719
297.104492 0.588778
301.108917 0.583556
301.108917 0.584716
301.108917 0.585796
301.108917 0.586833
301.108917 0.587872
301.108917 0.588902
301.108917 0.589930
301.108917 0.590923
301.108917 0.591978
301.108917 0.593047
301.108917 0.594061
301.108917 0.595025
301.108917 0.596016
301.108917 0.596992
301.108917 0.597978
301.108917 0.598941
301.108917 0.599949
301.108917 0.600999
301.108917 0.602049
301.108917 0.603109
301.108917 0.604249
301.108917 0.605364
301.108917 0.606508
301.108917 0.607681
301.108917 0.608832
301.108917 0.609963
301.108917 0.611068
301.108917 0.612182
305.349762 0.606529
309.558838 0.605229
309.558838 0.606309
313.746338 0.591368
317.902924 0.589063
317.902924 0.590140
317.902924 0.591200
317.902924 0.592249
317.902924 0.593289
317.902924 0.594391
317.902924 0.595461
317.902924 0.596485
317.902924 0.597523
317.902924 0.598539
317.902924 0.599637
317.902924 0.600810
317.902924 0.601956
317.902924 0.603091
317.902924 0.604197
322.164246 0.603786
322.164246 0.604784
322.164246 0.605742
322.164246 0.606772
326.423065 0.603468
330.650726 0.603553
330.650726 0.604660
330.650726 0.605767
330.650726 0.606830
330.650726 0.607978
330.650726 0.609106
330.650726 0.610160
334.904755 0.608578
334.904755 0.609569
334.904755 0.610511
334.904755 0.611469
334.904755 0.612414
334.904755 0.613403
334.904755 0.614427
339.184845 0.604994
343.433960 0.595240
343.433960 0.596320
343.433960 0.597450
343.433960 0.598616
343.433960 0.599767
343.433960 0.600919
343.433960 0.602056
343.433960 0.603140
343.433960 0.604147
343.433960 0.605071
347.737091 0.603045
352.009338 0.595435
352.009338 0.596423
352.009338 0.597447
352.009338 0.598546
352.009338 0.599697
352.009338 0.600814
352.009338 0.601947
352.009338 0.603064
352.009338 0.604260
352.009338 0.605413
352.009338 0.606554
352.009338 0.607663
356.353485 0.606536
356.353485 0.607618
356.353485 0.608662
356.353485 0.609703
356.353485 0.610692
356.353485 0.611732
360.712952 0.602488
360.712952 0.603514
360.712952 0.604563
365.059906 0.603065
365.059906 0.604081
369.385315 0.603674
369.385315 0.604691
369.385315 0.605671
369.385315 0.606650
369.385315 0.607654
369.385315 0.608690
369.385315 0.609729
369.385315 0.610769
369.385315 0.611803
369.385315 0.612901
369.385315 0.614052
369.385315 0.615147
378.136353 0.601257
378.136353 0.602212
378.136353 0.603203
378.136353 0.604147
378.136353 0.605109
378.136353 0.606090
378.136353 0.607148
378.136353 0.608189
378.136353 0.609127
382.533936 0.600605
382.533936 0.601458
382.533936 0.602288
382.533936 0.603119
382.533936 0.603985
382.533936 0.604875
382.533936 0.605785
382.533936 0.606664
382.533936 0.607547
382.533936 0.608451
382.533936 0.609436
382.533936 0.610312
382.533936 0.611217
382.533936 0.612163
382.533936 0.613104
382.533936 0.613995
382.533936 0.614969
382.533936 0.615882
382.533936 0.616826
382.533936 0.617781
387.072083 0.617003
387.072083 0.618002
387.072083 0.618916
387.072083 0.619892
387.072083 0.620869
387.072083 0.621842
387.072083 0.622793
387.072083 0.623713
387.072083 0.624669
387.072083 0.625606
387.072083 0.626510
387.072083 0.627535
387.072083 0.628541
387.072083 0.629525
387.072083 0.630560
387.072083 0.631579
387.072083 0.632589
387.072083 0.633552
387.072083 0.634530
387.072083 0.635517
391.748871 0.628135
391.748871 0.629129
391.748871 0.630078
391.748871 0.631144
391.748871 0.632189
391.748871 0.633190
391.748871 0.634137
391.748871 0.635085
391.748871 0.636073
396.464294 0.631719
401.146667 0.631678
401.146667 0.632626
401.146667 0.633589
401.146667 0.634520
401.146667 0.635454
401.146667 0.636485
401.146667 0.637446
401.146667 0.638436
405.858398 0.637741
405.858398 0.638720
405.858398 0.639703
405.858398 0.640634
405.858398 0.641521
405.858398 0.642416
405.858398 0.643280
405.858398 0.644195
405.858398 0.645088
405.858398 0.646033
405.858398 0.647045
415.350891 0.631912
415.350891 0.632837
415.350891 0.633857
415.350891 0.634855
415.350891 0.635795
415.350891 0.636691
415.350891 0.637543
415.350891 0.638445
415.350891 0.639351
415.350891 0.640241
415.350891 0.641145
415.350891 0.642132
415.350891 0.643089
415.350891 0.644050
415.350891 0.645142
415.350891 0.646170
415.350891 0.647128
420.183411 0.636331
420.183411 0.637248
420.183411 0.638112
425.000000 0.632490
429.783539 0.625496
429.783539 0.626230
429.783539 0.626978
429.783539 0.627749
429.783539 0.628570
429.783539 0.629412
429.783539 0.630228
429.783539 0.631029
429.783539 0.631853
429.783539 0.632707
429.783539 0.633636
434.620697 0.632435
439.424896 0.624876
439.424896 0.625778
448.944672 0.612462
448.944672 0.613393
448.944672 0.614280
448.944672 0.615234
448.944672 0.616208
448.944672 0.617140
448.944672 0.618117
448.944672 0.619129
448.944672 0.620148
453.720337 0.616210
453.720337 0.617206
458.472565 0.616434
458.472565 0.617450
458.472565 0.618373
458.472565 0.619269
467.924683 0.614471
467.924683 0.615310
467.924683 0.616183
467.924683 0.617088
467.924683 0.617947
467.924683 0.618761
467.924683 0.619546
472.649994 0.609831
472.649994 0.610669
472.649994 0.611451
472.649994 0.612225
472.649994 0.613092
472.649994 0.613962
472.649994 0.614833
472.649994 0.615670
472.649994 0.616466
477.410797 0.610063
477.410797 0.610937
477.410797 0.611832
477.410797 0.612716
477.410797 0.613635
477.410797 0.614566
482.181824 0.612901
482.181824 0.613802
482.181824 0.614726
482.181824 0.615689
482.181824 0.616713
482.181824 0.617712
482.181824 0.618641
482.181824 0.619521
482.181824 0.620385
482.181824 0.621274
482.181824 0.622141
482.181824 0.623004
487.012360 0.613532
487.012360 0.614471
487.012360 0.615522
487.012360 0.616495
491.836060 0.613637
491.836060 0.614645
491.836060 0.615622
491.836060 0.616546
491.836060 0.617377
491.836060 0.618248
491.836060 0.619093
491.836060 0.619944
491.836060 0.620890
496.693878 0.621317
496.693878 0.622272
496.693878 0.623205
496.693878 0.624177
501.544708 0.614741
501.544708 0.615574
501.544708 0.616411
501.544708 0.617294
501.544708 0.618324
501.544708 0.619306
501.544708 0.620293
501.544708 0.621198
501.544708 0.622060
501.544708 0.622878
501.544708 0.623676
501.544708 0.624412
501.544708 0.625174
501.544708 0.625965
501.544708 0.626748
501.544708 0.627588
501.544708 0.628472
501.544708 0.629386
501.544708 0.630248
501.544708 0.631097
501.544708 0.631978
501.544708 0.632808
506.534424 0.625529
506.534424 0.626308
506.534424 0.627127
506.534424 0.627913
506.534424 0.628698
511.524200 0.628543
511.524200 0.629336
511.524200 0.630095
511.524200 0.630829
516.506042 0.624769
516.506042 0.625561
516.506042 0.626319
516.506042 0.627002
516.506042 0.627776
516.506042 0.628553
516.506042 0.629344
521.504028 0.626950
521.504028 0.627799
521.504028 0.628585
521.504028 0.629414
521.504028 0.630216
521.504028 0.630983
521.504028 0.631759
521.504028 0.632558
521.504028 0.633391
521.504028 0.634246
521.504028 0.635209
521.504028 0.636098
521.504028 0.636922
521.504028 0.637730
521.504028 0.638545
521.504028 0.639410
521.504028 0.640281
521.504028 0.641082
521.504028 0.641891
521.504028 0.642712
521.504028 0.643550
521.504028 0.644386
521.504028 0.645189
521.504028 0.646012
521.504028 0.646877
521.504028 0.647668
521.504028 0.648440
521.504028 0.649244
521.504028 0.649959
521.504028 0.650662
521.504028 0.651452
521.504028 0.652274
521.504028 0.653095
521.504028 0.653885
521.504028 0.654694
521.504028 0.655486
521.504028 0.656252
521.504028 0.657044
521.504028 0.657792
521.504028 0.658532
521.504028 0.659329
521.504028 0.660091
521.504028 0.660867
521.504028 0.661645
521.504028 0.662442
521.504028 0.663257
521.504028 0.664112
521.504028 0.664993
521.504028 0.665872
521.504028 0.666709
521.504028 0.667575
521.504028 0.668507
521.504028 0.669386
521.504028 0.670416
521.504028 0.671427
521.504028 0.672369
521.504028 0.673363
521.504028 0.674294
521.504028 0.675152
526.932251 0.674241
526.932251 0.675067
526.932251 0.675822
526.932251 0.676605
526.932251 0.677481
526.932251 0.678307
526.932251 0.679061
526.932251 0.679864
526.932251 0.680712
526.932251 0.681613
526.932251 0.682525
526.932251 0.683377
526.932251 0.684244
526.932251 0.685114
526.932251 0.685925
526.932251 0.686758
526.932251 0.687591
526.932251 0.688441
526.932251 0.689295
532.468262 0.683660
532.468262 0.684562
532.468262 0.685506
532.468262 0.686373
532.468262 0.687238
532.468262 0.688096
532.468262 0.688975
532.468262 0.689892
532.468262 0.690781
532.468262 0.691732
532.468262 0.692641
532.468262 0.693530
532.468262 0.694353
532.468262 0.695165
532.468262 0.696015
532.468262 0.696888
532.468262 0.697784
532.468262 0.698597
532.468262 0.699523
538.110657 0.681835
538.110657 0.682613
538.110657 0.683461
538.110657 0.684268
538.110657 0.685038
538.110657 0.685801
538.110657 0.686570
538.110657 0.687378
538.110657 0.688152
538.110657 0.688955
538.110657 0.689721
538.110657 0.690484
538.110657 0.691232
538.110657 0.691962
538.110657 0.692754
538.110657 0.693526
538.110657 0.694368
538.110657 0.695179
538.110657 0.695998
538.110657 0.696766
538.110657 0.697477
538.110657 0.698290
538.110657 0.699027
538.110657 0.699757
538.110657 0.700472
538.110657 0.701153
538.110657 0.701885
538.110657 0.702579
538.110657 0.703271
538.110657 0.704007
538.110657 0.704721
538.110657 0.705463
538.110657 0.706204
538.110657 0.706955
538.110657 0.707756
543.984253 0.699063
543.984253 0.699805
543.984253 0.700593
543.984253 0.701461
543.984253 0.702365
543.984253 0.703244
543.984253 0.704101
543.984253 0.704934
543.984253 0.705788
543.984253 0.706666
543.984253 0.707482
543.984253 0.708254
543.984253 0.709020
543.984253 0.709745
543.984253 0.710467
543.984253 0.711141
543.984253 0.711813
543.984253 0.712518
543.984253 0.713269
543.984253 0.714044
543.984253 0.714881
549.976440 0.710385
549.976440 0.711192
549.976440 0.711995
549.976440 0.712790
549.976440 0.713602
549.976440 0.714423
555.968750 0.710602
555.968750 0.711450
555.968750 0.712258
555.968750 0.713109
555.968750 0.713953
555.968750 0.714818
555.968750 0.715701
561.968872 0.715588
561.968872 0.716468
567.937988 0.703746
567.937988 0.704603
567.937988 0.705416
567.937988 0.706197
567.937988 0.706966
567.937988 0.707780
567.937988 0.708624
567.937988 0.709459
567.937988 0.710293
573.930481 0.710987
573.930481 0.711802
573.930481 0.712590
573.930481 0.713407
573.930481 0.714221
573.930481 0.715076
573.930481 0.715916
573.930481 0.716718
573.930481 0.717528
579.946167 0.711487
579.946167 0.712298
585.931030 0.710668
585.931030 0.711500
585.931030 0.712416
585.931030 0.713326
585.931030 0.714238
585.931030 0.715110
585.931030 0.715994
585.931030 0.716931
585.931030 0.717798
585.931030 0.718628
585.931030 0.719432
585.931030 0.720296
585.931030 0.721102
585.931030 0.721945
585.931030 0.722753
585.931030 0.723495
585.931030 0.724211
585.931030 0.724999
585.931030 0.725776
585.931030 0.726528
585.931030 0.727284
585.931030 0.727980
585.931030 0.728686
585.931030 0.729402
592.053406 0.713177
592.053406 0.713878
592.053406 0.714614
592.053406 0.715342
592.053406 0.716048
592.053406 0.716724
592.053406 0.717478
592.053406 0.718249
592.053406 0.718980
592.053406 0.719727
592.053406 0.720442
592.053406 0.721161
592.053406 0.721894
592.053406 0.722631
592.053406 0.723387
592.053406 0.724191
592.053406 0.724983
592.053406 0.725769
592.053406 0.726543
592.053406 0.727290
592.053406 0.728015
592.053406 0.728736
592.053406 0.729477
592.053406 0.730171
592.053406 0.730838
592.053406 0.731541
592.053406 0.732248
592.053406 0.733016
592.053406 0.733811
592.053406 0.734597
592.053406 0.735359
592.053406 0.736085
592.053406 0.736770
592.053406 0.737476
592.053406 0.738216
592.053406 0.738983
592.053406 0.739768
592.053406 0.740554
592.053406 0.741295
592.053406 0.742116
598.433472 0.714796
598.433472 0.715629
598.433472 0.716473
598.433472 0.717320
598.433472 0.718143
598.433472 0.718904
598.433472 0.719609
598.433472 0.720300
598.433472 0.721016
598.433472 0.721753
598.433472 0.722480
598.433472 0.723301
598.433472 0.724094
598.433472 0.724918
604.871216 0.725339
604.871216 0.726198
604.871216 0.727048
604.871216 0.727835
604.871216 0.728635
604.871216 0.729380
604.871216 0.730073
604.871216 0.730738
604.871216 0.731370
604.871216 0.731977
604.871216 0.732588
604.871216 0.733254
604.871216 0.733916
611.358521 0.733216
611.358521 0.733947
611.358521 0.734728
611.358521 0.735513
611.358521 0.736281
611.358521 0.737093
611.358521 0.737850
611.358521 0.738587
611.358521 0.739348
611.358521 0.740114
611.358521 0.740889
611.358521 0.741674
611.358521 0.742519
611.358521 0.743331
611.358521 0.744093
611.358521 0.744856
611.358521 0.745700
611.358521 0.746531
611.358521 0.747328
611.358521 0.748070
611.358521 0.748774
611.358521 0.749578
611.358521 0.750391
611.358521 0.751161
611.358521 0.751940
611.358521 0.752755
611.358521 0.753522
611.358521 0.754309
611.358521 0.755056
611.358521 0.755829
611.358521 0.756602
611.358521 0.757365
611.358521 0.758062
611.358521 0.758771
611.358521 0.759546
611.358521 0.760306
611.358521 0.761037
611.358521 0.761785
611.358521 0.762613
611.358521 0.763412
611.358521 0.764270
611.358521 0.765158
611.358521 0.766038
611.358521 0.766907
611.358521 0.767815
611.358521 0.768706
611.358521 0.769552
611.358521 0.770357
611.358521 0.771128
611.358521 0.771929
611.358521 0.772694
611.358521 0.773418
611.358521 0.774117
611.358521 0.774844
611.358521 0.775629
618.210510 0.772229
618.210510 0.773029
618.210510 0.773798
618.210510 0.774547
618.210510 0.775316
618.210510 0.776092
618.210510 0.776868
618.210510 0.777630
618.210510 0.778416
618.210510 0.779152
618.210510 0.779898
618.210510 0.780566
618.210510 0.781214
618.210510 0.781896
618.210510 0.782538
618.210510 0.783228
618.210510 0.783963
618.210510 0.784673
618.210510 0.785393
618.210510 0.786082
618.210510 0.786809
618.210510 0.787557
618.210510 0.788289
618.210510 0.789010
618.210510 0.789763
618.210510 0.790510
618.210510 0.791256
618.210510 0.792014
618.210510 0.792807
618.210510 0.793527
618.210510 0.794272
618.210510 0.794982
618.210510 0.795645
618.210510 0.796419
618.210510 0.797203
618.210510 0.797982
618.210510 0.798774
618.210510 0.799603
618.210510 0.800430
618.210510 0.801236
618.210510 0.802041
618.210510 0.802798
618.210510 0.803623
618.210510 0.804498
618.210510 0.805408
618.210510 0.806311
618.210510 0.807128
618.210510 0.807877
618.210510 0.808622
618.210510 0.809413
625.385742 0.804090
632.514954 0.795029
632.514954 0.795743
632.514954 0.796449
632.514954 0.797170
632.514954 0.797928
632.514954 0.798713
632.514954 0.799478
632.514954 0.800230
632.514954 0.801089
632.514954 0.802047
632.514954 0.802917
632.514954 0.803774
632.514954 0.804552
632.514954 0.805310
632.514954 0.806107
639.702576 0.790179
639.702576 0.790985
639.702576 0.791737
639.702576 0.792706
639.702576 0.793631
639.702576 0.794535
639.702576 0.795381
639.702576 0.796153
639.702576 0.796987
639.702576 0.797879
639.702576 0.798712
639.702576 0.799662
639.702576 0.800565
639.702576 0.801437
639.702576 0.802276
639.702576 0.803112
639.702576 0.803927
639.702576 0.804761
639.702576 0.805604
639.702576 0.806406
639.702576 0.807199
639.702576 0.807966
639.702576 0.808709
639.702576 0.809547
639.702576 0.810381
639.702576 0.811284
639.702576 0.812245
639.702576 0.813139
639.702576 0.813979
639.702576 0.814798
639.702576 0.815497
639.702576 0.816245
639.702576 0.816994
639.702576 0.817719
639.702576 0.818423
639.702576 0.819218
639.702576 0.820057
639.702576 0.820858
639.702576 0.821628
639.702576 0.822353
639.702576 0.823047
639.702576 0.823700
639.702576 0.824328
639.702576 0.824979
639.702576 0.825623
639.702576 0.826281
639.702576 0.827003
639.702576 0.827745
639.702576 0.828417
639.702576 0.829119
639.702576 0.829878
639.702576 0.830726
639.702576 0.831561
639.702576 0.832395
639.702576 0.833220
639.702576 0.834015
639.702576 0.834882
639.702576 0.835661
639.702576 0.836484
639.702576 0.837274
639.702576 0.838026
639.702576 0.838811
639.702576 0.839621
639.702576 0.840383
639.702576 0.841227
639.702576 0.842017
639.702576 0.842846
639.702576 0.843636
639.702576 0.844426
639.702576 0.845242
639.702576 0.846040
639.702576 0.846813
639.702576 0.847604
639.702576 0.848439
639.702576 0.849277
639.702576 0.850124
639.702576 0.850976
639.702576 0.851773
639.702576 0.852534
639.702576 0.853301
639.702576 0.854090
639.702576 0.854880
639.702576 0.855635
639.702576 0.856431
639.702576 0.857186
639.702576 0.858012
639.702576 0.858803
639.702576 0.859622
639.702576 0.860481
639.702576 0.861399
639.702576 0.862313
639.702576 0.863339
639.702576 0.864413
647.525940 0.856829
647.525940 0.857751
655.306274 0.859311
655.306274 0.860214
655.306274 0.861097
663.051453 0.856959
663.051453 0.857789
670.754578 0.853248
670.754578 0.854045
670.754578 0.854858
670.754578 0.855678
670.754578 0.856513
670.754578 0.857314
670.754578 0.858118
670.754578 0.858966
670.754578 0.859859
670.754578 0.860826
670.754578 0.861737
670.754578 0.862588
670.754578 0.863394
670.754578 0.864230
670.754578 0.865114
670.754578 0.866001
670.754578 0.866874
670.754578 0.867674
670.754578 0.868436
670.754578 0.869178
670.754578 0.869921
670.754578 0.870704
670.754578 0.871489
670.754578 0.872287
670.754578 0.873074
670.754578 0.873804
670.754578 0.874594
670.754578 0.875425
670.754578 0.876221
670.754578 0.877049
670.754578 0.877831
670.754578 0.878632
670.754578 0.879436
670.754578 0.880171
670.754578 0.880902
670.754578 0.881598
670.754578 0.882301
670.754578 0.882995
670.754578 0.883721
670.754578 0.884421
670.754578 0.885105
670.754578 0.885766
670.754578 0.886473
670.754578 0.887184
670.754578 0.887866
670.754578 0.888562
670.754578 0.889311
670.754578 0.890059
670.754578 0.890844
670.754578 0.891618
670.754578 0.892408
670.754578 0.893184
670.754578 0.893905
670.754578 0.894692
670.754578 0.895514
670.754578 0.896296
670.754578 0.897082
670.754578 0.897919
670.754578 0.898788
670.754578 0.899629
670.754578 0.900455
670.754578 0.901281
670.754578 0.902090
678.861328 0.892483
678.861328 0.893227
678.861328 0.893986
678.861328 0.894696
678.861328 0.895360
686.945435 0.888500
686.945435 0.889185
686.945435 0.889886
686.945435 0.890608
686.945435 0.891293
686.945435 0.892004
686.945435 0.892796
695.021729 0.886350
695.021729 0.887136
695.021729 0.887899
695.021729 0.888616
703.068604 0.887437
711.064758 0.870838
711.064758 0.871532
711.064758 0.872193
711.064758 0.872810
711.064758 0.873467
711.064758 0.874120
711.064758 0.874844
711.064758 0.875621
711.064758 0.876384
711.064758 0.877131
711.064758 0.877839
711.064758 0.878548
711.064758 0.879246
711.064758 0.879968
719.103943 0.880583
719.103943 0.881288
719.103943 0.882002
719.103943 0.882692
719.103943 0.883376
719.103943 0.884081
719.103943 0.884842
719.103943 0.885600
719.103943 0.886321
719.103943 0.887084
719.103943 0.887893
719.103943 0.888735
719.103943 0.889606
719.103943 0.890435
719.103943 0.891274
719.103943 0.892159
719.103943 0.892983
719.103943 0.893757
719.103943 0.894572
719.103943 0.895351
719.103943 0.896079
719.103943 0.896807
719.103943 0.897549
719.103943 0.898247
719.103943 0.898961
719.103943 0.899673
719.103943 0.900364
719.103943 0.901106
719.103943 0.901880
719.103943 0.902639
719.103943 0.903345
719.103943 0.903982
719.103943 0.904619
719.103943 0.905273
719.103943 0.905981
727.335693 0.889204
727.335693 0.889891
727.335693 0.890639
727.335693 0.891439
727.335693 0.892255
727.335693 0.893024
727.335693 0.893841
727.335693 0.894638
727.335693 0.895484
727.335693 0.896291
727.335693 0.897102
727.335693 0.897924
727.335693 0.898683
735.601440 0.892074
735.601440 0.892736
735.601440 0.893363
735.601440 0.894013
735.601440 0.894624
735.601440 0.895240
735.601440 0.895959
735.601440 0.896671
735.601440 0.897449
735.601440 0.898292
735.601440 0.899123
735.601440 0.899909
735.601440 0.900616
735.601440 0.901350
735.601440 0.902038
735.601440 0.902691
735.601440 0.903381
735.601440 0.904078
735.601440 0.904807
735.601440 0.905564
735.601440 0.906284
735.601440 0.906979
735.601440 0.907701
735.601440 0.908435
735.601440 0.909257
735.601440 0.910071
735.601440 0.910880
735.601440 0.911639
735.601440 0.912341
735.601440 0.913103
744.021301 0.902339
744.021301 0.903086
744.021301 0.903769
744.021301 0.904445
744.021301 0.905172
744.021301 0.905855
744.021301 0.906578
744.021301 0.907410
744.021301 0.908219
744.021301 0.908968
744.021301 0.909708
744.021301 0.910421
744.021301 0.911254
744.021301 0.912065
744.021301 0.912845
744.021301 0.913627
744.021301 0.914342
744.021301 0.915071
744.021301 0.915832
744.021301 0.916529
744.021301 0.917252
744.021301 0.917968
744.021301 0.918704
752.544189 0.908579
752.544189 0.909366
752.544189 0.910142
752.544189 0.910928
752.544189 0.911714
752.544189 0.912416
752.544189 0.913119
752.544189 0.913891
752.544189 0.914695
752.544189 0.915492
752.544189 0.916230
752.544189 0.916948
752.544189 0.917714
752.544189 0.918405
752.544189 0.919071
752.544189 0.919861
752.544189 0.920635
752.544189 0.921404
752.544189 0.922114
752.544189 0.922819
752.544189 0.923538
752.544189 0.924213
752.544189 0.924861
752.544189 0.925499
752.544189 0.926164
752.544189 0.926827
752.544189 0.927489
761.197205 0.925531
769.796509 0.911204
769.796509 0.911874
769.796509 0.912539
769.796509 0.913297
769.796509 0.914063
769.796509 0.914904
769.796509 0.915773
769.796509 0.916592
769.796509 0.917378
769.796509 0.918140
769.796509 0.918832
769.796509 0.919524
769.796509 0.920257
769.796509 0.920969
778.433594 0.905744
778.433594 0.906428
787.024414 0.890804
787.024414 0.891471
787.024414 0.892129
787.024414 0.892786
787.024414 0.893484
787.024414 0.894181
787.024414 0.894993
787.024414 0.895774
787.024414 0.896504
787.024414 0.897263
787.024414 0.898049
787.024414 0.898818
787.024414 0.899660
787.024414 0.900446
787.024414 0.901203
787.024414 0.901892
787.024414 0.902601
787.024414 0.903324
787.024414 0.903965
787.024414 0.904615
787.024414 0.905316
787.024414 0.906002
787.024414 0.906609
787.024414 0.907211
787.024414 0.907884
787.024414 0.908550
787.024414 0.909214
787.024414 0.909848
795.750000 0.885879
795.750000 0.886598
795.750000 0.887379
804.435974 0.882782
804.435974 0.883557
804.435974 0.884271
804.435974 0.884973
804.435974 0.885727
804.435974 0.886542
804.435974 0.887345
804.435974 0.888114
804.435974 0.888822
804.435974 0.889512
804.435974 0.890219
804.435974 0.890944
804.435974 0.891658
813.151733 0.885966
813.151733 0.886696
813.151733 0.887373
813.151733 0.888014
813.151733 0.888707
813.151733 0.889410
813.151733 0.890091
813.151733 0.890782
813.151733 0.891516
813.151733 0.892207
813.151733 0.892872
813.151733 0.893566
813.151733 0.894220
813.151733 0.894966
813.151733 0.895713
813.151733 0.896452
813.151733 0.897264
813.151733 0.898097
813.151733 0.898907
813.151733 0.899706
813.151733 0.900504
813.151733 0.901345
813.151733 0.902171
813.151733 0.902936
813.151733 0.903696
813.151733 0.904423
813.151733 0.905092
813.151733 0.905737
813.151733 0.906389
813.151733 0.907031
813.151733 0.907701
813.151733 0.908369
813.151733 0.909052
813.151733 0.909739
813.151733 0.910445
813.151733 0.911164
813.151733 0.911925
813.151733 0.912620
822.068726 0.877855
822.068726 0.878577
822.068726 0.879283
822.068726 0.879972
822.068726 0.880633
822.068726 0.881300
822.068726 0.881942
822.068726 0.882546
822.068726 0.883140
822.068726 0.883768
822.068726 0.884412
822.068726 0.885043
822.068726 0.885673
822.068726 0.886285
822.068726 0.886856
822.068726 0.887451
822.068726 0.888109
822.068726 0.888727
822.068726 0.889365
822.068726 0.889991
822.068726 0.890589
822.068726 0.891203
822.068726 0.891851
822.068726 0.892504
822.068726 0.893147
822.068726 0.893897
822.068726 0.894558
822.068726 0.895194
822.068726 0.895876
822.068726 0.896587
822.068726 0.897263
822.068726 0.897966
831.143860 0.880796
831.143860 0.881466
831.143860 0.882149
831.143860 0.882836
831.143860 0.883528
831.143860 0.884171
831.143860 0.884761
831.143860 0.885354
831.143860 0.885917
831.143860 0.886473
831.143860 0.887050
831.143860 0.887687
831.143860 0.888383
831.143860 0.889008
831.143860 0.889591
831.143860 0.890297
831.143860 0.891004
831.143860 0.891743
831.143860 0.892472
831.143860 0.893256
831.143860 0.893994
831.143860 0.894724
831.143860 0.895432
831.143860 0.896085
831.143860 0.896858
831.143860 0.897574
831.143860 0.898277
831.143860 0.899021
831.143860 0.899763
831.143860 0.900508
831.143860 0.901269
831.143860 0.902003
831.143860 0.902712
831.143860 0.903427
831.143860 0.904130
831.143860 0.904798
831.143860 0.905426
831.143860 0.906104
831.143860 0.906752
831.143860 0.907377
831.143860 0.908057
840.436890 0.908458
840.436890 0.909125
840.436890 0.909787
840.436890 0.910433
840.436890 0.911081
840.436890 0.911767
840.436890 0.912468
840.436890 0.913159
840.436890 0.913858
840.436890 0.914479
840.436890 0.915052
840.436890 0.915654
840.436890 0.916207
840.436890 0.916728
840.436890 0.917275
840.436890 0.917886
840.436890 0.918464
849.782288 0.913611
849.782288 0.914231
849.782288 0.914853
849.782288 0.915527
859.091553 0.909431
859.091553 0.910019
859.091553 0.910641
859.091553 0.911232
859.091553 0.911813
859.091553 0.912377
859.091553 0.912955
859.091553 0.913586
859.091553 0.914242
859.091553 0.914905
859.091553 0.915518
859.091553 0.916123
859.091553 0.916709
859.091553 0.917349
859.091553 0.918044
859.091553 0.918796
859.091553 0.919527
859.091553 0.920287
859.091553 0.920997
859.091553 0.921650
859.091553 0.922332
859.091553 0.922981
859.091553 0.923665
859.091553 0.924283
859.091553 0.924948
859.091553 0.925610
859.091553 0.926288
859.091553 0.926942
859.091553 0.927599
859.091553 0.928226
859.091553 0.928861
859.091553 0.929492
859.091553 0.930236
859.091553 0.930952
859.091553 0.931696
868.574341 0.924567
868.574341 0.925240
868.574341 0.925939
868.574341 0.926600
868.574341 0.927219
868.574341 0.927813
868.574341 0.928450
868.574341 0.929207
868.574341 0.929935
868.574341 0.930632
868.574341 0.931260
868.574341 0.931914
868.574341 0.932543
878.080811 0.919396
878.080811 0.920080
878.080811 0.920723
878.080811 0.921307
878.080811 0.921932
878.080811 0.922522
878.080811 0.923139
878.080811 0.923750
878.080811 0.924340
878.080811 0.924931
878.080811 0.925473
878.080811 0.926015
878.080811 0.926558
878.080811 0.927131
878.080811 0.927701
878.080811 0.928242
878.080811 0.928787
878.080811 0.929402
878.080811 0.930024
878.080811 0.930679
878.080811 0.931365
887.664429 0.915571
887.664429 0.916195
887.664429 0.916853
887.664429 0.917527
887.664429 0.918272
887.664429 0.918980
887.664429 0.919618
887.664429 0.920260
887.664429 0.920898
887.664429 0.921518
887.664429 0.922226
887.664429 0.922937
887.664429 0.923600
887.664429 0.924287
887.664429 0.925085
887.664429 0.925809
887.664429 0.926557
887.664429 0.927319
887.664429 0.928059
887.664429 0.928762
887.664429 0.929434
887.664429 0.930142
887.664429 0.930821
887.664429 0.931473
887.664429 0.932098
887.664429 0.932705
887.664429 0.933296
887.664429 0.933886
887.664429 0.934456
887.664429 0.935039
887.664429 0.935601
887.664429 0.936164
897.398010 0.900582
897.398010 0.901117
897.398010 0.901627
897.398010 0.902160
897.398010 0.902696
897.398010 0.903191
897.398010 0.903684
897.398010 0.904214
897.398010 0.904729
897.398010 0.905215
897.398010 0.905702
897.398010 0.906277
897.398010 0.906897
897.398010 0.907515
897.398010 0.908073
897.398010 0.908604
897.398010 0.909191
897.398010 0.909730
897.398010 0.910240
897.398010 0.910745
897.398010 0.911270
897.398010 0.911770
897.398010 0.912366
897.398010 0.912918
897.398010 0.913542
897.398010 0.914160
897.398010 0.914770
897.398010 0.915436
897.398010 0.916091
897.398010 0.916770
897.398010 0.917487
897.398010 0.918220
897.398010 0.918907
917.109619 0.906857
917.109619 0.907476
917.109619 0.908101
917.109619 0.908732
926.894043 0.910784
926.894043 0.911463
926.894043 0.912105
926.894043 0.912781
926.894043 0.913449
926.894043 0.914085
926.894043 0.914659
926.894043 0.915273
926.894043 0.915898
926.894043 0.916537
926.894043 0.917224
926.894043 0.917913
926.894043 0.918608
926.894043 0.919384
926.894043 0.920129
926.894043 0.920861
926.894043 0.921589
926.894043 0.922368
926.894043 0.923102
926.894043 0.923740
926.894043 0.924364
926.894043 0.924945
926.894043 0.925497
926.894043 0.926023
926.894043 0.926543
926.894043 0.927039
926.894043 0.927521
926.894043 0.928023
926.894043 0.928624
926.894043 0.929215
926.894043 0.929816
926.894043 0.930398
926.894043 0.930970
926.894043 0.931553
926.894043 0.932187
926.894043 0.932787
926.894043 0.933425
926.894043 0.934070
926.894043 0.934686
926.894043 0.935399
926.894043 0.936067
926.894043 0.936729
926.894043 0.937402
926.894043 0.938138
926.894043 0.938844
926.894043 0.939576
926.894043 0.940273
926.894043 0.940922
926.894043 0.941573
926.894043 0.942211
926.894043 0.942816
926.894043 0.943432
926.894043 0.944050
926.894043 0.944607
926.894043 0.945161
926.894043 0.945650
926.894043 0.946155
926.894043 0.946772
926.894043 0.947338
926.894043 0.947900
926.894043 0.948440
926.894043 0.948949
926.894043 0.949525
926.894043 0.950155
926.894043 0.950810
926.894043 0.951441
926.894043 0.952064
926.894043 0.952647
926.894043 0.953250
926.894043 0.953828
926.894043 0.954419
926.894043 0.954998
926.894043 0.955616
926.894043 0.956212
926.894043 0.956846
926.894043 0.957544
926.894043 0.958342
926.894043 0.959091
926.894043 0.959853
926.894043 0.960667
926.894043 0.961448
926.894043 0.962189
926.894043 0.962907
926.894043 0.963616
926.894043 0.964286
926.894043 0.964930
926.894043 0.965554
926.894043 0.966154
926.894043 0.966684
926.894043 0.967291
926.894043 0.967876
926.894043 0.968492
926.894043 0.969191
926.894043 0.969872
926.894043 0.970610
926.894043 0.971265
926.894043 0.971875
926.894043 0.972591
926.894043 0.973323
926.894043 0.974015
926.894043 0.974698
926.894043 0.975376
926.894043 0.976058
926.894043 0.976747
926.894043 0.977431
926.894043 0.978126
926.894043 0.978804
926.894043 0.979476
926.894043 0.980211
926.894043 0.980938
937.339905 0.976664
937.339905 0.977326
937.339905 0.977977
937.339905 0.978601
937.339905 0.979187
937.339905 0.979778
937.339905 0.980374
937.339905 0.980908
937.339905 0.981426
937.339905 0.981953
937.339905 0.982526
947.789490 0.961405
947.789490 0.961885
947.789490 0.962407
947.789490 0.963038
947.789490 0.963646
947.789490 0.964196
947.789490 0.964711
958.216370 0.953218
958.216370 0.953689
958.216370 0.954162
958.216370 0.954644
958.216370 0.955214
958.216370 0.955799
958.216370 0.956402
958.216370 0.956964
958.216370 0.957521
958.216370 0.958071
958.216370 0.958599
958.216370 0.959141
958.216370 0.959709
958.216370 0.960276
958.216370 0.960889
958.216370 0.961496
958.216370 0.962115
958.216370 0.962723
958.216370 0.963302
958.216370 0.963888
958.216370 0.964488
958.216370 0.965162
958.216370 0.965852
958.216370 0.966531
958.216370 0.967266
958.216370 0.967971
958.216370 0.968642
958.216370 0.969277
958.216370 0.969871
958.216370 0.970512
958.216370 0.971122
958.216370 0.971722
958.216370 0.972329
958.216370 0.972913
958.216370 0.973479
958.216370 0.974080
958.216370 0.974650
958.216370 0.975185
958.216370 0.975699
958.216370 0.976227
958.216370 0.976741
958.216370 0.977385
958.216370 0.978010
958.216370 0.978621
958.216370 0.979221
958.216370 0.979822
958.216370 0.980401
958.216370 0.980947
958.216370 0.981469
968.895447 0.971431
968.895447 0.971949
968.895447 0.972507
979.524414 0.962175
979.524414 0.962731
979.524414 0.963316
979.524414 0.963913
979.524414 0.964478
979.524414 0.965046
979.524414 0.965603
979.524414 0.966181
979.524414 0.966744
979.524414 0.967287
979.524414 0.967835
979.524414 0.968390
979.524414 0.968945
979.524414 0.969553
979.524414 0.970166
979.524414 0.970793
979.524414 0.971372
979.524414 0.971929
979.524414 0.972469
979.524414 0.973031
979.524414 0.973604
979.524414 0.974230
979.524414 0.974836
979.524414 0.975417
979.524414 0.976018
979.524414 0.976586
979.524414 0.977201
979.524414 0.977822
979.524414 0.978437
979.524414 0.979013
979.524414 0.979585
979.524414 0.980185
979.524414 0.980756
979.524414 0.981333
979.524414 0.981908
979.524414 0.982519
979.524414 0.983106
979.524414 0.983687
979.524414 0.984277
979.524414 0.984862
979.524414 0.985418
979.524414 0.985940
979.524414 0.986409
979.524414 0.986899
979.524414 0.987455
979.524414 0.987989
979.524414 0.988475
979.524414 0.988974
979.524414 0.989471
979.524414 0.990007
979.524414 0.990498
979.524414 0.990976
979.524414 0.991432
979.524414 0.991889
979.524414 0.992382
979.524414 0.992868
979.524414 0.993391
979.524414 0.993887
979.524414 0.994375
990.467529 0.994112
990.467529 0.994630
990.467529 0.995195
990.467529 0.995746
990.467529 0.996304
990.467529 0.996871
990.467529 0.997457
990.467529 0.998014
990.467529 0.998610
990.467529 0.999192
990.467529 0.999772
990.467529 1.000347
990.467529 1.000900
990.467529 1.001488
990.467529 1.002088
990.467529 1.002700
1001.443359 0.966170
1001.443359 0.966709
1001.443359 0.967262
1012.367737 0.959463
1023.228271 0.959836
1023.228271 0.960405
1023.228271 0.960944
1023.228271 0.961516
1023.228271 0.962068
1023.228271 0.962609
1023.228271 0.963160
1023.228271 0.963677
1023.228271 0.964171
1023.228271 0.964707
1023.228271 0.965274
1023.228271 0.965834
1023.228271 0.966356
1023.228271 0.966857
1023.228271 0.967451
1023.228271 0.968019
1023.228271 0.968579
1023.228271 0.969146
1023.228271 0.969696
1023.228271 0.970241
1023.228271 0.970752
1023.228271 0.971260
1023.228271 0.971777
1023.228271 0.972276
1023.228271 0.972829
1023.228271 0.973339
1023.228271 0.973821
1023.228271 0.974313
1023.228271 0.974850
1023.228271 0.975403
1023.228271 0.975982
1023.228271 0.976587
1034.224365 0.942860
1034.224365 0.943400
1034.224365 0.943934
1034.224365 0.944457
1034.224365 0.944929
1034.224365 0.945431
1034.224365 0.945948
1034.224365 0.946466
1034.224365 0.946964
1034.224365 0.947425
1034.224365 0.947868
1034.224365 0.948375
1034.224365 0.948909
1034.224365 0.949404
1034.224365 0.949947
1034.224365 0.950475
1034.224365 0.950980
1034.224365 0.951553
1034.224365 0.952111
1034.224365 0.952643
1034.224365 0.953176
1034.224365 0.953690
1034.224365 0.954278
1034.224365 0.954854
1034.224365 0.955435
1034.224365 0.956019
1034.224365 0.956556
1034.224365 0.957101
1034.224365 0.957637
1034.224365 0.958168
1034.224365 0.958715
1034.224365 0.959249
1034.224365 0.959720
1034.224365 0.960185
1034.224365 0.960701
1034.224365 0.961263
1034.224365 0.961802
1034.224365 0.962378
1034.224365 0.962947
1034.224365 0.963511
1034.224365 0.964055
1034.224365 0.964602
1034.224365 0.965109
1034.224365 0.965621
1034.224365 0.966142
1034.224365 0.966652
1034.224365 0.967164
1034.224365 0.967666
1034.224365 0.968141
1034.224365 0.968702
1034.224365 0.969234
1034.224365 0.969803
1034.224365 0.970339
1034.224365 0.970876
1034.224365 0.971409
1034.224365 0.971942
1034.224365 0.972467
1034.224365 0.973003
1034.224365 0.973545
1034.224365 0.974071
1034.224365 0.974577
1034.224365 0.975091
1034.224365 0.975623
1034.224365 0.976132
1034.224365 0.976677
1034.224365 0.977211
1034.224365 0.977765
1034.224365 0.978304
1034.224365 0.978804
1034.224365 0.979339
1034.224365 0.979875
1034.224365 0.980413
1034.224365 0.980990
1034.224365 0.981583
1034.224365 0.982189
1034.224365 0.982782
1034.224365 0.983370
1034.224365 0.983963
1034.224365 0.984519
1034.224365 0.985120
1034.224365 0.985694
1034.224365 0.986256
1034.224365 0.986806
1034.224365 0.987375
1034.224365 0.987923
1034.224365 0.988482
1034.224365 0.989002
1034.224365 0.989517
1034.224365 0.990055
1034.224365 0.990613
1034.224365 0.991150
1034.224365 0.991680
1034.224365 0.992189
1034.224365 0.992703
1034.224365 0.993186
1045.757202 0.994624
1045.757202 0.995072
1045.757202 0.995550
1045.757202 0.996072
1045.757202 0.996621
1045.757202 0.997116
1045.757202 0.997638
1045.757202 0.998214
1045.757202 0.998763
1045.757202 0.999291
1045.757202 0.999794
1045.757202 1.000263
1045.757202 1.000745
1045.757202 1.001302
1045.757202 1.001903
1057.312134 0.997572
1057.312134 0.998148
1057.312134 0.998688
1057.312134 0.999248
1057.312134 0.999819
1057.312134 1.000399
1057.312134 1.000972
1057.312134 1.001522
1057.312134 1.002151
1057.312134 1.002733
1057.312134 1.003274
1057.312134 1.003770
1057.312134 1.004275
1057.312134 1.004802
1057.312134 1.005323
1057.312134 1.005871
1057.312134 1.006430
1057.312134 1.006998
1057.312134 1.007504
1057.312134 1.007985
1057.312134 1.008478
1057.312134 1.008939
1057.312134 1.009337
1057.312134 1.009778
1057.312134 1.010240
1057.312134 1.010729
1057.312134 1.011209
1057.312134 1.011746
1057.312134 1.012306
1057.312134 1.012876
1057.312134 1.013452
1057.312134 1.014008
1057.312134 1.014534
1057.312134 1.015067
1057.312134 1.015598
1057.312134 1.016134
1057.312134 1.016640
1057.312134 1.017184
1057.312134 1.017752
1057.312134 1.018399
1057.312134 1.019022
1057.312134 1.019596
1057.312134 1.020087
1057.312134 1.020536
1057.312134 1.020978
1057.312134 1.021511
1069.085693 1.024303
1069.085693 1.024861
1069.085693 1.025458
1069.085693 1.026007
1069.085693 1.026564
1069.085693 1.027179
1069.085693 1.027732
1069.085693 1.028227
1069.085693 1.028759
1069.085693 1.029250
1069.085693 1.029722
1069.085693 1.030240
1069.085693 1.030735
1069.085693 1.031241
1069.085693 1.031761
1069.085693 1.032264
1069.085693 1.032836
1069.085693 1.033407
1069.085693 1.033968
1069.085693 1.034535
1069.085693 1.035116
1069.085693 1.035684
1069.085693 1.036242
1069.085693 1.036774
1069.085693 1.037333
1069.085693 1.037900
1069.085693 1.038462
1069.085693 1.038997
1069.085693 1.039481
1069.085693 1.039964
1069.085693 1.040448
1069.085693 1.040931
1069.085693 1.041456
1069.085693 1.041927
1069.085693 1.042410
1069.085693 1.042951
1069.085693 1.043474
1069.085693 1.043992
1069.085693 1.044478
1069.085693 1.044954
1069.085693 1.045435
1069.085693 1.045949
1069.085693 1.046440
1069.085693 1.046889
1069.085693 1.047330
1069.085693 1.047752
1069.085693 1.048195
1069.085693 1.048679
1069.085693 1.049198
1069.085693 1.049748
1069.085693 1.050283
1069.085693 1.050798
1081.113892 1.034427
1081.113892 1.034961
1081.113892 1.035476
1081.113892 1.036002
1081.113892 1.036590
1081.113892 1.037146
1081.113892 1.037694
1081.113892 1.038258
1081.113892 1.038832
1081.113892 1.039387
1081.113892 1.040000
1081.113892 1.040618
1081.113892 1.041205
1081.113892 1.041826
1081.113892 1.042421
1081.113892 1.042961
1081.113892 1.043528
1081.113892 1.044078
1081.113892 1.044593
1081.113892 1.045135
1081.113892 1.045655
1081.113892 1.046146
1081.113892 1.046647
1081.113892 1.047146
1081.113892 1.047653
1081.113892 1.048183
1081.113892 1.048745
1081.113892 1.049327
1081.113892 1.049862
1081.113892 1.050341
1081.113892 1.050817
1081.113892 1.051291
1081.113892 1.051766
1081.113892 1.052266
1081.113892 1.052753
1081.113892 1.053243
1081.113892 1.053774
1081.113892 1.054312
1081.113892 1.054855
1081.113892 1.055355
1081.113892 1.055822
1081.113892 1.056317
1081.113892 1.056852
1081.113892 1.057371
1081.113892 1.057881
1081.113892 1.058371
1081.113892 1.058907
1081.113892 1.059415
1081.113892 1.059938
1081.113892 1.060439
1081.113892 1.060988
1081.113892 1.061502
1081.113892 1.062016
1081.113892 1.062551
1081.113892 1.063121
1081.113892 1.063695
1081.113892 1.064263
1081.113892 1.064845
1081.113892 1.065447
1093.438477 1.035197
1093.438477 1.035732
1093.438477 1.036287
1093.438477 1.036828
1105.710693 1.020324
1105.710693 1.020796
1105.710693 1.021264
1105.710693 1.021705
1105.710693 1.022188
1105.710693 1.022645
1105.710693 1.023104
1105.710693 1.023575
1105.710693 1.024084
1105.710693 1.024566
1105.710693 1.025013
1105.710693 1.025434
1105.710693 1.025864
1105.710693 1.026307
1105.710693 1.026757
1105.710693 1.027211
1105.710693 1.027675
1105.710693 1.028123
1105.710693 1.028566
1105.710693 1.029044
1105.710693 1.029529
1105.710693 1.030060
1105.710693 1.030564
1105.710693 1.031097
1105.710693 1.031597
1105.710693 1.032054
1105.710693 1.032562
1105.710693 1.033057
1105.710693 1.033562
1105.710693 1.034070
1105.710693 1.034540
1105.710693 1.034987
1105.710693 1.035497
1105.710693 1.036021
1105.710693 1.036572
1105.710693 1.037109
1105.710693 1.037620
1105.710693 1.038141
1105.710693 1.038656
1105.710693 1.039157
1105.710693 1.039641
1105.710693 1.040145
1105.710693 1.040633
1105.710693 1.041115
1105.710693 1.041594
1105.710693 1.042056
1105.710693 1.042497
1105.710693 1.042934
1105.710693 1.043377
1105.710693 1.043856
1105.710693 1.044320
1105.710693 1.044784
1105.710693 1.045260
1105.710693 1.045721
1105.710693 1.046198
1105.710693 1.046673
1118.257080 1.044819
1118.257080 1.045302
1118.257080 1.045780
1118.257080 1.046281
1118.257080 1.046815
1118.257080 1.047302
1118.257080 1.047787
1118.257080 1.048275
1118.257080 1.048741
1118.257080 1.049228
1118.257080 1.049753
1118.257080 1.050300
1130.800049 1.034758
1130.800049 1.035285
1130.800049 1.035807
1130.800049 1.036342
1130.800049 1.036858
1130.800049 1.037361
1130.800049 1.037880
1130.800049 1.038402
1143.314697 1.014806
1143.314697 1.015285
1143.314697 1.015810
1143.314697 1.016338
1143.314697 1.016875
1143.314697 1.017386
1143.314697 1.017907
1143.314697 1.018439
1143.314697 1.018942
1143.314697 1.019464
1143.314697 1.019970
1143.314697 1.020539
1143.314697 1.021081
1143.314697 1.021622
1143.314697 1.022114
1143.314697 1.022606
1155.850952 1.010931
1155.850952 1.011407
1155.850952 1.011888
1155.850952 1.012384
1155.850952 1.012890
1155.850952 1.013374
1155.850952 1.013883
1155.850952 1.014366
1155.850952 1.014842
1168.365356 0.996129
1168.365356 0.996609
1168.365356 0.997095
1168.365356 0.997565
1168.365356 0.998013
1168.365356 0.998449
1168.365356 0.998911
1168.365356 0.999393
1168.365356 0.999860
1168.365356 1.000329
1168.365356 1.000874
1168.365356 1.001369
1168.365356 1.001851
1168.365356 1.002297
1168.365356 1.002751
1168.365356 1.003150
1168.365356 1.003550
1168.365356 1.003922
1168.365356 1.004284
1168.365356 1.004699
1168.365356 1.005200
1180.932129 1.006147
1180.932129 1.006608
1180.932129 1.007083
1180.932129 1.007564
1180.932129 1.008015
1180.932129 1.008502
1180.932129 1.008993
1180.932129 1.009494
1180.932129 1.010033
1180.932129 1.010518
1180.932129 1.011011
1180.932129 1.011568
1180.932129 1.012108
1180.932129 1.012610
1180.932129 1.013092
1180.932129 1.013556
1180.932129 1.013998
1193.526123 1.003123
1193.526123 1.003580
1193.526123 1.004036
1193.526123 1.004523
1193.526123 1.004979
1193.526123 1.005405
1193.526123 1.005873
1193.526123 1.006335
1193.526123 1.006762
1193.526123 1.007212
1193.526123 1.007714
1193.526123 1.008251
1206.116577 0.980796
1206.116577 0.981290
1206.116577 0.981748
1206.116577 0.982165
1206.116577 0.982583
1206.116577 0.983011
1206.116577 0.983448
1206.116577 0.983840
1206.116577 0.984266
1206.116577 0.984683
1206.116577 0.985087
1206.116577 0.985457
1206.116577 0.985851
1206.116577 0.986251
1206.116577 0.986641
1206.116577 0.987073
1206.116577 0.987457
1206.116577 0.987852
1206.116577 0.988258
1206.116577 0.988659
1206.116577 0.989117
1206.116577 0.989540
1206.116577 0.989979
1206.116577 0.990390
1206.116577 0.990777
1206.116577 0.991148
1206.116577 0.991523
1206.116577 0.991933
1206.116577 0.992336
1206.116577 0.992752
1206.116577 0.993166
1206.116577 0.993586
1206.116577 0.993999
1206.116577 0.994419
1206.116577 0.994936
1206.116577 0.995457
1206.116577 0.995959
1206.116577 0.996442
1206.116577 0.996890
1206.116577 0.997341
1206.116577 0.997772
1206.116577 0.998221
1206.116577 0.998633
1206.116577 0.999021
1206.116577 0.999416
1206.116577 0.999866
1206.116577 1.000287
1206.116577 1.000718
1206.116577 1.001179
1206.116577 1.001663
1206.116577 1.002128
1206.116577 1.002666
1206.116577 1.003265
1206.116577 1.003817
1206.116577 1.004359
1206.116577 1.004943
1206.116577 1.005453
1206.116577 1.005929
1206.116577 1.006361
1206.116577 1.006812
1206.116577 1.007271
1206.116577 1.007726
1206.116577 1.008130
1206.116577 1.008511
1206.116577 1.008958
1206.116577 1.009404
1206.116577 1.009795
1206.116577 1.010209
1206.116577 1.010628
1206.116577 1.011020
1206.116577 1.011464
1206.116577 1.011977
1206.116577 1.012462
1206.116577 1.012902
1206.116577 1.013360
1206.116577 1.013841
1206.116577 1.014305
1206.116577 1.014830
1206.116577 1.015355
1206.116577 1.015838
1206.116577 1.016337
1206.116577 1.016901
1206.116577 1.017440
1206.116577 1.017910
1206.116577 1.018346
1206.116577 1.018782
1206.116577 1.019287
1206.116577 1.019811
1206.116577 1.020294
1206.116577 1.020727
1206.116577 1.021175
1206.116577 1.021563
1206.116577 1.021966
1206.116577 1.022384
1206.116577 1.022784
1206.116577 1.023216
1206.116577 1.023618
1206.116577 1.024027
1206.116577 1.024436
1206.116577 1.024835
1206.116577 1.025248
1206.116577 1.025649
1206.116577 1.026076
1206.116577 1.026533
1206.116577 1.026974
1206.116577 1.027411
1206.116577 1.027923
1206.116577 1.028414
1206.116577 1.028919
1206.116577 1.029404
1206.116577 1.029891
1206.116577 1.030359
1206.116577 1.030801
1206.116577 1.031231
1206.116577 1.031659
1206.116577 1.032058
1206.116577 1.032499
1206.116577 1.032947
1206.116577 1.033380
1206.116577 1.033799
1206.116577 1.034236
1206.116577 1.034744
1206.116577 1.035195
1206.116577 1.035681
1206.116577 1.036157
1206.116577 1.036648
1232.603638 1.017879
1232.603638 1.018338
1232.603638 1.018775
1232.603638 1.019227
1232.603638 1.019666
1232.603638 1.020079
1232.603638 1.020468
1232.603638 1.020842
1232.603638 1.021224
1232.603638 1.021701
1232.603638 1.022253
1232.603638 1.022755
1232.603638 1.023256
1232.603638 1.023727
1245.811523 1.010106
1245.811523 1.010514
1245.811523 1.010899
1245.811523 1.011309
1245.811523 1.011772
1245.811523 1.012253
1245.811523 1.012702
1245.811523 1.013179
1245.811523 1.013653
1245.811523 1.014114
1245.811523 1.014550
1245.811523 1.014963
1245.811523 1.015385
1245.811523 1.015793
1245.811523 1.016166
1245.811523 1.016531
1245.811523 1.016968
1245.811523 1.017386
1245.811523 1.017782
1245.811523 1.018157
1245.811523 1.018532
1245.811523 1.018867
1245.811523 1.019193
1245.811523 1.019521
1245.811523 1.019839
1245.811523 1.020160
1245.811523 1.020557
1245.811523 1.020943
1245.811523 1.021374
1245.811523 1.021865
1245.811523 1.022316
1245.811523 1.022743
1245.811523 1.023137
1245.811523 1.023543
1245.811523 1.023931
1245.811523 1.024360
1245.811523 1.024783
1245.811523 1.025209
1245.811523 1.025612
1245.811523 1.026025
1245.811523 1.026431
1245.811523 1.026837
1245.811523 1.027277
1245.811523 1.027741
1245.811523 1.028161
1245.811523 1.028607
1245.811523 1.029051
1245.811523 1.029454
1245.811523 1.029849
1245.811523 1.030217
1245.811523 1.030619
1245.811523 1.031014
1245.811523 1.031412
1245.811523 1.031810
1245.811523 1.032202
1245.811523 1.032586
1245.811523 1.032939
1245.811523 1.033296
1245.811523 1.033630
1245.811523 1.033936
1245.811523 1.034273
1245.811523 1.034644
1245.811523 1.035016
1245.811523 1.035407
1245.811523 1.035767
1245.811523 1.036162
1245.811523 1.036584
1245.811523 1.037030
1245.811523 1.037516
1245.811523 1.037954
1245.811523 1.038355
1245.811523 1.038773
1245.811523 1.039174
1245.811523 1.039604
1245.811523 1.040041
1245.811523 1.040471
1245.811523 1.040900
1245.811523 1.041336
1245.811523 1.041727
1245.811523 1.042129
1245.811523 1.042542
1245.811523 1.042966
1245.811523 1.043375
1245.811523 1.043786
1245.811523 1.044208
1245.811523 1.044623
1245.811523 1.045012
1245.811523 1.045390
1245.811523 1.045814
1245.811523 1.046267
1245.811523 1.046714
1245.811523 1.047147
1245.811523 1.047585
1245.811523 1.047953
1245.811523 1.048340
1245.811523 1.048707
1245.811523 1.049111
1245.811523 1.049511
1245.811523 1.049942
1245.811523 1.050354
1245.811523 1.050752
1245.811523 1.051130
1245.811523 1.051505
1245.811523 1.051865
1245.811523 1.052221
1245.811523 1.052549
1245.811523 1.052890
1245.811523 1.053250
1245.811523 1.053586
1245.811523 1.053949
1245.811523 1.054302
1245.811523 1.054699
1245.811523 1.055099
1245.811523 1.055478
1245.811523 1.055890
1245.811523 1.056332
1245.811523 1.056797
1245.811523 1.057263
1245.811523 1.057746
1245.811523 1.058209
1245.811523 1.058671
1245.811523 1.059127
1245.811523 1.059594
1245.811523 1.060047
1245.811523 1.060459
1245.811523 1.060881
1245.811523 1.061306
1245.811523 1.061692
1245.811523 1.062069
1245.811523 1.062470
1245.811523 1.062872
1245.811523 1.063315
1245.811523 1.063730
1245.811523 1.064121
1245.811523 1.064539
1245.811523 1.064925
1245.811523 1.065310
1245.811523 1.065685
1245.811523 1.066040
1245.811523 1.066406
1245.811523 1.066833
1245.811523 1.067262
1245.811523 1.067679
1245.811523 1.068066
1245.811523 1.068487
1245.811523 1.068891
1245.811523 1.069260
1245.811523 1.069667
1245.811523 1.070057
1245.811523 1.070436
1245.811523 1.070851
1245.811523 1.071287
1245.811523 1.071686
1245.811523 1.072033
1245.811523 1.072366
1245.811523 1.072707
1245.811523 1.073051
1245.811523 1.073420
1245.811523 1.073779
1245.811523 1.074118
1245.811523 1.074479
1245.811523 1.074936
1245.811523 1.075385
1245.811523 1.075820
1245.811523 1.076274
1245.811523 1.076731
1245.811523 1.077210
1245.811523 1.077649
1245.811523 1.078067
1245.811523 1.078462
1245.811523 1.078871
1245.811523 1.079256
1245.811523 1.079722
1245.811523 1.080174
1245.811523 1.080634
1245.811523 1.081115
1245.811523 1.081559
1245.811523 1.081946
1245.811523 1.082352
1245.811523 1.082748
1245.811523 1.083166
1245.811523 1.083569
1245.811523 1.083980
1245.811523 1.084372
1245.811523 1.084771
1245.811523 1.085179
1245.811523 1.085590
1245.811523 1.086044
1245.811523 1.086482
1245.811523 1.086936
1245.811523 1.087372
1245.811523 1.087804
1245.811523 1.088236
1245.811523 1.088619
1245.811523 1.089021
1245.811523 1.089387
1245.811523 1.089788
1245.811523 1.090194
1245.811523 1.090579
1245.811523 1.090941
1245.811523 1.091337
1245.811523 1.091676
1245.811523 1.092031
1245.811523 1.092446
1245.811523 1.092864
1245.811523 1.093299
1245.811523 1.093733
1245.811523 1.094191
1245.811523 1.094628
1245.811523 1.095048
1245.811523 1.095445
1245.811523 1.095874
1245.811523 1.096275
1245.811523 1.096675
1245.811523 1.097072
1245.811523 1.097486
1245.811523 1.097896
1245.811523 1.098291
1245.811523 1.098712
1245.811523 1.099117
1245.811523 1.099557
1245.811523 1.099988
1245.811523 1.100415
1245.811523 1.100851
1245.811523 1.101277
1245.811523 1.101695
1245.811523 1.102115
1245.811523 1.102527
1245.811523 1.102909
1245.811523 1.103304
1245.811523 1.103700
1245.811523 1.104077
1245.811523 1.104490
1245.811523 1.104903
1245.811523 1.105310
1245.811523 1.105754
1245.811523 1.106157
1245.811523 1.106551
1245.811523 1.106940
1245.811523 1.107349
1245.811523 1.107766
1245.811523 1.108217
1245.811523 1.108641
1245.811523 1.109030
1245.811523 1.109442
1245.811523 1.109842
1245.811523 1.110272
1245.811523 1.110715
1245.811523 1.111202
1245.811523 1.111679
1245.811523 1.112125
1245.811523 1.112533
1245.811523 1.112963
1245.811523 1.113365
1245.811523 1.113815
1245.811523 1.114234
1245.811523 1.114667
1245.811523 1.115064
1245.811523 1.115461
1245.811523 1.115842
1245.811523 1.116206
1245.811523 1.116586
1245.811523 1.116980
1245.811523 1.117393
1245.811523 1.117775
1245.811523 1.118173
1245.811523 1.118539
1245.811523 1.118933
1245.811523 1.119364
1245.811523 1.119795
1245.811523 1.120227
1245.811523 1.120624
1245.811523 1.121001
1245.811523 1.121377
1245.811523 1.121726
1245.811523 1.122090
1245.811523 1.122460
1245.811523 1.122851
1245.811523 1.123268
1245.811523 1.123648
1245.811523 1.124010
1245.811523 1.124352
1245.811523 1.124709
1245.811523 1.125049
1245.811523 1.125427
1245.811523 1.125834
1245.811523 1.126227
1245.811523 1.126643
1245.811523 1.127102
1245.811523 1.127580
1245.811523 1.128048
1245.811523 1.128508
1245.811523 1.128949
1245.811523 1.129378
1245.811523 1.129834
1245.811523 1.130290
1245.811523 1.130746
1245.811523 1.131227
1245.811523 1.131716
1245.811523 1.132211
1245.811523 1.132681
1245.811523 1.133106
1245.811523 1.133562
1245.811523 1.134022
1245.811523 1.134456
1245.811523 1.134876
1245.811523 1.135268
1245.811523 1.135684
1245.811523 1.136093
1245.811523 1.136493
1245.811523 1.136883
1245.811523 1.137289
1245.811523 1.137718
1245.811523 1.138140
1245.811523 1.138522
1245.811523 1.138878
1245.811523 1.139240
1245.811523 1.139609
1245.811523 1.139964
1245.811523 1.140310
1245.811523 1.140649
1245.811523 1.141014
1245.811523 1.141359
1245.811523 1.141731
1245.811523 1.142133
1245.811523 1.142552
1245.811523 1.142983
1245.811523 1.143412
1245.811523 1.143865
1245.811523 1.144280
1245.811523 1.144687
1245.811523 1.145082
1245.811523 1.145478
1245.811523 1.145846
1245.811523 1.146185
1245.811523 1.146552
1260.975708 1.114055
1260.975708 1.114400
1260.975708 1.114744
1260.975708 1.115071
1260.975708 1.115392
1260.975708 1.115735
1260.975708 1.116127
1260.975708 1.116510
1260.975708 1.116966
1260.975708 1.117400
1260.975708 1.117839
1260.975708 1.118249
1291.174683 1.086643
1291.174683 1.087067
1291.174683 1.087493
1291.174683 1.087978
1291.174683 1.088467
1291.174683 1.088925
1291.174683 1.089329
1291.174683 1.089738
1291.174683 1.090143
1291.174683 1.090550
1291.174683 1.091009
1291.174683 1.091461
1291.174683 1.091862
1291.174683 1.092250
1291.174683 1.092655
1291.174683 1.093069
1291.174683 1.093466
1291.174683 1.093858
1291.174683 1.094220
1291.174683 1.094571
1291.174683 1.094917
1291.174683 1.095313
1291.174683 1.095718
1291.174683 1.096094
1291.174683 1.096469
1291.174683 1.096816
1291.174683 1.097169
1291.174683 1.097536
1291.174683 1.097883
1291.174683 1.098230
1291.174683 1.098611
1291.174683 1.098965
1291.174683 1.099338
1291.174683 1.099711
1291.174683 1.100106
1291.174683 1.100495
1291.174683 1.100881
1291.174683 1.101266
1291.174683 1.101650
1291.174683 1.102043
1291.174683 1.102455
1291.174683 1.102834
1291.174683 1.103197
1291.174683 1.103557
1291.174683 1.103928
1291.174683 1.104296
1291.174683 1.104679
1291.174683 1.105040
1291.174683 1.105396
1291.174683 1.105743
1291.174683 1.106087
1291.174683 1.106396
1291.174683 1.106710
1291.174683 1.107041
1291.174683 1.107366
1291.174683 1.107722
1291.174683 1.108117
1291.174683 1.108499
1291.174683 1.108893
1291.174683 1.109325
1291.174683 1.109715
1291.174683 1.110117
1291.174683 1.110516
1291.174683 1.110904
1291.174683 1.111281
1291.174683 1.111676
1291.174683 1.112051
1291.174683 1.112403
1291.174683 1.112741
1291.174683 1.113120
1291.174683 1.113532
1291.174683 1.113933
1291.174683 1.114323
1291.174683 1.114739
1291.174683 1.115134
1291.174683 1.115490
1291.174683 1.115877
1291.174683 1.116257
1291.174683 1.116646
1291.174683 1.117020
1291.174683 1.117416
1291.174683 1.117779
1291.174683 1.118092
1291.174683 1.118417
1291.174683 1.118748
1291.174683 1.119043
1291.174683 1.119351
1291.174683 1.119685
1291.174683 1.120038
1291.174683 1.120368
1291.174683 1.120679
1291.174683 1.120967
1291.174683 1.121249
1291.174683 1.121572
1291.174683 1.121956
1291.174683 1.122300
1291.174683 1.122651
1291.174683 1.122986
1291.174683 1.123335
1291.174683 1.123735
1291.174683 1.124090
1291.174683 1.124456
1291.174683 1.124813
1291.174683 1.125161
1291.174683 1.125507
1291.174683 1.125862
1291.174683 1.126201
1291.174683 1.126536
1291.174683 1.126928
1291.174683 1.127311
1291.174683 1.127706
1291.174683 1.128099
1291.174683 1.128486
1291.174683 1.128877
1291.174683 1.129291
1291.174683 1.129696
1291.174683 1.130082
1291.174683 1.130453
1291.174683 1.130792
1291.174683 1.131150
1291.174683 1.131501
1291.174683 1.131848
1291.174683 1.132197
1291.174683 1.132561
1291.174683 1.132894
1291.174683 1.133237
1291.174683 1.133583
1291.174683 1.133917
1291.174683 1.134246
1291.174683 1.134620
1291.174683 1.134989
1291.174683 1.135377
1291.174683 1.135806
1291.174683 1.136223
1291.174683 1.136618
1291.174683 1.136999
1291.174683 1.137352
1291.174683 1.137740
1291.174683 1.138115
1291.174683 1.138473
1291.174683 1.138830
1291.174683 1.139192
1291.174683 1.139587
1291.174683 1.139974
1291.174683 1.140376
1291.174683 1.140802
1291.174683 1.141195
1291.174683 1.141547
1291.174683 1.141948
1291.174683 1.142320
1291.174683 1.142668
1291.174683 1.143041
1291.174683 1.143408
1291.174683 1.143813
1291.174683 1.144244
1291.174683 1.144675
1291.174683 1.145107
1291.174683 1.145507
1291.174683 1.145875
1291.174683 1.146229
1291.174683 1.146584
1291.174683 1.146966
1291.174683 1.147334
1291.174683 1.147691
1291.174683 1.148053
1291.174683 1.148426
1291.174683 1.148799
1291.174683 1.149180
1291.174683 1.149574
1291.174683 1.149937
1291.174683 1.150329
1291.174683 1.150733
1307.171143 1.149723
1307.171143 1.150131
1307.171143 1.150512
1307.171143 1.150877
1307.171143 1.151237
1307.171143 1.151591
1307.171143 1.151931
1307.171143 1.152274
1307.171143 1.152631
1307.171143 1.153001
1307.171143 1.153354
1307.171143 1.153702
1307.171143 1.154043
1307.171143 1.154370
1307.171143 1.154676
1307.171143 1.155017
1307.171143 1.155333
1307.171143 1.155681
1307.171143 1.156042
1307.171143 1.156433
1307.171143 1.156862
1307.171143 1.157310
1307.171143 1.157765
1307.171143 1.158177
1307.171143 1.158606
1307.171143 1.159066
1307.171143 1.159520
1307.171143 1.159972
1307.171143 1.160406
1307.171143 1.160811
1307.171143 1.161195
1307.171143 1.161589
1307.171143 1.161983
1307.171143 1.162364
1307.171143 1.162712
1307.171143 1.163075
1307.171143 1.163456
1307.171143 1.163828
1307.171143 1.164164
1307.171143 1.164572
1307.171143 1.165009
1307.171143 1.165407
1307.171143 1.165777
1307.171143 1.166179
1307.171143 1.166587
1307.171143 1.166997
1307.171143 1.167403
1307.171143 1.167832
1307.171143 1.168265
1307.171143 1.168678
1307.171143 1.169099
1307.171143 1.169496
1307.171143 1.169870
1307.171143 1.170251
1307.171143 1.170645
1307.171143 1.171044
1307.171143 1.171425
1307.171143 1.171816
1307.171143 1.172213
1307.171143 1.172599
1307.171143 1.172978
1307.171143 1.173362
1307.171143 1.173707
1307.171143 1.174077
1307.171143 1.174430
1307.171143 1.174807
1307.171143 1.175187
1307.171143 1.175585
1307.171143 1.175970
1307.171143 1.176344
1307.171143 1.176709
1307.171143 1.177107
1307.171143 1.177490
1307.171143 1.177883
1307.171143 1.178276
1307.171143 1.178681
1307.171143 1.179104
1307.171143 1.179603
1307.171143 1.180095
1307.171143 1.180543
1307.171143 1.180953
1307.171143 1.181389
1307.171143 1.181812
1307.171143 1.182234
1307.171143 1.182659
1307.171143 1.183076
1307.171143 1.183475
1307.171143 1.183909
1307.171143 1.184310
1307.171143 1.184746
1307.171143 1.185215
1307.171143 1.185656
1307.171143 1.186088
1307.171143 1.186496
1307.171143 1.186889
1307.171143 1.187259
1307.171143 1.187633
1307.171143 1.188022
1307.171143 1.188427
1307.171143 1.188816
1307.171143 1.189195
1307.171143 1.189572
1307.171143 1.189950
1307.171143 1.190320
1307.171143 1.190668
1307.171143 1.191032
1307.171143 1.191445
1307.171143 1.191851
1307.171143 1.192231
1307.171143 1.192576
1307.171143 1.192900
1307.171143 1.193224
1307.171143 1.193551
1307.171143 1.193916
1307.171143 1.194288
1307.171143 1.194661
1307.171143 1.195023
1307.171143 1.195386
1307.171143 1.195739
1307.171143 1.196150
1307.171143 1.196568
1307.171143 1.196979
1307.171143 1.197346
1307.171143 1.197695
1307.171143 1.198067
1307.171143 1.198437
1307.171143 1.198817
1307.171143 1.199241
1307.171143 1.199662
1307.171143 1.200066
1307.171143 1.200464
1307.171143 1.200848
1307.171143 1.201294
1307.171143 1.201739
1307.171143 1.202161
1307.171143 1.202598
1307.171143 1.203023
1307.171143 1.203444
1307.171143 1.203835
1307.171143 1.204213
1307.171143 1.204630
1307.171143 1.205003
1307.171143 1.205350
1307.171143 1.205706
1307.171143 1.206121
1307.171143 1.206556
1307.171143 1.206945
1307.171143 1.207336
1307.171143 1.207717
1307.171143 1.208095
1307.171143 1.208455
1307.171143 1.208806
1307.171143 1.209158
1307.171143 1.209490
1307.171143 1.209831
1307.171143 1.210169
1307.171143 1.210512
1307.171143 1.210863
1307.171143 1.211240
1307.171143 1.211636
1307.171143 1.212067
1307.171143 1.212472
1307.171143 1.212843
1307.171143 1.213187
1307.171143 1.213518
1307.171143 1.213854
1307.171143 1.214178
1307.171143 1.214557
1307.171143 1.214956
1307.171143 1.215384
1307.171143 1.215795
1307.171143 1.216208
1307.171143 1.216589
1307.171143 1.216966
1307.171143 1.217321
1307.171143 1.217651
1307.171143 1.217986
1307.171143 1.218365
1307.171143 1.218742
1307.171143 1.219185
1307.171143 1.219617
1307.171143 1.220002
1307.171143 1.220386
1307.171143 1.220752
1307.171143 1.221104
1307.171143 1.221478
1307.171143 1.221843
1307.171143 1.222234
1307.171143 1.222624
1307.171143 1.222999
1307.171143 1.223407
1307.171143 1.223804
1307.171143 1.224185
1307.171143 1.224570
1307.171143 1.224963
1307.171143 1.225320
1307.171143 1.225670
1307.171143 1.226017
1307.171143 1.226411
1307.171143 1.226778
1307.171143 1.227162
1307.171143 1.227542
1307.171143 1.227936
1307.171143 1.228335
1307.171143 1.228728
1307.171143 1.229155
1307.171143 1.229585
1307.171143 1.229988
1307.171143 1.230367
1307.171143 1.230745
1307.171143 1.231121
1307.171143 1.231488
1307.171143 1.231861
1307.171143 1.232244
1307.171143 1.232616
1307.171143 1.232981
1307.171143 1.233343
1307.171143 1.233671
1307.171143 1.233982
1307.171143 1.234315
1307.171143 1.234634
1307.171143 1.234983
1307.171143 1.235364
1307.171143 1.235715
1307.171143 1.236076
1307.171143 1.236446
1307.171143 1.236847
1307.171143 1.237244
1307.171143 1.237708
1307.171143 1.238140
1307.171143 1.238537
1307.171143 1.238886
1307.171143 1.239235
1307.171143 1.239606
1307.171143 1.239990
1307.171143 1.240379
1307.171143 1.240748
1307.171143 1.241107
1307.171143 1.241462
1307.171143 1.241794
1307.171143 1.242139
1307.171143 1.242493
1307.171143 1.242863
1307.171143 1.243223
1307.171143 1.243575
1307.171143 1.243955
1307.171143 1.244406
1307.171143 1.244865
1307.171143 1.245339
1307.171143 1.245785
1307.171143 1.246188
1307.171143 1.246563
1307.171143 1.246929
1307.171143 1.247273
1307.171143 1.247658
1307.171143 1.248042
1307.171143 1.248414
1307.171143 1.248774
1307.171143 1.249111
1307.171143 1.249465
1307.171143 1.249840
1307.171143 1.250232
1307.171143 1.250657
1307.171143 1.251085
1307.171143 1.251505
1307.171143 1.251946
1307.171143 1.252342
1307.171143 1.252747
1307.171143 1.253127
1307.171143 1.253516
1307.171143 1.253897
1307.171143 1.254284
1307.171143 1.254676
1307.171143 1.255082
1307.171143 1.255479
1307.171143 1.255848
1307.171143 1.256263
1307.171143 1.256672
1307.171143 1.257073
1307.171143 1.257458
1307.171143 1.257913
1307.171143 1.258363
1307.171143 1.258785
1324.766479 1.259586
1324.766479 1.260000
1324.766479 1.260401
1324.766479 1.260826
1324.766479 1.261223
1324.766479 1.261631
1324.766479 1.262086
1324.766479 1.262548
1324.766479 1.262969
1324.766479 1.263403
1324.766479 1.263807
1324.766479 1.264200
1324.766479 1.264599
1324.766479 1.265019
1324.766479 1.265410
1324.766479 1.265783
1324.766479 1.266121
1324.766479 1.266464
1324.766479 1.266852
1324.766479 1.267233
1324.766479 1.267626
1324.766479 1.268031
1324.766479 1.268424
1324.766479 1.268835
1324.766479 1.269251
1324.766479 1.269735
1324.766479 1.270217
1324.766479 1.270647
1324.766479 1.271047
1324.766479 1.271393
1324.766479 1.271785
1324.766479 1.272189
1324.766479 1.272557
1324.766479 1.272927
1324.766479 1.273342
1324.766479 1.273739
1324.766479 1.274153
1324.766479 1.274576
1324.766479 1.275032
1324.766479 1.275482
1324.766479 1.275920
1324.766479 1.276335
1324.766479 1.276769
1324.766479 1.277180
1324.766479 1.277582
1324.766479 1.277984
1324.766479 1.278412
1324.766479 1.278834
1324.766479 1.279230
1324.766479 1.279593
1324.766479 1.279979
1324.766479 1.280357
1324.766479 1.280707
1324.766479 1.281031
1324.766479 1.281360
1324.766479 1.281693
1324.766479 1.282040
1324.766479 1.282407
1324.766479 1.282771
1324.766479 1.283139
1324.766479 1.283531
1324.766479 1.283942
1324.766479 1.284334
1324.766479 1.284721
1324.766479 1.285127
1324.766479 1.285518
1324.766479 1.285894
1324.766479 1.286266
1324.766479 1.286644
1342.668701 1.291245
1342.668701 1.291646
1342.668701 1.292067
1342.668701 1.292463
1342.668701 1.292889
1342.668701 1.293298
1342.668701 1.293699
1342.668701 1.294104
1342.668701 1.294533
1342.668701 1.294943
1342.668701 1.295326
1342.668701 1.295690
1342.668701 1.296045
1360.541626 1.269373
1360.541626 1.269703
1360.541626 1.270086
1360.541626 1.270433
1360.541626 1.270760
1360.541626 1.271099
1360.541626 1.271431
1360.541626 1.271762
1360.541626 1.272089
1360.541626 1.272446
1360.541626 1.272851
1360.541626 1.273246
1360.541626 1.273615
1360.541626 1.274017
1360.541626 1.274400
1360.541626 1.274788
1360.541626 1.275208
1360.541626 1.275662
1360.541626 1.276106
1360.541626 1.276519
1360.541626 1.276914
1360.541626 1.277309
1360.541626 1.277711
1360.541626 1.278195
1360.541626 1.278700
1360.541626 1.279172
1360.541626 1.279616
1360.541626 1.280032
1360.541626 1.280460
1360.541626 1.280884
1360.541626 1.281258
1360.541626 1.281612
1360.541626 1.281966
1360.541626 1.282282
1360.541626 1.282608
1360.541626 1.282931
1360.541626 1.283310
1360.541626 1.283679
1360.541626 1.284057
1360.541626 1.284517
1360.541626 1.284951
1360.541626 1.285404
1360.541626 1.285841
1360.541626 1.286266
1360.541626 1.286685
1360.541626 1.287128
1360.541626 1.287576
1360.541626 1.288015
1360.541626 1.288434
1360.541626 1.288839
1360.541626 1.289227
1360.541626 1.289587
1360.541626 1.289939
1360.541626 1.290321
1360.541626 1.290682
1360.541626 1.291041
1360.541626 1.291449
1360.541626 1.291873
1360.541626 1.292324
1360.541626 1.292786
1360.541626 1.293234
1360.541626 1.293668
1360.541626 1.294111
1360.541626 1.294515
1360.541626 1.294933
1360.541626 1.295441
1360.541626 1.295929
1360.541626 1.296436
1360.541626 1.296906
1360.541626 1.297376
1360.541626 1.297791
1360.541626 1.298218
1360.541626 1.298636
1360.541626 1.299061
1360.541626 1.299493
1360.541626 1.299912
1360.541626 1.300312
1360.541626 1.300743
1360.541626 1.301152
1360.541626 1.301552
1360.541626 1.301971
1360.541626 1.302362
1360.541626 1.302756
1360.541626 1.303135
1360.541626 1.303516
1360.541626 1.303881
1360.541626 1.304246
1360.541626 1.304599
1360.541626 1.304994
1360.541626 1.305431
1360.541626 1.305877
1360.541626 1.306333
1360.541626 1.306763
1360.541626 1.307187
1360.541626 1.307595
1360.541626 1.308015
1360.541626 1.308456
1360.541626 1.308886
1360.541626 1.309310
1360.541626 1.309696
1360.541626 1.310104
1360.541626 1.310503
1360.541626 1.310890
1360.541626 1.311276
1360.541626 1.311641
1360.541626 1.312013
1360.541626 1.312391
1360.541626 1.312768
1360.541626 1.313141
1360.541626 1.313526
1360.541626 1.313948
1360.541626 1.314339
1360.541626 1.314707
1360.541626 1.315047
1360.541626 1.315399
1360.541626 1.315783
1360.541626 1.316136
1360.541626 1.316484
1360.541626 1.316821
1360.541626 1.317152
1360.541626 1.317432
1360.541626 1.317755
1360.541626 1.318078
1360.541626 1.318424
1360.541626 1.318773
1360.541626 1.319193
1360.541626 1.319583
1360.541626 1.319979
1360.541626 1.320366
1360.541626 1.320720
1360.541626 1.321119
1360.541626 1.321510
1360.541626 1.321855
1360.541626 1.322190
1360.541626 1.322538
1360.541626 1.322899
1360.541626 1.323273
1360.541626 1.323672
1360.541626 1.324119
1360.541626 1.324624
1360.541626 1.325148
1360.541626 1.325663
1360.541626 1.326135
1360.541626 1.326602
1360.541626 1.327006
1360.541626 1.327417
1360.541626 1.327821
1360.541626 1.328238
1360.541626 1.328656
1360.541626 1.329046
1360.541626 1.329476
1360.541626 1.329884
1360.541626 1.330311
1360.541626 1.330737
1360.541626 1.331146
1360.541626 1.331530
1360.541626 1.331950
1360.541626 1.332344
1360.541626 1.332720
1360.541626 1.333083
1360.541626 1.333438
1360.541626 1.333847
1360.541626 1.334251
1360.541626 1.334658
1360.541626 1.335049
1360.541626 1.335503
1360.541626 1.335953
1360.541626 1.336396
1360.541626 1.336869
1360.541626 1.337330
1360.541626 1.337783
1360.541626 1.338247
1360.541626 1.338736
1360.541626 1.339280
1360.541626 1.339804
1360.541626 1.340282
1360.541626 1.340751
1360.541626 1.341281
1360.541626 1.341790
1360.541626 1.342252
1360.541626 1.342705
1360.541626 1.343220
1360.541626 1.343734
1360.541626 1.344205
1360.541626 1.344634
1360.541626 1.345046
1360.541626 1.345466
1360.541626 1.345897
1360.541626 1.346329
1360.541626 1.346764
1360.541626 1.347209
1360.541626 1.347625
1360.541626 1.348040
1360.541626 1.348434
1360.541626 1.348835
1360.541626 1.349210
1360.541626 1.349599
1360.541626 1.350006
1360.541626 1.350443
1360.541626 1.350893
1360.541626 1.351327
1360.541626 1.351736
1360.541626 1.352134
1360.541626 1.352521
1360.541626 1.352891
1360.541626 1.353247
1360.541626 1.353635
1360.541626 1.354022
1360.541626 1.354398
1360.541626 1.354769
1360.541626 1.355150
1360.541626 1.355533
1360.541626 1.355915
1360.541626 1.356313
1360.541626 1.356709
1360.541626 1.357088
1360.541626 1.357481
1360.541626 1.357875
1360.541626 1.358262
1360.541626 1.358648
1360.541626 1.359046
1360.541626 1.359436
1360.541626 1.359871
1360.541626 1.360322
1360.541626 1.360764
1360.541626 1.361202
1360.541626 1.361658
1360.541626 1.362127
1360.541626 1.362564
1360.541626 1.362982
1360.541626 1.363396
1360.541626 1.363829
1360.541626 1.364251
1360.541626 1.364655
1360.541626 1.365069
1360.541626 1.365474
1360.541626 1.365862
1360.541626 1.366261
1360.541626 1.366646
1360.541626 1.366996
1360.541626 1.367329
1360.541626 1.367646
1360.541626 1.367981
1360.541626 1.368307
1360.541626 1.368681
1360.541626 1.369044
1360.541626 1.369397
1360.541626 1.369731
1360.541626 1.370074
1360.541626 1.370449
1360.541626 1.370866
1360.541626 1.371283
1360.541626 1.371712
1360.541626 1.372159
1360.541626 1.372606
1360.541626 1.373063
1360.541626 1.373515
1360.541626 1.373925
1360.541626 1.374337
1360.541626 1.374744
1360.541626 1.375117
1360.541626 1.375508
1360.541626 1.375891
1360.541626 1.376277
1360.541626 1.376655
1360.541626 1.377001
1360.541626 1.377376
1360.541626 1.377754
1360.541626 1.378167
1360.541626 1.378604
1360.541626 1.379043
1360.541626 1.379476
1360.541626 1.379852
1360.541626 1.380214
1360.541626 1.380583
1360.541626 1.380940
1360.541626 1.381313
1360.541626 1.381731
1360.541626 1.382174
1360.541626 1.382574
1360.541626 1.382941
1360.541626 1.383298
1360.541626 1.383665
1360.541626 1.384013
1360.541626 1.384398
1360.541626 1.384795
1360.541626 1.385229
1360.541626 1.385668
1360.541626 1.386097
1360.541626 1.386527
1360.541626 1.386928
1360.541626 1.387349
1360.541626 1.387742
1360.541626 1.388109
1360.541626 1.388453
1360.541626 1.388796
1360.541626 1.389163
1360.541626 1.389552
1360.541626 1.389937
1360.541626 1.390292
1360.541626 1.390640
1360.541626 1.390977
1360.541626 1.391351
1360.541626 1.391738
1360.541626 1.392128
1360.541626 1.392526
1360.541626 1.392927
1360.541626 1.393322
1360.541626 1.393712
1360.541626 1.394089
1360.541626 1.394478
1360.541626 1.394854
1360.541626 1.395256
1360.541626 1.395696
1360.541626 1.396151
1360.541626 1.396597
1360.541626 1.397071
1360.541626 1.397550
1360.541626 1.398022
1360.541626 1.398474
1360.541626 1.398906
1360.541626 1.399297
1360.541626 1.399663
1360.541626 1.400034
1360.541626 1.400402
1360.541626 1.400749
1360.541626 1.401086
1360.541626 1.401433
1360.541626 1.401796
1360.541626 1.402179
1360.541626 1.402567
1360.541626 1.402995
1360.541626 1.403432
1360.541626 1.403879
1360.541626 1.404354
1360.541626 1.404818
1360.541626 1.405259
1360.541626 1.405672
1360.541626 1.406052
1360.541626 1.406438
1360.541626 1.406853
1360.541626 1.407291
1360.541626 1.407730
1360.541626 1.408182
1360.541626 1.408644
1360.541626 1.409105
1360.541626 1.409532
1360.541626 1.409934
1360.541626 1.410351
1360.541626 1.410749
1360.541626 1.411150
1360.541626 1.411615
1360.541626 1.412055
1360.541626 1.412469
1360.541626 1.412853
1360.541626 1.413238
1360.541626 1.413580
1360.541626 1.413899
1360.541626 1.414210
1360.541626 1.414497
1360.541626 1.414804
1360.541626 1.415117
1360.541626 1.415465
1360.541626 1.415829
1360.541626 1.416202
1360.541626 1.416594
1360.541626 1.416986
1360.541626 1.417372
1360.541626 1.417788
1360.541626 1.418240
1360.541626 1.418656
1360.541626 1.419042
1360.541626 1.419403
1360.541626 1.419744
1360.541626 1.420090
1360.541626 1.420480
1360.541626 1.420888
1360.541626 1.421270
1360.541626 1.421648
1360.541626 1.422001
1360.541626 1.422363
1360.541626 1.422739
1360.541626 1.423146
1360.541626 1.423515
1360.541626 1.423874
1360.541626 1.424240
1360.541626 1.424596
1360.541626 1.424943
1360.541626 1.425291
1360.541626 1.425660
1360.541626 1.426029
1360.541626 1.426432
1360.541626 1.426817
1360.541626 1.427193
1360.541626 1.427619
1360.541626 1.428043
1360.541626 1.428490
1360.541626 1.428896
1360.541626 1.429325
1360.541626 1.429801
1360.541626 1.430243
1360.541626 1.430714
1360.541626 1.431158
1360.541626 1.431583
1360.541626 1.431994
1360.541626 1.432407
1360.541626 1.432820
1360.541626 1.433246
1360.541626 1.433646
1360.541626 1.434050
1360.541626 1.434423
1360.541626 1.434801
1360.541626 1.435167
1360.541626 1.435535
1360.541626 1.435892
1360.541626 1.436252
1360.541626 1.436620
1360.541626 1.436952
1360.541626 1.437279
1360.541626 1.437618
1360.541626 1.437971
1360.541626 1.438320
1360.541626 1.438672
1360.541626 1.439072
1360.541626 1.439460
1360.541626 1.439829
1360.541626 1.440210
1360.541626 1.440586
1360.541626 1.440937
1360.541626 1.441283
1360.541626 1.441646
1360.541626 1.441989
1360.541626 1.442363
1360.541626 1.442728
1360.541626 1.443108
1360.541626 1.443490
1360.541626 1.443847
1360.541626 1.444211
1360.541626 1.444594
1360.541626 1.444941
1360.541626 1.445269
1360.541626 1.445657
1360.541626 1.446018
1360.541626 1.446451
1360.541626 1.446931
1360.541626 1.447379
1360.541626 1.447804
1360.541626 1.448199
1360.541626 1.448596
1360.541626 1.449015
1360.541626 1.449453
1360.541626 1.449872
1360.541626 1.450296
1360.541626 1.450657
1360.541626 1.451030
1360.541626 1.451400
1360.541626 1.451790
1360.541626 1.452204
1360.541626 1.452620
1360.541626 1.453021
1360.541626 1.453396
1360.541626 1.453746
1360.541626 1.454092
1360.541626 1.454436
1360.541626 1.454751
1360.541626 1.455070
1360.541626 1.455432
1360.541626 1.455789
1360.541626 1.456163
1360.541626 1.456525
1360.541626 1.456909
1360.541626 1.457275
1360.541626 1.457645
1360.541626 1.458059
1360.541626 1.458460
1360.541626 1.458854
1360.541626 1.459261
1360.541626 1.459681
1360.541626 1.460125
1360.541626 1.460597
1360.541626 1.461009
1360.541626 1.461421
1381.169189 1.433621
1381.169189 1.433973
1381.169189 1.434320
1381.169189 1.434668
1381.169189 1.435027
1381.169189 1.435366
1381.169189 1.435713
1381.169189 1.436071
1381.169189 1.436458
1381.169189 1.436800
1381.169189 1.437157
1381.169189 1.437500
1381.169189 1.437854
1381.169189 1.438191
1401.757446 1.401554
1401.757446 1.401913
1401.757446 1.402279
1401.757446 1.402640
1401.757446 1.403032
1401.757446 1.403379
1401.757446 1.403802
1401.757446 1.404202
1401.757446 1.404647
1401.757446 1.405111
1401.757446 1.405558
1401.757446 1.406040
1401.757446 1.406559
1401.757446 1.407114
1401.757446 1.407635
1401.757446 1.408125
1401.757446 1.408655
1401.757446 1.409140
1401.757446 1.409624
1401.757446 1.410125
1401.757446 1.410578
1401.757446 1.411008
1401.757446 1.411401
1401.757446 1.411768
1401.757446 1.412122
1401.757446 1.412466
1401.757446 1.412832
1401.757446 1.413239
1401.757446 1.413655
1401.757446 1.414038
1401.757446 1.414419
1401.757446 1.414785
1401.757446 1.415129
1401.757446 1.415524
1401.757446 1.415905
1401.757446 1.416310
1401.757446 1.416707
1401.757446 1.417111
1401.757446 1.417485
1401.757446 1.417844
1401.757446 1.418179
1401.757446 1.418504
1401.757446 1.418818
1401.757446 1.419189
1401.757446 1.419543
1401.757446 1.419920
1401.757446 1.420299
1401.757446 1.420692
1401.757446 1.421078
1401.757446 1.421518
1401.757446 1.421927
1401.757446 1.422323
1401.757446 1.422697
1401.757446 1.423085
1401.757446 1.423458
1401.757446 1.423865
1401.757446 1.424292
1401.757446 1.424695
1401.757446 1.425086
1401.757446 1.425480
1401.757446 1.425881
1401.757446 1.426282
1401.757446 1.426716
1401.757446 1.427156
1401.757446 1.427561
1401.757446 1.427951
1401.757446 1.428340
1401.757446 1.428742
1401.757446 1.429134
1401.757446 1.429526
1401.757446 1.429923
1401.757446 1.430342
1422.648926 1.437000
1422.648926 1.437370
1422.648926 1.437737
1422.648926 1.438151
1422.648926 1.438566
1422.648926 1.438959
1422.648926 1.439347
1422.648926 1.439749
1422.648926 1.440105
1422.648926 1.440458
1422.648926 1.440811
1422.648926 1.441212
1422.648926 1.441623
1422.648926 1.442054
1422.648926 1.442433
1422.648926 1.442819
1422.648926 1.443179
1422.648926 1.443561
1422.648926 1.443918
1422.648926 1.444310
1422.648926 1.444720
1422.648926 1.445133
1422.648926 1.445539
1422.648926 1.445951
1422.648926 1.446366
1422.648926 1.446827
1422.648926 1.447275
1422.648926 1.447708
1422.648926 1.448114
1422.648926 1.448510
1422.648926 1.448893
1422.648926 1.449269
1422.648926 1.449641
1422.648926 1.450065
1422.648926 1.450500
1422.648926 1.450930
1422.648926 1.451378
1422.648926 1.451829
1422.648926 1.452251
1422.648926 1.452678
1422.648926 1.453100
1422.648926 1.453510
1422.648926 1.453941
1422.648926 1.454381
1422.648926 1.454872
1422.648926 1.455333
1422.648926 1.455812
1422.648926 1.456241
1422.648926 1.456694
1422.648926 1.457089
1422.648926 1.457513
1422.648926 1.457920
1422.648926 1.458343
1422.648926 1.458751
1422.648926 1.459204
1422.648926 1.459661
1422.648926 1.460068
1422.648926 1.460449
1422.648926 1.460846
1422.648926 1.461197
1422.648926 1.461536
1422.648926 1.461908
1422.648926 1.462300
1422.648926 1.462680
1422.648926 1.463026
1422.648926 1.463355
1422.648926 1.463734
1422.648926 1.464120
1422.648926 1.464489
1422.648926 1.464877
1422.648926 1.465264
1443.835327 1.449483
1443.835327 1.449927
1443.835327 1.450391
1443.835327 1.450812
1443.835327 1.451213
1443.835327 1.451596
1443.835327 1.451953
1443.835327 1.452314
1443.835327 1.452698
1443.835327 1.453079
1443.835327 1.453456
1443.835327 1.453785
1443.835327 1.454121
1443.835327 1.454523
1443.835327 1.454922
1443.835327 1.455335
1443.835327 1.455733
1443.835327 1.456155
1443.835327 1.456569
1443.835327 1.456962
1443.835327 1.457393
1443.835327 1.457822
1443.835327 1.458244
1443.835327 1.458645
1443.835327 1.459028
1443.835327 1.459468
1443.835327 1.459942
1443.835327 1.460369
1465.061523 1.455446
1465.061523 1.455849
1465.061523 1.456274
1465.061523 1.456731
1465.061523 1.457175
1465.061523 1.457587
1465.061523 1.457969
1465.061523 1.458319
1465.061523 1.458641
1465.061523 1.458962
1465.061523 1.459295
1465.061523 1.459604
1465.061523 1.459895
1465.061523 1.460189
1465.061523 1.460499
1465.061523 1.460802
1465.061523 1.461118
1465.061523 1.461484
1465.061523 1.461832
1465.061523 1.462174
1465.061523 1.462490
1465.061523 1.462913
1465.061523 1.463325
1465.061523 1.463738
1465.061523 1.464157
1465.061523 1.464588
1465.061523 1.465069
1465.061523 1.465514
1465.061523 1.465968
1465.061523 1.466438
1465.061523 1.466904
1465.061523 1.467321
1465.061523 1.467722
1465.061523 1.468081
1465.061523 1.468399
1465.061523 1.468705
1465.061523 1.468984
1465.061523 1.469264
1465.061523 1.469570
1465.061523 1.469908
1465.061523 1.470329
1465.061523 1.470747
1465.061523 1.471162
1465.061523 1.471588
1465.061523 1.472021
1465.061523 1.472436
1465.061523 1.472828
1465.061523 1.473197
1465.061523 1.473572
1465.061523 1.473954
1465.061523 1.474444
1465.061523 1.474922
1465.061523 1.475413
1465.061523 1.475878
1465.061523 1.476439
1465.061523 1.476966
1465.061523 1.477481
1465.061523 1.477936
1465.061523 1.478402
1465.061523 1.478815
1465.061523 1.479213
1465.061523 1.479679
1465.061523 1.480125
1465.061523 1.480537
1465.061523 1.481071
1465.061523 1.481597
1465.061523 1.482056
1465.061523 1.482479
1465.061523 1.482910
1465.061523 1.483322
1465.061523 1.483732
1465.061523 1.484126
1465.061523 1.484527
1465.061523 1.484950
1465.061523 1.485440
1465.061523 1.485917
1465.061523 1.486417
1465.061523 1.486904
1465.061523 1.487357
1465.061523 1.487761
1465.061523 1.488178
1465.061523 1.488585
1465.061523 1.488981
1465.061523 1.489386
1465.061523 1.489766
1465.061523 1.490156
1465.061523 1.490537
1465.061523 1.490914
1465.061523 1.491326
1465.061523 1.491736
1465.061523 1.492136
1465.061523 1.492575
1465.061523 1.493004
1465.061523 1.493459
1465.061523 1.493905
1465.061523 1.494308
1465.061523 1.494692
1465.061523 1.495113
1465.061523 1.495522
1465.061523 1.495913
1465.061523 1.496304
1465.061523 1.496703
1465.061523 1.497099
1465.061523 1.497540
1465.061523 1.497975
1465.061523 1.498396
1465.061523 1.498860
1465.061523 1.499297
1465.061523 1.499720
1465.061523 1.500158
1465.061523 1.500643
1465.061523 1.501114
1465.061523 1.501573
1465.061523 1.502060
1465.061523 1.502572
1465.061523 1.503076
1465.061523 1.503551
1465.061523 1.503999
1465.061523 1.504451
1465.061523 1.504878
1465.061523 1.505311
1465.061523 1.505697
1465.061523 1.506041
1465.061523 1.506384
1465.061523 1.506826
1465.061523 1.507241
1465.061523 1.507686
1465.061523 1.508100
1465.061523 1.508527
1465.061523 1.508978
1465.061523 1.509486
1465.061523 1.509976
1465.061523 1.510441
1465.061523 1.510910
1465.061523 1.511368
1465.061523 1.511854
1465.061523 1.512283
1465.061523 1.512684
1465.061523 1.513089
1465.061523 1.513552
1465.061523 1.513980
1465.061523 1.514378
1465.061523 1.514827
1465.061523 1.515331
1465.061523 1.515867
1465.061523 1.516353
1465.061523 1.516824
1465.061523 1.517259
1487.029297 1.527864
1487.029297 1.528237
1487.029297 1.528619
1487.029297 1.528998
1487.029297 1.529361
1487.029297 1.529728
1487.029297 1.530108
1487.029297 1.530499
1487.029297 1.530949
1487.029297 1.531366
1487.029297 1.531763
1487.029297 1.532146
1487.029297 1.532518
1487.029297 1.532889
1487.029297 1.533259
1487.029297 1.533620
1487.029297 1.533973
1487.029297 1.534353
1487.029297 1.534732
1487.029297 1.535103
1487.029297 1.535464
1487.029297 1.535861
1487.029297 1.536251
1487.029297 1.536651
1487.029297 1.537043
1487.029297 1.537440
1487.029297 1.537874
1487.029297 1.538268
1487.029297 1.538684
1487.029297 1.539164
1487.029297 1.539609
1487.029297 1.540037
1487.029297 1.540460
1487.029297 1.540879
1487.029297 1.541290
1487.029297 1.541697
1487.029297 1.542071
1487.029297 1.542482
1487.029297 1.542874
1487.029297 1.543278
1487.029297 1.543651
1487.029297 1.544067
1487.029297 1.544479
1487.029297 1.544969
1487.029297 1.545423
1487.029297 1.545853
1487.029297 1.546269
1487.029297 1.546712
1487.029297 1.547162
1487.029297 1.547586
1487.029297 1.548029
1487.029297 1.548440
1487.029297 1.548857
1487.029297 1.549258
1487.029297 1.549663
1487.029297 1.550054
1487.029297 1.550423
1487.029297 1.550805
1487.029297 1.551206
1487.029297 1.551612
1487.029297 1.552017
1487.029297 1.552410
1487.029297 1.552781
1487.029297 1.553153
1487.029297 1.553545
1487.029297 1.553915
1487.029297 1.554329
1487.029297 1.554720
1487.029297 1.555099
1487.029297 1.555506
1487.029297 1.555889
1487.029297 1.556253
1487.029297 1.556649
1487.029297 1.557087
1487.029297 1.557493
1487.029297 1.557924
1487.029297 1.558386
1487.029297 1.558844
1487.029297 1.559281
1487.029297 1.559750
1487.029297 1.560188
1487.029297 1.560610
1509.346924 1.561735
1509.346924 1.562127
1509.346924 1.562481
1509.346924 1.562831
1509.346924 1.563201
1509.346924 1.563582
1509.346924 1.563941
1509.346924 1.564305
1509.346924 1.564645
1509.346924 1.565008
1509.346924 1.565355
1509.346924 1.565710
1509.346924 1.566069
1509.346924 1.566501
1509.346924 1.566896
1509.346924 1.567298
1509.346924 1.567739
1509.346924 1.568189
1509.346924 1.568646
1509.346924 1.569175
1509.346924 1.569655
1509.346924 1.570121
1509.346924 1.570590
1509.346924 1.571043
1509.346924 1.571460
1509.346924 1.571871
1509.346924 1.572298
1509.346924 1.572753
1509.346924 1.573170
1509.346924 1.573591
1509.346924 1.573971
1509.346924 1.574335
1509.346924 1.574704
1509.346924 1.575064
1509.346924 1.575441
1509.346924 1.575808
1509.346924 1.576181
1509.346924 1.576570
1509.346924 1.576982
1531.761597 1.535125
1531.761597 1.535525
1531.761597 1.535914
1531.761597 1.536294
1531.761597 1.536665
1531.761597 1.537028
1554.081177 1.506444
1554.081177 1.506767
1554.081177 1.507220
1554.081177 1.507631
1554.081177 1.508025
1554.081177 1.508446
1554.081177 1.508930
1554.081177 1.509380
1554.081177 1.509826
1554.081177 1.510256
1554.081177 1.510644
1554.081177 1.511032
1554.081177 1.511394
1554.081177 1.511735
1554.081177 1.512088
1554.081177 1.512419
1554.081177 1.512776
1554.081177 1.513139
1554.081177 1.513511
1554.081177 1.513896
1554.081177 1.514257
1554.081177 1.514647
1554.081177 1.514994
1554.081177 1.515313
1576.410400 1.489755
1576.410400 1.490058
1576.410400 1.490375
1576.410400 1.490714
1576.410400 1.491046
1576.410400 1.491361
1576.410400 1.491687
1576.410400 1.491974
1576.410400 1.492295
1576.410400 1.492571
1576.410400 1.492854
1576.410400 1.493158
1576.410400 1.493443
1576.410400 1.493754
1576.410400 1.494056
1576.410400 1.494387
1576.410400 1.494749
1576.410400 1.495091
1576.410400 1.495413
1576.410400 1.495742
1576.410400 1.496084
1576.410400 1.496425
1576.410400 1.496790
1576.410400 1.497132
1576.410400 1.497467
1576.410400 1.497827
1576.410400 1.498160
1576.410400 1.498495
1576.410400 1.498806
1576.410400 1.499122
1576.410400 1.499458
1576.410400 1.499778
1576.410400 1.500087
1576.410400 1.500435
1576.410400 1.500776
1576.410400 1.501109
1576.410400 1.501446
1576.410400 1.501774
1576.410400 1.502130
1576.410400 1.502506
1576.410400 1.502856
1576.410400 1.503170
1576.410400 1.503449
1576.410400 1.503735
1576.410400 1.504021
1576.410400 1.504287
1576.410400 1.504576
1576.410400 1.504905
1576.410400 1.505259
1576.410400 1.505620
1576.410400 1.505968
1576.410400 1.506328
1576.410400 1.506680
1576.410400 1.507020
1576.410400 1.507378
1576.410400 1.507730
1576.410400 1.508098
1576.410400 1.508471
1576.410400 1.508835
1576.410400 1.509227
1576.410400 1.509627
1576.410400 1.510017
1576.410400 1.510422
1576.410400 1.510791
1576.410400 1.511147
1576.410400 1.511516
1576.410400 1.511901
1576.410400 1.512292
1576.410400 1.512669
1576.410400 1.513003
1576.410400 1.513309
1576.410400 1.513632
1576.410400 1.513947
1576.410400 1.514244
1576.410400 1.514575
1576.410400 1.514910
1576.410400 1.515257
1576.410400 1.515612
1576.410400 1.516005
1576.410400 1.516372
1576.410400 1.516750
1576.410400 1.517104
1576.410400 1.517471
1576.410400 1.517798
1576.410400 1.518124
1576.410400 1.518469
1576.410400 1.518821
1576.410400 1.519168
1576.410400 1.519493
1576.410400 1.519809
1576.410400 1.520134
1576.410400 1.520428
1576.410400 1.520710
1576.410400 1.520982
1576.410400 1.521263
1576.410400 1.521545
1576.410400 1.521840
1576.410400 1.522119
1576.410400 1.522439
1576.410400 1.522761
1576.410400 1.523075
1576.410400 1.523402
1576.410400 1.523766
1576.410400 1.524147
1576.410400 1.524525
1576.410400 1.524921
1576.410400 1.525299
1576.410400 1.525691
1576.410400 1.526061
1576.410400 1.526414
1576.410400 1.526759
1576.410400 1.527137
1576.410400 1.527513
1576.410400 1.527877
1576.410400 1.528233
1576.410400 1.528564
1576.410400 1.528880
1576.410400 1.529201
1576.410400 1.529512
1576.410400 1.529802
1576.410400 1.530092
1576.410400 1.530428
1576.410400 1.530795
1576.410400 1.531160
1576.410400 1.531528
1576.410400 1.531857
1576.410400 1.532188
1576.410400 1.532518
1576.410400 1.532860
1576.410400 1.533205
1576.410400 1.533540
1576.410400 1.533891
1576.410400 1.534221
1576.410400 1.534575
1576.410400 1.534893
1576.410400 1.535208
1576.410400 1.535508
1576.410400 1.535802
1576.410400 1.536139
1576.410400 1.536473
1576.410400 1.536795
1576.410400 1.537133
1576.410400 1.537463
1576.410400 1.537774
1576.410400 1.538081
1576.410400 1.538359
1576.410400 1.538656
1576.410400 1.538965
1576.410400 1.539278
1576.410400 1.539615
1576.410400 1.539975
1576.410400 1.540375
1576.410400 1.540756
1576.410400 1.541131
1576.410400 1.541493
1576.410400 1.541867
1576.410400 1.542220
1576.410400 1.542568
1576.410400 1.542928
1576.410400 1.543278
1576.410400 1.543655
1576.410400 1.544024
1576.410400 1.544386
1576.410400 1.544741
1576.410400 1.545109
1576.410400 1.545484
1576.410400 1.545853
1576.410400 1.546249
1576.410400 1.546654
1576.410400 1.547022
1576.410400 1.547359
1576.410400 1.547725
1576.410400 1.548068
1576.410400 1.548448
1576.410400 1.548808
1576.410400 1.549156
1576.410400 1.549517
1576.410400 1.549859
1576.410400 1.550177
1576.410400 1.550480
1576.410400 1.550769
1576.410400 1.551035
1576.410400 1.551280
1576.410400 1.551539
1576.410400 1.551840
1576.410400 1.552182
1576.410400 1.552510
1576.410400 1.552840
1576.410400 1.553140
1576.410400 1.553430
1576.410400 1.553710
1576.410400 1.553995
1576.410400 1.554274
1576.410400 1.554568
1576.410400 1.554890
1576.410400 1.555206
1576.410400 1.555526
1576.410400 1.555816
1576.410400 1.556119
1576.410400 1.556420
1599.763672 1.519567
1599.763672 1.519874
1599.763672 1.520210
1599.763672 1.520566
1599.763672 1.520950
1599.763672 1.521351
1599.763672 1.521729
1599.763672 1.522087
1599.763672 1.522423
1599.763672 1.522752
1599.763672 1.523103
1599.763672 1.523444
1599.763672 1.523821
1599.763672 1.524191
1599.763672 1.524573
1599.763672 1.525024
1599.763672 1.525449
1599.763672 1.525845
1599.763672 1.526236
1599.763672 1.526602
1599.763672 1.526977
1599.763672 1.527327
1599.763672 1.527653
1599.763672 1.527976
1599.763672 1.528276
1599.763672 1.528573
1599.763672 1.528846
1599.763672 1.529100
1599.763672 1.529360
1599.763672 1.529605
1599.763672 1.529867
1599.763672 1.530143
1599.763672 1.530414
1599.763672 1.530685
1599.763672 1.530948
1599.763672 1.531185
1599.763672 1.531412
1599.763672 1.531682
1599.763672 1.531994
1599.763672 1.532278
1599.763672 1.532580
1599.763672 1.532898
1599.763672 1.533227
1599.763672 1.533552
1599.763672 1.533896
1599.763672 1.534223
1599.763672 1.534577
1599.763672 1.534912
1599.763672 1.535222
1599.763672 1.535527
1599.763672 1.535844
1599.763672 1.536151
1599.763672 1.536517
1599.763672 1.536867
1599.763672 1.537225
1599.763672 1.537529
1599.763672 1.537806
1599.763672 1.538074
1599.763672 1.538347
1599.763672 1.538633
1599.763672 1.538911
1599.763672 1.539188
1599.763672 1.539487
1599.763672 1.539761
1599.763672 1.540028
1599.763672 1.540326
1599.763672 1.540655
1599.763672 1.540986
1599.763672 1.541313
1599.763672 1.541624
1599.763672 1.541931
1599.763672 1.542199
1599.763672 1.542461
1599.763672 1.542720
1599.763672 1.542991
1599.763672 1.543281
1599.763672 1.543603
1599.763672 1.543897
1599.763672 1.544200
1599.763672 1.544492
1599.763672 1.544801
1599.763672 1.545105
1599.763672 1.545414
1599.763672 1.545706
1599.763672 1.545992
1599.763672 1.546277
1599.763672 1.546557
1599.763672 1.546844
1599.763672 1.547134
1599.763672 1.547437
1599.763672 1.547742
1599.763672 1.548070
1599.763672 1.548394
1599.763672 1.548709
1599.763672 1.549026
1599.763672 1.549318
1599.763672 1.549599
1599.763672 1.549871
1599.763672 1.550171
1599.763672 1.550483
1599.763672 1.550804
1599.763672 1.551091
1599.763672 1.551414
1599.763672 1.551696
1599.763672 1.552015
1599.763672 1.552371
1599.763672 1.552747
1599.763672 1.553147
1599.763672 1.553537
1599.763672 1.553917
1599.763672 1.554326
1599.763672 1.554731
1623.626465 1.487710
1623.626465 1.488105
1623.626465 1.488478
1623.626465 1.488829
1623.626465 1.489170
1623.626465 1.489519
1647.386841 1.480945
1647.386841 1.481269
1647.386841 1.481610
1647.386841 1.481934
1647.386841 1.482297
1647.386841 1.482654
1647.386841 1.482980
1647.386841 1.483290
1647.386841 1.483623
1647.386841 1.483982
1647.386841 1.484300
1647.386841 1.484623
1647.386841 1.484984
1647.386841 1.485304
1647.386841 1.485586
1647.386841 1.485872
1647.386841 1.486140
1647.386841 1.486420
1647.386841 1.486673
1647.386841 1.486928
1647.386841 1.487184
1647.386841 1.487455
1647.386841 1.487739
1647.386841 1.488039
1647.386841 1.488345
1647.386841 1.488630
1647.386841 1.488903
1647.386841 1.489208
1647.386841 1.489495
1647.386841 1.489834
1647.386841 1.490162
1647.386841 1.490482
1647.386841 1.490772
1647.386841 1.491112
1647.386841 1.491439
1647.386841 1.491778
1647.386841 1.492101
1647.386841 1.492451
1647.386841 1.492792
1647.386841 1.493144
1647.386841 1.493501
1647.386841 1.493848
1647.386841 1.494176


==> fig/data/avgq-vs-success-2/banditstd-linf-cdf.tex <==
0.000000 0.289285
1.538462 0.277368
2.608696 0.289178
3.891892 0.293925
4.897959 0.320921
5.901639 0.347615
6.904109 0.369859
8.179775 0.364499
8.897959 0.396675
9.663551 0.429785
9.853211 0.424296
10.178572 0.428605
10.655172 0.422945
10.655172 0.432223
10.655172 0.438714
10.820513 0.442417
11.000000 0.449184
11.193277 0.457409
12.193548 0.437867
12.193548 0.446680
12.634921 0.442655
12.866141 0.444056
13.584616 0.441100
13.584616 0.450931
14.859260 0.439722
16.114286 0.429636
16.114286 0.438036
16.909090 0.434866
17.448277 0.433920
18.000000 0.436734
19.112583 0.429218
19.394737 0.435466
20.538462 0.417295
20.828026 0.422139
21.126583 0.421365
21.126583 0.427309
21.126583 0.432630
21.459120 0.434851
21.459120 0.439270
21.812500 0.439925
22.173914 0.440486
22.173914 0.443338
22.555555 0.441446
22.944786 0.442669
22.944786 0.446529
23.353659 0.442032
23.769697 0.444783
24.610779 0.444267
25.035715 0.448214
25.467455 0.449662
25.905882 0.448977
26.350878 0.451397
26.350878 0.456599
27.271677 0.448798
27.271677 0.451246
27.747126 0.449211
27.747126 0.451740
27.747126 0.454892
27.747126 0.458481
27.747126 0.462718
27.747126 0.466540
28.285715 0.466706
28.829546 0.467902
29.378531 0.467449
29.932585 0.469472
29.932585 0.475829
29.932585 0.481108
29.932585 0.485457
29.932585 0.490755
29.932585 0.496207
29.932585 0.502057
29.932585 0.508570
31.823204 0.502910
32.450550 0.506382
32.450550 0.512373
33.092896 0.508915
33.092896 0.513375
33.750000 0.514248
33.750000 0.519087
35.086021 0.514273
35.086021 0.519706
35.086021 0.526361
35.775402 0.528358
35.775402 0.532878
36.478722 0.536420
37.185184 0.539023
37.185184 0.545690
37.905262 0.546638
38.628273 0.547485
40.072540 0.536559
40.072540 0.541242
40.072540 0.543225
40.814434 0.539135
41.558975 0.528888
41.558975 0.530744
42.316326 0.524672
42.316326 0.526488
43.848484 0.515887
43.848484 0.519023
43.848484 0.521900
43.848484 0.526247
43.848484 0.531752
43.848484 0.536829
43.848484 0.543496
44.673367 0.536551
45.500000 0.538640
45.500000 0.543455
46.338310 0.542566
46.338310 0.547289
46.338310 0.552425
46.338310 0.556840
48.068966 0.552683
48.068966 0.559166
48.068966 0.565884
48.068966 0.571635
49.843903 0.566639
50.728157 0.564712
51.613525 0.555755
52.500000 0.550768
52.500000 0.553489
52.500000 0.555230
53.406700 0.556003
53.406700 0.558727
53.406700 0.562492
54.333332 0.562849
54.333332 0.565663
55.270142 0.566179
55.270142 0.569388
56.216980 0.566879
57.164318 0.566045
59.981480 0.546846
61.834862 0.538216
61.834862 0.542990
63.690910 0.531547
64.615387 0.531654
64.615387 0.534814
64.615387 0.539238
64.615387 0.544428
64.615387 0.549427
65.576576 0.549527
65.576576 0.554240
65.576576 0.557631
65.576576 0.562407
66.565025 0.544529
66.565025 0.550017
67.562500 0.552152
67.562500 0.556271
67.562500 0.560638
68.577774 0.563056
68.577774 0.567831
68.577774 0.571442
69.610619 0.557886
69.610619 0.563072
69.610619 0.569243
70.660789 0.571514
70.660789 0.576029
70.660789 0.581473
70.660789 0.586594
71.736839 0.580927
73.878258 0.573914
74.943726 0.564812
76.008621 0.555738
76.008621 0.559135
76.008621 0.561399
76.008621 0.564456
76.008621 0.567233
76.008621 0.572839
77.115883 0.567425
77.115883 0.570914
79.336174 0.560902
81.535866 0.544382
81.535866 0.547590
81.535866 0.550205
81.535866 0.551411
82.655464 0.546159
82.655464 0.546878
83.782425 0.539079
84.908333 0.537345
84.908333 0.538132
86.041496 0.532791
87.173553 0.527883
87.173553 0.530028
88.312759 0.529767
88.312759 0.533090
89.459015 0.528571
89.459015 0.533075
89.459015 0.536540
89.459015 0.540287
89.459015 0.544083
89.459015 0.547377
89.459015 0.550855
89.459015 0.554355
91.853661 0.542233
91.853661 0.544648
91.853661 0.546640
91.853661 0.549652
91.853661 0.552490
94.290321 0.546726
95.502007 0.539144
95.502007 0.542509
95.502007 0.545109
95.502007 0.547681
95.502007 0.551527
95.502007 0.555376
95.502007 0.558684
95.502007 0.561832
95.502007 0.565062
95.502007 0.568404
95.502007 0.571290
95.502007 0.573940
96.800003 0.575617
96.800003 0.578282
98.103584 0.576421
99.404762 0.569607
99.404762 0.572313
99.404762 0.574568
99.404762 0.577985
100.727272 0.561747
102.047241 0.557609
102.047241 0.561115
102.047241 0.563979
102.047241 0.565726
102.047241 0.568541
102.047241 0.569833
102.047241 0.571233
102.047241 0.571596
102.047241 0.572251
102.047241 0.572763
102.047241 0.575414
102.047241 0.579342
103.450981 0.577491
103.450981 0.579761
103.450981 0.582475
103.450981 0.584931
103.450981 0.588382
103.450981 0.592906
103.450981 0.596529
104.898438 0.595267
104.898438 0.597746
106.350197 0.594982
106.350197 0.596402
106.350197 0.597853
106.350197 0.599592
106.350197 0.601355
106.350197 0.604025
106.350197 0.608383
106.350197 0.612887
107.852715 0.606293
109.351349 0.586096
109.351349 0.589637
109.351349 0.593284
110.861542 0.581709
110.861542 0.584191
110.861542 0.587708
110.861542 0.590387
110.861542 0.592562
112.398468 0.583917
112.398468 0.587949
112.398468 0.592243
112.398468 0.594569
112.398468 0.596200
113.961830 0.576273
113.961830 0.578545
113.961830 0.579867
113.961830 0.582798
113.961830 0.584373
113.961830 0.585724
113.961830 0.588176
113.961830 0.588619
113.961830 0.588700
113.961830 0.589244
115.589355 0.587516
115.589355 0.587364
115.589355 0.589102
117.227272 0.587398
117.227272 0.588892
117.227272 0.590449
117.227272 0.591600
118.883018 0.589473
120.533836 0.581932
122.179779 0.571878
122.179779 0.572829
122.179779 0.573972
122.179779 0.576185
122.179779 0.577314
122.179779 0.579361
122.179779 0.581817
122.179779 0.584869
122.179779 0.587244
122.179779 0.588035
123.888062 0.585558
123.888062 0.586625
123.888062 0.587177
125.605949 0.565434
125.605949 0.567129
125.605949 0.568615
125.605949 0.570176
125.605949 0.571404
125.605949 0.573258
125.605949 0.577919
127.362961 0.577397
129.114395 0.576460
129.114395 0.580685
129.114395 0.585904
129.114395 0.590436
129.114395 0.593724
129.114395 0.597979
130.897064 0.595830
130.897064 0.599089
130.897064 0.601153
130.897064 0.603026
130.897064 0.603907
130.897064 0.604551
130.897064 0.605489
130.897064 0.606176
130.897064 0.606814
130.897064 0.609262
130.897064 0.610709
130.897064 0.612940
130.897064 0.615452
130.897064 0.618552
132.769226 0.607465
132.769226 0.609072
134.642334 0.609166
134.642334 0.611239
136.516357 0.610981
136.516357 0.611391
136.516357 0.611443
136.516357 0.611334
136.516357 0.609427
136.516357 0.609142
136.516357 0.607511
136.516357 0.607615
136.516357 0.607133
138.442032 0.598371
138.442032 0.598948
138.442032 0.600953
138.442032 0.604068
138.442032 0.607451
138.442032 0.610849
138.442032 0.614541
140.404327 0.598853
140.404327 0.601660
140.404327 0.602107
140.404327 0.605267
140.404327 0.609612
140.404327 0.612086
140.404327 0.615255
140.404327 0.620205
140.404327 0.624368
140.404327 0.627577
140.404327 0.630364
140.404327 0.633813
140.404327 0.636894
140.404327 0.639899
142.453232 0.622483
142.453232 0.626291
142.453232 0.631451
142.453232 0.634912
144.516129 0.621120
144.516129 0.623572
144.516129 0.625930
146.585709 0.617570
146.585709 0.621429
146.585709 0.625097
146.585709 0.629184
146.585709 0.634396
146.585709 0.640199
146.585709 0.645247
146.585709 0.648442
146.585709 0.652441
148.704620 0.653613
148.704620 0.655344
148.704620 0.656960
148.704620 0.659010
148.704620 0.662122
148.704620 0.663481
148.704620 0.664734
148.704620 0.664313
148.704620 0.664427
148.704620 0.663198
150.879425 0.661579
150.879425 0.661097
150.879425 0.663409
150.879425 0.666260
150.879425 0.669067
150.879425 0.672002
153.081268 0.655745
153.081268 0.657061
155.281693 0.651718
155.281693 0.650929
157.480698 0.630808
157.480698 0.631828
157.480698 0.631680
157.480698 0.633206
157.480698 0.633528
157.480698 0.634369
159.706299 0.632947
161.923340 0.623826
161.923340 0.626385
161.923340 0.628704
161.923340 0.631225
161.923340 0.634037
161.923340 0.637445
161.923340 0.640558
161.923340 0.643391
161.923340 0.645317
161.923340 0.648585
164.194443 0.639582
164.194443 0.641417
166.463669 0.638778
166.463669 0.638842
166.463669 0.640362
166.463669 0.641294
166.463669 0.644797
166.463669 0.648551
171.037796 0.648542
173.308212 0.644753
173.308212 0.647024
173.308212 0.649919
173.308212 0.651839
173.308212 0.653760
173.308212 0.656681
173.308212 0.658773
173.308212 0.662458
173.308212 0.665244
173.308212 0.668974
173.308212 0.671642
173.308212 0.675069
173.308212 0.679172
173.308212 0.681962
173.308212 0.684634
173.308212 0.686890
173.308212 0.688424
173.308212 0.690018
173.308212 0.689727
173.308212 0.691031
173.308212 0.692717
173.308212 0.693605
173.308212 0.695941
173.308212 0.698228
173.308212 0.699679
173.308212 0.701239
175.740616 0.693320
175.740616 0.695635
175.740616 0.696705
175.740616 0.699199
175.740616 0.699775
178.190475 0.683960
178.190475 0.687179
178.190475 0.690599
178.190475 0.694537
178.190475 0.697777
178.190475 0.700828
178.190475 0.702362
178.190475 0.704412
180.677963 0.684266
180.677963 0.686956
180.677963 0.688624
180.677963 0.688043
183.175674 0.684798
183.175674 0.685283
183.175674 0.687844
183.175674 0.688338
185.683502 0.685654
188.181213 0.667346
188.181213 0.666703
188.181213 0.666059
188.181213 0.666506
188.181213 0.666171
188.181213 0.667812
188.181213 0.669684
188.181213 0.670456
190.715714 0.654697
190.715714 0.656918
193.246674 0.657474
193.246674 0.659164
195.774094 0.660586
195.774094 0.664482
195.774094 0.667715
198.304642 0.662677
198.304642 0.665402
198.304642 0.667896
198.304642 0.670608
198.304642 0.675700
198.304642 0.680158
198.304642 0.683262
200.864685 0.680026
200.864685 0.683010
200.864685 0.687352
200.864685 0.691121
200.864685 0.692668
200.864685 0.693262
200.864685 0.695009
200.864685 0.698376
203.460526 0.694574
203.460526 0.698173
206.052460 0.695780
206.052460 0.699542
206.052460 0.701729
206.052460 0.703185
206.052460 0.705058
206.052460 0.705721
206.052460 0.705502
206.052460 0.706385
208.679733 0.704387
211.296417 0.695722
211.296417 0.696977
211.296417 0.697561
213.915588 0.677559
213.915588 0.679339
213.915588 0.680772
213.915588 0.682031
213.915588 0.683014
213.915588 0.685197
213.915588 0.688281
213.915588 0.692247
213.915588 0.697022
219.219360 0.688534
219.219360 0.691006
219.219360 0.694614
219.219360 0.698492
219.219360 0.701465
219.219360 0.704402
219.219360 0.707639
219.219360 0.712864
219.219360 0.714982
219.219360 0.720151
219.219360 0.723257
219.219360 0.726364
219.219360 0.728686
219.219360 0.731445
219.219360 0.734270
219.219360 0.737399
219.219360 0.740659
219.219360 0.744981
219.219360 0.746572
219.219360 0.749228
221.974274 0.747075
224.717941 0.743825
224.717941 0.748177
224.717941 0.751413
224.717941 0.753248
224.717941 0.755513
224.717941 0.758699
230.229294 0.724611
230.229294 0.726954
232.971436 0.705887
232.971436 0.708785
232.971436 0.711267
232.971436 0.714816
232.971436 0.717739
235.727844 0.696257
238.473190 0.691973
238.473190 0.694107
238.473190 0.697737
238.473190 0.700052
238.473190 0.703650
241.232712 0.692585
241.232712 0.695903
241.232712 0.696557
241.232712 0.696693
241.232712 0.697149
241.232712 0.700350
241.232712 0.701541
241.232712 0.702631
241.232712 0.703284
241.232712 0.702169
241.232712 0.700963
241.232712 0.700873
241.232712 0.700879
241.232712 0.701121
241.232712 0.702579
241.232712 0.705043
241.232712 0.707445
241.232712 0.709587
241.232712 0.711136
241.232712 0.713682
241.232712 0.717324
241.232712 0.721810
241.232712 0.725712
241.232712 0.731068
241.232712 0.734911
241.232712 0.739440
241.232712 0.742171
241.232712 0.745805
241.232712 0.750677
241.232712 0.751627
244.163010 0.737686
244.163010 0.737252
244.163010 0.737459
244.163010 0.737223
244.163010 0.738298
244.163010 0.738521
244.163010 0.739818
244.163010 0.740070
244.163010 0.740998
244.163010 0.740946
244.163010 0.741272
247.143753 0.723415
247.143753 0.725576
247.143753 0.727495
247.143753 0.729639
247.143753 0.733065
250.137070 0.706987
250.137070 0.707969
250.137070 0.710527
250.137070 0.712212
250.137070 0.713049
250.137070 0.714117
250.137070 0.715527
250.137070 0.717162
250.137070 0.722040
250.137070 0.724993
253.173920 0.701163
253.173920 0.702631
253.173920 0.703105
253.173920 0.702165
253.173920 0.704320
253.173920 0.705370
253.173920 0.708817
253.173920 0.709737
253.173920 0.710497
253.173920 0.710625
253.173920 0.709817
253.173920 0.710313
253.173920 0.710739
253.173920 0.711776
253.173920 0.713829
256.284821 0.692814
256.284821 0.696036
256.284821 0.697757
256.284821 0.700639
256.284821 0.702573
256.284821 0.705225
256.284821 0.707182
256.284821 0.707012
256.284821 0.707385
256.284821 0.705354
256.284821 0.706251
256.284821 0.707782
256.284821 0.707620
256.284821 0.709601
256.284821 0.712254
256.284821 0.714944
256.284821 0.717647
256.284821 0.720917
256.284821 0.724290
256.284821 0.726511
256.284821 0.728536
262.707703 0.708565
262.707703 0.711667
262.707703 0.713807
262.707703 0.717411
262.707703 0.721130
262.707703 0.723158
262.707703 0.725399
262.707703 0.727448
262.707703 0.728769
262.707703 0.728969
265.950928 0.722107
265.950928 0.724428
265.950928 0.725453
265.950928 0.724676
265.950928 0.726211
265.950928 0.728450
265.950928 0.730275
265.950928 0.730383
265.950928 0.731418
265.950928 0.731254
265.950928 0.731350
269.241577 0.726063
269.241577 0.726367
269.241577 0.726584
272.530487 0.718056
272.530487 0.720293
272.530487 0.722573
272.530487 0.724663
272.530487 0.726605
272.530487 0.728608
272.530487 0.731098
272.530487 0.732535
272.530487 0.735222
272.530487 0.737898
272.530487 0.739590
272.530487 0.742537
272.530487 0.745641
272.530487 0.749368
272.530487 0.752900
272.530487 0.755440
272.530487 0.756897
272.530487 0.759260
272.530487 0.761122
272.530487 0.762817
272.530487 0.765166
272.530487 0.768148
272.530487 0.769778
272.530487 0.769639
272.530487 0.770596
272.530487 0.773021
275.957458 0.775978
275.957458 0.775741
279.375763 0.758800
279.375763 0.758856
279.375763 0.758973
279.375763 0.759629
279.375763 0.760945
279.375763 0.763554
282.809662 0.726590
282.809662 0.728284
282.809662 0.729525
282.809662 0.729714
282.809662 0.732155
282.809662 0.735914
282.809662 0.738254
282.809662 0.739981
282.809662 0.741688
282.809662 0.742360
282.809662 0.742105
282.809662 0.744087
282.809662 0.745080
282.809662 0.746402
286.307220 0.719788
286.307220 0.720257
286.307220 0.722067
286.307220 0.723334
286.307220 0.724929
286.307220 0.727414
286.307220 0.728891
286.307220 0.730562
286.307220 0.732099
286.307220 0.734997
286.307220 0.737878
286.307220 0.743735
286.307220 0.748076
286.307220 0.751385
286.307220 0.755588
286.307220 0.758344
286.307220 0.758536
286.307220 0.758524
286.307220 0.759011
289.897888 0.752326
289.897888 0.753026
289.897888 0.753355
289.897888 0.753119
289.897888 0.752730
289.897888 0.753707
289.897888 0.755071
289.897888 0.758912
289.897888 0.760183
289.897888 0.763103
293.526947 0.761277
293.526947 0.762796
293.526947 0.763940
293.526947 0.762053
293.526947 0.762876
293.526947 0.762065
293.526947 0.763289
293.526947 0.763063
293.526947 0.763786
293.526947 0.765232
293.526947 0.766075
293.526947 0.766715
293.526947 0.767641
293.526947 0.766447
293.526947 0.766434
293.526947 0.768505
293.526947 0.769928
293.526947 0.773252
293.526947 0.774997
293.526947 0.775831
293.526947 0.776062
293.526947 0.776294
293.526947 0.777035
293.526947 0.778760
293.526947 0.780719
293.526947 0.783408
293.526947 0.786383
293.526947 0.789037
301.053558 0.774866
301.053558 0.775552
301.053558 0.777037
301.053558 0.777552
301.053558 0.779411
301.053558 0.780936
301.053558 0.782587
301.053558 0.784524
301.053558 0.786245
301.053558 0.788571
301.053558 0.790478
301.053558 0.792117
301.053558 0.793136
304.860535 0.773703
304.860535 0.776039
304.860535 0.779636
304.860535 0.783268
304.860535 0.785785
304.860535 0.788030
304.860535 0.789782
304.860535 0.791450
304.860535 0.792784
304.860535 0.793075
304.860535 0.793637
304.860535 0.794890
304.860535 0.795830
304.860535 0.796273
304.860535 0.796516
304.860535 0.799059
304.860535 0.801099
304.860535 0.803425
304.860535 0.806184
304.860535 0.807436
304.860535 0.809382
308.769226 0.793724
308.769226 0.794889
308.769226 0.797291
308.769226 0.799003
308.769226 0.802310
308.769226 0.807358
308.769226 0.809506
308.769226 0.813040
308.769226 0.815757
308.769226 0.818079
308.769226 0.820167
308.769226 0.821909
308.769226 0.823924
308.769226 0.825592
308.769226 0.826753
308.769226 0.827330
308.769226 0.827758
308.769226 0.827523
308.769226 0.827836
308.769226 0.829990
308.769226 0.831388
308.769226 0.834864
312.784668 0.811814
312.784668 0.815685
312.784668 0.818633
312.784668 0.821346
312.784668 0.826096
312.784668 0.829577
312.784668 0.830170
312.784668 0.830543
312.784668 0.831293
312.784668 0.832183
316.835297 0.788457
316.835297 0.788808
316.835297 0.787621
316.835297 0.787443
316.835297 0.785993
316.835297 0.784732
316.835297 0.784082
316.835297 0.783291
316.835297 0.782292
316.835297 0.782177
316.835297 0.782973
316.835297 0.784867
316.835297 0.786417
316.835297 0.787630
316.835297 0.788715
316.835297 0.790204
316.835297 0.790648
316.835297 0.792016
316.835297 0.794176
316.835297 0.794640
320.979462 0.768188
320.979462 0.767763
320.979462 0.768653
320.979462 0.768095
320.979462 0.768127
320.979462 0.769082
320.979462 0.769000
320.979462 0.767527
320.979462 0.766866
320.979462 0.768463
320.979462 0.768238
320.979462 0.767719
320.979462 0.768264
320.979462 0.770061
320.979462 0.771045
320.979462 0.772129
320.979462 0.775392
320.979462 0.777981
320.979462 0.779805
320.979462 0.779931
320.979462 0.779958
320.979462 0.779771
320.979462 0.779907
320.979462 0.783438
320.979462 0.784274
320.979462 0.785802
320.979462 0.785216
320.979462 0.787167
320.979462 0.787732
320.979462 0.788758
320.979462 0.792686
320.979462 0.796488
320.979462 0.799824
320.979462 0.800582
320.979462 0.802198
320.979462 0.802747
320.979462 0.804710
320.979462 0.807308
320.979462 0.809868
320.979462 0.811750
320.979462 0.813733
320.979462 0.816737
320.979462 0.821576
320.979462 0.825291
320.979462 0.829583
320.979462 0.834208
325.368408 0.788523
325.368408 0.790312
325.368408 0.790654
325.368408 0.789968
325.368408 0.788178
325.368408 0.787787
325.368408 0.787323
325.368408 0.786959
325.368408 0.787963
325.368408 0.787048
325.368408 0.785111
325.368408 0.784857
325.368408 0.785838
325.368408 0.786419
325.368408 0.790356
325.368408 0.793816
325.368408 0.796224
325.368408 0.797793
325.368408 0.798934
325.368408 0.799295
325.368408 0.802106
325.368408 0.804751
325.368408 0.805338
325.368408 0.804480
325.368408 0.804157
325.368408 0.802568
325.368408 0.800982
325.368408 0.800123
325.368408 0.800674
325.368408 0.802104
325.368408 0.802011
325.368408 0.803976
325.368408 0.806589
325.368408 0.807422
325.368408 0.808346
325.368408 0.810934
325.368408 0.811946
325.368408 0.813603
325.368408 0.816715
329.959198 0.813731
329.959198 0.818916
329.959198 0.822506
329.959198 0.826002
329.959198 0.827882
329.959198 0.828587
329.959198 0.829359
329.959198 0.832208
329.959198 0.834754
329.959198 0.838839
329.959198 0.842055
329.959198 0.844963
329.959198 0.844453
329.959198 0.846725
329.959198 0.847034
329.959198 0.849514
329.959198 0.852118
334.622101 0.808134
334.622101 0.808919
334.622101 0.812642
334.622101 0.815811
334.622101 0.819822
334.622101 0.824269
334.622101 0.826496
334.622101 0.827668
334.622101 0.827751
334.622101 0.827043
334.622101 0.826898
334.622101 0.826268
334.622101 0.826743
334.622101 0.826855
334.622101 0.827031
334.622101 0.828507
334.622101 0.828391
334.622101 0.829944
334.622101 0.831292
334.622101 0.830151
334.622101 0.830016
334.622101 0.829358
334.622101 0.829673
334.622101 0.830619
334.622101 0.832972
334.622101 0.835622
334.622101 0.838539
334.622101 0.843157
334.622101 0.846070
334.622101 0.850140
334.622101 0.853968
334.622101 0.857862
334.622101 0.861957
334.622101 0.866436
334.622101 0.870247
334.622101 0.875260
334.622101 0.879947
334.622101 0.884529
334.622101 0.887917
334.622101 0.892648
334.622101 0.897860
334.622101 0.903117
334.622101 0.904722
334.622101 0.905461
334.622101 0.905899
334.622101 0.905483
334.622101 0.905762
334.622101 0.905338
334.622101 0.906593
334.622101 0.906453
334.622101 0.904579
334.622101 0.902984
334.622101 0.902875
334.622101 0.904344
334.622101 0.906376
334.622101 0.908957
334.622101 0.912670
339.588409 0.857464
339.588409 0.860917
339.588409 0.864626
339.588409 0.867609
339.588409 0.869207
339.588409 0.870482
339.588409 0.869856
339.588409 0.870525
339.588409 0.872291
339.588409 0.873316
339.588409 0.875668
339.588409 0.877021
339.588409 0.877670
339.588409 0.877158
339.588409 0.877697
339.588409 0.878343
339.588409 0.878910
339.588409 0.879484
339.588409 0.880545
339.588409 0.879844
339.588409 0.879428
339.588409 0.881015
339.588409 0.884127
339.588409 0.887785
339.588409 0.889303
339.588409 0.892430
339.588409 0.896622
344.682068 0.868150
344.682068 0.871412
344.682068 0.872737
344.682068 0.876996
344.682068 0.881565
344.682068 0.886489
344.682068 0.891379
344.682068 0.894654
344.682068 0.898019
344.682068 0.899907
344.682068 0.901989
344.682068 0.902444
344.682068 0.903497
349.821320 0.862826
349.821320 0.864363
349.821320 0.866543
349.821320 0.868890
349.821320 0.869961
349.821320 0.870403
349.821320 0.870200
349.821320 0.870188
349.821320 0.870196
349.821320 0.870881
349.821320 0.870864
349.821320 0.870650
349.821320 0.872095
349.821320 0.871906
349.821320 0.872299
349.821320 0.871581
349.821320 0.871482
349.821320 0.871599
349.821320 0.871674
349.821320 0.869648
349.821320 0.870881
349.821320 0.869643
349.821320 0.868919
355.063232 0.849335
355.063232 0.850994
360.286530 0.839099
360.286530 0.839858
360.286530 0.840889
360.286530 0.841887
360.286530 0.842961
365.508575 0.820991
365.508575 0.821477
365.508575 0.823129
365.508575 0.826151
365.508575 0.829799
365.508575 0.832775
370.735046 0.816066
370.735046 0.817067
370.735046 0.817303
370.735046 0.819518
370.735046 0.822167
370.735046 0.825789
375.965912 0.812654
375.965912 0.814511
375.965912 0.818504
375.965912 0.821207
375.965912 0.824199
375.965912 0.825186
375.965912 0.826406
375.965912 0.826594
375.965912 0.826363
375.965912 0.827779
375.965912 0.827299
375.965912 0.827015
375.965912 0.827542
375.965912 0.828214
375.965912 0.829497
375.965912 0.829633
375.965912 0.828641
375.965912 0.828542
375.965912 0.828586
375.965912 0.829873
375.965912 0.830686
375.965912 0.829335
375.965912 0.828248
375.965912 0.829712
375.965912 0.831214
375.965912 0.831923
375.965912 0.832624
375.965912 0.833388
375.965912 0.833380
375.965912 0.834716
375.965912 0.833512
375.965912 0.831354
375.965912 0.830217
375.965912 0.829369
375.965912 0.827020
375.965912 0.824769
375.965912 0.824124
375.965912 0.822473
375.965912 0.821604
375.965912 0.820620
375.965912 0.820335
375.965912 0.820062
375.965912 0.820063
375.965912 0.819942
375.965912 0.820386
375.965912 0.822992
375.965912 0.825634
375.965912 0.828479
381.439087 0.781484
381.439087 0.782974
386.892670 0.734915
386.892670 0.736940
386.892670 0.739357
386.892670 0.740386
386.892670 0.741417
386.892670 0.740233
386.892670 0.739639
386.892670 0.740934
386.892670 0.741179
392.366211 0.684203
392.366211 0.686332
392.366211 0.688518
392.366211 0.688137
392.366211 0.688540
392.366211 0.689303
392.366211 0.689598
392.366211 0.691112
392.366211 0.693603
392.366211 0.695503
392.366211 0.698314
392.366211 0.700922
392.366211 0.704007
392.366211 0.705793
392.366211 0.706613
392.366211 0.707678
392.366211 0.707600
392.366211 0.708912
392.366211 0.709495
392.366211 0.709373
392.366211 0.709720
392.366211 0.710612
392.366211 0.710716
392.366211 0.712130
392.366211 0.713586
392.366211 0.715848
392.366211 0.716419
392.366211 0.716422
392.366211 0.717837
392.366211 0.719663
392.366211 0.720187
392.366211 0.721946
392.366211 0.723364
392.366211 0.725726
392.366211 0.727790
392.366211 0.729616
392.366211 0.730879
392.366211 0.733653
392.366211 0.737209
392.366211 0.740178
392.366211 0.742230
392.366211 0.744226
392.366211 0.749307
392.366211 0.754359
392.366211 0.758802
392.366211 0.762928
392.366211 0.766562
392.366211 0.769860
392.366211 0.771274
392.366211 0.774197
392.366211 0.776171
392.366211 0.780364
398.101135 0.722012
398.101135 0.724033
398.101135 0.725994
398.101135 0.727633
398.101135 0.728633
398.101135 0.727841
398.101135 0.729028
398.101135 0.730083
398.101135 0.732218
398.101135 0.733390
398.101135 0.735791
398.101135 0.737616
398.101135 0.740306
398.101135 0.742977
398.101135 0.746443
398.101135 0.746957
398.101135 0.749753
398.101135 0.749992
398.101135 0.750324
398.101135 0.752690
398.101135 0.753741
398.101135 0.753724
398.101135 0.753423
398.101135 0.752577
398.101135 0.752600
398.101135 0.753612
398.101135 0.753753
398.101135 0.753551
398.101135 0.753161
398.101135 0.751591
398.101135 0.750268
398.101135 0.750272
398.101135 0.750217
398.101135 0.750390
398.101135 0.752154
398.101135 0.754052
398.101135 0.756819
398.101135 0.759198
398.101135 0.762208
398.101135 0.763602
398.101135 0.765651
398.101135 0.765647
398.101135 0.765538
398.101135 0.765922
398.101135 0.767102
398.101135 0.767064
398.101135 0.768148
398.101135 0.769997
398.101135 0.771658
398.101135 0.771950
398.101135 0.771167
398.101135 0.770323
398.101135 0.770990
398.101135 0.772596
404.106445 0.715929
404.106445 0.717228
404.106445 0.716787
404.106445 0.717853
404.106445 0.719010
404.106445 0.719541
404.106445 0.720694
404.106445 0.721502
404.106445 0.722736
404.106445 0.725578
404.106445 0.728208
404.106445 0.729578
404.106445 0.732488
404.106445 0.734332
404.106445 0.735182
404.106445 0.734900
404.106445 0.735579
404.106445 0.736165
404.106445 0.738968
404.106445 0.740439
404.106445 0.742395
404.106445 0.745073
404.106445 0.747626
404.106445 0.748645
404.106445 0.747382
404.106445 0.750181
404.106445 0.750803
404.106445 0.752379
404.106445 0.752443
404.106445 0.751519
404.106445 0.751219
404.106445 0.751706
404.106445 0.751494
404.106445 0.751610
404.106445 0.750241
404.106445 0.751023
404.106445 0.751473
404.106445 0.750942
404.106445 0.752734
404.106445 0.753871
404.106445 0.755380
404.106445 0.756238
404.106445 0.756826
404.106445 0.756604
404.106445 0.755253
404.106445 0.756967
404.106445 0.758151
404.106445 0.758818
404.106445 0.759246
404.106445 0.758750
404.106445 0.760202
404.106445 0.761322
404.106445 0.763843
404.106445 0.765087
404.106445 0.768260
404.106445 0.770338
404.106445 0.773502
404.106445 0.775027
404.106445 0.776940
404.106445 0.776696
404.106445 0.773209
404.106445 0.772593
404.106445 0.773713
404.106445 0.775595
404.106445 0.773692
404.106445 0.772391
404.106445 0.773321
404.106445 0.774955
404.106445 0.777265
404.106445 0.777713
404.106445 0.776918
404.106445 0.778018
404.106445 0.778793
404.106445 0.779250
404.106445 0.780684
404.106445 0.782548
404.106445 0.785700
404.106445 0.786495
404.106445 0.787805
404.106445 0.788989
404.106445 0.788381
404.106445 0.788154
404.106445 0.789849
404.106445 0.791928
404.106445 0.794214
404.106445 0.796219
404.106445 0.798373
404.106445 0.798147
410.569824 0.763306
410.569824 0.766859
410.569824 0.771191
410.569824 0.774981
410.569824 0.777095
410.569824 0.778178
410.569824 0.779053
410.569824 0.779211
410.569824 0.777331
410.569824 0.775082
410.569824 0.774259
410.569824 0.770983
410.569824 0.767994
410.569824 0.764955
410.569824 0.761482
410.569824 0.758097
410.569824 0.754840
410.569824 0.752752
410.569824 0.752793
410.569824 0.753547
410.569824 0.752864
410.569824 0.752019
410.569824 0.752091
410.569824 0.753022
410.569824 0.753456
410.569824 0.753635
410.569824 0.754062
410.569824 0.755000
410.569824 0.756295
410.569824 0.758480
410.569824 0.759465
417.169922 0.737559
417.169922 0.737834
417.169922 0.737347
417.169922 0.738073
417.169922 0.737072
417.169922 0.737314
417.169922 0.738346
417.169922 0.740038
417.169922 0.741454
417.169922 0.743052
417.169922 0.742062
417.169922 0.740828
417.169922 0.741103
417.169922 0.740855
417.169922 0.739664
417.169922 0.738854
417.169922 0.737494
417.169922 0.735184
417.169922 0.732975
417.169922 0.732488
417.169922 0.732504
417.169922 0.732743
417.169922 0.732283
417.169922 0.731418
417.169922 0.732437
417.169922 0.733081
417.169922 0.734068
417.169922 0.733318
417.169922 0.732848
417.169922 0.731870
417.169922 0.731949
417.169922 0.731947
417.169922 0.731241
417.169922 0.731494
417.169922 0.732775
417.169922 0.735470
417.169922 0.737887
417.169922 0.739995
417.169922 0.740718
417.169922 0.741864
417.169922 0.742667
417.169922 0.744958
417.169922 0.747455
417.169922 0.749844
417.169922 0.750481
417.169922 0.752388
417.169922 0.753548
417.169922 0.753300
417.169922 0.753920
417.169922 0.755266
417.169922 0.758053
417.169922 0.762688
417.169922 0.766556
417.169922 0.770252
417.169922 0.773792
417.169922 0.777305
417.169922 0.782424
417.169922 0.788811
417.169922 0.797119
417.169922 0.804557
417.169922 0.811414
417.169922 0.816956
417.169922 0.822326
417.169922 0.827798
417.169922 0.832622
417.169922 0.837365
417.169922 0.841042
417.169922 0.843135
417.169922 0.846064
417.169922 0.852350
417.169922 0.856877
417.169922 0.860823
417.169922 0.863126
417.169922 0.866098
417.169922 0.869097
417.169922 0.870253
417.169922 0.872005
417.169922 0.870955
417.169922 0.869997
417.169922 0.869441
417.169922 0.869515
417.169922 0.870317
417.169922 0.870134
417.169922 0.869287
417.169922 0.867448
417.169922 0.867154
417.169922 0.869010
417.169922 0.871112
417.169922 0.872759
417.169922 0.873196
417.169922 0.872972
417.169922 0.873176
417.169922 0.873845
417.169922 0.874459
417.169922 0.876936
417.169922 0.880393
417.169922 0.881978
417.169922 0.882232
417.169922 0.883983
417.169922 0.885867
417.169922 0.887589
417.169922 0.890784
417.169922 0.889879
417.169922 0.891095
417.169922 0.893249
417.169922 0.898478
417.169922 0.904373
417.169922 0.907230
424.333344 0.877615
424.333344 0.877781
424.333344 0.875350
424.333344 0.874724
424.333344 0.873478
424.333344 0.871662
424.333344 0.870566
424.333344 0.869976
424.333344 0.870359
424.333344 0.868124
424.333344 0.864512
424.333344 0.861963
424.333344 0.859739
424.333344 0.858048
424.333344 0.856209
424.333344 0.856752
424.333344 0.858608
424.333344 0.860215
424.333344 0.862102
424.333344 0.863705
424.333344 0.864681
424.333344 0.866530
424.333344 0.868420
424.333344 0.868938
424.333344 0.868723
424.333344 0.868762
424.333344 0.867808
424.333344 0.866776
424.333344 0.865694
424.333344 0.865118
424.333344 0.865404
424.333344 0.865260
424.333344 0.864550
424.333344 0.865300
424.333344 0.864454
424.333344 0.865009
424.333344 0.864288
424.333344 0.863835
424.333344 0.865516
424.333344 0.868864
424.333344 0.871481
424.333344 0.873386
424.333344 0.875504
424.333344 0.876653
424.333344 0.877906
424.333344 0.882485
424.333344 0.885662
424.333344 0.887304
424.333344 0.886930
424.333344 0.890131
424.333344 0.892443
424.333344 0.893315
424.333344 0.894474
424.333344 0.898054
424.333344 0.902370
424.333344 0.907000
424.333344 0.909780
424.333344 0.912876
424.333344 0.916115
424.333344 0.918194
424.333344 0.922478
424.333344 0.925702
424.333344 0.929765
424.333344 0.934328
424.333344 0.936615
424.333344 0.939548
424.333344 0.941374
424.333344 0.944044
424.333344 0.944758
424.333344 0.945692
424.333344 0.943807
424.333344 0.943242
424.333344 0.942889
424.333344 0.941389
424.333344 0.940840
424.333344 0.944699
424.333344 0.947625
424.333344 0.949353
424.333344 0.951662
424.333344 0.954936
431.900269 0.960635
431.900269 0.963425
431.900269 0.966634
439.441986 0.964806
439.441986 0.965326
439.441986 0.964224
439.441986 0.963951
439.441986 0.964760
439.441986 0.965784
439.441986 0.967172
439.441986 0.966126
439.441986 0.963948
439.441986 0.962600
439.441986 0.959887
439.441986 0.958652
439.441986 0.958228
439.441986 0.957598
439.441986 0.960970
439.441986 0.964373
439.441986 0.968013
439.441986 0.969868
439.441986 0.972311
439.441986 0.975241
439.441986 0.978115
439.441986 0.981998
439.441986 0.986054
439.441986 0.988012
439.441986 0.990353
439.441986 0.991482
439.441986 0.992418
439.441986 0.990767
439.441986 0.990537
439.441986 0.993976
439.441986 0.997131
439.441986 0.999857
447.118469 0.984764
447.118469 0.984129
447.118469 0.984440
447.118469 0.982922
447.118469 0.981485
447.118469 0.977997
447.118469 0.976834
447.118469 0.977980
447.118469 0.979648
447.118469 0.980229
447.118469 0.982012
447.118469 0.982602
447.118469 0.983293
447.118469 0.983216
447.118469 0.981697
447.118469 0.980208
447.118469 0.980270
447.118469 0.979203
447.118469 0.980152
447.118469 0.979676
447.118469 0.981409
447.118469 0.983165
447.118469 0.987269
447.118469 0.990909
447.118469 0.993609
447.118469 0.996648
447.118469 0.998024
447.118469 1.001582
447.118469 1.003572
447.118469 1.005370
447.118469 1.004997
447.118469 1.004074
447.118469 1.001514
447.118469 1.001168
447.118469 1.001736
447.118469 1.003111
447.118469 1.002710
447.118469 1.002973
447.118469 0.999886
447.118469 0.998352
447.118469 0.997512
447.118469 0.995183
447.118469 0.993436
447.118469 0.993513
447.118469 0.992112
447.118469 0.991685
447.118469 0.992381
447.118469 0.992584
447.118469 0.992343
447.118469 0.994445
447.118469 0.995374
447.118469 0.996883
447.118469 0.997488
447.118469 0.999513
447.118469 0.999813
447.118469 1.000794
447.118469 0.999688
447.118469 0.999418
447.118469 1.001368
455.076935 1.000132
455.076935 1.003968
455.076935 1.005324
455.076935 1.009021
455.076935 1.012534
455.076935 1.013830
455.076935 1.016341
455.076935 1.018658
455.076935 1.018529
455.076935 1.017908
455.076935 1.017585
455.076935 1.018593
455.076935 1.019969
455.076935 1.020810
455.076935 1.022172
455.076935 1.023664
455.076935 1.025690
455.076935 1.028296
455.076935 1.031925
455.076935 1.036210
455.076935 1.040046
455.076935 1.044583
455.076935 1.047208
455.076935 1.048476
455.076935 1.049570
455.076935 1.050530
455.076935 1.050121
455.076935 1.049977
455.076935 1.049305
455.076935 1.048778
455.076935 1.048686
455.076935 1.047261
455.076935 1.047072
455.076935 1.047131
455.076935 1.047809
455.076935 1.049406
455.076935 1.051789
455.076935 1.053387
455.076935 1.055753
455.076935 1.057849
455.076935 1.060426
455.076935 1.062000
455.076935 1.063592
455.076935 1.063083
455.076935 1.063989
455.076935 1.064759
455.076935 1.063209
455.076935 1.062046
455.076935 1.060874
455.076935 1.062259
455.076935 1.064398
455.076935 1.065520
455.076935 1.066117
455.076935 1.066885
455.076935 1.067317
455.076935 1.068148
455.076935 1.069491
455.076935 1.071352
455.076935 1.071420
455.076935 1.072759
455.076935 1.075597
455.076935 1.078622
455.076935 1.079473
455.076935 1.081790
455.076935 1.084841
455.076935 1.089272
455.076935 1.092315
455.076935 1.093656
455.076935 1.095529
455.076935 1.097236
455.076935 1.098434
455.076935 1.098309
455.076935 1.099331
455.076935 1.101507
455.076935 1.104726
455.076935 1.107669
455.076935 1.108821
455.076935 1.106869
455.076935 1.105713
455.076935 1.103766
455.076935 1.101682
455.076935 1.100230
455.076935 1.097663
455.076935 1.096541
455.076935 1.095710
463.457520 1.070439
463.457520 1.069945
463.457520 1.069306
463.457520 1.068743
463.457520 1.067425
463.457520 1.066817
463.457520 1.064027
463.457520 1.062846
463.457520 1.059194
463.457520 1.058687
463.457520 1.058368
463.457520 1.059990
463.457520 1.060998
463.457520 1.064166
463.457520 1.068751
463.457520 1.073343
463.457520 1.075703
463.457520 1.079079
463.457520 1.081383
463.457520 1.085430
463.457520 1.087375
463.457520 1.089830
463.457520 1.092067
463.457520 1.092174
463.457520 1.093110
463.457520 1.093598
463.457520 1.093339
463.457520 1.094437
463.457520 1.095506
463.457520 1.098311
463.457520 1.101252
463.457520 1.105185
463.457520 1.109601
471.972687 1.001538
471.972687 1.002618
471.972687 1.003314
471.972687 1.002987
471.972687 1.002433
471.972687 1.001040
471.972687 1.002297
471.972687 1.003863
471.972687 1.004604
471.972687 1.008040
471.972687 1.013276
471.972687 1.015156
471.972687 1.017132
471.972687 1.018596
471.972687 1.018214
471.972687 1.016625
471.972687 1.013991
471.972687 1.012532
471.972687 1.011484
471.972687 1.009878
471.972687 1.007058
471.972687 1.002814
471.972687 1.004549
471.972687 1.005353
471.972687 1.005901
471.972687 1.005818
471.972687 1.004208
471.972687 1.003103
471.972687 1.003286
471.972687 1.004446
471.972687 1.004569
471.972687 1.006222
471.972687 1.007766
471.972687 1.010040
471.972687 1.014120
471.972687 1.016534
471.972687 1.017513
471.972687 1.018839
471.972687 1.021807
471.972687 1.023756
471.972687 1.026232
471.972687 1.028033
471.972687 1.027029
471.972687 1.028794
471.972687 1.029940
471.972687 1.030964
471.972687 1.033238
471.972687 1.034273
471.972687 1.035942
471.972687 1.038634
471.972687 1.040983
471.972687 1.040956
471.972687 1.041531
471.972687 1.045008
471.972687 1.049108
471.972687 1.051320
471.972687 1.053334
471.972687 1.053510
471.972687 1.052617
471.972687 1.052701
471.972687 1.053362
471.972687 1.055071
471.972687 1.057197
471.972687 1.060653
471.972687 1.062805
480.795654 1.015902
480.795654 1.016403
480.795654 1.017547
480.795654 1.018198
480.795654 1.018143
480.795654 1.018443
480.795654 1.016772
480.795654 1.016796
480.795654 1.016526
480.795654 1.014943
480.795654 1.015152
480.795654 1.015452
480.795654 1.015010
480.795654 1.015884
480.795654 1.015381
480.795654 1.016098
480.795654 1.015626
480.795654 1.016263
480.795654 1.018613
480.795654 1.018998
480.795654 1.021706
480.795654 1.023634
480.795654 1.026070
480.795654 1.028117
480.795654 1.028216
480.795654 1.028614
480.795654 1.028554
480.795654 1.029768
480.795654 1.031046
480.795654 1.031758
480.795654 1.032883
480.795654 1.035021
480.795654 1.035791
480.795654 1.036943
480.795654 1.038396
480.795654 1.038677
480.795654 1.039446
480.795654 1.041622
480.795654 1.044015
480.795654 1.045638
480.795654 1.045378
480.795654 1.046819
480.795654 1.047634
480.795654 1.048596
480.795654 1.050074
480.795654 1.050709
489.820648 1.025347
489.820648 1.023886
489.820648 1.022708
489.820648 1.020610
489.820648 1.019045
489.820648 1.017764
489.820648 1.016150
489.820648 1.016872
489.820648 1.016327
489.820648 1.017713
489.820648 1.019393
489.820648 1.020965
489.820648 1.021142
489.820648 1.019159
489.820648 1.016042
489.820648 1.014372
489.820648 1.015475
489.820648 1.016054
489.820648 1.017109
489.820648 1.019063
489.820648 1.020302
489.820648 1.021458
489.820648 1.023118
489.820648 1.024613
489.820648 1.024633
489.820648 1.025677
489.820648 1.027609
489.820648 1.028014
489.820648 1.026768
489.820648 1.026802
489.820648 1.026724
489.820648 1.024875
489.820648 1.022460
489.820648 1.020166
489.820648 1.016763
489.820648 1.013853
489.820648 1.011186
489.820648 1.012250
489.820648 1.012467
489.820648 1.012265
489.820648 1.010322
489.820648 1.006919
489.820648 1.005924
489.820648 1.003963
489.820648 1.004617
489.820648 1.005637
489.820648 1.006764
489.820648 1.006874
489.820648 1.007902
489.820648 1.010514
489.820648 1.013355
489.820648 1.015464
489.820648 1.015840
489.820648 1.016610
489.820648 1.018247
489.820648 1.018660
489.820648 1.021267
489.820648 1.023671
489.820648 1.025937
489.820648 1.025326
489.820648 1.026417
489.820648 1.024130
489.820648 1.024133
489.820648 1.022532
489.820648 1.022006
489.820648 1.024308
489.820648 1.026409
489.820648 1.029267
489.820648 1.031712
489.820648 1.033671
489.820648 1.034809
489.820648 1.035986
489.820648 1.035573
489.820648 1.035073
489.820648 1.032245
489.820648 1.029621
489.820648 1.030601
489.820648 1.031118
489.820648 1.032104
489.820648 1.033138
489.820648 1.034110
489.820648 1.038480
489.820648 1.042542
489.820648 1.047188
489.820648 1.048592
489.820648 1.047874
489.820648 1.048753
489.820648 1.050865
489.820648 1.050096
489.820648 1.052242
489.820648 1.055158
489.820648 1.056191
489.820648 1.057159
489.820648 1.055639
489.820648 1.055134
489.820648 1.054915
489.820648 1.054688
489.820648 1.053776
489.820648 1.052852
489.820648 1.052045
489.820648 1.051274
489.820648 1.050953
489.820648 1.051472
489.820648 1.050138
489.820648 1.050234
489.820648 1.049457
489.820648 1.049576
489.820648 1.048300
489.820648 1.046235
489.820648 1.044110
489.820648 1.040851
489.820648 1.040293
489.820648 1.038422
489.820648 1.037885
489.820648 1.038585
489.820648 1.038216
489.820648 1.036611
489.820648 1.035732
489.820648 1.035049
489.820648 1.036404
489.820648 1.039347
489.820648 1.039952
489.820648 1.041289
489.820648 1.041288
489.820648 1.043531
489.820648 1.044445
489.820648 1.045449
489.820648 1.046809
489.820648 1.049946
489.820648 1.053781
489.820648 1.056539
489.820648 1.059502
489.820648 1.062878
489.820648 1.065366
489.820648 1.068834
489.820648 1.073245
489.820648 1.074099
489.820648 1.074085
489.820648 1.074382
489.820648 1.075853
489.820648 1.075771
489.820648 1.076215
489.820648 1.078868
489.820648 1.082493
489.820648 1.083610
489.820648 1.082731
489.820648 1.081973
489.820648 1.080448
489.820648 1.078874
489.820648 1.076864
489.820648 1.075100
489.820648 1.072692
489.820648 1.071487
489.820648 1.072033
489.820648 1.072938
489.820648 1.074509
489.820648 1.073848
489.820648 1.072855
489.820648 1.073123
489.820648 1.072016
489.820648 1.073652
489.820648 1.074803
489.820648 1.074821
489.820648 1.076590
489.820648 1.077195
489.820648 1.077096
489.820648 1.076501
489.820648 1.073618
489.820648 1.074919
489.820648 1.076177
489.820648 1.077901
489.820648 1.079255
489.820648 1.080236
489.820648 1.079635
489.820648 1.081552
489.820648 1.084262
489.820648 1.087052
489.820648 1.087063
489.820648 1.087780
489.820648 1.090928
489.820648 1.092087
489.820648 1.092840
489.820648 1.093083
489.820648 1.096582
489.820648 1.100821
489.820648 1.102176
489.820648 1.104859
489.820648 1.106104
489.820648 1.107350
489.820648 1.106352
489.820648 1.106080
489.820648 1.107167
489.820648 1.109555
489.820648 1.111540
489.820648 1.112085
489.820648 1.113659
489.820648 1.114752
489.820648 1.114131
489.820648 1.118450
489.820648 1.125343
489.820648 1.130586
489.820648 1.134812
499.891602 1.113871
499.891602 1.115523
499.891602 1.117513
499.891602 1.119776
499.891602 1.121503
499.891602 1.124518
499.891602 1.125669
499.891602 1.124566
499.891602 1.125413
499.891602 1.124971
499.891602 1.124324
499.891602 1.124612
499.891602 1.124595
499.891602 1.123758
499.891602 1.123821
499.891602 1.124715
499.891602 1.125510
499.891602 1.126498
499.891602 1.127350
499.891602 1.127758
499.891602 1.127956
499.891602 1.129164
499.891602 1.130971
499.891602 1.133895
499.891602 1.136766
499.891602 1.140078
499.891602 1.142705
499.891602 1.144043
510.059448 1.111047
510.059448 1.110454
510.059448 1.111995
510.059448 1.113010
510.059448 1.115630
510.059448 1.118984
510.059448 1.123111
510.059448 1.127442
510.059448 1.131700
510.059448 1.134625
510.059448 1.137381
510.059448 1.142498
510.059448 1.146482
510.059448 1.151864
510.059448 1.153622
510.059448 1.156640
510.059448 1.158303
510.059448 1.158877
510.059448 1.157562
510.059448 1.158032
510.059448 1.158855
510.059448 1.157987
510.059448 1.156144
510.059448 1.155270
510.059448 1.153440
510.059448 1.153453
510.059448 1.152394
510.059448 1.153243
510.059448 1.152291
510.059448 1.151713
510.059448 1.150766
510.059448 1.151541
510.059448 1.151444
510.059448 1.152404
510.059448 1.151594
510.059448 1.151648
510.059448 1.151641
510.059448 1.152936
510.059448 1.153790
510.059448 1.154768
510.059448 1.156009
510.059448 1.157676
510.059448 1.159396
510.059448 1.159125
510.059448 1.157692
510.059448 1.157465
510.059448 1.157561
510.059448 1.157733
510.059448 1.157889
510.059448 1.158967
510.059448 1.158284
510.059448 1.156530
510.059448 1.153755
510.059448 1.153934
510.059448 1.153619
510.059448 1.153165
510.059448 1.154508
510.059448 1.154055
510.059448 1.152557
510.059448 1.151289
510.059448 1.150928
510.059448 1.149958
510.059448 1.148031
510.059448 1.147521
510.059448 1.148504
510.059448 1.148883
510.059448 1.150549
510.059448 1.150958
510.059448 1.150802
510.059448 1.149088
510.059448 1.149447
510.059448 1.149944
510.059448 1.150261
510.059448 1.151042
510.059448 1.150673
510.059448 1.149281
510.059448 1.148569
510.059448 1.149043
510.059448 1.147056
510.059448 1.146782
510.059448 1.147385
510.059448 1.147013
510.059448 1.146554
510.059448 1.144405
510.059448 1.145011
510.059448 1.145187
510.059448 1.146071
510.059448 1.147525
510.059448 1.148830
510.059448 1.150374
510.059448 1.155091
510.059448 1.158690
510.059448 1.162161
510.059448 1.164900
510.059448 1.169784
510.059448 1.172136
510.059448 1.174920
510.059448 1.177760
510.059448 1.179870
510.059448 1.180336
510.059448 1.181910
510.059448 1.182780
510.059448 1.183463
510.059448 1.184234
510.059448 1.185244
510.059448 1.185833
510.059448 1.187325
510.059448 1.188588
510.059448 1.189542
510.059448 1.188062
510.059448 1.187696
510.059448 1.186672
510.059448 1.188925
510.059448 1.190680
510.059448 1.193439
510.059448 1.193981
510.059448 1.196152
510.059448 1.197119
510.059448 1.198194
510.059448 1.200027
510.059448 1.200308
510.059448 1.201160
510.059448 1.201083
510.059448 1.200168
510.059448 1.200478
510.059448 1.202976
510.059448 1.204976
510.059448 1.205956
510.059448 1.206529
510.059448 1.207314
510.059448 1.210055
510.059448 1.214329
510.059448 1.216262
510.059448 1.216490
510.059448 1.215629
510.059448 1.214554
510.059448 1.214598
510.059448 1.214604
510.059448 1.214558
510.059448 1.215306
510.059448 1.216946
510.059448 1.218818
510.059448 1.223268
510.059448 1.226404
510.059448 1.225865
510.059448 1.226592
510.059448 1.228275
510.059448 1.231802
510.059448 1.235373
510.059448 1.238047
510.059448 1.243845
510.059448 1.247617
510.059448 1.250890
510.059448 1.252521
510.059448 1.254872
510.059448 1.255813
510.059448 1.257230
510.059448 1.260131
510.059448 1.264730
510.059448 1.266273
510.059448 1.267973
510.059448 1.267551
510.059448 1.268407
510.059448 1.270680
510.059448 1.272427
510.059448 1.272282
510.059448 1.270551
510.059448 1.274640
510.059448 1.278429
510.059448 1.281997
510.059448 1.284516
510.059448 1.284828
510.059448 1.285791
510.059448 1.288135
510.059448 1.291819
510.059448 1.294071
510.059448 1.297951
510.059448 1.299056
510.059448 1.298810
510.059448 1.299008
510.059448 1.299919
510.059448 1.299245
510.059448 1.300743
510.059448 1.302333
510.059448 1.304175
510.059448 1.303603
510.059448 1.304440
510.059448 1.303659
510.059448 1.305619
510.059448 1.306368
510.059448 1.304461
510.059448 1.304308
510.059448 1.305976
510.059448 1.305980
510.059448 1.306681
510.059448 1.307444
510.059448 1.308179
510.059448 1.308907
510.059448 1.308588
510.059448 1.307274
510.059448 1.307544
510.059448 1.309727
510.059448 1.309946
510.059448 1.310524
510.059448 1.310212
510.059448 1.310558
510.059448 1.309853
510.059448 1.310493
510.059448 1.308662
510.059448 1.306761
510.059448 1.305207
510.059448 1.305313
510.059448 1.303103
510.059448 1.303473
510.059448 1.301174
510.059448 1.298882
510.059448 1.299809
510.059448 1.303343
510.059448 1.308318
510.059448 1.314807
510.059448 1.319235
510.059448 1.322092
510.059448 1.325057
510.059448 1.327912
510.059448 1.330226
521.385437 1.213565
521.385437 1.215796
521.385437 1.216798
521.385437 1.218463
521.385437 1.221788
521.385437 1.223574
521.385437 1.225459
521.385437 1.227246
521.385437 1.228651
521.385437 1.228398
532.704285 1.175599
532.704285 1.177592
532.704285 1.181543
532.704285 1.184769
532.704285 1.186112
532.704285 1.186413
532.704285 1.184652
532.704285 1.183020
532.704285 1.180038
532.704285 1.179355
532.704285 1.176658
532.704285 1.175843
532.704285 1.175156
532.704285 1.176394
532.704285 1.178467
532.704285 1.180759
532.704285 1.183256
532.704285 1.188228
532.704285 1.193964
532.704285 1.195833
532.704285 1.198020
532.704285 1.197827
532.704285 1.198593
532.704285 1.199340
532.704285 1.196358
532.704285 1.194319
532.704285 1.191812
532.704285 1.189395
532.704285 1.187670
532.704285 1.185897
532.704285 1.185112
532.704285 1.184306
532.704285 1.185402
532.704285 1.185743
532.704285 1.185559
532.704285 1.186227
532.704285 1.186383
532.704285 1.186428
532.704285 1.185997
532.704285 1.186847
532.704285 1.187946
532.704285 1.187110
532.704285 1.188078
532.704285 1.190157
532.704285 1.194241
532.704285 1.198203
532.704285 1.201093
532.704285 1.204000
532.704285 1.206437
532.704285 1.207737
532.704285 1.209045
532.704285 1.211045
532.704285 1.213032
532.704285 1.215094
532.704285 1.216289
532.704285 1.218472
532.704285 1.217991
532.704285 1.219708
532.704285 1.219806
532.704285 1.220128
532.704285 1.223578
532.704285 1.226734
532.704285 1.228357
532.704285 1.230922
532.704285 1.234455
532.704285 1.238525
532.704285 1.241640
532.704285 1.243914
532.704285 1.246881
532.704285 1.247182
532.704285 1.246072
532.704285 1.247685
532.704285 1.250453
544.353882 1.234894
544.353882 1.236210
544.353882 1.237805
544.353882 1.238215
544.353882 1.241093
544.353882 1.242485
544.353882 1.243822
544.353882 1.246504
544.353882 1.248945
544.353882 1.250377
544.353882 1.249302
544.353882 1.247740
544.353882 1.245905
544.353882 1.245216
544.353882 1.242694
544.353882 1.242054
544.353882 1.241281
544.353882 1.240360
544.353882 1.241696
544.353882 1.241787
544.353882 1.241861
544.353882 1.242893
544.353882 1.243242
544.353882 1.242845
544.353882 1.243017
544.353882 1.243456
544.353882 1.245973
544.353882 1.245376
544.353882 1.249489
544.353882 1.252677
544.353882 1.254335
544.353882 1.255622
544.353882 1.256853
544.353882 1.259919
544.353882 1.262035
544.353882 1.263364
544.353882 1.263614
544.353882 1.263935
544.353882 1.263249
544.353882 1.264109
544.353882 1.264840
544.353882 1.266257
544.353882 1.267626
544.353882 1.268694
556.176453 1.156473
556.176453 1.157807
556.176453 1.160265
556.176453 1.163889
556.176453 1.168466
556.176453 1.173095
556.176453 1.177767
556.176453 1.181836
556.176453 1.185661
556.176453 1.189308
556.176453 1.191986
556.176453 1.192422
556.176453 1.192676
556.176453 1.193085
556.176453 1.193262
556.176453 1.191826
556.176453 1.192700
556.176453 1.192797
556.176453 1.192123
556.176453 1.190536
556.176453 1.191191
556.176453 1.190925
556.176453 1.189326
556.176453 1.188624
556.176453 1.190691
556.176453 1.192788
556.176453 1.193271
556.176453 1.192567
556.176453 1.192405
556.176453 1.190968
556.176453 1.188947
556.176453 1.189251
556.176453 1.189266
556.176453 1.188280
556.176453 1.185698
556.176453 1.182092
556.176453 1.177058
556.176453 1.176493
556.176453 1.175588
556.176453 1.175438
556.176453 1.175931
556.176453 1.176162
556.176453 1.176018
556.176453 1.177208
556.176453 1.179208
556.176453 1.180322
556.176453 1.182847
580.132996 1.039689
580.132996 1.044258
580.132996 1.046839
580.132996 1.049105
580.132996 1.051396
580.132996 1.053674
580.132996 1.054426
580.132996 1.055436
580.132996 1.057408
580.132996 1.059380
580.132996 1.060063
580.132996 1.061880
580.132996 1.060546
580.132996 1.057918
580.132996 1.057503
580.132996 1.055926
580.132996 1.053599
580.132996 1.050807
580.132996 1.049235
580.132996 1.046875
580.132996 1.045535
580.132996 1.043553
580.132996 1.044486
580.132996 1.046810
580.132996 1.049310
580.132996 1.049243
580.132996 1.048929
580.132996 1.048195
580.132996 1.047150
580.132996 1.046624
580.132996 1.046372
580.132996 1.044550
580.132996 1.043071
580.132996 1.042936
580.132996 1.042706
580.132996 1.042353
580.132996 1.043633
580.132996 1.046664
580.132996 1.051009
580.132996 1.055413
580.132996 1.058321
580.132996 1.062659
580.132996 1.067342
580.132996 1.070621
580.132996 1.073819
580.132996 1.074993
580.132996 1.077733
580.132996 1.079407
580.132996 1.081142
580.132996 1.080961
580.132996 1.080065
580.132996 1.079249
580.132996 1.080352
580.132996 1.079296
580.132996 1.077498
580.132996 1.077529
580.132996 1.076372
580.132996 1.074984
580.132996 1.074046
580.132996 1.074617
580.132996 1.076759
580.132996 1.079234
580.132996 1.080547
580.132996 1.079994
580.132996 1.080253
580.132996 1.081337
580.132996 1.083628
580.132996 1.084599
580.132996 1.085732
580.132996 1.087358
580.132996 1.089329
580.132996 1.090858
580.132996 1.093097
580.132996 1.095056
580.132996 1.096933
580.132996 1.098643
580.132996 1.100698
580.132996 1.101820
580.132996 1.101216
580.132996 1.103648
580.132996 1.104352
580.132996 1.104757
580.132996 1.104359
580.132996 1.103449
580.132996 1.103429
580.132996 1.105506
580.132996 1.106391
580.132996 1.106061
580.132996 1.105266
580.132996 1.102550
580.132996 1.103067
580.132996 1.101737
580.132996 1.102157
580.132996 1.101356
580.132996 1.102334
580.132996 1.100029
580.132996 1.100061
580.132996 1.098869
580.132996 1.097460
580.132996 1.096320
580.132996 1.099272
580.132996 1.099165
580.132996 1.100974
580.132996 1.102859
580.132996 1.104950
580.132996 1.106852
580.132996 1.107918
580.132996 1.108293
580.132996 1.110385
580.132996 1.111267
580.132996 1.113194
580.132996 1.113674
580.132996 1.115016
580.132996 1.114989
580.132996 1.116121
580.132996 1.116782
580.132996 1.120421
580.132996 1.123093
580.132996 1.126254
580.132996 1.127648
580.132996 1.130039
580.132996 1.133520
580.132996 1.137391
580.132996 1.139630
580.132996 1.141458
580.132996 1.143903
580.132996 1.144145
580.132996 1.146664
580.132996 1.147952
580.132996 1.149371
580.132996 1.152275
580.132996 1.154609
580.132996 1.156950
580.132996 1.158090
580.132996 1.158833
580.132996 1.160669
580.132996 1.161926
580.132996 1.161222
580.132996 1.161626
580.132996 1.161807
580.132996 1.161034
580.132996 1.160133
580.132996 1.160800
580.132996 1.160136
580.132996 1.160247
580.132996 1.159171
580.132996 1.159325
580.132996 1.158031
580.132996 1.154940
580.132996 1.153466
580.132996 1.152131
580.132996 1.149732
580.132996 1.147766
580.132996 1.146755
580.132996 1.146310
580.132996 1.145591
580.132996 1.144470
580.132996 1.144354
580.132996 1.142942
580.132996 1.142341
580.132996 1.142408
580.132996 1.142978
580.132996 1.142840
580.132996 1.143011
580.132996 1.143867
580.132996 1.146138
580.132996 1.149403
580.132996 1.148943
592.907166 1.094159
592.907166 1.093893
592.907166 1.095044
592.907166 1.092821
592.907166 1.090843
592.907166 1.087551
592.907166 1.085113
592.907166 1.086320
592.907166 1.085316
592.907166 1.084921
592.907166 1.086405
592.907166 1.088387
592.907166 1.091115
592.907166 1.093360
592.907166 1.094705
592.907166 1.093789
592.907166 1.093458
592.907166 1.095657
592.907166 1.097294
592.907166 1.098985
592.907166 1.100075
592.907166 1.101463
592.907166 1.103697
605.735474 1.038290
605.735474 1.037612
605.735474 1.036765
605.735474 1.035019
605.735474 1.031955
605.735474 1.030691
605.735474 1.030311
605.735474 1.029422
605.735474 1.029864
605.735474 1.030541
605.735474 1.031672
605.735474 1.029731
605.735474 1.026499
605.735474 1.030313
605.735474 1.034012
605.735474 1.038563
605.735474 1.041704
605.735474 1.044251
605.735474 1.046167
605.735474 1.047318
605.735474 1.046435
605.735474 1.046830
605.735474 1.045437
605.735474 1.045513
605.735474 1.046298
605.735474 1.047860
605.735474 1.049595
605.735474 1.050562
605.735474 1.052431
605.735474 1.052318
605.735474 1.052402
605.735474 1.050320
605.735474 1.048729
605.735474 1.052013
605.735474 1.053526
605.735474 1.055560
605.735474 1.057490
605.735474 1.058919
605.735474 1.061213
605.735474 1.064743
605.735474 1.067295
605.735474 1.067960
605.735474 1.070545
605.735474 1.072009
605.735474 1.071204
605.735474 1.072191
605.735474 1.073681
605.735474 1.079679
605.735474 1.082936
605.735474 1.085277
605.735474 1.088204
605.735474 1.092019
605.735474 1.092525
605.735474 1.094083
605.735474 1.095468
605.735474 1.095372
605.735474 1.095402
605.735474 1.094137
605.735474 1.093088
605.735474 1.091452
605.735474 1.091240
605.735474 1.094018
605.735474 1.095300
605.735474 1.097929
605.735474 1.099401
605.735474 1.103519
605.735474 1.104458
605.735474 1.105001
605.735474 1.107816
605.735474 1.109891
605.735474 1.112453
605.735474 1.114108
605.735474 1.113732
605.735474 1.115176
605.735474 1.116497
605.735474 1.119676
605.735474 1.121152
605.735474 1.120223
605.735474 1.120647
605.735474 1.121672
605.735474 1.119641
605.735474 1.120708
605.735474 1.121184
605.735474 1.121598
605.735474 1.119528
605.735474 1.120336
605.735474 1.123573
605.735474 1.124330
605.735474 1.124044
605.735474 1.123823
605.735474 1.124398
605.735474 1.123281
605.735474 1.121808
605.735474 1.123066
605.735474 1.124310
605.735474 1.124547
605.735474 1.122554
605.735474 1.123087
605.735474 1.121952
605.735474 1.119063
605.735474 1.118199
605.735474 1.118397
605.735474 1.116445
605.735474 1.115910
605.735474 1.114957
605.735474 1.115804
605.735474 1.116662
605.735474 1.117609
605.735474 1.122111
605.735474 1.125783
605.735474 1.127121
605.735474 1.127105
605.735474 1.126432
605.735474 1.124541
605.735474 1.122493
605.735474 1.120119
605.735474 1.117157
605.735474 1.115680
605.735474 1.114102
605.735474 1.111783
605.735474 1.109442
605.735474 1.107620
605.735474 1.106581
605.735474 1.106095
605.735474 1.108514
605.735474 1.110766
605.735474 1.113378
605.735474 1.115049
605.735474 1.117414
605.735474 1.118941
605.735474 1.121458
605.735474 1.124428
605.735474 1.128910
605.735474 1.130875
605.735474 1.133453
605.735474 1.133948
605.735474 1.134066
605.735474 1.134395
605.735474 1.134959
605.735474 1.134719
605.735474 1.135133
605.735474 1.135352
605.735474 1.134001
605.735474 1.133426
605.735474 1.131837
605.735474 1.130822
605.735474 1.129203
605.735474 1.125590
605.735474 1.125661
605.735474 1.122357
605.735474 1.122722
605.735474 1.123195
605.735474 1.124128
605.735474 1.123497
605.735474 1.123409
605.735474 1.123828
605.735474 1.124286
605.735474 1.123796
605.735474 1.125002
605.735474 1.124701
605.735474 1.124273
605.735474 1.123026
605.735474 1.121621
605.735474 1.121730
605.735474 1.121915
605.735474 1.121593
605.735474 1.123022
605.735474 1.123605
605.735474 1.125172
605.735474 1.126321
605.735474 1.128584
605.735474 1.130679
605.735474 1.131111
605.735474 1.131408
605.735474 1.134630
605.735474 1.137148
605.735474 1.139002
605.735474 1.140349
605.735474 1.140766
605.735474 1.139982
605.735474 1.140385
605.735474 1.139260
605.735474 1.139527
605.735474 1.141767
605.735474 1.142324
605.735474 1.145503
605.735474 1.148136
605.735474 1.149708
605.735474 1.151143
605.735474 1.152740
605.735474 1.153903
605.735474 1.155377
605.735474 1.156892
605.735474 1.158475
605.735474 1.158199
605.735474 1.158045
605.735474 1.156568
605.735474 1.154108
605.735474 1.151896
605.735474 1.149836
605.735474 1.150395
605.735474 1.151034
605.735474 1.150843
605.735474 1.152624
605.735474 1.155092
605.735474 1.157394
605.735474 1.160575
605.735474 1.161929
605.735474 1.164038
605.735474 1.163190
605.735474 1.163835
605.735474 1.164428
605.735474 1.164890
605.735474 1.166813
605.735474 1.168397
605.735474 1.170761
605.735474 1.173688
605.735474 1.175490
605.735474 1.178769
605.735474 1.181276
605.735474 1.185801
605.735474 1.187469
605.735474 1.190633
605.735474 1.192393
605.735474 1.193041
605.735474 1.193982
605.735474 1.196722
605.735474 1.197757
605.735474 1.203526
605.735474 1.207201
605.735474 1.208992
605.735474 1.212010
605.735474 1.213554
605.735474 1.215555
605.735474 1.216069
605.735474 1.215646
605.735474 1.214440
605.735474 1.214397
605.735474 1.211080
605.735474 1.209998
605.735474 1.208782
605.735474 1.205700
605.735474 1.203318
605.735474 1.202548
605.735474 1.201223
605.735474 1.200068
605.735474 1.197187
605.735474 1.194623
605.735474 1.192941
605.735474 1.191186
605.735474 1.189452
605.735474 1.188888
605.735474 1.188341
605.735474 1.185642
605.735474 1.182919
605.735474 1.181702
605.735474 1.182622
605.735474 1.183290
605.735474 1.184307
605.735474 1.182671
605.735474 1.181774
605.735474 1.180461
605.735474 1.179500
605.735474 1.179051
605.735474 1.178936
605.735474 1.177549
605.735474 1.177432
605.735474 1.177132
605.735474 1.176614
605.735474 1.173977
605.735474 1.175948
605.735474 1.176195
605.735474 1.175844
605.735474 1.175961
605.735474 1.177723
605.735474 1.177558
605.735474 1.178479
605.735474 1.177645
605.735474 1.175797
605.735474 1.173003
605.735474 1.172210
605.735474 1.171628
605.735474 1.173183
605.735474 1.174643
605.735474 1.177058
605.735474 1.179772
605.735474 1.184193
605.735474 1.188666
605.735474 1.191276
605.735474 1.192031
605.735474 1.191844
605.735474 1.191635
605.735474 1.193267
605.735474 1.194399
605.735474 1.194738
605.735474 1.196738
605.735474 1.196820
605.735474 1.196186
605.735474 1.193054
605.735474 1.193060
605.735474 1.192129
605.735474 1.192023
605.735474 1.192884
605.735474 1.191597
605.735474 1.191259
605.735474 1.188909
605.735474 1.187023
605.735474 1.184622
605.735474 1.182177
605.735474 1.180451
605.735474 1.179626
605.735474 1.178885
605.735474 1.178700
605.735474 1.177609
605.735474 1.179417
605.735474 1.180932
605.735474 1.183424
605.735474 1.185701
605.735474 1.186994
605.735474 1.190071
605.735474 1.192831
605.735474 1.194563
605.735474 1.195356
605.735474 1.195095
605.735474 1.195714
605.735474 1.197040
605.735474 1.196314
605.735474 1.196932
605.735474 1.195677
605.735474 1.193210
605.735474 1.189834
605.735474 1.184178
605.735474 1.179443
605.735474 1.179016
605.735474 1.178202
605.735474 1.176745
605.735474 1.173426
605.735474 1.172495
605.735474 1.172422
605.735474 1.173598
605.735474 1.174292
605.735474 1.172944
605.735474 1.172965
605.735474 1.174832
605.735474 1.176061
605.735474 1.177076
605.735474 1.178412
605.735474 1.179827
605.735474 1.182384
605.735474 1.185589
605.735474 1.187381
605.735474 1.190630
605.735474 1.192423
605.735474 1.192696
605.735474 1.192749
605.735474 1.190533
605.735474 1.192914
605.735474 1.194055
605.735474 1.195666
605.735474 1.197077
605.735474 1.198105
605.735474 1.201312
605.735474 1.203880
605.735474 1.203686
605.735474 1.204518
605.735474 1.203394
605.735474 1.204521
605.735474 1.206545
605.735474 1.208603
605.735474 1.206425
605.735474 1.205737
605.735474 1.203438
605.735474 1.200151
605.735474 1.196510
605.735474 1.194296
605.735474 1.191998
605.735474 1.190336
605.735474 1.190101
605.735474 1.189423
605.735474 1.187823
605.735474 1.185778
605.735474 1.183744
605.735474 1.184107
605.735474 1.184996
605.735474 1.185849
605.735474 1.183597
605.735474 1.182218
605.735474 1.180461
605.735474 1.178431
605.735474 1.175857
605.735474 1.173943
605.735474 1.172779
605.735474 1.172033
605.735474 1.171734
605.735474 1.172329
605.735474 1.172933
605.735474 1.177190
605.735474 1.178343
605.735474 1.180150
605.735474 1.182881
605.735474 1.185444
605.735474 1.184388
605.735474 1.181591
605.735474 1.182561
605.735474 1.184013
605.735474 1.184601
605.735474 1.185211
605.735474 1.185419
605.735474 1.188054
605.735474 1.189193
605.735474 1.190712
605.735474 1.191770
605.735474 1.192373
605.735474 1.194411
605.735474 1.194149
605.735474 1.194068
605.735474 1.191737
605.735474 1.188687
605.735474 1.187036
605.735474 1.183988
605.735474 1.180253
605.735474 1.175940
605.735474 1.174227
605.735474 1.174587
605.735474 1.174755
605.735474 1.177284
605.735474 1.178384
605.735474 1.180516
605.735474 1.181413
605.735474 1.181408
605.735474 1.180848
605.735474 1.180867
605.735474 1.180428
605.735474 1.180942
605.735474 1.180859
605.735474 1.183690
605.735474 1.187094
605.735474 1.190219
605.735474 1.193975
605.735474 1.197247
605.735474 1.200478
605.735474 1.202675
605.735474 1.204090
605.735474 1.203841
605.735474 1.207743
605.735474 1.210710
605.735474 1.214556
605.735474 1.216635
605.735474 1.221035
605.735474 1.223629
605.735474 1.227054
605.735474 1.228775
605.735474 1.229707
605.735474 1.230936
605.735474 1.232287
605.735474 1.234254
605.735474 1.234878
605.735474 1.235886
605.735474 1.236356
605.735474 1.236818
605.735474 1.238850
605.735474 1.240380
605.735474 1.244421
605.735474 1.247991
605.735474 1.252293
605.735474 1.255179
605.735474 1.253650
605.735474 1.253597
605.735474 1.254103
605.735474 1.252945
605.735474 1.252601
605.735474 1.253422
605.735474 1.255691
605.735474 1.256732
605.735474 1.255415
605.735474 1.253934
605.735474 1.254240
605.735474 1.253162
605.735474 1.251002
605.735474 1.249174
605.735474 1.248177
605.735474 1.244643
605.735474 1.248292
605.735474 1.249942
605.735474 1.251760
605.735474 1.252338
605.735474 1.250029
605.735474 1.250769
605.735474 1.250410
605.735474 1.249893
605.735474 1.251518
605.735474 1.253112
605.735474 1.254608
605.735474 1.257434
605.735474 1.261432
605.735474 1.264306
605.735474 1.265926
605.735474 1.268894
605.735474 1.271866
605.735474 1.275165
605.735474 1.277008
605.735474 1.280379
605.735474 1.284912
605.735474 1.287707
605.735474 1.289246
605.735474 1.291230
605.735474 1.291414
605.735474 1.289129
605.735474 1.287162
605.735474 1.288286
605.735474 1.291156
605.735474 1.296366
605.735474 1.299423
605.735474 1.301495
605.735474 1.303879
605.735474 1.305576
605.735474 1.304413
605.735474 1.303107
605.735474 1.300923
605.735474 1.299867
605.735474 1.298652
605.735474 1.296993
605.735474 1.296236
605.735474 1.294598
605.735474 1.293644
605.735474 1.291690
605.735474 1.287263
605.735474 1.282793
605.735474 1.282289
605.735474 1.282243
605.735474 1.280591
605.735474 1.280632
605.735474 1.278060
605.735474 1.275477
605.735474 1.274004
605.735474 1.274287
605.735474 1.274516
605.735474 1.275888
605.735474 1.275585
605.735474 1.276893
605.735474 1.279770
605.735474 1.283028
605.735474 1.284467
605.735474 1.284441
605.735474 1.289751
605.735474 1.292437
605.735474 1.293207
605.735474 1.293359
605.735474 1.293338
605.735474 1.295365
605.735474 1.295843
605.735474 1.297050
605.735474 1.299022
605.735474 1.300084
605.735474 1.300782
605.735474 1.299946
605.735474 1.298511
605.735474 1.298028
605.735474 1.298524
605.735474 1.299816
605.735474 1.299205
605.735474 1.296186
605.735474 1.293799
605.735474 1.291514
605.735474 1.291840
605.735474 1.294883
605.735474 1.298919
605.735474 1.301471
605.735474 1.303732
605.735474 1.303863
605.735474 1.307669
605.735474 1.310151
605.735474 1.310505
605.735474 1.310766
605.735474 1.310118
605.735474 1.310143
605.735474 1.309464
605.735474 1.308383
605.735474 1.308113
605.735474 1.307795
605.735474 1.310361
605.735474 1.314422
605.735474 1.320990
605.735474 1.324479
605.735474 1.327147
605.735474 1.329995
605.735474 1.333213
605.735474 1.334390
605.735474 1.336636
605.735474 1.338080
605.735474 1.339176
605.735474 1.339391
605.735474 1.341684
605.735474 1.344107
605.735474 1.345758
605.735474 1.348353
605.735474 1.347122
605.735474 1.345260
605.735474 1.345156
605.735474 1.344153
605.735474 1.341607
605.735474 1.339686
605.735474 1.341075
605.735474 1.342708
605.735474 1.343318
605.735474 1.342621
605.735474 1.340964
605.735474 1.344098
605.735474 1.346404
605.735474 1.345966
605.735474 1.346099
605.735474 1.345804
605.735474 1.346751
605.735474 1.345161
605.735474 1.344977
605.735474 1.344467
605.735474 1.348080
605.735474 1.349944
605.735474 1.353607
605.735474 1.353019
605.735474 1.351953
605.735474 1.352643
605.735474 1.355403
605.735474 1.359925
605.735474 1.361413
605.735474 1.364311
605.735474 1.369025
605.735474 1.371363
605.735474 1.373490
605.735474 1.375281
621.820557 1.285434
621.820557 1.288309
621.820557 1.288980
621.820557 1.291325
621.820557 1.294218
621.820557 1.294305
621.820557 1.293474
621.820557 1.294759
621.820557 1.293068
621.820557 1.295087
621.820557 1.294938
621.820557 1.295542
621.820557 1.294747
621.820557 1.295805
621.820557 1.296844
621.820557 1.297053
621.820557 1.297944
621.820557 1.296354
621.820557 1.294904
621.820557 1.294044
621.820557 1.294176
621.820557 1.294508
621.820557 1.296340
621.820557 1.298339
621.820557 1.300704
621.820557 1.303014
621.820557 1.305796
621.820557 1.308101
621.820557 1.311658
621.820557 1.315723
621.820557 1.319853
621.820557 1.321893
621.820557 1.324152
621.820557 1.326142
621.820557 1.327050
621.820557 1.327162
621.820557 1.330861
621.820557 1.331176
621.820557 1.332540
621.820557 1.334005
621.820557 1.336335
621.820557 1.338301
621.820557 1.339265
621.820557 1.339167
621.820557 1.338520
621.820557 1.338440
621.820557 1.339276
621.820557 1.338321
621.820557 1.338096
621.820557 1.339651
621.820557 1.339576
621.820557 1.342092
621.820557 1.341888
621.820557 1.342492
621.820557 1.342211
621.820557 1.343728
621.820557 1.344061
621.820557 1.344881
621.820557 1.345287
621.820557 1.345379
621.820557 1.342840
621.820557 1.339151
621.820557 1.337183
621.820557 1.334877
621.820557 1.334448
621.820557 1.336520
621.820557 1.337718
621.820557 1.339992
621.820557 1.344494
621.820557 1.347966
621.820557 1.350372
621.820557 1.351443
621.820557 1.353030
621.820557 1.355451
621.820557 1.358630
621.820557 1.360207
621.820557 1.360335
621.820557 1.360476
621.820557 1.359089
621.820557 1.356519
621.820557 1.354046
621.820557 1.351869
621.820557 1.350772
621.820557 1.348508
621.820557 1.344889
621.820557 1.342567
621.820557 1.339318
621.820557 1.336993
621.820557 1.333146
621.820557 1.331835
621.820557 1.329035
621.820557 1.324939
621.820557 1.324225
621.820557 1.323869
621.820557 1.324217
621.820557 1.322395
621.820557 1.320768
621.820557 1.322956
621.820557 1.324312
621.820557 1.325315
621.820557 1.328341
621.820557 1.330620
621.820557 1.331932
621.820557 1.333411
621.820557 1.333072
621.820557 1.333945
621.820557 1.335065
621.820557 1.336503
621.820557 1.335376
621.820557 1.334635
621.820557 1.336575
621.820557 1.340456
621.820557 1.341992
621.820557 1.340629
621.820557 1.338910
621.820557 1.336275
621.820557 1.336530
621.820557 1.338362
621.820557 1.338630
621.820557 1.340048
621.820557 1.339189
621.820557 1.338266
621.820557 1.336120
621.820557 1.335357
621.820557 1.334150
621.820557 1.334001
621.820557 1.333157
621.820557 1.331444
621.820557 1.330343
621.820557 1.329596
621.820557 1.328687
621.820557 1.327708
621.820557 1.325086
621.820557 1.321615
621.820557 1.318036
621.820557 1.315434
621.820557 1.313605
621.820557 1.311258
621.820557 1.309155
621.820557 1.306582
621.820557 1.304312
621.820557 1.302932
621.820557 1.303216
621.820557 1.302048
621.820557 1.301890
621.820557 1.301729
621.820557 1.301648
621.820557 1.301466
621.820557 1.302317
621.820557 1.304939
621.820557 1.308051
621.820557 1.310268
621.820557 1.312563
621.820557 1.316289
621.820557 1.319055
621.820557 1.322402
621.820557 1.325907
621.820557 1.329958
621.820557 1.332825
621.820557 1.335011
621.820557 1.336258
621.820557 1.338695
621.820557 1.342655
621.820557 1.343249
621.820557 1.346395
621.820557 1.349153
621.820557 1.348670
621.820557 1.347822
621.820557 1.348456
621.820557 1.351683
621.820557 1.353967
621.820557 1.357749
621.820557 1.358890
621.820557 1.360140
621.820557 1.362042
621.820557 1.364475
621.820557 1.367912
621.820557 1.369476
621.820557 1.369427
621.820557 1.370080
621.820557 1.370063
621.820557 1.370725
621.820557 1.370728
621.820557 1.371603
621.820557 1.373113
621.820557 1.375207
621.820557 1.377014
621.820557 1.376317
621.820557 1.376992
621.820557 1.377494
621.820557 1.378879
621.820557 1.380388
621.820557 1.382464
621.820557 1.384759
621.820557 1.385305
621.820557 1.384891
621.820557 1.384964
621.820557 1.384548
621.820557 1.382614
621.820557 1.380797
621.820557 1.380965
621.820557 1.382905
621.820557 1.388143
621.820557 1.392162
621.820557 1.395827
621.820557 1.399702
621.820557 1.405998
621.820557 1.410505
621.820557 1.414559
621.820557 1.417395
621.820557 1.421043
621.820557 1.424292
621.820557 1.428046
621.820557 1.429803
621.820557 1.429813
621.820557 1.429928
621.820557 1.427272
621.820557 1.425488
621.820557 1.419933
621.820557 1.413121
621.820557 1.406100
621.820557 1.398256
621.820557 1.392486
621.820557 1.385839
621.820557 1.383487
621.820557 1.379082
621.820557 1.376572
621.820557 1.374195
621.820557 1.370429
621.820557 1.367129
621.820557 1.367228
621.820557 1.366929
621.820557 1.367141
621.820557 1.365629
621.820557 1.363821
621.820557 1.362053
621.820557 1.361111
621.820557 1.360162
621.820557 1.358840
621.820557 1.356576
621.820557 1.355867
621.820557 1.354247
621.820557 1.353661
621.820557 1.352320
621.820557 1.352183
621.820557 1.351831
621.820557 1.352594
621.820557 1.352394
621.820557 1.352423
621.820557 1.352178
621.820557 1.349964
621.820557 1.349237
621.820557 1.347189
621.820557 1.347776
621.820557 1.347272
621.820557 1.348227
621.820557 1.348966
621.820557 1.348736
621.820557 1.348978
621.820557 1.348156
621.820557 1.349169
621.820557 1.348604
621.820557 1.348072
621.820557 1.348280
621.820557 1.347205
621.820557 1.346428
621.820557 1.346934
621.820557 1.347930
621.820557 1.349951
621.820557 1.353252
621.820557 1.355455
621.820557 1.358106
621.820557 1.360903
621.820557 1.361856
621.820557 1.363261
621.820557 1.364922
621.820557 1.367380
621.820557 1.370700
621.820557 1.373546
621.820557 1.373756
621.820557 1.374355
621.820557 1.374348
621.820557 1.375104
621.820557 1.375451
621.820557 1.374357
621.820557 1.373232
621.820557 1.372242
621.820557 1.370597
621.820557 1.370269
621.820557 1.369022
621.820557 1.367234
621.820557 1.368960
621.820557 1.371200
621.820557 1.372309
621.820557 1.373149
621.820557 1.374767
621.820557 1.375383
621.820557 1.375192
621.820557 1.375736
621.820557 1.376960
621.820557 1.377493
621.820557 1.378084
621.820557 1.377775
621.820557 1.378100
621.820557 1.378839
621.820557 1.380837
621.820557 1.381832
621.820557 1.382832
621.820557 1.382720
621.820557 1.382431
621.820557 1.381856
621.820557 1.382673
621.820557 1.382218
621.820557 1.382378
621.820557 1.383028
621.820557 1.386265
621.820557 1.389132
621.820557 1.391541
621.820557 1.392223
621.820557 1.394284
621.820557 1.396406
621.820557 1.397724
621.820557 1.398164
621.820557 1.400074
621.820557 1.398118
621.820557 1.395959
621.820557 1.394510
621.820557 1.393460
621.820557 1.393630
621.820557 1.393514
621.820557 1.392647
621.820557 1.391918
621.820557 1.393599
621.820557 1.394403
621.820557 1.395585
621.820557 1.397528
621.820557 1.397622
621.820557 1.397211
621.820557 1.396990
621.820557 1.395070
621.820557 1.394963
621.820557 1.396076
621.820557 1.398040
621.820557 1.398658
621.820557 1.400755
621.820557 1.402552
621.820557 1.403143
621.820557 1.403762
621.820557 1.404094
621.820557 1.406552
621.820557 1.409194
621.820557 1.414406
621.820557 1.418142
621.820557 1.419414
621.820557 1.422992
621.820557 1.424417
621.820557 1.426840
621.820557 1.426892
621.820557 1.426912
621.820557 1.426362
621.820557 1.426770
621.820557 1.428753
621.820557 1.430042
621.820557 1.430666
621.820557 1.429870
621.820557 1.429654
621.820557 1.429677
621.820557 1.428497
621.820557 1.429527
621.820557 1.431329
621.820557 1.430955
621.820557 1.428597
621.820557 1.429998
621.820557 1.427919
621.820557 1.428147
621.820557 1.427735
621.820557 1.427045
621.820557 1.427834
621.820557 1.428393
621.820557 1.429682
621.820557 1.428144
621.820557 1.427016
621.820557 1.424974
621.820557 1.425082
621.820557 1.424156
621.820557 1.423162
621.820557 1.420740
621.820557 1.419004
621.820557 1.419253
621.820557 1.419880
621.820557 1.419101
621.820557 1.419119
621.820557 1.419884
621.820557 1.419495
621.820557 1.420874
621.820557 1.423404
621.820557 1.425407
621.820557 1.426923
621.820557 1.426882
621.820557 1.427608
621.820557 1.429606
621.820557 1.433992
621.820557 1.437573
621.820557 1.440171
621.820557 1.443914
621.820557 1.446633
621.820557 1.448590
621.820557 1.450123
621.820557 1.449762
621.820557 1.452254
621.820557 1.452411
621.820557 1.452572
621.820557 1.451939
621.820557 1.450076
621.820557 1.447046
621.820557 1.444920
621.820557 1.443168
621.820557 1.442099
621.820557 1.439958
621.820557 1.436200
621.820557 1.431775
621.820557 1.431103
621.820557 1.430757
621.820557 1.431248
621.820557 1.430967
621.820557 1.432757
621.820557 1.433995
621.820557 1.435174
621.820557 1.436903
621.820557 1.436829
621.820557 1.439600
621.820557 1.441014
621.820557 1.442641
621.820557 1.443057
621.820557 1.444873
621.820557 1.445487
621.820557 1.445148
621.820557 1.445977
621.820557 1.443155
621.820557 1.443225
621.820557 1.441710
621.820557 1.443290
621.820557 1.443658
621.820557 1.444743
621.820557 1.445568
621.820557 1.446616
621.820557 1.447274
621.820557 1.449940
621.820557 1.453252
621.820557 1.454994
621.820557 1.456863
621.820557 1.457022
621.820557 1.458762
621.820557 1.459640
621.820557 1.460606
621.820557 1.461858
621.820557 1.463482
621.820557 1.465875
621.820557 1.468915
621.820557 1.469828
621.820557 1.468754
621.820557 1.466459
621.820557 1.466663
621.820557 1.469390
621.820557 1.473164
621.820557 1.475283
621.820557 1.476181
621.820557 1.476870
621.820557 1.480190
621.820557 1.479393
621.820557 1.480469
621.820557 1.477647
621.820557 1.478158
621.820557 1.481478
621.820557 1.482477
621.820557 1.483203
621.820557 1.484829
621.820557 1.486239
621.820557 1.485820
621.820557 1.485677
621.820557 1.486871
621.820557 1.487246
621.820557 1.488030
621.820557 1.489990
621.820557 1.494328
621.820557 1.494486
621.820557 1.492398
621.820557 1.489694
621.820557 1.487862
621.820557 1.485516
621.820557 1.483343
621.820557 1.482881
621.820557 1.483636
621.820557 1.484355
621.820557 1.484973
621.820557 1.484891
621.820557 1.484158
621.820557 1.485219
621.820557 1.486081
621.820557 1.486542
621.820557 1.487675
621.820557 1.487609
621.820557 1.487404
621.820557 1.487628
621.820557 1.489620
621.820557 1.492006
621.820557 1.494180
621.820557 1.494993
621.820557 1.497970
621.820557 1.501843
621.820557 1.505121
621.820557 1.505011
621.820557 1.505051
621.820557 1.506644
621.820557 1.507989
621.820557 1.507767
621.820557 1.507034
621.820557 1.504608
621.820557 1.503757
621.820557 1.503644
621.820557 1.502102
621.820557 1.503987
621.820557 1.507289
621.820557 1.510269
621.820557 1.512653
621.820557 1.513876
621.820557 1.516143
621.820557 1.516255
621.820557 1.514570
621.820557 1.513197
621.820557 1.513400
621.820557 1.513806
621.820557 1.516286
621.820557 1.518436
621.820557 1.523046
621.820557 1.524911
621.820557 1.526911
621.820557 1.526596
621.820557 1.528373
621.820557 1.530396
621.820557 1.532435
621.820557 1.532965
621.820557 1.533136
621.820557 1.534327
621.820557 1.536302
621.820557 1.540150
621.820557 1.543300
621.820557 1.545020
621.820557 1.549387
621.820557 1.551937
621.820557 1.555273
621.820557 1.557804
621.820557 1.559247
621.820557 1.561176
621.820557 1.563758
621.820557 1.559593
621.820557 1.556105
621.820557 1.553104
621.820557 1.549592
621.820557 1.547984
621.820557 1.546669
621.820557 1.544643
621.820557 1.541905
621.820557 1.543352
621.820557 1.543096
621.820557 1.541847
621.820557 1.543330
621.820557 1.542007
621.820557 1.539660
621.820557 1.536680
621.820557 1.532528
621.820557 1.528813
621.820557 1.526193
621.820557 1.524886
621.820557 1.524088
621.820557 1.523274
621.820557 1.521684
621.820557 1.520781
621.820557 1.520286
621.820557 1.521690
621.820557 1.521208
621.820557 1.521615
621.820557 1.522384
621.820557 1.522952
621.820557 1.520998
621.820557 1.519977
621.820557 1.517227
621.820557 1.511817
621.820557 1.509465
621.820557 1.511216
621.820557 1.512309
621.820557 1.512009
621.820557 1.510660
621.820557 1.511930
621.820557 1.511374
621.820557 1.511046
621.820557 1.512000
621.820557 1.514424
621.820557 1.515446
621.820557 1.516446
621.820557 1.517977
621.820557 1.521186
621.820557 1.523141
621.820557 1.525007
621.820557 1.527761
621.820557 1.528895
621.820557 1.530767
621.820557 1.532208
621.820557 1.533053
621.820557 1.533132
621.820557 1.533225
621.820557 1.533806
621.820557 1.534452
621.820557 1.535377
621.820557 1.538692
621.820557 1.541219
621.820557 1.543428
621.820557 1.543568
621.820557 1.546157
621.820557 1.546645
621.820557 1.546908
621.820557 1.546112
621.820557 1.543712
621.820557 1.544407
621.820557 1.545368
621.820557 1.545453
621.820557 1.549571
621.820557 1.553429
621.820557 1.558771
621.820557 1.562829
621.820557 1.564107
621.820557 1.564797
621.820557 1.564568
621.820557 1.565194
621.820557 1.566028
621.820557 1.565722
621.820557 1.569835
621.820557 1.571127
621.820557 1.572310
621.820557 1.571854
621.820557 1.572582
621.820557 1.573363
621.820557 1.573866
621.820557 1.576151
621.820557 1.577128
621.820557 1.580879
621.820557 1.582634
621.820557 1.583846
621.820557 1.584280
621.820557 1.584942
621.820557 1.585781
621.820557 1.586929
621.820557 1.587556
621.820557 1.588009
621.820557 1.591525
621.820557 1.592662
621.820557 1.592886
621.820557 1.595760
621.820557 1.596193
621.820557 1.594844
621.820557 1.593583
621.820557 1.593915
621.820557 1.594267
621.820557 1.592732
641.315796 1.284380
641.315796 1.280837
641.315796 1.276297
641.315796 1.271112
641.315796 1.273710
641.315796 1.275217
641.315796 1.274828
641.315796 1.275020
641.315796 1.274491
641.315796 1.274696
641.315796 1.276925
641.315796 1.278716
641.315796 1.278647
641.315796 1.276224
641.315796 1.272739
641.315796 1.270460
641.315796 1.268942
641.315796 1.266349
641.315796 1.263750
641.315796 1.262302
641.315796 1.263814
641.315796 1.266046
641.315796 1.265865
641.315796 1.267333
641.315796 1.266144
641.315796 1.270727
641.315796 1.276106
641.315796 1.278755
641.315796 1.283102
641.315796 1.284211
641.315796 1.284008
641.315796 1.284908
641.315796 1.284616
641.315796 1.284857
641.315796 1.284916
641.315796 1.285139
641.315796 1.286751
641.315796 1.286362
641.315796 1.285524
641.315796 1.284552
641.315796 1.287030
641.315796 1.289351
641.315796 1.292452
641.315796 1.295799
641.315796 1.297563
641.315796 1.298687
641.315796 1.299261
641.315796 1.301086
641.315796 1.301416
641.315796 1.298201
641.315796 1.296454
641.315796 1.294678
641.315796 1.292007
641.315796 1.288969
641.315796 1.288178
641.315796 1.290236
641.315796 1.292314
661.007874 1.256996
661.007874 1.257165
661.007874 1.256721
661.007874 1.255560
661.007874 1.254530
661.007874 1.254572
661.007874 1.254412
661.007874 1.254363
661.007874 1.253299
661.007874 1.252432
661.007874 1.252741
661.007874 1.253738
661.007874 1.257416
661.007874 1.260935
661.007874 1.264082
661.007874 1.268150
661.007874 1.271013
661.007874 1.272082
661.007874 1.274598
661.007874 1.275540
661.007874 1.276925
661.007874 1.277821
661.007874 1.277558
661.007874 1.275972
661.007874 1.273207
661.007874 1.272648
661.007874 1.273538
661.007874 1.273532
661.007874 1.274409
661.007874 1.272634
661.007874 1.272335
661.007874 1.272874
661.007874 1.272477
661.007874 1.273253
661.007874 1.274317
661.007874 1.277152
661.007874 1.278382
661.007874 1.279407
661.007874 1.279842
661.007874 1.279853
661.007874 1.279929
661.007874 1.278512
661.007874 1.278663
661.007874 1.277926
661.007874 1.276350
661.007874 1.277579
661.007874 1.280393
661.007874 1.283162
661.007874 1.284618
661.007874 1.286506
661.007874 1.288100
661.007874 1.286862
661.007874 1.287204
661.007874 1.288117
661.007874 1.288527
661.007874 1.289038
661.007874 1.290326
661.007874 1.289728
661.007874 1.287902
661.007874 1.284702
661.007874 1.281705
661.007874 1.280491
661.007874 1.279090
661.007874 1.278324
661.007874 1.279135
661.007874 1.279738
661.007874 1.280173
661.007874 1.279241
661.007874 1.277562
661.007874 1.276970
661.007874 1.275580
661.007874 1.276594
661.007874 1.277396
661.007874 1.277894
661.007874 1.278370
661.007874 1.278827
661.007874 1.279022
661.007874 1.281219
661.007874 1.282027
661.007874 1.283639
661.007874 1.283464
661.007874 1.283937
661.007874 1.286394
661.007874 1.287738
661.007874 1.288490
661.007874 1.288611
661.007874 1.287170
661.007874 1.285819
661.007874 1.285733
661.007874 1.287771
661.007874 1.290473
661.007874 1.291243
661.007874 1.293320
661.007874 1.294089
661.007874 1.295943
661.007874 1.296263
661.007874 1.296494
661.007874 1.298952
661.007874 1.300452
661.007874 1.301074
661.007874 1.299707
661.007874 1.298285
661.007874 1.298386
661.007874 1.297779
661.007874 1.299876
661.007874 1.303092
661.007874 1.303334
661.007874 1.302063
661.007874 1.301070
661.007874 1.300913
661.007874 1.299223
661.007874 1.298726
661.007874 1.296681
661.007874 1.297553
661.007874 1.297123
661.007874 1.295550
661.007874 1.296044
661.007874 1.296993
661.007874 1.296040
661.007874 1.295082
661.007874 1.295866
661.007874 1.296584
661.007874 1.296559
661.007874 1.297824
661.007874 1.298036
661.007874 1.295643
661.007874 1.292570
661.007874 1.290633
661.007874 1.289388
661.007874 1.286787
661.007874 1.285490
661.007874 1.285730
661.007874 1.284895
661.007874 1.283609
661.007874 1.283362
661.007874 1.282070
661.007874 1.281723
661.007874 1.284776
661.007874 1.287227
661.007874 1.288940
661.007874 1.289639
661.007874 1.288549
661.007874 1.287056
661.007874 1.284418
661.007874 1.282786
661.007874 1.283255
661.007874 1.284297
661.007874 1.284517
661.007874 1.286582
661.007874 1.286894
661.007874 1.288323
661.007874 1.291287
661.007874 1.292323
661.007874 1.293378
661.007874 1.295101
661.007874 1.297750
661.007874 1.301040
661.007874 1.305133
661.007874 1.306392
661.007874 1.307358
661.007874 1.310399
661.007874 1.315215
661.007874 1.319395
661.007874 1.321813
661.007874 1.326147
661.007874 1.330121
661.007874 1.331214
661.007874 1.330645
661.007874 1.330113
661.007874 1.328593
661.007874 1.328030
661.007874 1.328320
661.007874 1.328538
661.007874 1.329521
661.007874 1.329444
661.007874 1.328614
661.007874 1.327888
661.007874 1.328568
661.007874 1.327630
661.007874 1.325512
661.007874 1.324708
661.007874 1.324733
661.007874 1.324595
661.007874 1.327202
661.007874 1.329661
661.007874 1.331845
661.007874 1.336199
661.007874 1.338800
661.007874 1.339504
661.007874 1.339312
661.007874 1.340681
661.007874 1.342568
661.007874 1.345320
661.007874 1.346225
661.007874 1.347586
661.007874 1.348027
661.007874 1.348910
661.007874 1.348997
661.007874 1.350616
661.007874 1.351179
661.007874 1.350736
661.007874 1.350927
661.007874 1.351438
661.007874 1.351155
661.007874 1.352221
661.007874 1.353572
661.007874 1.354308
661.007874 1.354397
661.007874 1.353907
661.007874 1.355881
661.007874 1.359078
661.007874 1.361627
661.007874 1.364545
661.007874 1.365671
661.007874 1.368413
661.007874 1.371227
661.007874 1.373430
661.007874 1.373607
661.007874 1.370536
661.007874 1.368753
661.007874 1.365567
661.007874 1.363241
661.007874 1.359838
661.007874 1.355951
661.007874 1.352458
661.007874 1.353359
661.007874 1.351005
661.007874 1.349403
661.007874 1.349035
661.007874 1.347862
661.007874 1.347189
661.007874 1.347462
661.007874 1.345841
661.007874 1.346411
661.007874 1.346349
661.007874 1.347598
661.007874 1.350181
661.007874 1.353301
661.007874 1.357350
661.007874 1.359018
661.007874 1.360949
661.007874 1.361020
661.007874 1.361548
661.007874 1.362448
661.007874 1.363125
661.007874 1.361211
661.007874 1.359009
661.007874 1.357059
661.007874 1.357559
661.007874 1.356428
661.007874 1.355096
661.007874 1.351558
661.007874 1.350129
661.007874 1.350076
661.007874 1.347821
661.007874 1.349123
661.007874 1.352231
661.007874 1.353559
661.007874 1.355790
661.007874 1.355628
661.007874 1.357576
661.007874 1.359425
661.007874 1.359805
661.007874 1.360193
661.007874 1.361420
661.007874 1.360686
661.007874 1.360483
661.007874 1.359078
661.007874 1.356110
661.007874 1.353607
661.007874 1.351707
661.007874 1.348968
661.007874 1.344283
661.007874 1.342631
661.007874 1.341482
661.007874 1.340149
661.007874 1.339796
661.007874 1.338256
661.007874 1.336788
661.007874 1.336702
661.007874 1.337844
661.007874 1.339133
661.007874 1.339437
661.007874 1.338796
661.007874 1.338939
661.007874 1.340316
661.007874 1.341453
661.007874 1.342296
661.007874 1.342645
661.007874 1.343225
661.007874 1.344790
661.007874 1.345433
661.007874 1.344537
661.007874 1.342664
661.007874 1.340534
661.007874 1.338645
661.007874 1.337135
661.007874 1.335546
661.007874 1.336018
661.007874 1.334319
661.007874 1.334655
661.007874 1.334643
661.007874 1.334769
661.007874 1.334594
661.007874 1.334082
661.007874 1.334154
661.007874 1.333887
661.007874 1.334567
661.007874 1.335285
661.007874 1.335612
661.007874 1.335452
661.007874 1.336156
661.007874 1.334432
661.007874 1.334798
661.007874 1.334979
661.007874 1.335159
661.007874 1.335464
661.007874 1.336295
661.007874 1.337407
661.007874 1.338497
661.007874 1.341348
661.007874 1.342047
661.007874 1.344435
661.007874 1.345066
661.007874 1.346420
661.007874 1.345878
661.007874 1.346941
661.007874 1.347306
661.007874 1.348370
661.007874 1.348312
661.007874 1.348042
661.007874 1.349146
661.007874 1.347473
661.007874 1.347228
661.007874 1.345171
661.007874 1.344250
682.356018 1.045223
682.356018 1.044093
682.356018 1.042406
682.356018 1.041525
682.356018 1.039852
682.356018 1.038602
682.356018 1.038120
682.356018 1.037763
682.356018 1.039241
682.356018 1.041228
682.356018 1.041492
682.356018 1.042434
682.356018 1.043180
682.356018 1.045105
682.356018 1.045946
682.356018 1.045985
682.356018 1.044719
682.356018 1.044356
682.356018 1.042917
682.356018 1.042548
682.356018 1.042283
682.356018 1.041395
682.356018 1.041177
682.356018 1.040159
682.356018 1.039636
682.356018 1.039098
682.356018 1.039192
682.356018 1.040563
682.356018 1.040907
682.356018 1.043969
682.356018 1.048425
682.356018 1.050550
682.356018 1.052894
682.356018 1.056194
682.356018 1.057846
682.356018 1.060265
682.356018 1.062588
682.356018 1.063797
682.356018 1.064139
682.356018 1.063952
682.356018 1.063990
682.356018 1.063447
682.356018 1.062558
682.356018 1.061641
682.356018 1.060088
682.356018 1.057487
682.356018 1.055337
682.356018 1.055167
682.356018 1.055359
682.356018 1.055266
682.356018 1.055330
682.356018 1.055305
682.356018 1.055052
682.356018 1.056073
682.356018 1.056000
682.356018 1.056145
682.356018 1.056932
682.356018 1.055954
682.356018 1.055251
682.356018 1.054704
682.356018 1.057942
682.356018 1.060555
682.356018 1.063470
682.356018 1.065215
682.356018 1.066050
682.356018 1.066190
682.356018 1.067363
682.356018 1.069485
682.356018 1.071029
682.356018 1.072350
682.356018 1.073111
682.356018 1.073777
682.356018 1.074644
682.356018 1.074505
682.356018 1.073646
682.356018 1.074204
682.356018 1.076023
682.356018 1.076500
682.356018 1.074541
682.356018 1.074155
682.356018 1.076329
682.356018 1.079372
682.356018 1.081344
682.356018 1.083999
682.356018 1.085439
682.356018 1.085414
682.356018 1.086214
682.356018 1.087382
682.356018 1.088220
682.356018 1.086884
682.356018 1.084901
682.356018 1.083618
682.356018 1.081946
682.356018 1.081393
682.356018 1.081630
682.356018 1.082648
682.356018 1.081520
682.356018 1.081419
682.356018 1.079418
682.356018 1.077899
682.356018 1.079007
682.356018 1.079207
682.356018 1.078816
682.356018 1.078891
682.356018 1.081379
682.356018 1.083379
682.356018 1.084761
682.356018 1.084447
682.356018 1.082803
682.356018 1.081094
682.356018 1.080283
682.356018 1.080171
682.356018 1.080717
682.356018 1.081915
682.356018 1.083524
682.356018 1.084715
682.356018 1.085763
682.356018 1.088001
682.356018 1.090953
682.356018 1.093602
682.356018 1.096694
682.356018 1.100630
682.356018 1.102684
682.356018 1.102575
682.356018 1.101871
682.356018 1.099940
682.356018 1.098981
682.356018 1.098018
682.356018 1.095062
682.356018 1.092998
682.356018 1.091901
682.356018 1.090076
682.356018 1.090396
682.356018 1.090773
682.356018 1.091581
682.356018 1.092620
682.356018 1.092672
682.356018 1.093553
682.356018 1.093503
682.356018 1.094015
682.356018 1.095356
682.356018 1.096136
682.356018 1.097773
682.356018 1.098149
682.356018 1.098860
682.356018 1.099478
682.356018 1.100512
682.356018 1.101826
682.356018 1.102307
682.356018 1.103026
682.356018 1.103557
682.356018 1.103597
682.356018 1.104044
682.356018 1.105922
682.356018 1.106374
682.356018 1.106272
682.356018 1.106135
682.356018 1.104352
682.356018 1.103121
682.356018 1.100835
682.356018 1.099662
682.356018 1.100847
682.356018 1.101048
682.356018 1.101066
682.356018 1.103191
682.356018 1.105346
682.356018 1.107748
682.356018 1.109170
682.356018 1.109905
682.356018 1.111094
682.356018 1.112187
682.356018 1.111794
682.356018 1.111168
682.356018 1.111395
682.356018 1.111483
682.356018 1.110217
682.356018 1.108585
682.356018 1.108979
682.356018 1.108269
682.356018 1.107875
682.356018 1.107656
682.356018 1.109869
682.356018 1.110892
682.356018 1.110717
682.356018 1.112844
682.356018 1.116508
682.356018 1.118934
682.356018 1.121218
682.356018 1.123962
682.356018 1.125456
682.356018 1.126274
682.356018 1.127914
682.356018 1.128605
682.356018 1.128476
682.356018 1.128375
682.356018 1.127939
682.356018 1.128225
682.356018 1.127337
682.356018 1.126161
682.356018 1.124932
682.356018 1.125373
682.356018 1.125260
682.356018 1.124424
682.356018 1.123706
682.356018 1.122277
682.356018 1.121464
682.356018 1.122668
682.356018 1.123008
682.356018 1.122898
682.356018 1.121858
682.356018 1.120435
682.356018 1.118509
682.356018 1.116480
682.356018 1.116476
682.356018 1.115779
682.356018 1.115123
682.356018 1.112989
682.356018 1.112803
682.356018 1.114081
682.356018 1.113892
682.356018 1.114593
682.356018 1.115151
682.356018 1.116031
682.356018 1.118243
682.356018 1.120459
682.356018 1.121881
682.356018 1.124472
682.356018 1.130064
682.356018 1.134399
682.356018 1.138468
682.356018 1.142177
682.356018 1.144038
682.356018 1.145587
682.356018 1.146415
682.356018 1.147774
682.356018 1.149203
682.356018 1.149928
682.356018 1.150886
682.356018 1.151759
682.356018 1.152026
682.356018 1.154086
682.356018 1.155002
682.356018 1.155463
682.356018 1.155979
682.356018 1.156596
682.356018 1.157014
682.356018 1.156999
682.356018 1.154820
682.356018 1.154431
682.356018 1.154091
682.356018 1.155179
682.356018 1.154908
682.356018 1.157813
682.356018 1.159123
682.356018 1.162438
682.356018 1.164596
682.356018 1.164991
682.356018 1.164693
682.356018 1.165627
682.356018 1.165276
682.356018 1.163701
682.356018 1.162513
682.356018 1.161922
682.356018 1.160845
682.356018 1.161184
682.356018 1.162078
682.356018 1.162982
682.356018 1.163273
682.356018 1.164486
682.356018 1.165892
682.356018 1.166790
682.356018 1.166170
682.356018 1.166108
682.356018 1.165707
682.356018 1.165966
682.356018 1.165385
682.356018 1.164881
682.356018 1.165084
682.356018 1.164935
682.356018 1.165531
682.356018 1.167271
682.356018 1.169047
682.356018 1.170899
682.356018 1.171576
682.356018 1.171696
682.356018 1.172565
682.356018 1.172137
682.356018 1.170762
682.356018 1.170887
682.356018 1.170203
682.356018 1.170278
682.356018 1.170338
682.356018 1.169362
682.356018 1.167715
682.356018 1.164997
682.356018 1.163954
682.356018 1.164190
682.356018 1.164737
682.356018 1.165024
682.356018 1.166036
682.356018 1.165266
682.356018 1.167048
682.356018 1.168955
682.356018 1.170397
682.356018 1.172320
682.356018 1.174339
682.356018 1.174126
682.356018 1.174702
682.356018 1.176220
682.356018 1.176951
682.356018 1.175819
682.356018 1.174892
682.356018 1.176080
682.356018 1.175702
682.356018 1.175705
682.356018 1.175223
682.356018 1.174237
682.356018 1.173948
682.356018 1.173208
682.356018 1.173622
682.356018 1.173215
682.356018 1.171811
682.356018 1.170390
682.356018 1.168601
682.356018 1.167144
682.356018 1.164841
682.356018 1.162094
682.356018 1.159556
682.356018 1.158725
682.356018 1.158251
682.356018 1.157966
682.356018 1.156416
682.356018 1.156341
682.356018 1.156385
682.356018 1.157518
682.356018 1.157262
682.356018 1.155107
682.356018 1.154484
682.356018 1.153639
682.356018 1.155677
682.356018 1.156079
682.356018 1.156133
682.356018 1.155844
682.356018 1.155475
682.356018 1.155327
682.356018 1.156261
682.356018 1.155279
682.356018 1.157202
682.356018 1.157516
682.356018 1.157658
682.356018 1.158055
682.356018 1.157070
682.356018 1.154376
682.356018 1.154483
682.356018 1.153193
682.356018 1.151355
682.356018 1.149412
682.356018 1.148400
682.356018 1.146695
682.356018 1.145990
682.356018 1.143350
682.356018 1.142039
682.356018 1.141680
682.356018 1.141281
682.356018 1.140387
682.356018 1.141748
682.356018 1.142139
682.356018 1.142569
682.356018 1.144069
682.356018 1.143499
682.356018 1.143431
682.356018 1.143190
682.356018 1.142410
682.356018 1.141126
682.356018 1.139363
682.356018 1.138989
682.356018 1.138335
682.356018 1.138429
682.356018 1.138858
682.356018 1.138214
682.356018 1.139135
682.356018 1.139014
682.356018 1.138648
682.356018 1.138597
682.356018 1.143615
682.356018 1.145051
682.356018 1.144506
682.356018 1.144463
682.356018 1.146438
682.356018 1.146874
682.356018 1.147379
682.356018 1.148272
682.356018 1.150071
682.356018 1.152381
682.356018 1.152144
682.356018 1.152319
682.356018 1.152958
682.356018 1.155904
682.356018 1.158713
682.356018 1.160611
682.356018 1.162095
682.356018 1.162810
682.356018 1.162252
682.356018 1.162432
682.356018 1.162708
682.356018 1.161212
682.356018 1.161205
682.356018 1.159393
682.356018 1.159489
682.356018 1.159263
682.356018 1.157790
682.356018 1.158338
682.356018 1.157074
682.356018 1.154878
682.356018 1.151702
682.356018 1.149350
682.356018 1.146875
682.356018 1.144568
682.356018 1.140432
682.356018 1.137452
682.356018 1.136775
682.356018 1.137213
682.356018 1.137868
682.356018 1.137470
682.356018 1.135793
682.356018 1.134769
682.356018 1.133777
682.356018 1.133462
682.356018 1.135155
682.356018 1.137947
682.356018 1.139853
682.356018 1.139970
682.356018 1.142824
682.356018 1.143744
682.356018 1.144409
682.356018 1.147468
682.356018 1.149073
682.356018 1.151266
682.356018 1.154100
682.356018 1.155952
682.356018 1.158391
682.356018 1.161019
682.356018 1.164034
682.356018 1.168335
682.356018 1.171019
682.356018 1.175322
682.356018 1.179093
682.356018 1.182152
682.356018 1.186312
682.356018 1.189586
682.356018 1.192445
682.356018 1.194389
682.356018 1.195876
682.356018 1.199798
682.356018 1.202200
682.356018 1.202956
682.356018 1.202396
682.356018 1.201206
682.356018 1.201607
682.356018 1.203548
682.356018 1.204002
682.356018 1.203004
682.356018 1.200222
682.356018 1.199852
682.356018 1.203487
682.356018 1.208533
682.356018 1.209327
682.356018 1.209339
682.356018 1.210351
682.356018 1.210877
682.356018 1.213347
682.356018 1.213200
682.356018 1.212772
682.356018 1.214720
682.356018 1.215862
682.356018 1.220037
682.356018 1.224185
682.356018 1.225683
682.356018 1.226773
682.356018 1.227969
682.356018 1.229027
682.356018 1.231825
682.356018 1.233418
682.356018 1.235898
682.356018 1.237602
682.356018 1.239610
682.356018 1.240974
682.356018 1.243711
682.356018 1.246713
682.356018 1.251055
682.356018 1.254821
682.356018 1.259342
682.356018 1.262602
682.356018 1.263849
682.356018 1.266329
682.356018 1.266859
682.356018 1.268063
682.356018 1.270225
682.356018 1.272516
682.356018 1.276774
682.356018 1.281767
682.356018 1.283589
682.356018 1.286272
682.356018 1.287910
682.356018 1.287871
682.356018 1.285417
682.356018 1.285125
682.356018 1.286057
682.356018 1.287609
682.356018 1.286901
682.356018 1.283736
682.356018 1.282789
682.356018 1.279083
682.356018 1.276077
682.356018 1.274909
682.356018 1.274285
682.356018 1.274183
682.356018 1.271458
682.356018 1.270223
682.356018 1.268037
682.356018 1.264327
682.356018 1.260780
682.356018 1.257714
682.356018 1.254881
682.356018 1.253038
682.356018 1.253831
682.356018 1.257232
682.356018 1.260709
682.356018 1.264953
682.356018 1.271057
682.356018 1.272849
682.356018 1.274966
682.356018 1.276369
682.356018 1.277437
682.356018 1.276133
682.356018 1.274720
682.356018 1.273298
682.356018 1.272494
682.356018 1.270048
682.356018 1.269422
682.356018 1.270015
682.356018 1.272621
682.356018 1.272634
682.356018 1.273417
682.356018 1.273988
682.356018 1.273944
682.356018 1.272371
682.356018 1.271602
682.356018 1.271780
682.356018 1.270516
682.356018 1.269512
682.356018 1.268353
682.356018 1.266773
682.356018 1.265386
682.356018 1.266067
682.356018 1.266345
682.356018 1.266719
682.356018 1.268334
682.356018 1.270270
682.356018 1.272188
682.356018 1.273689
682.356018 1.274912
682.356018 1.275924
682.356018 1.275937
682.356018 1.280705
682.356018 1.283565
682.356018 1.288440
682.356018 1.290789
682.356018 1.292367
682.356018 1.295052
682.356018 1.297488
682.356018 1.296471
682.356018 1.296097
682.356018 1.294504
682.356018 1.291333
682.356018 1.288452
682.356018 1.285439
682.356018 1.283241
682.356018 1.285031
682.356018 1.288165
682.356018 1.288499
682.356018 1.288769
682.356018 1.286962
682.356018 1.286254
682.356018 1.286462
682.356018 1.286535
682.356018 1.285022
682.356018 1.282133
682.356018 1.284070
682.356018 1.284663
682.356018 1.287265
682.356018 1.290519
682.356018 1.291657


==> fig/data/avgq-vs-success-2/bt-l2-cdf.tex <==
0 0.281216
78.468086 0.331157
161.378372 0.346344
215.415726 0.376683
288.514282 0.380493
350.854706 0.392640
413.078125 0.393546
440.469696 0.412830
506.170227 0.421702
546.821899 0.438462
591.562927 0.458514
630.890320 0.479395
693.788818 0.483051
727.963440 0.500711
763.676636 0.520069
800.517639 0.535003
840.289001 0.551876
882.431824 0.554064
925.754211 0.570484
1016.032410 0.578620
1091.463135 0.578786
1138.673584 0.591166
1201.705566 0.600195
1267.323364 0.608405
1302.009888 0.621434
1319.460815 0.637393
1392.528809 0.636152
1464.801880 0.644126
1557.087524 0.644217
1613.709106 0.653749
1670.780273 0.660735
1748.643188 0.671030
1788.960693 0.688583
1829.740234 0.706568
1911.863770 0.703043
1974.865601 0.714582
2017.441650 0.733977
2083.440430 0.737159
2105.368896 0.747754
2173.522217 0.763643
2173.522217 0.787305
2173.522217 0.810399
2222.770996 0.811871
2322.790527 0.807291
2347.692871 0.826111
2373.678467 0.847702
2400.218750 0.860007
2531.072754 0.850455
2558.015381 0.874160
2584.798584 0.890207
2584.798584 0.913007


==> fig/data/avgq-vs-success-2/bt-linf-cdf.tex <==
0.000000 0.280978
79.413330 0.359312
132.435638 0.441775
218.000000 0.519249
309.629639 0.581056
406.590668 0.584604
445.756104 0.679812
528.343628 0.682452
592.065857 0.720201
626.573730 0.782952
671.746155 0.825484
714.708984 0.873712
755.461792 0.929869
799.368774 0.978271
851.717224 0.998265
872.593872 1.071844
953.388184 1.027919
990.951477 1.028410
1030.942627 1.050187
1080.043701 1.081123
1105.795654 1.103199
1142.330322 1.127447
1161.531860 1.165692
1171.624268 1.220989
1182.096680 1.266988
1215.634766 1.288651
1261.520752 1.293473
1308.801147 1.288599
1333.732544 1.352157
1358.497070 1.356106
1358.497070 1.418083
1358.497070 1.468975
1358.497070 1.527079
1373.365967 1.590863
1404.022949 1.599658
1451.079590 1.560889
1499.104248 1.526739
1531.837524 1.483279
1548.413452 1.513593
1565.493042 1.536319
1583.300049 1.547239
1601.301880 1.510457
1656.516479 1.560436
1656.516479 1.606562
1694.907104 1.652824
1714.288818 1.652371
1734.298950 1.700373
1754.812988 1.638189
1754.812988 1.691710
1776.464844 1.643199
1798.544434 1.590239


==> fig/data/avgq-vs-success-2/btd-l2-cdf.tex <==
0 0.283590
74.433960 0.381287
131.208328 0.416682
174.134964 0.469554
231.530060 0.505449
266.062164 0.577107
317.902924 0.604197
387.072083 0.620869
467.924683 0.618761
521.504028 0.640281
538.110657 0.696766
592.053406 0.716048
611.358521 0.761785
639.702576 0.803927
670.754578 0.866874
719.103943 0.897549
752.544189 0.924213
813.151733 0.909739
859.091553 0.910019
897.398010 0.900582
926.894043 0.950155
958.216370 0.974080
1023.228271 0.962068
1034.224365 0.980990
1069.085693 1.032836
1105.710693 1.020796
1168.365356 0.996129
1206.116577 1.002128
1245.811523 1.014550
1245.811523 1.054302
1245.811523 1.095445
1245.811523 1.136883
1291.174683 1.110516
1291.174683 1.147334
1307.171143 1.185215
1307.171143 1.223407
1324.766479 1.262548
1360.541626 1.279172
1360.541626 1.319193
1360.541626 1.361202
1360.541626 1.400749
1360.541626 1.439829
1401.757446 1.414038
1422.648926 1.460449
1465.061523 1.478402
1487.029297 1.531763
1509.346924 1.573170
1576.410400 1.509227
1576.410400 1.543278
1599.763672 1.538633
1647.386841 1.493848


==> fig/data/avgq-vs-success-2/btd-linf-cdf.tex <==
0.000000 0.289285
43.848484 0.521900
95.502007 0.542509
125.605949 0.577919
161.923340 0.626385
206.052460 0.701729
247.143753 0.723415
272.530487 0.773021
304.860535 0.791450
320.979462 0.802198
334.622101 0.861957
365.508575 0.832775
392.366211 0.727790
404.106445 0.752443
417.169922 0.743052
424.333344 0.877781
439.441986 0.972311
455.076935 1.049977
471.972687 1.008040
480.795654 1.050074
489.820648 1.052852
489.820648 1.118450
510.059448 1.150802
510.059448 1.278429
532.704285 1.185743
556.176453 1.192700
580.132996 1.087358
592.907166 1.093893
605.735474 1.120647
605.735474 1.140766
605.735474 1.175797
605.735474 1.189423
605.735474 1.251002
605.735474 1.308113
621.820557 1.338096
621.820557 1.302317
621.820557 1.352423
621.820557 1.404094
621.820557 1.453252
621.820557 1.549387
621.820557 1.584280
661.007874 1.273532
661.007874 1.290633
661.007874 1.349403
661.007874 1.347306
682.356018 1.083618
682.356018 1.127914
682.356018 1.170338
682.356018 1.148272
682.356018 1.259342
682.356018 1.290519


==> fig/data/avgq-vs-success-2/nes-l2-cdf.tex <==
0 0.282171
0 0.285060
0 0.288035
30.000000 0.284903
30.000000 0.287910
30.000000 0.291048
30.000000 0.294138
30.000000 0.297159
30.000000 0.300133
60.000000 0.297407
60.000000 0.300296
67.142860 0.299868
73.750000 0.296637
73.750000 0.299559
73.750000 0.302592
73.750000 0.305443
83.333336 0.305184
99.090912 0.304585
99.090912 0.307578
113.076920 0.304110
113.076920 0.307028
120.000000 0.305577
120.000000 0.308618
120.000000 0.311733
128.000000 0.312881
128.000000 0.316043
136.250000 0.317520
136.250000 0.320502
144.705887 0.318338
144.705887 0.321303
161.052628 0.311822
175.238098 0.309870
181.818176 0.311347
181.818176 0.314188
181.818176 0.317106
189.130432 0.316629
189.130432 0.319579
203.600006 0.318327
203.600006 0.321383
210.769226 0.322733
217.777771 0.322880
224.642853 0.322791
224.642853 0.325859
231.724136 0.324560
231.724136 0.327392
245.806458 0.327686
252.500000 0.324936
259.090912 0.324344
265.588226 0.321942
272.000000 0.322129
272.000000 0.324924
278.611115 0.323798
278.611115 0.326583
278.611115 0.329455
285.675690 0.328241
299.230774 0.327924
305.750000 0.329500
312.195129 0.328452
318.571442 0.326009
318.571442 0.328843
331.363647 0.328100
337.555542 0.324733
343.695648 0.325965
349.787231 0.326264
349.787231 0.329292
356.041656 0.330559
356.041656 0.333470
362.448975 0.329739
362.448975 0.332619
369.000000 0.332642
369.000000 0.335356
375.686279 0.336831
382.307678 0.337966
382.307678 0.340856
382.307678 0.343818
382.307678 0.346762
389.433960 0.348584
389.433960 0.351630
410.357147 0.342477
410.357147 0.345583
436.333344 0.334734
442.459015 0.336205
442.459015 0.339126
442.459015 0.341915
461.093750 0.336336
461.093750 0.339196
467.230774 0.339835
467.230774 0.342833
473.484863 0.344062
479.701508 0.345473
485.882355 0.345358
498.000000 0.343034
503.943665 0.342704
503.943665 0.345441
510.000000 0.342591
510.000000 0.345236
510.000000 0.348093
510.000000 0.350736
510.000000 0.353678
516.575317 0.355264
529.466675 0.346672
535.789490 0.347877
542.077942 0.344880
548.333313 0.345879
554.556946 0.344762
554.556946 0.347382
554.556946 0.349968
554.556946 0.352571
561.125000 0.353916
567.654297 0.354721
567.654297 0.357432
580.722900 0.352142
580.722900 0.354833
580.722900 0.357568
587.380981 0.352303
594.000000 0.352944
594.000000 0.355753
600.697693 0.352914
600.697693 0.355524
600.697693 0.358203
607.586182 0.357509
621.123596 0.356708
627.777771 0.357753
634.395630 0.359027
634.395630 0.361723
634.395630 0.364428
634.395630 0.367114
641.304321 0.366675
648.172058 0.365930
648.172058 0.368496
655.106384 0.370187
662.000000 0.370620
662.000000 0.373493
668.958313 0.373389
668.958313 0.376287
682.857117 0.371309
682.857117 0.373980
682.857117 0.376864
689.898987 0.376297
689.898987 0.379092
689.898987 0.381893
689.898987 0.384595
689.898987 0.387455
704.554443 0.383886
704.554443 0.386553
704.554443 0.389510
719.223328 0.388513
719.223328 0.391240
719.223328 0.394182
733.904785 0.388931
733.904785 0.391658
733.904785 0.394475
733.904785 0.397364
733.904785 0.400237
733.904785 0.403171
741.603760 0.399699
741.603760 0.402628
741.603760 0.405368
741.603760 0.408320
741.603760 0.411300
765.229370 0.403754
780.450439 0.400174
787.946411 0.400515
787.946411 0.403163
802.894714 0.399609
817.500000 0.389309
817.500000 0.391965
824.786316 0.392161
824.786316 0.394839
832.118652 0.392466
832.118652 0.395007
839.495789 0.393392
839.495789 0.395937
839.495789 0.398569
847.000000 0.398348
847.000000 0.401153
854.545471 0.402174
854.545471 0.404903
854.545471 0.407582
854.545471 0.410238
854.545471 0.412953
854.545471 0.415752
862.459045 0.410401
870.325195 0.406177
878.145142 0.407564
878.145142 0.410075
886.000000 0.410997
901.496033 0.398977
909.140625 0.395639
916.744202 0.396609
916.744202 0.399130
916.744202 0.401523
916.744202 0.404172
924.538452 0.399838
924.538452 0.402486
924.538452 0.404980
924.538452 0.407571
924.538452 0.409977
924.538452 0.412487
932.671753 0.410610
948.721802 0.406064
948.721802 0.408671
948.721802 0.410959
948.721802 0.413292
972.794128 0.397259
972.794128 0.399755
980.729919 0.400226
988.623169 0.401202
988.623169 0.403531
988.623169 0.406155
996.618713 0.403018
996.618713 0.405450
996.618713 0.408014
996.618713 0.410404
996.618713 0.412828
996.618713 0.415236
1004.928589 0.413505
1004.928589 0.415922
1004.928589 0.418279
1021.619690 0.417107
1021.619690 0.419647
1021.619690 0.422028
1021.619690 0.424595
1021.619690 0.427075
1021.619690 0.429561
1021.619690 0.431966
1021.619690 0.434528
1021.619690 0.437106
1021.619690 0.439652
1021.619690 0.442111
1021.619690 0.444585
1021.619690 0.447044
1021.619690 0.449602
1021.619690 0.452284
1021.619690 0.454657
1021.619690 0.457195
1040.208374 0.455234
1040.208374 0.457824
1040.208374 0.460318
1040.208374 0.462829
1040.208374 0.465420
1040.208374 0.468160
1049.724121 0.462308
1049.724121 0.464983
1059.246582 0.466100
1068.707520 0.462408
1078.108154 0.462594
1078.108154 0.465158
1078.108154 0.468000
1078.108154 0.470596
1078.108154 0.473130
1078.108154 0.475771
1078.108154 0.478574
1078.108154 0.481324
1087.919434 0.483195
1097.666626 0.483917
1107.350952 0.485262
1107.350952 0.488034
1107.350952 0.490844
1107.350952 0.493604
1107.350952 0.496336
1107.350952 0.499123
1117.302612 0.499712
1117.302612 0.502468
1117.302612 0.505320
1117.302612 0.508206
1117.302612 0.510941
1137.467529 0.509091
1137.467529 0.511867
1137.467529 0.514775
1137.467529 0.517645
1137.467529 0.520272
1137.467529 0.523102
1137.467529 0.526097
1147.806396 0.523680
1147.806396 0.526611
1158.140991 0.525477
1158.140991 0.527994
1158.140991 0.530149
1168.535034 0.530819
1178.860718 0.527250
1189.119507 0.519218
1199.312500 0.512161
1199.312500 0.513914
1199.312500 0.515567
1199.312500 0.517449
1199.312500 0.519007
1199.312500 0.520700
1199.312500 0.522402
1209.813721 0.520796
1209.813721 0.522260
1209.813721 0.523744
1209.813721 0.525448
1209.813721 0.527128
1209.813721 0.528656
1209.813721 0.530390
1209.813721 0.531902
1220.678955 0.527091
1220.678955 0.528533
1231.533691 0.526666
1231.533691 0.528323
1231.533691 0.529783
1231.533691 0.531338
1231.533691 0.533019
1242.561035 0.527300
1242.561035 0.528957
1253.575806 0.525112
1253.575806 0.526803
1253.575806 0.528354
1253.575806 0.529689
1253.575806 0.531282
1264.759033 0.524873
1264.759033 0.526211
1264.759033 0.527757
1264.759033 0.529413
1264.759033 0.530773
1276.107788 0.528233
1276.107788 0.529726
1276.107788 0.531135
1276.107788 0.532526
1287.559570 0.531325
1287.559570 0.532653
1298.994141 0.529576
1298.994141 0.531142
1310.411743 0.528530
1310.411743 0.529932
1310.411743 0.531399
1310.411743 0.532977
1310.411743 0.534519
1310.411743 0.535977
1310.411743 0.537442
1310.411743 0.538826
1310.411743 0.540206
1310.411743 0.541685
1310.411743 0.543102
1310.411743 0.544466
1310.411743 0.545828
1310.411743 0.547156
1310.411743 0.548526
1310.411743 0.549966
1310.411743 0.551318
1310.411743 0.552747
1310.411743 0.554115
1310.411743 0.555798
1310.411743 0.557303
1322.923950 0.552985
1322.923950 0.554372
1335.406982 0.552274
1335.406982 0.553654
1335.406982 0.555142
1335.406982 0.556690
1335.406982 0.558178
1335.406982 0.559527
1335.406982 0.560837
1335.406982 0.562178
1335.406982 0.563441
1335.406982 0.564998
1335.406982 0.566544
1335.406982 0.567948
1335.406982 0.569537
1335.406982 0.571106
1348.554932 0.571012
1348.554932 0.572398
1361.666626 0.572364
1361.666626 0.573788
1361.666626 0.575313
1361.666626 0.576773
1361.666626 0.578088
1374.914307 0.572447
1374.914307 0.573881
1374.914307 0.575243
1388.181763 0.559567
1401.355957 0.555891
1401.355957 0.557188
1401.355957 0.558431
1414.550537 0.558739
1414.550537 0.560102
1427.709473 0.557424
1427.709473 0.558751
1440.833374 0.552457
1440.833374 0.553699
1440.833374 0.555072
1453.977905 0.552133
1453.977905 0.553352
1453.977905 0.554744
1467.142822 0.554583
1467.142822 0.555899
1467.142822 0.557133
1467.142822 0.558408
1467.142822 0.559692
1467.142822 0.560983
1467.142822 0.562354
1467.142822 0.563820
1467.142822 0.564918
1467.142822 0.566230
1467.142822 0.567548
1467.142822 0.568837
1467.142822 0.570081
1467.142822 0.571397
1467.142822 0.572769
1467.142822 0.573928
1467.142822 0.575297
1467.142822 0.576712
1467.142822 0.578042
1467.142822 0.579476
1467.142822 0.580843
1467.142822 0.582028
1467.142822 0.583252
1467.142822 0.584625
1467.142822 0.586026
1467.142822 0.587413
1467.142822 0.588966
1467.142822 0.590287
1467.142822 0.591869
1467.142822 0.593349
1467.142822 0.594623
1467.142822 0.595931
1481.912598 0.593290
1481.912598 0.594642
1481.912598 0.595942
1481.912598 0.597246
1481.912598 0.598493
1481.912598 0.599683
1481.912598 0.600822
1496.902222 0.601089
1496.902222 0.602402
1511.837891 0.599547
1526.666626 0.591630
1526.666626 0.592911
1526.666626 0.593947
1526.666626 0.595254
1526.666626 0.596435
1526.666626 0.597737
1541.657715 0.597777
1541.657715 0.598894
1541.657715 0.600129
1556.648926 0.594671
1571.534424 0.591480
1571.534424 0.592688
1571.534424 0.593994
1571.534424 0.595339
1571.534424 0.596544
1571.534424 0.597864
1571.534424 0.599288
1571.534424 0.600458
1586.684204 0.593974
1616.614624 0.573690
1631.398926 0.573522
1631.398926 0.574646
1631.398926 0.575889
1646.185547 0.572714
1646.185547 0.574057
1646.185547 0.575224
1646.185547 0.576573
1646.185547 0.577858
1646.185547 0.578895
1646.185547 0.579940
1646.185547 0.581186
1646.185547 0.582240
1646.185547 0.583495
1646.185547 0.584878
1646.185547 0.586193
1646.185547 0.587364
1646.185547 0.588422
1646.185547 0.589646
1646.185547 0.590813
1646.185547 0.591978
1646.185547 0.593238
1646.185547 0.594475
1646.185547 0.595818
1646.185547 0.597118
1661.897461 0.595649
1661.897461 0.596807
1661.897461 0.597938
1661.897461 0.599190
1677.653076 0.594337
1677.653076 0.595423
1677.653076 0.596547
1677.653076 0.597888
1677.653076 0.598872
1677.653076 0.600034
1677.653076 0.601441
1693.604004 0.592033
1693.604004 0.593239
1709.494995 0.593078
1709.494995 0.593840
1709.494995 0.595067
1709.494995 0.596164
1725.427124 0.595034
1725.427124 0.596369
1725.427124 0.597294
1725.427124 0.598329
1725.427124 0.599442
1725.427124 0.600619
1725.427124 0.601826
1725.427124 0.603074
1725.427124 0.604240
1725.427124 0.605355
1741.699951 0.594930
1741.699951 0.596289
1741.699951 0.597595
1741.699951 0.598688
1741.699951 0.599793
1758.059692 0.595192
1758.059692 0.596117
1758.059692 0.597247
1758.059692 0.598224
1758.059692 0.599397
1758.059692 0.600713
1758.059692 0.601713
1758.059692 0.603055
1758.059692 0.604135
1758.059692 0.605516
1758.059692 0.606939
1758.059692 0.608105
1758.059692 0.609195
1758.059692 0.610285
1758.059692 0.611412
1758.059692 0.612446
1758.059692 0.613511
1758.059692 0.614881
1758.059692 0.616013
1758.059692 0.617224
1758.059692 0.618248
1758.059692 0.619321
1775.346558 0.608481
1775.346558 0.609694
1775.346558 0.610978
1775.346558 0.612070
1775.346558 0.612988
1775.346558 0.614035
1775.346558 0.615414
1775.346558 0.616509
1775.346558 0.617674
1775.346558 0.618839
1775.346558 0.620051
1775.346558 0.621052
1775.346558 0.621928
1775.346558 0.623002
1775.346558 0.623971
1793.202026 0.623958
1793.202026 0.624903
1793.202026 0.625999
1793.202026 0.627108
1793.202026 0.628213
1811.127441 0.626230
1811.127441 0.627237
1811.127441 0.628354
1811.127441 0.629453
1811.127441 0.630453
1811.127441 0.631689
1811.127441 0.632852
1811.127441 0.634144
1811.127441 0.635257
1811.127441 0.636061
1811.127441 0.637331
1811.127441 0.638376
1811.127441 0.639351
1811.127441 0.640417
1811.127441 0.641527
1811.127441 0.642415
1829.658569 0.636473
1829.658569 0.637492
1829.658569 0.638499
1829.658569 0.639622
1829.658569 0.640703
1829.658569 0.641757
1829.658569 0.643016
1829.658569 0.644161
1829.658569 0.645158
1848.446655 0.639110
1867.101440 0.630927
1867.101440 0.631977
1867.101440 0.633047
1867.101440 0.634072
1867.101440 0.635143
1867.101440 0.636508
1885.865356 0.636466
1885.865356 0.637348
1885.865356 0.638410
1885.865356 0.639345
1885.865356 0.640450
1885.865356 0.641574
1885.865356 0.642611
1885.865356 0.643557
1885.865356 0.644804
1885.865356 0.645922
1885.865356 0.647064
1885.865356 0.648311
1885.865356 0.649398
1885.865356 0.650235
1885.865356 0.651352
1905.167480 0.649699
1905.167480 0.650686
1905.167480 0.651866
1905.167480 0.652784
1924.476196 0.652441
1924.476196 0.653383
1924.476196 0.654579
1924.476196 0.655820
1924.476196 0.656787
1924.476196 0.657845
1924.476196 0.658875
1924.476196 0.659610
1924.476196 0.660526
1924.476196 0.661435
1924.476196 0.662597
1924.476196 0.663861
1924.476196 0.664984
1924.476196 0.666054
1924.476196 0.666965
1963.962280 0.654818
1963.962280 0.655873
1963.962280 0.656821
1983.568115 0.652926
1983.568115 0.653974
1983.568115 0.654783
1983.568115 0.655971
1983.568115 0.656992
1983.568115 0.658005
1983.568115 0.658949
1983.568115 0.659929
1983.568115 0.660975
1983.568115 0.661999
1983.568115 0.662917
2003.504639 0.661748
2003.504639 0.662682
2003.504639 0.663448
2003.504639 0.664475
2003.504639 0.665615
2003.504639 0.666571
2003.504639 0.667576
2003.504639 0.668409
2023.627930 0.668260
2023.627930 0.669351
2023.627930 0.670259
2023.627930 0.671253
2023.627930 0.672308
2023.627930 0.673492
2023.627930 0.674545
2023.627930 0.675431
2023.627930 0.676344
2023.627930 0.677298
2023.627930 0.678340
2023.627930 0.679135
2023.627930 0.680229
2023.627930 0.681193
2023.627930 0.681819
2023.627930 0.682695
2023.627930 0.683852
2023.627930 0.684859
2023.627930 0.685842
2023.627930 0.686980
2023.627930 0.688092
2023.627930 0.688966
2023.627930 0.689817
2023.627930 0.691006
2023.627930 0.691753
2023.627930 0.692650
2044.768555 0.686879
2044.768555 0.687863
2044.768555 0.688726
2044.768555 0.689585
2044.768555 0.690575
2065.944580 0.687153
2065.944580 0.687780
2065.944580 0.688631
2065.944580 0.689771
2087.110107 0.682914
2087.110107 0.683990
2087.110107 0.684930
2087.110107 0.685822
2087.110107 0.686692
2108.310547 0.678904
2150.226318 0.676944
2150.226318 0.677950
2170.990967 0.676532
2170.990967 0.677312
2170.990967 0.678166
2170.990967 0.678918
2170.990967 0.679724
2170.990967 0.680792
2170.990967 0.681657
2191.883301 0.676967
2191.883301 0.677627
2191.883301 0.678387
2191.883301 0.679442
2212.767822 0.678579
2212.767822 0.679391
2212.767822 0.680307
2212.767822 0.681190
2233.644531 0.673710
2233.644531 0.674837
2233.644531 0.675543
2233.644531 0.676522
2233.644531 0.677663
2233.644531 0.678486
2233.644531 0.679576
2233.644531 0.680404
2233.644531 0.681438
2233.644531 0.682195
2233.644531 0.683215
2233.644531 0.684019
2233.644531 0.684926
2233.644531 0.685581
2233.644531 0.686523
2233.644531 0.687843
2233.644531 0.688399
2233.644531 0.689352
2233.644531 0.690393
2233.644531 0.691102
2233.644531 0.692043
2233.644531 0.692856
2233.644531 0.693833
2233.644531 0.694434
2233.644531 0.695184
2233.644531 0.696173
2233.644531 0.696883
2233.644531 0.697750
2233.644531 0.698522
2255.619385 0.688744
2255.619385 0.689711
2255.619385 0.690784
2255.619385 0.691641
2255.619385 0.692224
2255.619385 0.693183
2255.619385 0.694181
2255.619385 0.695163
2255.619385 0.695962
2255.619385 0.696716
2255.619385 0.697264
2255.619385 0.698175
2255.619385 0.699025
2255.619385 0.699661
2255.619385 0.700576
2278.061768 0.685875
2278.061768 0.686643
2278.061768 0.687430
2278.061768 0.688452
2278.061768 0.689227
2278.061768 0.690236
2300.570068 0.689684
2300.570068 0.690725
2300.570068 0.691610
2300.570068 0.692430
2300.570068 0.693337
2323.100342 0.693316
2323.100342 0.694081
2323.100342 0.695085
2345.565186 0.693718
2345.565186 0.694262
2345.565186 0.694896
2345.565186 0.695626
2345.565186 0.696511
2345.565186 0.697407
2368.095215 0.697498
2368.095215 0.698453
2368.095215 0.699090
2368.095215 0.700000
2368.095215 0.700932
2368.095215 0.701682
2368.095215 0.702813
2368.095215 0.703614
2368.095215 0.704493
2368.095215 0.705244
2368.095215 0.706291
2368.095215 0.707020
2368.095215 0.707995
2368.095215 0.708865
2368.095215 0.709408
2368.095215 0.710213
2368.095215 0.710921
2368.095215 0.711590
2368.095215 0.712285
2368.095215 0.712896
2368.095215 0.713776
2391.336182 0.705430
2391.336182 0.706235
2391.336182 0.707013
2414.506348 0.705910
2437.521484 0.706047
2437.521484 0.707011
2437.521484 0.707799
2437.521484 0.708609
2437.521484 0.709554
2437.521484 0.710499
2437.521484 0.711401
2437.521484 0.712290
2437.521484 0.712679
2460.723389 0.711794
2460.723389 0.712498
2460.723389 0.713252
2460.723389 0.713903
2460.723389 0.714628
2460.723389 0.715456
2460.723389 0.716129
2460.723389 0.716886
2460.723389 0.717559
2460.723389 0.718264
2460.723389 0.719081
2460.723389 0.719799
2460.723389 0.720346
2460.723389 0.721203
2460.723389 0.721854
2484.364502 0.720968
2484.364502 0.721608
2484.364502 0.722399
2484.364502 0.723267
2484.364502 0.724042
2484.364502 0.724854
2484.364502 0.725708
2484.364502 0.726493
2484.364502 0.727192
2484.364502 0.728288
2484.364502 0.729038
2484.364502 0.729843
2484.364502 0.730587
2484.364502 0.731731
2484.364502 0.732643
2484.364502 0.733606
2484.364502 0.734457
2484.364502 0.735243
2484.364502 0.735876
2484.364502 0.736395
2484.364502 0.737403
2484.364502 0.738074
2484.364502 0.738832
2484.364502 0.739449
2484.364502 0.740460
2484.364502 0.741170
2508.902832 0.742404
2508.902832 0.743145
2508.902832 0.744008
2508.902832 0.744837
2508.902832 0.745825
2508.902832 0.746588
2508.902832 0.747451
2508.902832 0.748427
2533.571533 0.740935
2533.571533 0.741976
2533.571533 0.742894
2533.571533 0.743514
2533.571533 0.744217
2533.571533 0.744905
2533.571533 0.745642
2533.571533 0.746420
2533.571533 0.747047
2533.571533 0.747835
2533.571533 0.748531
2533.571533 0.749472
2533.571533 0.750166
2533.571533 0.750976
2533.571533 0.751404
2533.571533 0.752064
2533.571533 0.752787
2533.571533 0.753518
2533.571533 0.754566
2533.571533 0.755362
2533.571533 0.755886
2533.571533 0.756543
2558.953857 0.756260
2584.166748 0.755116
2584.166748 0.755795
2584.166748 0.756561
2584.166748 0.757695
2584.166748 0.758389
2584.166748 0.759282
2584.166748 0.760274
2584.166748 0.761027
2584.166748 0.761790
2584.166748 0.762485
2584.166748 0.763189
2584.166748 0.764013
2584.166748 0.764802
2584.166748 0.765705
2584.166748 0.766434
2584.166748 0.767176
2584.166748 0.767874
2584.166748 0.768666
2584.166748 0.769481
2584.166748 0.770182
2584.166748 0.770436
2584.166748 0.771150
2584.166748 0.771877
2584.166748 0.772752
2584.166748 0.773345
2584.166748 0.774273
2584.166748 0.775142
2584.166748 0.775955
2584.166748 0.776986
2584.166748 0.777742
2584.166748 0.778624
2584.166748 0.779317
2584.166748 0.780298
2610.539307 0.775406
2610.539307 0.776022
2610.539307 0.776802
2610.539307 0.777586
2610.539307 0.778213
2610.539307 0.779020
2610.539307 0.779412
2610.539307 0.780214
2610.539307 0.780815
2610.539307 0.781521
2610.539307 0.782266
2610.539307 0.783044
2610.539307 0.783928
2610.539307 0.784634
2610.539307 0.785366
2610.539307 0.786023
2610.539307 0.786643
2610.539307 0.787492
2610.539307 0.788183
2610.539307 0.788709
2610.539307 0.789460
2610.539307 0.790308
2610.539307 0.790930
2610.539307 0.791447
2610.539307 0.792171
2610.539307 0.793008
2610.539307 0.793723
2610.539307 0.794618
2637.851318 0.778297
2637.851318 0.779112
2637.851318 0.779970
2637.851318 0.780750
2637.851318 0.781538
2637.851318 0.782287
2637.851318 0.782941
2637.851318 0.783783
2637.851318 0.784378
2637.851318 0.785199
2637.851318 0.785886
2637.851318 0.786455
2637.851318 0.787404
2637.851318 0.788328
2665.514404 0.780803
2665.514404 0.781504
2665.514404 0.782181
2665.514404 0.782814
2665.514404 0.783535
2665.514404 0.784326
2665.514404 0.784895
2665.514404 0.785500
2665.514404 0.786349
2665.514404 0.787227
2665.514404 0.788002
2665.514404 0.788710
2665.514404 0.789434
2665.514404 0.790030
2665.514404 0.790752
2665.514404 0.791460
2665.514404 0.792185
2665.514404 0.792693
2665.514404 0.793454
2665.514404 0.794090
2665.514404 0.795006
2665.514404 0.796045
2665.514404 0.796838
2665.514404 0.797735
2693.934326 0.797059
2693.934326 0.797588
2693.934326 0.798445
2693.934326 0.799223
2693.934326 0.799812
2722.326416 0.796450
2722.326416 0.797050
2722.326416 0.797596
2722.326416 0.798210
2722.326416 0.798730
2722.326416 0.799846
2722.326416 0.800677
2750.772461 0.798399
2779.028320 0.788851
2779.028320 0.789533
2779.028320 0.790230
2779.028320 0.790863
2779.028320 0.791475
2779.028320 0.792017
2779.028320 0.792688
2779.028320 0.792939
2779.028320 0.793467
2779.028320 0.794032
2779.028320 0.794646
2779.028320 0.795492
2779.028320 0.796462
2779.028320 0.796961
2807.620850 0.792923
2807.620850 0.793716
2807.620850 0.794296
2807.620850 0.794792
2807.620850 0.795273
2807.620850 0.795952
2807.620850 0.796489
2807.620850 0.797315
2807.620850 0.797792
2807.620850 0.798300
2807.620850 0.798925
2807.620850 0.799618
2807.620850 0.800167
2807.620850 0.800771


==> fig/losses_cosines_infty.tex <==
% This file was created by matplotlib2tikz v0.6.15.
\begin{tikzpicture}

\begin{groupplot}[group style={group size=2 by 1}]
\nextgroupplot[
title={$\ell_\infty$ threat model: losses},
xlabel={queries},
ylabel={loss},
xmin=0, xmax=100,
ymin=0, ymax=1,
axis on top,
ytick={0,0.2,0.4,0.6,0.8,1},
yticklabels={0.0,0.2,0.4,0.6,0.8,1.0},
tick pos=both,
legend cell align={left},
legend style={at={(0.03,0.97)}, anchor=north west},
legend entries={{nes},{bandits},{bandits with tiling}}
]
\addlegendimage{no markers, blue}
\addlegendimage{no markers, green!50.0!black}
\addlegendimage{no markers, red}
\addplot [blue]
table {%
0 0.0032635633219894
1 0.00388944676696823
2 0.0250053009868988
3 0.0251488700052391
4 0.0792979523108565
5 0.0942054648076629
6 0.0994493768502038
7 0.101781691013701
8 0.106047335533487
9 0.11332696200203
10 0.116965928732369
11 0.124841719334477
12 0.128644955056283
13 0.129943081765582
14 0.14309709003925
15 0.14561061748298
16 0.160607682880705
17 0.165817566769969
18 0.166895434282219
19 0.176674412011399
20 0.187663147487399
21 0.193437152493396
22 0.207790536328987
23 0.209726490577804
24 0.212216684432088
25 0.216974427631074
26 0.241277106052609
27 0.244583537338208
28 0.244739384299764
29 0.248988332483545
30 0.26211011713656
31 0.27814752574185
32 0.285124790392602
33 0.29494225173698
34 0.298011038175454
35 0.303566872195377
36 0.304890992466471
37 0.306593285165539
38 0.320552142994593
39 0.335904998017112
40 0.33660513172326
41 0.336671033992087
42 0.356612715670073
43 0.367131979621511
44 0.374240133588218
45 0.391943923377678
46 0.413351581285283
47 0.420043300526973
48 0.424703073131317
49 0.428930877676575
50 0.429295718774435
51 0.431283896419769
52 0.457191636139072
53 0.462837587728704
54 0.468471818620762
55 0.473793899824027
56 0.47946729613422
57 0.49504060982361
58 0.502842965617551
59 0.595478012212291
60 0.597524281698089
61 0.614800665131597
62 0.614849753147843
63 0.616385275163957
64 0.635358310801722
65 0.646195980069143
66 0.648497001300342
67 0.670251263264158
68 0.682433943391468
69 0.691939688840064
70 0.695870015542812
71 0.696588396668379
72 0.702552637468748
73 0.707028436678932
74 0.717602402424274
75 0.761625025099985
76 0.770498206187047
77 0.772481411647162
78 0.78042725585392
79 0.781425966167523
80 0.79626856070516
81 0.799833521835982
82 0.810793518619334
83 0.812400138677276
84 0.822229415920728
85 0.833824447752178
86 0.834333171502823
87 0.866080068625481
88 0.884748761441896
89 0.884924709378076
90 0.90389213947818
91 0.920811446210205
92 0.926618287045532
93 0.929010122944322
94 0.929092912490238
95 0.949225229092222
96 0.960071740279436
97 0.967187553265598
98 0.97179359693551
99 0.996111905143816
};
\addplot [green!50.0!black]
table {%
0 0.0400251473396693
1 0.0532831736876478
2 0.0537090402491788
3 0.0590438898420721
4 0.0663646086186251
5 0.0739272607389901
6 0.0760344231238992
7 0.0789788263023482
8 0.100439113958327
9 0.100556037738503
10 0.121888551560927
11 0.128934814209964
12 0.129176107068968
13 0.132503312887539
14 0.138497597599248
15 0.152706828092281
16 0.170388363297586
17 0.17480354801486
18 0.179575209807769
19 0.200719581878428
20 0.208673743977035
21 0.211342869967781
22 0.216345228176522
23 0.231487957389484
24 0.244887911148161
25 0.251848938528159
26 0.255057610851396
27 0.266227635942439
28 0.270421206571254
29 0.278496867031217
30 0.334589921066933
31 0.3413158594454
32 0.371653476489882
33 0.394481343886827
34 0.401824911250413
35 0.406501163576243
36 0.412389146303562
37 0.424231023306785
38 0.43621878962437
39 0.444640053123949
40 0.447388390577901
41 0.451377875084502
42 0.45775157144285
43 0.46412838051434
44 0.466475014264333
45 0.471592873418627
46 0.477737139132773
47 0.493908735404083
48 0.497988907060158
49 0.506122504085875
50 0.507450125036131
51 0.515974876985142
52 0.521246068569394
53 0.52799265600758
54 0.552212504901208
55 0.570748206618011
56 0.571679046864598
57 0.587206585405094
58 0.590995228709475
59 0.619763819837982
60 0.635081522107675
61 0.638705612985385
62 0.640940421892968
63 0.644700168659886
64 0.649168865733813
65 0.649292217716777
66 0.650686195520957
67 0.652341765971977
68 0.656386093724387
69 0.66264328123696
70 0.674343826196057
71 0.676551706587824
72 0.684156749250107
73 0.699606071552188
74 0.704941348221535
75 0.71250559495083
76 0.719581534731227
77 0.732475820315521
78 0.741963142337838
79 0.746073055119112
80 0.751965466821513
81 0.756461697451164
82 0.757787512088616
83 0.770840683101314
84 0.793570961239777
85 0.806816178989973
86 0.821388799234601
87 0.823493999405221
88 0.824680802739761
89 0.832878412308236
90 0.842555670833155
91 0.860762832741238
92 0.866098961591055
93 0.872433800854537
94 0.884581156162491
95 0.908249724348274
96 0.936194091495883
97 0.939445591161573
98 0.950517955696339
99 0.961269426646287
};
\addplot [red]
table {%
0 0.00579629648469959
1 0.0333880310025126
2 0.0368997693712851
3 0.0394551285547745
4 0.0429790078841005
5 0.0452387670335236
6 0.0547244785353203
7 0.0598187621350916
8 0.0698056219497104
9 0.0853709065614959
10 0.0868241502977609
11 0.0964363777146836
12 0.10575409777373
13 0.118218448001854
14 0.123190242171884
15 0.127601348287294
16 0.148819328185766
17 0.150549245650384
18 0.184935098781711
19 0.191010048503952
20 0.194109787684739
21 0.194565850892842
22 0.197060918443697
23 0.205771783878231
24 0.207073202468864
25 0.231647942757515
26 0.234583581698261
27 0.236565789964875
28 0.257629978957141
29 0.261975962875823
30 0.270191305524552
31 0.270522538742563
32 0.29395304207378
33 0.301285456284379
34 0.313169598969196
35 0.320697122955215
36 0.328285145381411
37 0.335346810657068
38 0.343935182073104
39 0.349701014165688
40 0.371970566827378
41 0.37487442395947
42 0.404961558385784
43 0.405759333011294
44 0.410952806191371
45 0.415070956486996
46 0.421206216369101
47 0.42677625601058
48 0.452462382074594
49 0.453788307989276
50 0.459560425343318
51 0.460878070466172
52 0.474201996920818
53 0.490025028252302
54 0.545555094582242
55 0.558288723361786
56 0.559543912640726
57 0.570857505916094
58 0.576114206240571
59 0.577934850263489
60 0.594755045305581
61 0.596736852619225
62 0.607686260332763
63 0.617960269196792
64 0.628045842437172
65 0.63641249698323
66 0.640176047091955
67 0.663274008377533
68 0.671559502414124
69 0.678471465584633
70 0.683660012383737
71 0.686402821552504
72 0.709856508257163
73 0.71865061495348
74 0.721410856449116
75 0.721710192246523
76 0.736027661273562
77 0.73687328141653
78 0.743074989706914
79 0.764480620363834
80 0.770949923362678
81 0.784976455897122
82 0.795153104821587
83 0.795910582090441
84 0.805384244946631
85 0.808320194720788
86 0.809876494021276
87 0.820037185264683
88 0.821380618601263
89 0.853099527816547
90 0.881261804679564
91 0.912606578304113
92 0.938677338849039
93 0.952715314041119
94 0.967281038685973
95 0.974357638162402
96 0.987004824199575
97 0.991655193852829
98 0.993691908780809
99 0.999148999094244
};
\nextgroupplot[
title={$\ell_\infty$ threat model: cosine distances},
xlabel={queries},
ylabel={cosine distance},
xmin=0, xmax=100,
ymin=0, ymax=1,
axis on top,
ytick={0,0.2,0.4,0.6,0.8,1},
yticklabels={0.0,0.2,0.4,0.6,0.8,1.0},
tick pos=both,
legend cell align={left},
legend style={at={(0.97,0.03)}, anchor=south east},
legend entries={{nes},{bandits},{bandits with tiling}}
]
\addlegendimage{no markers, blue}
\addlegendimage{no markers, green!50.0!black}
\addlegendimage{no markers, red}
\addlegendimage{no markers, blue}
\addlegendimage{no markers, green!50.0!black}
\addlegendimage{no markers, red}
\addplot [blue]
table {%
0 0.00744001001366468
1 0.0116528741041581
2 0.0168907129390427
3 0.018343824685722
4 0.0202834942371439
5 0.0334258951133637
6 0.0515676782253514
7 0.0584937836829754
8 0.0717722959922041
9 0.0735942434521899
10 0.0845431878830148
11 0.120581269911113
12 0.143828470633901
13 0.149906690319282
14 0.185572518359806
15 0.208929237360291
16 0.210654129787685
17 0.219613140172278
18 0.224024866935833
19 0.23088502417322
20 0.27311826372781
21 0.274870727370623
22 0.296873112165768
23 0.326747838910152
24 0.355862209229283
25 0.363326381299346
26 0.36413783972659
27 0.364983798754882
28 0.367423850701174
29 0.379909379271469
30 0.385715917560245
31 0.392092096912147
32 0.397447510650557
33 0.43407860717515
34 0.439660021587314
35 0.445854608752552
36 0.462967252292028
37 0.49239442307301
38 0.497308093791546
39 0.504722870840889
40 0.504877910733946
41 0.505142262708438
42 0.531560890501752
43 0.536433983793331
44 0.540701387709534
45 0.565774633805264
46 0.567831465149464
47 0.580439203864748
48 0.580819046129559
49 0.58344924509502
50 0.597785765604557
51 0.623237573817587
52 0.639735050735355
53 0.641044741626556
54 0.641084888690098
55 0.64184152614569
56 0.646353993044088
57 0.647463939247703
58 0.656875454819102
59 0.696054394557912
60 0.697348114508393
61 0.699774841827507
62 0.726792708808817
63 0.730883901876238
64 0.731517577853722
65 0.749178505802073
66 0.759041626071121
67 0.763974643972388
68 0.771478169787129
69 0.778542424153631
70 0.780458675294384
71 0.780872981153138
72 0.791784672582774
73 0.800748786293983
74 0.805155531059728
75 0.814775520022557
76 0.823238983168437
77 0.824262761376392
78 0.833282406077107
79 0.838172509490898
80 0.84434812697537
81 0.847008552361244
82 0.858838900869561
83 0.86135108151171
84 0.870909945731323
85 0.872242984094059
86 0.873449315762526
87 0.876297835444042
88 0.886464229837218
89 0.887176031670271
90 0.895866837550707
91 0.92617005574874
92 0.928869072306149
93 0.931680608864752
94 0.93773583598939
95 0.94724615770041
96 0.955774756165032
97 0.962260474222979
98 0.967116666629084
99 0.976577018750724
};
\addplot [green!50.0!black]
table {%
0 0.00867423111658272
1 0.0527434842241229
2 0.0576995096007341
3 0.109390811165392
4 0.109757899553705
5 0.113588482781533
6 0.116117249146037
7 0.118118375207113
8 0.143457058582136
9 0.145230644699191
10 0.157681182300191
11 0.172095335520989
12 0.172632162526828
13 0.192981669319347
14 0.198789674884387
15 0.209592724949433
16 0.216568955538406
17 0.217728658196329
18 0.256400460791085
19 0.263458117631938
20 0.270883467608737
21 0.273473758490643
22 0.28374501237657
23 0.295203370048917
24 0.298756843408376
25 0.319750445361394
26 0.321427300202515
27 0.33338303066881
28 0.336222231965462
29 0.35650681207662
30 0.382887229891301
31 0.386478608725816
32 0.397003876607295
33 0.399628689586449
34 0.402408784484549
35 0.454847954315646
36 0.46044898275098
37 0.464247202328884
38 0.465646401657449
39 0.477836591859914
40 0.486355631004769
41 0.488009091470136
42 0.48936435741041
43 0.496548542878316
44 0.500847897379393
45 0.518219731086799
46 0.519902180423105
47 0.540518616167979
48 0.549024906351813
49 0.564007812496013
50 0.57279327754498
51 0.611323419330601
52 0.611396573387183
53 0.613142355418511
54 0.625391368725921
55 0.654120275377068
56 0.658315857039192
57 0.659459297378153
58 0.676463110446129
59 0.679235538632307
60 0.710481333864788
61 0.727186492778922
62 0.728592907397852
63 0.73168557821974
64 0.733579866289499
65 0.738388213986015
66 0.740380407987428
67 0.745443425497672
68 0.748040009115558
69 0.752340204985014
70 0.754554319133237
71 0.758118778664572
72 0.758580208760688
73 0.764863610223049
74 0.764940475708614
75 0.769871447593237
76 0.780379058454364
77 0.781833114021172
78 0.801072317356727
79 0.803009114003871
80 0.808855529914104
81 0.81201877016146
82 0.81926092912828
83 0.819656214918757
84 0.828317464917511
85 0.83458840806798
86 0.852990656777823
87 0.865397454668436
88 0.865563946925127
89 0.884813441167678
90 0.903764597764771
91 0.927317466133566
92 0.935307317732956
93 0.938748839356099
94 0.945098760068156
95 0.950982220291691
96 0.952551594423097
97 0.959421717282598
98 0.983555269833358
99 0.986364891378025
};
\addplot [red]
table {%
0 0.00162403263452238
1 0.0197695474602503
2 0.0226017660007398
3 0.0434522951269982
4 0.0531345006589595
5 0.0828727635034673
6 0.101411885787843
7 0.119432837331239
8 0.125643016825463
9 0.132235150577198
10 0.134726963353257
11 0.150092401998774
12 0.154074468371077
13 0.161582813380894
14 0.165590038388728
15 0.180026386945448
16 0.20256024910133
17 0.206936231919665
18 0.209107020837632
19 0.232379216880143
20 0.25498727927567
21 0.255684108603471
22 0.261611907054599
23 0.26227835381886
24 0.275815313481092
25 0.30083879750855
26 0.303303105539541
27 0.311261709721619
28 0.312196918008941
29 0.331808549471864
30 0.332022850905496
31 0.332949516773911
32 0.373090731478921
33 0.373864831565592
34 0.393283589168077
35 0.39545507245349
36 0.397899943706172
37 0.418795716157417
38 0.422151958443765
39 0.436155248671762
40 0.449670528173101
41 0.474431319524184
42 0.477675592768617
43 0.479238335839502
44 0.485195451588404
45 0.486220861361306
46 0.487956988728426
47 0.488084161555014
48 0.488572200403373
49 0.488599783067868
50 0.497545922510926
51 0.513196239358351
52 0.533473448227915
53 0.534532720650796
54 0.540065418951164
55 0.542969063379883
56 0.551249461038264
57 0.560154684421991
58 0.587618951295343
59 0.590074543136861
60 0.592034102918833
61 0.598049926581706
62 0.617798224966605
63 0.647739412507351
64 0.681850006798503
65 0.712794906126466
66 0.713891215948256
67 0.71993827130047
68 0.72196820554434
69 0.725963219777513
70 0.733833585205364
71 0.737581611427113
72 0.741682553843402
73 0.746598812881468
74 0.751147459892055
75 0.783675358428816
76 0.803198400068862
77 0.809405860552922
78 0.8125874884457
79 0.813647263307165
80 0.850086612007417
81 0.87026667945189
82 0.885456557680122
83 0.902799215810832
84 0.909151811972748
85 0.918679644234261
86 0.921498893861209
87 0.923986606539484
88 0.942389711123278
89 0.944998135156254
90 0.954848957216482
91 0.956651299928998
92 0.96257117112886
93 0.972696510433354
94 0.975026379209489
95 0.9772901024776
96 0.980908472635054
97 0.993463619455213
98 0.996471341212699
99 0.998773565440282
};
\end{groupplot}

\end{tikzpicture}

==> pseudocode/linf-alg.tex <==
\begin{algorithm}
\caption{Adversarial Example Generation with Bandit Optimization
($\ell_\infty$)}\label{alg:linf}
\begin{algorithmic}[1]
    \Procedure{Adversarial-Bandit-LInf}{$x_{init}, y_{init}$} 
    \State $//\ C(\cdot)$ returns top class, $f(\cdot;y)$ returns softmax loss wrt $y$
    \State $p \gets {\bf \frac{1}{2}}_{1\times d}\ //$ Latent vector for temporal prior
    \State $x \gets x_{init}\ //$ Adversarial Image
    \While{$C(x) = y_{init}$}
    \State $l_t \gets f(x; y_{init})\ //$ Current loss (for logging)
    \State $u \gets \mathcal{N}(0, \frac{1}{d}I)$
    \State $\{d_1, d_2\} \gets \{2\cdot (p + \delta\cdot u) - 1, 2\cdot (p
- \delta\cdot u) - 1\}$
    \State 
    \State $//$ Estimate $g_t \approx \nabla_p\inner{\nabla_xf(x)}{p}$ via two-query spherical estimate:
    \State $q_1 \gets \frac{f(x+\epsilon\cdot d_1)}{\epsilon} \approx
    \inner{\nabla_xf(x)}{p + \delta u}$
    \State $q_2 \gets \frac{f(x+\epsilon\cdot d_2)}{\epsilon} \approx
    \inner{\nabla_xf(x)}{p - \delta u}$
    \State $g_t \gets q_1\bm{u} + q_2(-\bm{u}) = (q_1 - q_2)\bm{u}$
    \State $p \gets \frac{p\cdot \exp\{\eta\cdot g_t\}}{p\cdot
\exp\{\eta\cdot g_t\} + (1-p)\exp\{-\eta g_t\}}$
    \State $x \gets x + h \cdot \text{sgn}(p)$
    \EndWhile
    \Return $x$
\EndProcedure
\end{algorithmic}
\end{algorithm}


==> tiling.tex <==
\begin{figure}
\centering
\begin{subfigure}{.45\textwidth}
  \centering
  \includegraphics[width=.85\linewidth]{fig/pooling/unpooled_grad.png}
  \caption{Gradient}
  \label{fig:avg-blur-sub1}
\end{subfigure}
\begin{subfigure}{.45\textwidth}
  \centering
  \includegraphics[width=.85\linewidth]{fig/pooling/pooled_grad.png}
  \caption{Tiled gradient}
  \label{fig:avg-blu-sub2}
\end{subfigure}
  \caption{Average blurred gradient with kernel size or ``tile length'' 5. The original gradient can be seen in~\ref{fig:avg-blur-sub1}, and the ``tiled'' or average blurred gradient can be seen in~\ref{fig:avg-blu-sub2}}
  \label{fig:avg-blur}
\end{figure}

